Formation of large-scale structures by turbulence in rotating planets

This thesis presents a newly developed theory for the formation and maintenance of eddy-driven jets in planetary turbulence. The novelty is that jet formation and maintenance is studied as a dynamics of the statistics of the flow rather than a dynamics of individual realizations. This is pursued using Stochastic Structural Stability Theory (S3T), which studies the closed dynamics of the first two cumulants of the full statistical state dynamics of the flow after neglecting or parameterizing third and higher-order cumulants. Using this statistical closure, large-scale structure formation is studied in barotropic turbulence on a $\beta$-plane. It is demonstrated that at analytically predicted critical parameter values the homogeneous turbulent state undergoes a bifurcation becoming inhomogeneous with the emergence of large-scale zonal and/or non-zonal flows. The mechanisms by which the turbulent Reynolds stresses organize to reinforce infinitesimal mean flow inhomogeneities, thus leading to this statistical state instability, are studied for various regimes of parameter values. It is also demonstrated that the S3T instabilities equilibrate to turbulent states with finite-amplitude jets. Moreover, the relation between large-scale structure formation through modulational instability and the S3T instability of the homogeneous turbulent state is also investigated and it is shown that the modulational instability results are subsumed by the S3T results. Finally, the study of the S3T stability of inhomogeneous turbulent jet equilibria is presented and the relation with the phenomenon of jet merging is investigated. Although all these phenomena cannot be predicted by analysis of the dynamics of single realizations of the flow, it is demonstrated that the predictions of S3T are reflected in individual realizations of the flow.

==> chapters/app-S3Tgr_copy.tex <==
% !TEX root = ../thesis.tex


\chapter{Derivation of the dispersion relation for the S3T stability of a homogeneous equilibrium}
\label{app:S3Tgr}

\section{Eigenvalue relation for homogeneous S3T equilibrium} 
\label{appsec:eigenvalue}

Here we derive an analytic expression satisfied by  the eigenvalue $\s$  that determines the stability of the homogeneous equilibrium~\eqref{eq:ZeCe}. The eigenvalue problem to be solved is~\eqref{eq:s3t_dZdC_s}, %\textcolor{red}{\textbf{(Petro the equations do not change with the inclusion of hyperdiffusion, only $\Acal^e$ changes. Do you think I should repeat them anyway?)}}
\begin{subequations}\begin{align}
s \,\dZ &=\Acal^e\,\dZ+ \Rcal( \dC )\ ,\label{eq:s3t_pert_dZ_s_app}\\
s \,\dC_{ab} & = \(\bit\Acal^e_a + \Acal^e_b \)\dC_{ab} +\(\bit\d\tilde{\Acal}_a + \d\tilde{\Acal}_b\)C^e_{ab}\ .\label{eq:s3t_pert_dC_s}
\end{align}\label{eq:s3t_dZdC_s_app}\end{subequations}
We have included in~\eqref{eq:s3t_dZdC_s_app} also hyperdiffusive damping of the form: $-(-1)^h\nu_{2h} \Delta^{h}\,\z$. For $h=1$ this is normal diffusion, while for $h>1$ is hyperdiffusion of order $2h$. With this damping the operator $\Acal^e$ becomes:
\be
\Acal^e =\zhat\cdot\( \bv\times\nablav\)\Del^{-1} -1 + (-1)^h\nu_{2h} \Delta^{h}\ .
\ee
Equations~\eqref{eq:s3t_dZdC_s_app} is a linear system in $\dZ$ and $\dC$ and can be written symbolically as:\footnote{To find explicitly the form of $\Lcal$ one needs to manipulate $\d\tilde{\Acal}_a\,C^e_{ab}$ in the following manner:
\begin{align}
\d\tilde{\Acal}_a \,C^e_{ab} &   =-\d\tilde{\Uv}_a\cdot \nablav_a C^e_{ab} + (\Del_a\d\tilde{\Uv}_a)\cdot \nablav_a\Del_a^{-1}C^e_{ab} \nonumber\\
&   =-\(\zhat\times\nablav_a\d\tilde{\Psi}_a\) \cdot\nablav_a C^e_{ab} + \(\zhat\times\nablav_a\dZ_a\) \cdot \nablav_a \Del_a^{-1}C^e_{ab} \nonumber\\
&   =\(\zhat\times\nablav_a C^e_{ab}\) \cdot \nablav_a\d\tilde{\Psi}_a-\(\zhat\times\nablav_a \Del_a^{-1}C^e_{ab}\) \cdot\nablav_a\dZ_a \nonumber\\
&   =\[ \(\zhat\times\nablav_a C^e_{ab}\) \cdot \nablav_a\Del_a^{-1}-\(\zhat\times\nablav_a \Del_a^{-1}C^e_{ab}\) \cdot\nablav_a\]\dZ_a\ .\nonumber
\end{align}
Similarly for $\d\tilde{\Acal}_a\,C^e_{ab}$.}
\be
s\,\[\dZ,\dC\]^\transp = \Lcal(C^e)\,\[\dZ,\dC\]^\transp\ .
\ee
Because the only spatial dependence of the coefficients of $\Lcal$ is through $C^e(\xv_a-\xv_b)$ it is advantageous to consider the eigenvalue problem in terms of the relative coordinate $\xv_a-\xv_b$ and centroid coordinate $(\xv_a+\xv_b)/2$. Since~\eqref{eq:s3t_pert_dZ_s_app} is homogeneous in $\xv$ and~\eqref{eq:s3t_dZdC_s_app} homogeneous in $(\xv_a+\xv_b)/2$ the eigenfunctions $\dZ$ and $\dC$ will be single harmonics of their homogeneous coordinate (cf. Appendix~\ref{app:bloch}) and can be assumed to be of the form:
\begin{subequations}\begin{align}
\dZ_\nv(\xv) &= e^{\i\nv \cdot\xv}\ ,\\
\dC_\nv(\xv_a,\xv_b) &=\tilde{C}_\nv^{(\textrm{h})}\(\bit\xv_a-\xv_b\)\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\ .
\end{align}\end{subequations}
The homogeneous part of the perturbation covariance eigenfunction, $\tilde{C}_\nv^{(\textrm{h})}$, is expanded as
\be
C_\nv^{\textrm{(h)}}(\xv_a-\xv_b) = \int\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\ ,\label{eq:Cnv_Cnvhat}
\ee
and introducing~\eqref{eq:Cnv_Cnvhat} to the perturbation covariance equation~\eqref{eq:s3t_pert_dC_s}, we obtain:
\begin{subequations}\begin{align}
%s \,\dC_{ab}  & = \int\frac{\df^2\kv}{(2\pi)^2}(\s-\i\om_{\nv})\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\ ,\\
\(\bit\Acal^e_a + \Acal^e_b \)\dC_{ab}  & = -\int\frac{\df^2\kv}{(2\pi)^2}\[ 2+\nu_{2h} (k^{2h}_+ + k^{2h}_-) + \i\(\om_{\kv_+}-\om_{\kv_-}\)\]\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\ ,\end{align}
with $\kv_{\pm} \equiv \kv\pm\nv/2$. We also have that \begin{align}
\d\tilde{\Acal}_a \,C^e_{ab} &=\int\!\frac{\df^2\kv}{(2\pi)^2}\,\hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2}-\frac1{n^2}\)\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b}\nonumber\\
&= e^{\i\nv\cdot(\xv_a+\xv_b)/2} \int\!\frac{\df^2\kv}{(2\pi)^2}\,\hat{\mathbf{z}}\cdot(\nv\times\kv_-)\(\frac1{k_-^2}-\frac1{n^2}\)\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\ ,
\end{align}
and similarly,
\begin{align}\d\tilde{\Acal}_b \,C^e_{ab} &=\int\!\frac{\df^2\kv}{(2\pi)^2}\,\hat{\mathbf{z}}\cdot(\kv\times\nv)\(\frac1{k^2}-\frac1{n^2}\)\,\hat{C}^e(\kv)\,e^{\i\kv\cdot\xv_a-\i(\kv+\nv)\cdot\xv_b}\nonumber\\
&=- e^{\i\nv\cdot(\xv_a+\xv_b)/2} \int\!\frac{\df^2\kv}{(2\pi)^2}\,\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\frac1{k_+^2}-\frac1{n^2}\)\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\ .
\end{align}\label{eq:dCpert_terms}\end{subequations}
From~\eqref{eq:s3t_pert_dC_s} we then obtain that
\begin{align}
\hat{C}^{\textrm{(h)}}(\kv)&=\dfrac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\dfrac1{k^2_{-}}-\dfrac1{n^2}\)\,\hat{C}^e(\kv_-)-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\dfrac1{k^2_{+}}-\dfrac1{n^2}\)\,\hat{C}^e(\kv_+)}{\s+2 + \nu_{2h} (k^{2h}_+ + k^{2h}_-) +\i \(  \om_{\kv_+}- \om_{\kv_-} - \om_\nv\)}e^{\i\nv\cdot(\xv_a+\xv_b)/2}\nonumber\\
  &\equiv \[\bit F(\kv_-)-F(\kv_+)\]e^{\i\nv\cdot(\xv_a+\xv_b)/2} \ .\label{eq:Chk}
\end{align}
with $\s\equiv s+\i\om_\nv$. Further,
\begin{align}
&\Rcal (\dC_\nv)     =\nonumber\\
&\hspace{.3em}  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\!\times\!\(\nablav_a \Del_{a}^{-1}+\nablav_b \Del_{b}^{-1}\) \dC\]_{\xv_a=\xv_b}\nonumber\\
%&  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\times\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) \int\frac{\df^2\kv}{(2\pi)^2} \hat{C}^{\textrm{(h)}}(\kv) e^{\i\kv\cdot(\xv_a-\xv_b)} \]_{\xv_a=\xv_b}\nonumber\\
&\hspace{.3em}  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\!\times\!\(\nablav_a \Del_{a}^{-1}+\nablav_b \Del_{b}^{-1}\) \int\!\frac{\df^2\kv}{(2\pi)^2} \[\bit F(\kv_-)-F(\kv_+)\] e^{\i\nv\cdot(\xv_a+\xv_b)/2}e^{\i\kv\cdot(\xv_a-\xv_b)} \]_{\xv_a=\xv_b}\nonumber\\
%&  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\times \iint\frac{\df^2\kv}{(2\pi)^2} \(\frac{\i \kv_+}{-k^2_{\la+}}-\frac{\i \kv_-}{-k^2_{\la-}} \)\[\bit F(\kv_-)-F(\kv_+)\] e^{\i (\kv_+\cdot \xv_a-\kv_-\xv_b)} \]_{\xv_a=\xv_b}\nonumber\\
&\hspace{.3em}  =-\nablav\cdot \int\!\frac{\df^2\kv}{(2\pi)^2} \frac{\hat{\mathbf{z}}}{2}\!\times\!\(\frac{\i \kv_-}{k^2_{-}}-\frac{\i \kv_+}{k^2_{+}} \)\[\bit F(\kv_-)-F(\kv_+)\] e^{\i \nv\cdot\xv}\ ,\label{eq:app8}
\end{align}
and since under the transformation $\kv\to-\kv$ we have that $\kv_+ \to- \kv_-$, $k^2_{+} \to k^2_{-}$ and $F(\kv_+)\to -F(\kv_-)$,~\eqref{eq:app8} becomes
\begin{align}
\Rcal (\dC_\nv)    &   =-\nablav\cdot \int\!\frac{\df^2\kv}{(2\pi)^2}\, \hat{\mathbf{z}}\times\(\frac{\i \kv_-}{k^2_{-}}-\frac{\i \kv_+}{k^2_{+}} \)\, F(\kv_-)  e^{\i \nv\cdot\xv}~.\label{eq:RdC_prefinal}
\end{align}
Using $\nablav\cdot\( \hat{\mathbf{z}}\times\pv\,e^{\i\nv\cdot\xv}\) = -\i\,\hat{\mathbf{z}}\cdot(\nv\times\pv)\,e^{\i\nv\cdot\xv}$, we then obtain,
\begin{align}
\Rcal (\dC_\nv)  &   = \int\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2_{+}} -\frac1{k^2_{-}}\)\, F(\kv_-)  e^{\i \nv\cdot\xv} \nonumber\\
%& = \d\tilde Q\iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2_{s}} -\frac1{k^2}\)\, F(\kv)   \nonumber\\
&   =\dZ \int\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{s}}-\dfrac1{k^2} \)\(\dfrac1{k^2}-\dfrac1{n^2}\)}{\s+2+ \nu_{2h} (k^{2h}_s + k^{2h}) +\i \(  \om_{\kv+\nv}- \om_{\kv} - \om_\nv\)}  \frac{\e\hat{Q}(\kv)}{2}\ ,\label{eq:RdC_efdZ}
\end{align}
with $\kv_s\equiv \kv+\nv$ and $k_s\equiv|\kv_s|$. The last equality was obtained with the substitution $\kv\to\kv-\nv/2$. For $\nu_{2h}=0$~\eqref{eq:RdC_efdZ} gives~\eqref{eq:f_factor}. Finally, using~\eqref{eq:s3t_pert_dZ_s} we obtain the dispersion relation for the stability
of the homogeneous equilibrium:
\begin{align}
\s + 1 + \nu_{2h} n^{2h} &=\e \int\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{s}}-\dfrac1{k^2} \)\(\dfrac1{k^2}-\dfrac1{n^2}\)}{\s+2+ \nu_{2h} (k^{2h}_s + k^{2h}) +\i \(  \om_{\kv+\nv}- \om_{\kv}  - \om_\nv\)}  \frac{\hat{Q}(\kv)}{2} \ .\label{eq:s3tgr}
%&= \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(k^2_{s}-k^2\)\(k^2-n^2\)\,\hat{C}^e(\kv)}{k_{s}^2k^4 n^2 \[\s+2r + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)\bit\]}  
\end{align}


Equation~\eqref{eq:s3tgr} can be written in terms of the real and
imaginary part of the eigenvalue $s$ as:\begin{subequations}
\begin{align}
s_r&=-1+\varepsilon\,\real[f(\s)] ~,\label{eq:s3t_slanted_real}\\
s_i&=-\om_\nv+\varepsilon\,\imag[f(\s)]~.\label{eq:s3t_slanted_imag}
\end{align}\label{eq:s3t_slanted}\end{subequations}
The real part of the eddy feedback contributes to the growth rate of the mean flow and the imaginary part determines the departure of the phase speed of the mean flow from the Rossby wave frequency. For $\b\gg1$ the marginally unstable eigenfunctions have $\s_i=-\om_\nv$ as it can be readily shown that $f_i$ is at most of $\mathcal{O}(1)$ and therefore produces only a small correction to the Rossby phase speed which is of $\mathcal{O}(\b)$.


Equation~\eqref{eq:s3tgr} is solved numerically for $\s$ for a given $\nv$, $\b$, $\e$ and $\hat{Q}(\kv)$. However, in some special cases $\s$ can be solved in closed form. Such an example is when $\b=0$ and with $\nu_{2h}=0$. Then~\eqref{eq:s3tgr} takes the form:
\be
(s + 1)(s+2) =\e \underbrace{\int \frac{\df^2 \kv}{(2\pi)^2}\;\frac{|\mathbf{k}\times{\mathbf{n}}|^2\, (k^2_s-k^2) (k^2-n^2) }{k^4 k^2_s n^2 }\frac{\hat{Q}(\kv)}{2}}_{J}\equiv\e\, J\ ,\label{eq:s3tgr_b0}
\ee
and the eigenvalues are $s=-3/2\pm\(1/4+\e J\)^{1/2}$. The value of the integral, $J$, depends only on the wavevector $\nv$ and the forcing spectrum. For the ring forcing spectrum~\eqref{eq:Qhat_deltaG} and by using the definitions of Fig.~\ref{fig:einx_angles},
\begin{align}
|\mathbf{k}\times{\mathbf{n}}|^2 &= n^2\cos^2\thet\ ,\ \ k_s^2 = 1+n^2+2n\sin\thet\ ,\label{eq:defs_inangles}
\end{align}
 $J$ takes the form:
\begin{align}
J&=  \int\limits_{0}^{2\pi}\frac{\df \thet}{2\pi} \frac{2n\(1-n^2\)\,\cos^2{\thet} (\sin\thet+n/2) }{1 +n^2+2n\sin{\thet} }   \,\Gcal(\thet-\varphi)\nonumber\\
&=\frac{\mu}{4} n^2(1-n^2)\,\cos(2\varphi)\ ,\ \ \text{for }n\le 1\ .
\end{align}
For isotropic forcing $J=0$ and there is no instability since $\s=-1$ or $\s=-2$. When $\mu\ne0$ we have instability when $\e\ge 32/[\mu\cos(2\phi)]>0$, which occurs either when $\mu>0$ and $0\le \phi<45\deg$ or when $\mu<0$ and $45\deg<\phi\le 90\deg$.





\section{Derivation of expression for $\fr$ for the ring forcing spectrum}
\label{appsec:fr_theta_phi_n}

In this section we will derive the expression~\eqref{eq:fr} for $\fr\equiv\real\[f(0)\]$ for the ring forcing spectrum~\eqref{eq:Qhat_deltaG}. For $\nu_{2h}=0$, $\s=0$ and for spectrum~\eqref{eq:Qhat_deltaG} we have that
\begin{align}
 f(0) &= \int\frac{k\df k\df \thet}{(2\pi)^2} \frac{|\mathbf{k}\times{\mathbf{n}}|^2\, (k^2_s-k^2) (k^2-n^2) }{k^4 k^2_s n^2  \[ 2 +\i\( \om_{\kv+\nv}- \om_{\nv} - \om_{\kv} \)\bit \] }  \,2\pi\,\Gcal(\thet-\varphi)\,\d(k-1)\nonumber\\
 &= \int\limits_{0}^{2\pi}\frac{\df \thet}{2\pi} \frac{|\mathbf{k}\times{\mathbf{n}}|^2\, (k^2_s-1) (1-n^2) }{k^2_s n^2  \[ 2 +\i\( \om_{\kv+\nv}- \om_{\nv} - \om_{\kv} \)\bit \] }   \,\Gcal(\thet-\varphi)\ .
\end{align}
Again using the definitions of Fig.~\ref{fig:einx_angles} we have:
\begin{align}
\om_\nv = -\b \sin\varphi/n \ ,\ \ \om_\kv = -\b \cos(\thet-\varphi) \ ,\ \ \om_{\kv+\nv} = -\b \frac{n\sin\varphi+\cos(\thet-\varphi)}{1+n^2+2n\sin\thet}\ .
\end{align}
and together with~\eqref{eq:defs_inangles} we have that
\begin{align}
\fr &=\real\[\f(0)\bit\]  = \real\(\spa\right.\int\limits_{0}^{2\pi} { \frac{\Ncal}{\Dcal_0 +\i\b\,\Db }}\df \thet\left.\spa \)\nonumber\\
&=\int\limits_{0}^{2\pi}\frac{\Ncal\,\Dcal_0}{ \Dcal_0^2 + \b^2\,\Db^2 }\,\df \thet\equiv\int\limits_{0}^{2\pi} F(\thet,\nv)\,\df \thet\ ,\label{eq:dvz}
\end{align}
with $F(\thet,\nv)$ defined by~\eqref{eq:defF} and
\begin{subequations}
\begin{align}
\Dcal_0(\thet,\nv)&=2(1 +n^2+2n\sin{\thet})~,\\
%\Db(\thet,n)&=\sin{\varphi}/n+(1+n^2)\cos{(\thet-\varphi)} - \cos{(\thet+\varphi)} + 2n\sin\thet\cos(\thet-\varphi)~,\\
%\Db(\thet,n)&=\sin{\varphi}/n+\cos{(\thet-\varphi)}\(1+n^2+2n\sin{\thet}\) - \cos{(\thet+\varphi)}~,\\
\Db(\thet,\nv)&=(1 +n^2+2n\sin{\thet})\sin{\varphi}/n+n^2\cos{(\thet-\varphi)} + n \sin{(2\thet-\varphi)}~,\\
%\Db(\thet,n)&=(1 +n^2+2n\sin{\thet})\[\frac{\sin{\varphi}}{n} + \cos{(\thet-\varphi)} - \frac{\cos{(\thet-\varphi)} + n\sin{\varphi}}{1 +n^2+2n\sin{\thet}}\]~,\\
%N(\thet)&=4\pi n\(1-n^2\)\,\cos^2{\thet} (\st+n/2) \left\{ 1-\mu \cos[2(\thet-\varphi)] \bit\right\}\,D_0(\thet)~,
\Ncal(\thet,\nv)&= \frac1{\pi}\, n\(1-n^2\)\,\cos^2{\thet} (\sin\thet+n/2) \, \mathcal{G}(\thet-\varphi) ~.\label{eq:defNcal}\end{align}\label{eq:defD0DbN}\end{subequations}

Note that $\b\Db$ is 
\be
\b\,\Db(\thet,\nv)= k^2_s (\om_{\kv+\nv}-\om_{\nv}-\om_{\kv})~,\label{eq:D2zero}
\ee
and therefore vanishing of $\Db$ occurs when the resonant condition is satisfied:
\be
\om_{\nv}+\om_{\kv}=\om_{\kv+\nv}~.\label{eq:res}
\ee 

Also note that the $F$ defined by~\eqref{eq:defF} remains unchanged when the angle $\varphi$ is shifted by
$180\deg$ ($\varphi\to180\deg+\varphi$) or when there is a simultaneous shift of $\varphi\to180\deg-\varphi$
and $\thet\to180\deg-\thet$. As a result, it suffices to only consider cases with $0\le\varphi\le 90\deg$.



%
\begin{comment}

\vspace{10em}


and satisfy
\begin{align}
\s \,\d \tilde{Q} &+ J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d\tilde C  )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\,\d \tilde{Q}\ ,\label{eq1}\\
\s \,\d \tilde{C} & = \(\bit\Acal^e_a + \Acal^e_b \)\d \tilde C +\(\bit\d\tilde\Acal_a + \d\tilde\Acal_b\)C^e\ ,\label{eq2}
\end{align}
with
\begin{align}
\d\Acal&=-\d\Uv\cdot\nablav + \[\bit(\Del_\la\,\d\Uv)\cdot\nablav \]\Del^{-1}_\la ~
\end{align}

Since $\d\tilde Q=e^{\i\nv\cdot\xv}$ we have
\be
\d\tilde\Psi = -\frac{\d\tilde Q}{n^2+\la^2}~,~\d\tilde U = \frac{\i n_y \d\tilde Q}{n^2+\la^2}~,~\d\tilde V = -\frac{\i n_x\,\d\tilde Q}{n^2+\la^2}~.
\ee

{\color{red} Define Rossby wave frequency as:
\be
\om_{\kv} = \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k^2+\la^2} \equiv  \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k_\la^2}
\ee
}

Calculate each term of~\eqref{eq1} and \eqref{eq2}.

\begin{enumerate}
\item
\be\boxed{
J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \frac{\i(\b_x n_y-\b_y n_x)}{n^2+\la^2}\d\tilde Q = \i\om_{\nv}\d\tilde Q }
\ee
\item
\be\boxed{
\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\,\d \tilde{Q}= \[ r+\nu_{2h} n^{2h}\]\d\tilde Q  }
\ee
\item
\begin{align}
\[ 2r+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C=?
\end{align}
We have that
\begin{align}
\nablav_a \,\d\tilde C &= \nablav_a \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
&= \iint\frac{\df^2\kv}{(2\pi)^2} (\i\kv_+)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
\nablav_b \, \d\tilde C &= \nablav_b \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
&= \iint\frac{\df^2\kv}{(2\pi)^2} (-\i\kv_-)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with $\kv_{\pm} = \kv\pm\nv/2$. Therefore $\[ 2r+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C$ translated in wavenumber space as
\begin{align}
\[ 2r+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C &=  \iint\frac{\df^2\kv}{(2\pi)^2} \[ 2r + \nu_{2h} (k^{2h}_+ + k^{2h}_-)\]\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\end{align}
or 
\begin{align}
\[ 2r+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C &\leftrightarrow  \[ 2r + \nu_{2h} (k^{2h}_+ + k^{2h}_-)\]\hat{C}^{\textrm{(h)}}(\kv)
\end{align}
\item
\begin{align}
& \[\bit\hat{\mathbf{z}}\cdot(\bv\times\nablav_a) \Del^{-1}_{\la,a}+\hat{\mathbf{z}}\cdot(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\d\tilde C= \nonumber\\
%&\qquad= \hat{\mathbf{z}}\cdot \[\bit(\bv\times\nablav_a) \Del^{-1}_{\la,a}+(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\Del_{\la,a}\Del_{\la,b}\d\tilde S ~\nonumber\\
% &\qquad=  \hat{\mathbf{z}}\cdot\[\bit(\bv\times\nablav_a) \Del_{\la,b}+(\bv\times\nablav_b) \Del_{\la,a}\] \d\tilde S \leftrightarrow~\\
 &\leftrightarrow \hat{\mathbf{z}}\cdot\[\i\bit(\bv\times \kv_{+} ) /(-k^2_{\la+})-\i\bit(\bv\times \kv_{-} ) /(-k^2_{\la-})\] \hat{C}^{\textrm{(h)}}(\kv)\\
% &\qquad=  -\i k^2_{\la+} k^2_{\la-}\, \hat{\mathbf{z}}\cdot\[\bit(\bv\times \kv_{+} )/k^2_{\la+} -\bit(\bv\times \kv_{-} )/ k^2_{\la-} \] \hat{S}^{\textrm{(h)}}(\kv)\\
 &\qquad=  -\i \, \( \om_{\kv_+} - \om_{\kv_-} \) \hat{C}^{\textrm{(h)}}(\kv)
\end{align}

Therefore
\be
\boxed{(\Acal^e_a+\Acal^e_b)\d\tilde C \leftrightarrow \[\bit- 2r - \nu_{2h} (k^{2h}_+ + k^{2h}_-) -\i \, \( \om_{\kv_+} - \om_{\kv_-} \)\] \hat{C}^{\textrm{(h)}}(\kv)}
\ee
\end{enumerate}


Some useful identities:
\begin{align}
\uv\cdot\nablav F &= J(\psi,F) = \hat{\mathbf{z}}\cdot(\nablav\psi\times\nablav F)\\
(\Del_\la\uv)\cdot\nablav F &= J(q,F) = \hat{\mathbf{z}}\cdot(\nablav q\times\nablav F)
\end{align}
Using these we calculate the term $(\d\Acal_a+\d\Acal_b) C^e$.

\begin{enumerate}
\item
\begin{align}
(\d\Uv_a\cdot\nablav_a) C^e &= J_a(\d\tilde \Psi_a,C^e)\nonumber\\
&= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)
\end{align}
we have that $\nablav_a\d\tilde \Psi_a = -\i\nv/(n^2_\la)\,e^{\i\nv\cdot\xv_a}$, where $n^2_\la = n^2+\la^2$ and therefore
\begin{align}
(\d\Uv_a\cdot\nablav_a) C^e &= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)\nonumber\\
&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}(\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{n^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{n^2_\la}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
\end{align}
\item similarly
\begin{align}
(\d\Uv_b\cdot\nablav_b) C^e &= \hat{\mathbf{z}}\cdot (\nablav_b\d\tilde \Psi_b\times\nablav_b C^E)\nonumber\\
&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}(-\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{n^2_\la}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
\end{align}
\item
\begin{align}
\[\bit(\Del_{\la,a}\d\Uv_a)\cdot\nablav_a\]\Del_{\la,a}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_a\d\tilde Q_a\times\nablav_a \Del_{\la,a}^{-1}C^e)\nonumber\\
&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{k^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{k^2_{\la-}}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
\end{align}
\item and similarly
\begin{align}
\[\bit(\Del_{\la,b}\d\Uv_b)\cdot\nablav_b\]\Del_{\la,b}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_b\d\tilde Q_b\times\nablav_b \Del_{\la,b}^{-1}C^e)\nonumber\\
&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{k^2_{\la+}}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
\end{align}
\end{enumerate}


Therefore
\begin{empheq}[box=\fbox]{align}
&(\d\Acal_a+\d\Acal_b) C^e = \nonumber\\
&\hspace{2em}=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\iint\frac{\df^2\kv}{(2\pi)^2}\[\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\frac1{k^2_{\la-}}-\frac1{n^2_\la}\)\,\hat{C}^e(\kv_-)-\right.\nonumber\\
&\hspace{15em}\left.-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\frac1{k^2_{\la+}}-\frac1{n^2_\la}\)\,\hat{C}^e(\kv_+)\]\,e^{\i\kv\cdot(\xv_a-\xv_b)} 
\end{empheq}


We are now in the position to solve the perturbation covariance equation and obtain $\hat{C}^{\textrm{(h)}}(\kv)$ as

\begin{empheq}[box=\fbox]{align}
&\hat{C}^{\textrm{(h)}}(\kv)=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\times\nonumber\\
 &\vspace{2em}\times\dfrac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\dfrac1{k^2_{\la-}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv_-)-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\dfrac1{k^2_{\la+}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv_+)}{\s+2r + \nu_{2h} (k^{2h}_+ + k^{2h}_-) -\i \, \( \om_{\kv_-} - \om_{\kv_+}\)}\nonumber\\
  &\vspace{1em}\equiv e^{\i\nv\cdot(\xv_a+\xv_b)/2} \[\bit F(\kv_-)-F(\kv_+)\]
\end{empheq}


How much is $\Rcal (\dC)$ ?

\begin{align}
&\Rcal (\dC)     =\nonumber\\
&\hspace{.3em}  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\!\times\!\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) \dC\]_{\xv_a=\xv_b}\nonumber\\
%&  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\times\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) \iint\frac{\df^2\kv}{(2\pi)^2} \hat{C}^{\textrm{(h)}}(\kv) e^{\i\kv\cdot(\xv_a-\xv_b)} \]_{\xv_a=\xv_b}\nonumber\\
&\hspace{.3em}  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\!\times\!\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) \iint\!\frac{\df^2\kv}{(2\pi)^2} \[\bit F(\kv_-)-F(\kv_+)\] e^{\i\nv\cdot(\xv_a+\xv_b)/2}e^{\i\kv\cdot(\xv_a-\xv_b)} \]_{\xv_a=\xv_b}\nonumber\\
%&  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\times \iint\frac{\df^2\kv}{(2\pi)^2} \(\frac{\i \kv_+}{-k^2_{\la+}}-\frac{\i \kv_-}{-k^2_{\la-}} \)\[\bit F(\kv_-)-F(\kv_+)\] e^{\i (\kv_+\cdot \xv_a-\kv_-\xv_b)} \]_{\xv_a=\xv_b}\nonumber\\
&\hspace{.3em}  =-\nablav\cdot \iint\!\frac{\df^2\kv}{(2\pi)^2} \frac{\hat{\mathbf{z}}}{2}\!\times\!\(\frac{\i \kv_-}{k^2_{\la-}}-\frac{\i \kv_+}{k^2_{\la+}} \)\[\bit F(\kv_-)-F(\kv_+)\] e^{\i \nv\cdot\xv}
\end{align}
Moreover, since under $\kv\to-\kv$ we have that $\kv_+ \to- \kv_-$, $k^2_{\la+} \to k^2_{\la-}$ and $F(\kv_+)\to -F(\kv_-)$ we get that 
\begin{align}
\Rcal (\dC)    &   =-\nablav\cdot \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\times\(\frac{\i \kv_-}{k^2_{\la-}}-\frac{\i \kv_+}{k^2_{\la+}} \)\, F(\kv_-)  e^{\i \nv\cdot\xv}~.
\end{align}
It is easy to derive that for any vector $\pv$,
\be
\nablav\cdot\( \hat{\mathbf{z}}\times\pv\,e^{\i\nv\cdot\xv}\) = -\i\,\hat{\mathbf{z}}\cdot(\nv\times\pv)\,e^{\i\nv\cdot\xv}\ ,
\ee
and therefore
\begin{align}
\Rcal (\dC)  &   = \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2_{\la,+}} -\frac1{k^2_{\la,-}}\)\, F(\kv_-)  e^{\i \nv\cdot\xv} \nonumber\\
& = \d\tilde Q\iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2_{\la,s}} -\frac1{k^2_{\la}}\)\, F(\kv)   \nonumber\\
&   =\d\tilde Q \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv)}{\s+2r + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  
\end{align}

Using the above we find that from the mean flow perturbation equation $\s$ must satisfy:
\begin{align}
\sigma + r + \nu_{2h} n^{2h} + \i\om_{\nv}&= \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv)}{\s+2r + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  \\
&= \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(k^2_{\la,s}-k^2_{\la}\)\(k^2_{\la}-n^2_\la\)\,\hat{C}^e(\kv)}{k_{\la,s}^2k_{\la}^4 n_\la^2 \[\s+2r + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)\bit\]}  
\end{align}





\subsection{dissipate only kinetic energy, $-r\Delta\psi$}
We will write with red only the differences from $- rq$. 

For the NL system:
\begin{align}
\partial_t q + J(\psi,q) + \beta v  =\xi +\textrm{Diss}
\end{align}
with
\begin{align}
\textrm{Diss}&= - r \textcolor{red}{\Delta \psi} - (-1)^h\nu_{2h} \Delta^{h}\textcolor{red}{\Delta \psi} = -\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Delta \psi}\ \\
q &=\Delta \psi - \lambda^2 \psi~~,~~u =-\partial_y \psi ~~,~~v= \partial_x \psi~.
\end{align}
$h=1$ is diffusion, $h>1$ hyperdiffusion

Define $q=Q+q'$, etc. Then
\begin{align}
&\partial_t Q + J(\Psi,Q + \bv\cdot\xv) =- r \textcolor{red}{\Del\Psi} - (-1)^h\nu_{2h}  \Delta^{h}\textcolor{red}{\Del\Psi} - \Tcal[ J(\psi',q') ]~\\
&\partial_t q' = \Acal(\Uv) \,q' + f_{\textrm{nl}} + \xi
\end{align}
with
\begin{align}
\Acal(\Uv)&=-\Uv\cdot\nablav + \[\bit(\Del_\la\Uv)\cdot\nablav + \hat{\mathbf{z}}\cdot(\bv\times\nablav)\]\Del^{-1}_\la - \[r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Del\Del_\la^{-1}}~\\
f_{\textrm{nl}}&=\Tcal[ J(\psi',q') ]-J(\psi',q')
\end{align}

Eddy vorticity covariance is again $C(\xv_a,\xv_b,t)=\<q'(\xv_a,t)q'(\xv_b,t)\>$ and using the ergodic hypothesis $\Tcal(\bullet) = \<\bullet\>$ the Reynolds stress divergence can be expressed as:
\begin{align}
 -\Tcal[ J(\psi',q') ]&=-\nablav\cdot \<(\uv'\,q')\>\\
    &  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\times\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) C\]_{\xv_a=\xv_b}\nonumber\\
  &\equiv \Rcal(C)\ .
\end{align}


S3T system is
\begin{align}
\partial_t \, Q &+ J \(\Psi,Q+ {\bm\beta}\cdot\mathbf{x} \) = \Rcal( C )-\[r+(-1)^{h}\nu_{2h} \Del^h\]\,\textcolor{red}{\Del\Del_\la^{-1}}Q\ ,\\
\partial_t \, C & = \[\bit\Acal_a(\Uv) + \Acal_b(\Uv) \] C +\varepsilon\,Q\ ,
\end{align}

Consider a homogeneous, stationary equilibrium solution, $Q^e$, $C^e(\xv_a-\xv_b)$. Expanding $C^e$ as
\be
C^e(\xv_a-\xv_b) = \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}
\ee
(and similarly for $Q(\xv_a-\xv_b)$), we find that
\be
\textcolor{red}{\hat{C}^e(\kv) }= \frac{\varepsilon\,\hat{Q}(\kv)}{2(r+\nu_{2h} k^{2h})}\textcolor{red}{\frac{k^2_\la}{k^2}}\ ,
\ee

Perturbations $\d Q$, $\d C$ about this equilibrium satisfy:
\begin{align}
\partial_t \,\d Q &+ J \(\d\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d C )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\,\textcolor{red}{\Del\Del_\la^{-1}}\d Q\ ,\label{eq1}\\
\partial_t \,\d C & = \(\bit\Acal^e_a + \Acal^e_b \)\d C +\(\bit\d\Acal_a + \d\Acal_b\)C^e\ ,\label{eq2}
\end{align}


The spatial component of the eigenfunction, $\d Q = \d\tilde{Q}\,e^{\s t}$, $\d C = \d\tilde{C}\,e^{\s t}$ about the homogeneous equilibrium are
\begin{align}
\d\tilde{Q}(\xv) &= e^{\i\nv\cdot\xv} ~\\
\d\tilde{C}(\xv_a,\xv_b) &= C^{\textrm{(h)}}(\xv_a-\xv_b)\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with
\be
C^{\textrm{(h)}}(\xv_a-\xv_b) = \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}
\ee
and satisfy
\begin{align}
\s \,\d \tilde{Q} &+ J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d\tilde C  )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Del\Del_\la^{-1}}\d \tilde{Q}\ ,\label{eq1}\\
\s \,\d \tilde{C} & = \(\bit\Acal^e_a + \Acal^e_b \)\d \tilde C +\(\bit\d\tilde\Acal_a + \d\tilde\Acal_b\)C^e\ ,\label{eq2}
\end{align}
with
\begin{align}
\d\Acal&=-\d\Uv\cdot\nablav + \[\bit(\Del_\la\,\d\Uv)\cdot\nablav \]\Del^{-1}_\la ~
\end{align}

Since $\d\tilde Q=e^{\i\nv\cdot\xv}$ we have
\be
\d\tilde\Psi = -\frac{\d\tilde Q}{n^2+\la^2}~,~\d\tilde U = \frac{\i n_y \d\tilde Q}{n^2+\la^2}~,~\d\tilde V = -\frac{\i n_x\,\d\tilde Q}{n^2+\la^2}~.
\ee

 Define Rossby wave frequency as:
\be
\om_{\kv} = \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k^2+\la^2} \equiv  \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k_\la^2}
\ee

Calculate each term of~\eqref{eq1} and \eqref{eq2}.

\begin{enumerate}
\item
\be\boxed{
J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \frac{\i(\b_x n_y-\b_y n_x)}{n^2+\la^2}\d\tilde Q = \i\om_{\nv}\d\tilde Q }
\ee
\item
\be\boxed{
\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Del\Del_\la^{-1}}\d \tilde{Q}= \[ r+\nu_{2h} n^{2h}\]\textcolor{red}{(n^2/n^2_\la)}\d\tilde Q  }
\ee
\item
\begin{align}
\[ 2r\textcolor{red}{(\Del_a\Del_{\la,a}^{-1}+\Del_b\Del_{\la,b}^{-1})}+(-1)^h\nu_{2h} (\Delta_a^{h}\textcolor{red}{\Del_a\Del_{\la,a}^{-1}}+\Delta_b^{h}\textcolor{red}{\Del_b\Del_{\la,b}^{-1}})\]\d\tilde C=?
\end{align}
We have that
\begin{align}
\nablav_a \,\d\tilde C &= \iint\frac{\df^2\kv}{(2\pi)^2} (\i\kv_+)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
\nablav_b \, \d\tilde C &= \iint\frac{\df^2\kv}{(2\pi)^2} (-\i\kv_-)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with $\kv_{\pm} = \kv\pm\nv/2$. Therefore $\[ 2r\textcolor{red}{(\Del_a\Del_{\la,a}^{-1}+\Del_b\Del_{\la,b}^{-1})}+(-1)^h\nu_{2h} (\Delta_a^{h}\textcolor{red}{\Del_a\Del_{\la,a}^{-1}}+\Delta_b^{h}\textcolor{red}{\Del_b\Del_{\la,b}^{-1}})\]\d\tilde C$ translated in wavenumber space as
\begin{align}
&\[ 2r\textcolor{red}{(\Del_a\Del_{\la,a}^{-1}+\Del_b\Del_{\la,b}^{-1})}+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C \leftrightarrow \nonumber\\
&\qquad\leftrightarrow \[ 2r\textcolor{red}{(k^2_+/ k^2_{\la,+} + k^2_-/ k^2_{\la,-})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_+/k^2_{\la,+} + k^{2h+2}_-/k^2_{\la,-}})\]\hat{C}^{\textrm{(h)}}(\kv)
\end{align}
\item
\begin{align}
& \[\bit\hat{\mathbf{z}}\cdot(\bv\times\nablav_a) \Del^{-1}_{\la,a}+\hat{\mathbf{z}}\cdot(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\d\tilde C= \nonumber\\
%&\qquad= \hat{\mathbf{z}}\cdot \[\bit(\bv\times\nablav_a) \Del^{-1}_{\la,a}+(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\Del_{\la,a}\Del_{\la,b}\d\tilde S ~\nonumber\\
% &\qquad=  \hat{\mathbf{z}}\cdot\[\bit(\bv\times\nablav_a) \Del_{\la,b}+(\bv\times\nablav_b) \Del_{\la,a}\] \d\tilde S \leftrightarrow~\\
 &\leftrightarrow \hat{\mathbf{z}}\cdot\[\i\bit(\bv\times \kv_{+} ) /(-k^2_{\la+})-\i\bit(\bv\times \kv_{-} ) /(-k^2_{\la-})\] \hat{C}^{\textrm{(h)}}(\kv)\\
% &\qquad=  -\i k^2_{\la+} k^2_{\la-}\, \hat{\mathbf{z}}\cdot\[\bit(\bv\times \kv_{+} )/k^2_{\la+} -\bit(\bv\times \kv_{-} )/ k^2_{\la-} \] \hat{S}^{\textrm{(h)}}(\kv)\\
 &\qquad=  -\i \, \( \om_{\kv_+} - \om_{\kv_-} \) \hat{C}^{\textrm{(h)}}(\kv)
\end{align}

Therefore
\be
\boxed{(\Acal^e_a+\Acal^e_b)\d\tilde C \leftrightarrow \[\bit- 2r \textcolor{red}{(k^2_+/ k^2_{\la,+} + k^2_-/ k^2_{\la,-})}- \nu_{2h} (\textcolor{red}{k^{2h+2}_+/k^2_{\la,+} + k^{2h+2}_-/k^2_{\la,-}}) -\i \, \( \om_{\kv_+} - \om_{\kv_-} \)\] \hat{C}^{\textrm{(h)}}(\kv)}
\ee
\end{enumerate}


Some useful identities:
\begin{align}
\uv\cdot\nablav F &= J(\psi,F) = \hat{\mathbf{z}}\cdot(\nablav\psi\times\nablav F)\\
(\Del_\la\uv)\cdot\nablav F &= J(q,F) = \hat{\mathbf{z}}\cdot(\nablav q\times\nablav F)
\end{align}
Using these we calculate the term $(\d\Acal_a+\d\Acal_b) C^e$. Everything is the same, except $C^e$.
%
%\begin{enumerate}
%\item
%\begin{align}
%(\d\Uv_a\cdot\nablav_a) C^e &= J_a(\d\tilde \Psi_a,C^e)\nonumber\\
%&= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)
%\end{align}
%we have that $\nablav_a\d\tilde \Psi_a = -\i\nv/(n^2_\la)\,e^{\i\nv\cdot\xv_a}$, where $n^2_\la = n^2+\la^2$ and therefore
%\begin{align}
%(\d\Uv_a\cdot\nablav_a) C^e &= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}(\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{n^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
%\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{n^2_\la}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\item similarly
%\begin{align}
%(\d\Uv_b\cdot\nablav_b) C^e &= \hat{\mathbf{z}}\cdot (\nablav_b\d\tilde \Psi_b\times\nablav_b C^E)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}(-\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{n^2_\la}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\item
%\begin{align}
%\[\bit(\Del_{\la,a}\d\Uv_a)\cdot\nablav_a\]\Del_{\la,a}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_a\d\tilde Q_a\times\nablav_a \Del_{\la,a}^{-1}C^e)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{k^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
%\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{k^2_{\la-}}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\item and similarly
%\begin{align}
%\[\bit(\Del_{\la,b}\d\Uv_b)\cdot\nablav_b\]\Del_{\la,b}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_b\d\tilde Q_b\times\nablav_b \Del_{\la,b}^{-1}C^e)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{k^2_{\la+}}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\end{enumerate}
Therefore
\begin{empheq}[box=\fbox]{align}
&(\d\Acal_a+\d\Acal_b) \textcolor{red}{C^e} = \nonumber\\
&\hspace{2em}=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\iint\frac{\df^2\kv}{(2\pi)^2}\[\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\frac1{k^2_{\la-}}-\frac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_-)}-\right.\nonumber\\
&\hspace{15em}\left.-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\frac1{k^2_{\la+}}-\frac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_+)}\]\,e^{\i\kv\cdot(\xv_a-\xv_b)} 
\end{empheq}


We are now in the position to solve the perturbation covariance equation and obtain $\hat{C}^{\textrm{(h)}}(\kv)$ as

\begin{empheq}[box=\fbox]{align}
&\hat{C}^{\textrm{(h)}}(\kv)=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\times\nonumber\\
 &\vspace{2em}\times\dfrac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\dfrac1{k^2_{\la-}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_-)}-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\dfrac1{k^2_{\la+}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_+)}}{\s+2r\textcolor{red}{(k^2_+/ k^2_{\la,+} + k^2_-/ k^2_{\la,-})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_+/k^2_{\la,+} + k^{2h+2}_-/k^2_{\la,-}}) -\i \, \( \om_{\kv_-} - \om_{\kv_+}\)}\nonumber\\
  &\vspace{1em}\equiv e^{\i\nv\cdot(\xv_a+\xv_b)/2} \[\bit F(\kv_-)-F(\kv_+)\]
\end{empheq}


How much is $\Rcal (\d C)$ ?

\begin{align}
\Rcal (\d C)    &   =-\nablav\cdot \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\times\(\frac{\i \kv}{k^2_{\la}}-\frac{\i (\kv+\nv)}{k^2_{\la,s}} \)\, \textcolor{red}{F(\kv)}  e^{\i \nv\cdot\xv} \nonumber\\
\end{align}

Now after some algebra we get that:
\begin{align}
\nablav\cdot\( \hat{\mathbf{z}}\times\kv\,e^{\i\nv\cdot\xv}\) &= -\i\hat{\mathbf{z}}\cdot(\nv\times\kv)\\
\nablav\cdot\( \hat{\mathbf{z}}\times\nv\,e^{\i\nv\cdot\xv}\) &= 0
\end{align}
therefore
\begin{align}
\Rcal (\d C)  &   = \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2_{\la,s}} -\frac1{k^2_{\la}}\)\, \textcolor{red}{F(\kv)}  e^{\i \nv\cdot\xv} \nonumber\\
&   =\d\tilde Q \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv)}}{\s+2r\textcolor{red}{(k^2_s/ k^2_{\la,s} + k^2/ k^2_{\la})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_s/k^2_{\la,s} + k^{2h+2}/k^2_{\la}}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  
\end{align}

Using the above we find that from the mean flow perturbation equation $\s$ must satisfy:
\begin{align}
&\sigma + (r + \nu_{2h} n^{2h})\textcolor{red}{(n^2/n^2_\la)} + \i\om_{\nv}=\nonumber\\
&\qquad= \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv)}}{\s+2r\textcolor{red}{(k^2_s/ k^2_{\la,s} + k^2/ k^2_{\la})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_s/k^2_{\la,s} + k^{2h+2}/k^2_{\la}}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  \\
&\qquad=  \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(k^2_{\la,s}-k^2_{\la}\)\(k^2_{\la}-n^2_\la\)\,\textcolor{red}{(k^2_\la/k^2)}\,\hat{C}^{e,OLD}(\kv)}{k_{\la,s}^2k_{\la}^4 n_\la^2 \[\s+2r\textcolor{red}{(k^2_s/ k^2_{\la,s} + k^2/ k^2_{\la})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_s/k^2_{\la,s} + k^{2h+2}/k^2_{\la}}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)\bit\]}  
\end{align}










%
%
%
%
%\textcolor{green}{H E R E }
%
%
%
%the generalized S3T dispersion relation is:
%\begin{align}
%\sigma\, N^2_\la/N^2+& r + \nu_4 N^4 - \i\b m/N^2 =\intinf\intinf\frac{\df k}{2\pi}\frac{\df \l}{2\pi} \frac{\Ncal~(K^2/N^2-1)}{K^2_\la\(\sigma \Dcal_\sigma +  \Dcal_0 + \i\b\,\Dcal_\b\)}\,C^E(k,\l)
%\end{align}
%
%
%where $\<\xi_a\xi_b\>=\d(t_a-t_b) Q(x_a-x_b,y_a-y_b)$ and 
%\begin{subequations}
%\begin{align}
%C^E(k,\l)&=\frac{\varepsilon\,K^2_{\la} \,Q(k,\l) }{2 r K^2 + 2 \nu_4 K^6 }~,\\
%\Ncal &= 2(nk-m\l)\[\bit mn(k^2_+ - \l^2_+) - (m^2-n^2) k_+\l_+ \]=\nonumber\\
%&=(nk-m\l)^2 (K^2_s-K^2)~,\\
%\Dcal_\sigma &= K^2_\la K^2_{s,\la}~,\\
%\Dcal_0 &= r  \,(K^2 K^2_{s,\la} + K^2_{\la}K^2_{s}) + \nu_4  (K^6 K^2_{s,\la} + K^6_{s} K^2_{\la})~,\\
%\Dcal_\b &= k\,K^2_{s,\la} -(k+m)K^2_{\la}~.
%\end{align}
%\end{subequations}
%with
%\begin{subequations}
%\begin{align}
%N^2 = m^2+n^2~~&,~~N^2_\la = N^2+\la^2~,\\
%K^2 = k^2+\l^2~~&,~~K^2_\la = K^2+\la^2~,\\
%K^2_{s} = (k+m)^2+(\l+n)^2~~&,~~K^2_{s,\la} = K^2_{s}+\la^2~.
%\end{align}
%\end{subequations}
%%    B1 = K2la.^2.*Ks2la;
%%    B2 = r*K2la.*(K2.*Ks2la + K2la.*Ks2) + nu4*K2la.*(K2.^3.*Ks2la + Ks2.^3.*K2la);
%%    B3 = beta*K2la.*(k.*Ks2la -(k+m).*K2la);
%%        
%%    Denom = s*B1+B2+1i*B3 ;
%%    
%%    SP_f  =   A1    ./ Denom;
%


\end{comment}







==> chapters/app-S3Tgr_lambda.tex <==
% !TEX root = ../thesis.tex


\chapter{Calculation of the S3T growth rates for the homogeneous turbulent equilibrium}
\label{app:S3Tgr_lambda}

In this appendix we will calculate the eigenvalues of~\eqref{??}\textcolor{red}{??} about the homogeneous S3T equilibrium~\eqref{eq:hom_equil}. We will do the calculation including finite deformation radius, $1/\lambda$ (cf.~chapter~\ref{??}\textcolor{red}{??}). The infinite deformation radius case, as discussed in chapter~\ref{ch:st3hom} is recovered by setting $\lambda=0$.


Consider the NL system:
\begin{align}
\partial_t q + J\(\psi,\z- \lambda^2 \psi+\bv\cdot\xv\bit\) =\sqrt{\varepsilon}\xi +\textrm{Diss}
\end{align}
where $q=\Delta \psi - \lambda^2 \psi$ and the dissipation is taken to be
\begin{align}
\textrm{Diss}&=- r q - (-1)^h\nu_{2h} \Delta^{h}q\ .
\end{align}
Besides linear dissipation we have also included also dissipation of the form $-(-1)^h\nu_{2h} \Delta^{h}\,q$. For $h=1$ this is normal diffusion, while for $h>1$ is hyperdiffusion of order $2h$.

Define $q=Q+q'$, etc. Then
\begin{align}
&\partial_t Q + J(\Psi,Q + \bv\cdot\xv) =- \[ r+(-1)^h\nu_{2h} \Delta^{h}\] Q - \Tcal[ J(\psi',q') ]~\\
&\partial_t q' = \Acal(\Uv) \,q' + f_{\textrm{nl}} + \xi
\end{align}
with
\begin{align}
\Acal(\Uv)&=-\Uv\cdot\nablav + \[\bit(\Del_\la\Uv)\cdot\nablav + \hat{\mathbf{z}}\cdot(\bv\times\nablav)\]\Del^{-1}_\la - \[r+(-1)^h\nu_{2h} \Delta^{h}\]~\\
f_{\textrm{nl}}&=\Tcal[ J(\psi',q') ]-J(\psi',q')
\end{align}

After defining the eddy vorticity covariance as $C(\xv_a,\xv_b,t)=\<q'(\xv_a,t)q'(\xv_b,t)\>$ and using the ergodic hypothesis that $\Tcal(\bullet) = \<\bullet\>$, the Reynolds stress divergence can be expressed as: $\Rcal(C)=-\nablav\cdot\[\zhat\times \frac1{2}\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) C\]_{\xv_a=\xv_b}$ (cf.~\eqref{eq:def_Rcal}).


S3T system is
\begin{align}
\partial_t \, Q &+ J \(\Psi,Q+ {\bm\beta}\cdot\mathbf{x} \) = \Rcal( C )-\[r+(-1)^h\nu_{2h} \Delta^{h}\]Q\ ,\\
\partial_t \, C & = \[\bit\Acal_a(\Uv) + \Acal_b(\Uv) \] C +\varepsilon\,Q\ ,
\end{align}

Consider a homogeneous, stationary equilibrium solution, $Q^e$, $C^e(\xv_a-\xv_b)$. Expanding $C^e$ as
\be
C^e(\xv_a-\xv_b) = \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}
\ee
(and similarly for $Q(\xv_a-\xv_b)$), we find that
\be
\hat{C}^e(\kv) = \frac{\varepsilon\,\hat{Q}(\kv)}{2(r+\nu_{2h} k^{2h})}\ ,
\ee

Perturbations $\d Q$, $\d C$ about this equilibrium satisfy:
\begin{align}
\partial_t \,\d Q &+ J \(\d\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d C )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\,\d Q\ ,\label{eq1}\\
\partial_t \,\d C & = \(\bit\Acal^e_a + \Acal^e_b \)\d C +\(\bit\d\Acal_a + \d\Acal_b\)C^e\ ,\label{eq2}
\end{align}


The spatial component of the eigenfunction, $\d Q = \d\tilde{Q}\,e^{\s t}$, $\d C = \d\tilde{C}\,e^{\s t}$ about the homogeneous equilibrium are
\begin{align}
\d\tilde{Q}(\xv) &= e^{\i\nv\cdot\xv} ~\\
\d\tilde{C}(\xv_a,\xv_b) &= C^{\textrm{(h)}}(\xv_a-\xv_b)\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with
\be
C^{\textrm{(h)}}(\xv_a-\xv_b) = \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}
\ee
and satisfy
\begin{align}
\s \,\d \tilde{Q} &+ J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d\tilde C  )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\,\d \tilde{Q}\ ,\label{eq1}\\
\s \,\d \tilde{C} & = \(\bit\Acal^e_a + \Acal^e_b \)\d \tilde C +\(\bit\d\tilde\Acal_a + \d\tilde\Acal_b\)C^e\ ,\label{eq2}
\end{align}
with
\begin{align}
\d\Acal&=-\d\Uv\cdot\nablav + \[\bit(\Del_\la\,\d\Uv)\cdot\nablav \]\Del^{-1}_\la ~
\end{align}

Since $\d\tilde Q=e^{\i\nv\cdot\xv}$ we have
\be
\d\tilde\Psi = -\frac{\d\tilde Q}{n^2+\la^2}~,~\d\tilde U = \frac{\i n_y \d\tilde Q}{n^2+\la^2}~,~\d\tilde V = -\frac{\i n_x\,\d\tilde Q}{n^2+\la^2}~.
\ee

{\color{red} Define Rossby wave frequency as:
\be
\om_{\kv} = \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k^2+\la^2} \equiv  \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k_\la^2}
\ee
}

Calculate each term of~\eqref{eq1} and \eqref{eq2}.

\begin{enumerate}
\item
\be\boxed{
J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \frac{\i(\b_x n_y-\b_y n_x)}{n^2+\la^2}\d\tilde Q = \i\om_{\nv}\d\tilde Q }
\ee
\item
\be\boxed{
\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\,\d \tilde{Q}= \[ r+\nu_{2h} n^{2h}\]\d\tilde Q  }
\ee
\item
\begin{align}
\[ 2r+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C=?
\end{align}
We have that
\begin{align}
\nablav_a \,\d\tilde C &= \nablav_a \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
&= \iint\frac{\df^2\kv}{(2\pi)^2} (\i\kv_+)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
\nablav_b \, \d\tilde C &= \nablav_b \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
&= \iint\frac{\df^2\kv}{(2\pi)^2} (-\i\kv_-)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with $\kv_{\pm} = \kv\pm\nv/2$. Therefore $\[ 2r+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C$ translated in wavenumber space as
\begin{align}
\[ 2r+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C &=  \iint\frac{\df^2\kv}{(2\pi)^2} \[ 2r + \nu_{2h} (k^{2h}_+ + k^{2h}_-)\]\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\end{align}
or 
\begin{align}
\[ 2r+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C &\leftrightarrow  \[ 2r + \nu_{2h} (k^{2h}_+ + k^{2h}_-)\]\hat{C}^{\textrm{(h)}}(\kv)
\end{align}
\item
\begin{align}
& \[\bit\hat{\mathbf{z}}\cdot(\bv\times\nablav_a) \Del^{-1}_{\la,a}+\hat{\mathbf{z}}\cdot(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\d\tilde C= \nonumber\\
%&\qquad= \hat{\mathbf{z}}\cdot \[\bit(\bv\times\nablav_a) \Del^{-1}_{\la,a}+(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\Del_{\la,a}\Del_{\la,b}\d\tilde S ~\nonumber\\
% &\qquad=  \hat{\mathbf{z}}\cdot\[\bit(\bv\times\nablav_a) \Del_{\la,b}+(\bv\times\nablav_b) \Del_{\la,a}\] \d\tilde S \leftrightarrow~\\
 &\leftrightarrow \hat{\mathbf{z}}\cdot\[\i\bit(\bv\times \kv_{+} ) /(-k^2_{\la+})-\i\bit(\bv\times \kv_{-} ) /(-k^2_{\la-})\] \hat{C}^{\textrm{(h)}}(\kv)\\
% &\qquad=  -\i k^2_{\la+} k^2_{\la-}\, \hat{\mathbf{z}}\cdot\[\bit(\bv\times \kv_{+} )/k^2_{\la+} -\bit(\bv\times \kv_{-} )/ k^2_{\la-} \] \hat{S}^{\textrm{(h)}}(\kv)\\
 &\qquad=  -\i \, \( \om_{\kv_+} - \om_{\kv_-} \) \hat{C}^{\textrm{(h)}}(\kv)
\end{align}

Therefore
\be
\boxed{(\Acal^e_a+\Acal^e_b)\d\tilde C \leftrightarrow \[\bit- 2r - \nu_{2h} (k^{2h}_+ + k^{2h}_-) -\i \, \( \om_{\kv_+} - \om_{\kv_-} \)\] \hat{C}^{\textrm{(h)}}(\kv)}
\ee
\end{enumerate}


Some useful identities:
\begin{align}
\uv\cdot\nablav F &= J(\psi,F) = \hat{\mathbf{z}}\cdot(\nablav\psi\times\nablav F)\\
(\Del_\la\uv)\cdot\nablav F &= J(q,F) = \hat{\mathbf{z}}\cdot(\nablav q\times\nablav F)
\end{align}
Using these we calculate the term $(\d\Acal_a+\d\Acal_b) C^e$.

\begin{enumerate}
\item
\begin{align}
(\d\Uv_a\cdot\nablav_a) C^e &= J_a(\d\tilde \Psi_a,C^e)\nonumber\\
&= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)
\end{align}
we have that $\nablav_a\d\tilde \Psi_a = -\i\nv/(n^2_\la)\,e^{\i\nv\cdot\xv_a}$, where $n^2_\la = n^2+\la^2$ and therefore
\begin{align}
(\d\Uv_a\cdot\nablav_a) C^e &= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)\nonumber\\
&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}(\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{n^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{n^2_\la}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
\end{align}
\item similarly
\begin{align}
(\d\Uv_b\cdot\nablav_b) C^e &= \hat{\mathbf{z}}\cdot (\nablav_b\d\tilde \Psi_b\times\nablav_b C^E)\nonumber\\
&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}(-\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{n^2_\la}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
\end{align}
\item
\begin{align}
\[\bit(\Del_{\la,a}\d\Uv_a)\cdot\nablav_a\]\Del_{\la,a}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_a\d\tilde Q_a\times\nablav_a \Del_{\la,a}^{-1}C^e)\nonumber\\
&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{k^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{k^2_{\la-}}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
\end{align}
\item and similarly
\begin{align}
\[\bit(\Del_{\la,b}\d\Uv_b)\cdot\nablav_b\]\Del_{\la,b}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_b\d\tilde Q_b\times\nablav_b \Del_{\la,b}^{-1}C^e)\nonumber\\
&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{k^2_{\la+}}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
\end{align}
\end{enumerate}


Therefore
\begin{empheq}[box=\fbox]{align}
&(\d\Acal_a+\d\Acal_b) C^e = \nonumber\\
&\hspace{2em}=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\iint\frac{\df^2\kv}{(2\pi)^2}\[\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\frac1{k^2_{\la-}}-\frac1{n^2_\la}\)\,\hat{C}^e(\kv_-)-\right.\nonumber\\
&\hspace{15em}\left.-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\frac1{k^2_{\la+}}-\frac1{n^2_\la}\)\,\hat{C}^e(\kv_+)\]\,e^{\i\kv\cdot(\xv_a-\xv_b)} 
\end{empheq}


We are now in the position to solve the perturbation covariance equation and obtain $\hat{C}^{\textrm{(h)}}(\kv)$ as

\begin{empheq}[box=\fbox]{align}
&\hat{C}^{\textrm{(h)}}(\kv)=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\times\nonumber\\
 &\vspace{2em}\times\dfrac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\dfrac1{k^2_{\la-}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv_-)-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\dfrac1{k^2_{\la+}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv_+)}{\s+2r + \nu_{2h} (k^{2h}_+ + k^{2h}_-) -\i \, \( \om_{\kv_-} - \om_{\kv_+}\)}\nonumber\\
  &\vspace{1em}\equiv e^{\i\nv\cdot(\xv_a+\xv_b)/2} \[\bit F(\kv_-)-F(\kv_+)\]
\end{empheq}


How much is $\Rcal (\dC)$ ?

\begin{align}
&\Rcal (\dC)     =\nonumber\\
&\hspace{.3em}  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\!\times\!\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) \dC\]_{\xv_a=\xv_b}\nonumber\\
%&  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\times\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) \iint\frac{\df^2\kv}{(2\pi)^2} \hat{C}^{\textrm{(h)}}(\kv) e^{\i\kv\cdot(\xv_a-\xv_b)} \]_{\xv_a=\xv_b}\nonumber\\
&\hspace{.3em}  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\!\times\!\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) \iint\!\frac{\df^2\kv}{(2\pi)^2} \[\bit F(\kv_-)-F(\kv_+)\] e^{\i\nv\cdot(\xv_a+\xv_b)/2}e^{\i\kv\cdot(\xv_a-\xv_b)} \]_{\xv_a=\xv_b}\nonumber\\
%&  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\times \iint\frac{\df^2\kv}{(2\pi)^2} \(\frac{\i \kv_+}{-k^2_{\la+}}-\frac{\i \kv_-}{-k^2_{\la-}} \)\[\bit F(\kv_-)-F(\kv_+)\] e^{\i (\kv_+\cdot \xv_a-\kv_-\xv_b)} \]_{\xv_a=\xv_b}\nonumber\\
&\hspace{.3em}  =-\nablav\cdot \iint\!\frac{\df^2\kv}{(2\pi)^2} \frac{\hat{\mathbf{z}}}{2}\!\times\!\(\frac{\i \kv_-}{k^2_{\la-}}-\frac{\i \kv_+}{k^2_{\la+}} \)\[\bit F(\kv_-)-F(\kv_+)\] e^{\i \nv\cdot\xv}
\end{align}
Moreover, since under $\kv\to-\kv$ we have that $\kv_+ \to- \kv_-$, $k^2_{\la+} \to k^2_{\la-}$ and $F(\kv_+)\to -F(\kv_-)$ we get that 
\begin{align}
\Rcal (\dC)    &   =-\nablav\cdot \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\times\(\frac{\i \kv_-}{k^2_{\la-}}-\frac{\i \kv_+}{k^2_{\la+}} \)\, F(\kv_-)  e^{\i \nv\cdot\xv}~.
\end{align}
It is easy to derive that for any vector $\pv$,
\be
\nablav\cdot\( \hat{\mathbf{z}}\times\pv\,e^{\i\nv\cdot\xv}\) = -\i\,\hat{\mathbf{z}}\cdot(\nv\times\pv)\,e^{\i\nv\cdot\xv}\ ,
\ee
and therefore
\begin{align}
\Rcal (\dC)  &   = \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2_{\la,+}} -\frac1{k^2_{\la,-}}\)\, F(\kv_-)  e^{\i \nv\cdot\xv} \nonumber\\
& = \d\tilde Q\iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2_{\la,s}} -\frac1{k^2_{\la}}\)\, F(\kv)   \nonumber\\
&   =\d\tilde Q \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv)}{\s+2r + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  
\end{align}

Using the above we find that from the mean flow perturbation equation $\s$ must satisfy:
\begin{align}
\sigma + r + \nu_{2h} n^{2h} + \i\om_{\nv}&= \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv)}{\s+2r + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  \\
&= \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(k^2_{\la,s}-k^2_{\la}\)\(k^2_{\la}-n^2_\la\)\,\hat{C}^e(\kv)}{k_{\la,s}^2k_{\la}^4 n_\la^2 \[\s+2r + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)\bit\]}  
\end{align}





\subsection{dissipate only kinetic energy, $-r\Delta\psi$}
We will write with red only the differences from $- rq$. 

For the NL system:
\begin{align}
\partial_t q + J(\psi,q) + \beta v  =\xi +\textrm{Diss}
\end{align}
with
\begin{align}
\textrm{Diss}&= - r \textcolor{red}{\Delta \psi} - (-1)^h\nu_{2h} \Delta^{h}\textcolor{red}{\Delta \psi} = -\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Delta \psi}\ \\
q &=\Delta \psi - \lambda^2 \psi~~,~~u =-\partial_y \psi ~~,~~v= \partial_x \psi~.
\end{align}
$h=1$ is diffusion, $h>1$ hyperdiffusion

Define $q=Q+q'$, etc. Then
\begin{align}
&\partial_t Q + J(\Psi,Q + \bv\cdot\xv) =- r \textcolor{red}{\Del\Psi} - (-1)^h\nu_{2h}  \Delta^{h}\textcolor{red}{\Del\Psi} - \Tcal[ J(\psi',q') ]~\\
&\partial_t q' = \Acal(\Uv) \,q' + f_{\textrm{nl}} + \xi
\end{align}
with
\begin{align}
\Acal(\Uv)&=-\Uv\cdot\nablav + \[\bit(\Del_\la\Uv)\cdot\nablav + \hat{\mathbf{z}}\cdot(\bv\times\nablav)\]\Del^{-1}_\la - \[r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Del\Del_\la^{-1}}~\\
f_{\textrm{nl}}&=\Tcal[ J(\psi',q') ]-J(\psi',q')
\end{align}

Eddy vorticity covariance is again $C(\xv_a,\xv_b,t)=\<q'(\xv_a,t)q'(\xv_b,t)\>$ and using the ergodic hypothesis $\Tcal(\bullet) = \<\bullet\>$ the Reynolds stress divergence can be expressed as:
\begin{align}
 -\Tcal[ J(\psi',q') ]&=-\nablav\cdot \<(\uv'\,q')\>\\
    &  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\times\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) C\]_{\xv_a=\xv_b}\nonumber\\
  &\equiv \Rcal(C)\ .
\end{align}


S3T system is
\begin{align}
\partial_t \, Q &+ J \(\Psi,Q+ {\bm\beta}\cdot\mathbf{x} \) = \Rcal( C )-\[r+(-1)^{h}\nu_{2h} \Del^h\]\,\textcolor{red}{\Del\Del_\la^{-1}}Q\ ,\\
\partial_t \, C & = \[\bit\Acal_a(\Uv) + \Acal_b(\Uv) \] C +\varepsilon\,Q\ ,
\end{align}

Consider a homogeneous, stationary equilibrium solution, $Q^e$, $C^e(\xv_a-\xv_b)$. Expanding $C^e$ as
\be
C^e(\xv_a-\xv_b) = \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}
\ee
(and similarly for $Q(\xv_a-\xv_b)$), we find that
\be
\textcolor{red}{\hat{C}^e(\kv) }= \frac{\varepsilon\,\hat{Q}(\kv)}{2(r+\nu_{2h} k^{2h})}\textcolor{red}{\frac{k^2_\la}{k^2}}\ ,
\ee

Perturbations $\d Q$, $\d C$ about this equilibrium satisfy:
\begin{align}
\partial_t \,\d Q &+ J \(\d\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d C )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\,\textcolor{red}{\Del\Del_\la^{-1}}\d Q\ ,\label{eq1}\\
\partial_t \,\d C & = \(\bit\Acal^e_a + \Acal^e_b \)\d C +\(\bit\d\Acal_a + \d\Acal_b\)C^e\ ,\label{eq2}
\end{align}


The spatial component of the eigenfunction, $\d Q = \d\tilde{Q}\,e^{\s t}$, $\d C = \d\tilde{C}\,e^{\s t}$ about the homogeneous equilibrium are
\begin{align}
\d\tilde{Q}(\xv) &= e^{\i\nv\cdot\xv} ~\\
\d\tilde{C}(\xv_a,\xv_b) &= C^{\textrm{(h)}}(\xv_a-\xv_b)\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with
\be
C^{\textrm{(h)}}(\xv_a-\xv_b) = \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}
\ee
and satisfy
\begin{align}
\s \,\d \tilde{Q} &+ J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d\tilde C  )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Del\Del_\la^{-1}}\d \tilde{Q}\ ,\label{eq1}\\
\s \,\d \tilde{C} & = \(\bit\Acal^e_a + \Acal^e_b \)\d \tilde C +\(\bit\d\tilde\Acal_a + \d\tilde\Acal_b\)C^e\ ,\label{eq2}
\end{align}
with
\begin{align}
\d\Acal&=-\d\Uv\cdot\nablav + \[\bit(\Del_\la\,\d\Uv)\cdot\nablav \]\Del^{-1}_\la ~
\end{align}

Since $\d\tilde Q=e^{\i\nv\cdot\xv}$ we have
\be
\d\tilde\Psi = -\frac{\d\tilde Q}{n^2+\la^2}~,~\d\tilde U = \frac{\i n_y \d\tilde Q}{n^2+\la^2}~,~\d\tilde V = -\frac{\i n_x\,\d\tilde Q}{n^2+\la^2}~.
\ee

 Define Rossby wave frequency as:
\be
\om_{\kv} = \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k^2+\la^2} \equiv  \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k_\la^2}
\ee

Calculate each term of~\eqref{eq1} and \eqref{eq2}.

\begin{enumerate}
\item
\be\boxed{
J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \frac{\i(\b_x n_y-\b_y n_x)}{n^2+\la^2}\d\tilde Q = \i\om_{\nv}\d\tilde Q }
\ee
\item
\be\boxed{
\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Del\Del_\la^{-1}}\d \tilde{Q}= \[ r+\nu_{2h} n^{2h}\]\textcolor{red}{(n^2/n^2_\la)}\d\tilde Q  }
\ee
\item
\begin{align}
\[ 2r\textcolor{red}{(\Del_a\Del_{\la,a}^{-1}+\Del_b\Del_{\la,b}^{-1})}+(-1)^h\nu_{2h} (\Delta_a^{h}\textcolor{red}{\Del_a\Del_{\la,a}^{-1}}+\Delta_b^{h}\textcolor{red}{\Del_b\Del_{\la,b}^{-1}})\]\d\tilde C=?
\end{align}
We have that
\begin{align}
\nablav_a \,\d\tilde C &= \iint\frac{\df^2\kv}{(2\pi)^2} (\i\kv_+)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
\nablav_b \, \d\tilde C &= \iint\frac{\df^2\kv}{(2\pi)^2} (-\i\kv_-)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with $\kv_{\pm} = \kv\pm\nv/2$. Therefore $\[ 2r\textcolor{red}{(\Del_a\Del_{\la,a}^{-1}+\Del_b\Del_{\la,b}^{-1})}+(-1)^h\nu_{2h} (\Delta_a^{h}\textcolor{red}{\Del_a\Del_{\la,a}^{-1}}+\Delta_b^{h}\textcolor{red}{\Del_b\Del_{\la,b}^{-1}})\]\d\tilde C$ translated in wavenumber space as
\begin{align}
&\[ 2r\textcolor{red}{(\Del_a\Del_{\la,a}^{-1}+\Del_b\Del_{\la,b}^{-1})}+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C \leftrightarrow \nonumber\\
&\qquad\leftrightarrow \[ 2r\textcolor{red}{(k^2_+/ k^2_{\la,+} + k^2_-/ k^2_{\la,-})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_+/k^2_{\la,+} + k^{2h+2}_-/k^2_{\la,-}})\]\hat{C}^{\textrm{(h)}}(\kv)
\end{align}
\item
\begin{align}
& \[\bit\hat{\mathbf{z}}\cdot(\bv\times\nablav_a) \Del^{-1}_{\la,a}+\hat{\mathbf{z}}\cdot(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\d\tilde C= \nonumber\\
%&\qquad= \hat{\mathbf{z}}\cdot \[\bit(\bv\times\nablav_a) \Del^{-1}_{\la,a}+(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\Del_{\la,a}\Del_{\la,b}\d\tilde S ~\nonumber\\
% &\qquad=  \hat{\mathbf{z}}\cdot\[\bit(\bv\times\nablav_a) \Del_{\la,b}+(\bv\times\nablav_b) \Del_{\la,a}\] \d\tilde S \leftrightarrow~\\
 &\leftrightarrow \hat{\mathbf{z}}\cdot\[\i\bit(\bv\times \kv_{+} ) /(-k^2_{\la+})-\i\bit(\bv\times \kv_{-} ) /(-k^2_{\la-})\] \hat{C}^{\textrm{(h)}}(\kv)\\
% &\qquad=  -\i k^2_{\la+} k^2_{\la-}\, \hat{\mathbf{z}}\cdot\[\bit(\bv\times \kv_{+} )/k^2_{\la+} -\bit(\bv\times \kv_{-} )/ k^2_{\la-} \] \hat{S}^{\textrm{(h)}}(\kv)\\
 &\qquad=  -\i \, \( \om_{\kv_+} - \om_{\kv_-} \) \hat{C}^{\textrm{(h)}}(\kv)
\end{align}

Therefore
\be
\boxed{(\Acal^e_a+\Acal^e_b)\d\tilde C \leftrightarrow \[\bit- 2r \textcolor{red}{(k^2_+/ k^2_{\la,+} + k^2_-/ k^2_{\la,-})}- \nu_{2h} (\textcolor{red}{k^{2h+2}_+/k^2_{\la,+} + k^{2h+2}_-/k^2_{\la,-}}) -\i \, \( \om_{\kv_+} - \om_{\kv_-} \)\] \hat{C}^{\textrm{(h)}}(\kv)}
\ee
\end{enumerate}


Some useful identities:
\begin{align}
\uv\cdot\nablav F &= J(\psi,F) = \hat{\mathbf{z}}\cdot(\nablav\psi\times\nablav F)\\
(\Del_\la\uv)\cdot\nablav F &= J(q,F) = \hat{\mathbf{z}}\cdot(\nablav q\times\nablav F)
\end{align}
Using these we calculate the term $(\d\Acal_a+\d\Acal_b) C^e$. Everything is the same, except $C^e$.
%
%\begin{enumerate}
%\item
%\begin{align}
%(\d\Uv_a\cdot\nablav_a) C^e &= J_a(\d\tilde \Psi_a,C^e)\nonumber\\
%&= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)
%\end{align}
%we have that $\nablav_a\d\tilde \Psi_a = -\i\nv/(n^2_\la)\,e^{\i\nv\cdot\xv_a}$, where $n^2_\la = n^2+\la^2$ and therefore
%\begin{align}
%(\d\Uv_a\cdot\nablav_a) C^e &= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}(\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{n^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
%\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{n^2_\la}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\item similarly
%\begin{align}
%(\d\Uv_b\cdot\nablav_b) C^e &= \hat{\mathbf{z}}\cdot (\nablav_b\d\tilde \Psi_b\times\nablav_b C^E)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}(-\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{n^2_\la}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\item
%\begin{align}
%\[\bit(\Del_{\la,a}\d\Uv_a)\cdot\nablav_a\]\Del_{\la,a}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_a\d\tilde Q_a\times\nablav_a \Del_{\la,a}^{-1}C^e)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{k^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
%\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{k^2_{\la-}}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\item and similarly
%\begin{align}
%\[\bit(\Del_{\la,b}\d\Uv_b)\cdot\nablav_b\]\Del_{\la,b}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_b\d\tilde Q_b\times\nablav_b \Del_{\la,b}^{-1}C^e)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{k^2_{\la+}}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\end{enumerate}
Therefore
\begin{empheq}[box=\fbox]{align}
&(\d\Acal_a+\d\Acal_b) \textcolor{red}{C^e} = \nonumber\\
&\hspace{2em}=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\iint\frac{\df^2\kv}{(2\pi)^2}\[\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\frac1{k^2_{\la-}}-\frac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_-)}-\right.\nonumber\\
&\hspace{15em}\left.-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\frac1{k^2_{\la+}}-\frac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_+)}\]\,e^{\i\kv\cdot(\xv_a-\xv_b)} 
\end{empheq}


We are now in the position to solve the perturbation covariance equation and obtain $\hat{C}^{\textrm{(h)}}(\kv)$ as

\begin{empheq}[box=\fbox]{align}
&\hat{C}^{\textrm{(h)}}(\kv)=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\times\nonumber\\
 &\vspace{2em}\times\dfrac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\dfrac1{k^2_{\la-}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_-)}-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\dfrac1{k^2_{\la+}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_+)}}{\s+2r\textcolor{red}{(k^2_+/ k^2_{\la,+} + k^2_-/ k^2_{\la,-})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_+/k^2_{\la,+} + k^{2h+2}_-/k^2_{\la,-}}) -\i \, \( \om_{\kv_-} - \om_{\kv_+}\)}\nonumber\\
  &\vspace{1em}\equiv e^{\i\nv\cdot(\xv_a+\xv_b)/2} \[\bit F(\kv_-)-F(\kv_+)\]
\end{empheq}


How much is $\Rcal (\d C)$ ?

\begin{align}
\Rcal (\d C)    &   =-\nablav\cdot \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\times\(\frac{\i \kv}{k^2_{\la}}-\frac{\i (\kv+\nv)}{k^2_{\la,s}} \)\, \textcolor{red}{F(\kv)}  e^{\i \nv\cdot\xv} \nonumber\\
\end{align}

Now after some algebra we get that:
\begin{align}
\nablav\cdot\( \hat{\mathbf{z}}\times\kv\,e^{\i\nv\cdot\xv}\) &= -\i\hat{\mathbf{z}}\cdot(\nv\times\kv)\\
\nablav\cdot\( \hat{\mathbf{z}}\times\nv\,e^{\i\nv\cdot\xv}\) &= 0
\end{align}
therefore
\begin{align}
\Rcal (\d C)  &   = \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2_{\la,s}} -\frac1{k^2_{\la}}\)\, \textcolor{red}{F(\kv)}  e^{\i \nv\cdot\xv} \nonumber\\
&   =\d\tilde Q \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv)}}{\s+2r\textcolor{red}{(k^2_s/ k^2_{\la,s} + k^2/ k^2_{\la})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_s/k^2_{\la,s} + k^{2h+2}/k^2_{\la}}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  
\end{align}

Using the above we find that from the mean flow perturbation equation $\s$ must satisfy:
\begin{align}
&\sigma + (r + \nu_{2h} n^{2h})\textcolor{red}{(n^2/n^2_\la)} + \i\om_{\nv}=\nonumber\\
&\qquad= \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv)}}{\s+2r\textcolor{red}{(k^2_s/ k^2_{\la,s} + k^2/ k^2_{\la})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_s/k^2_{\la,s} + k^{2h+2}/k^2_{\la}}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  \\
&\qquad=  \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(k^2_{\la,s}-k^2_{\la}\)\(k^2_{\la}-n^2_\la\)\,\textcolor{red}{(k^2_\la/k^2)}\,\hat{C}^{e,OLD}(\kv)}{k_{\la,s}^2k_{\la}^4 n_\la^2 \[\s+2r\textcolor{red}{(k^2_s/ k^2_{\la,s} + k^2/ k^2_{\la})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_s/k^2_{\la,s} + k^{2h+2}/k^2_{\la}}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)\bit\]}  
\end{align}










%
%
%
%
%\textcolor{green}{H E R E }
%
%
%
%the generalized S3T dispersion relation is:
%\begin{align}
%\sigma\, N^2_\la/N^2+& r + \nu_4 N^4 - \i\b m/N^2 =\intinf\intinf\frac{\df k}{2\pi}\frac{\df \l}{2\pi} \frac{\Ncal~(K^2/N^2-1)}{K^2_\la\(\sigma \Dcal_\sigma +  \Dcal_0 + \i\b\,\Dcal_\b\)}\,C^E(k,\l)
%\end{align}
%
%
%where $\<\xi_a\xi_b\>=\d(t_a-t_b) Q(x_a-x_b,y_a-y_b)$ and 
%\begin{subequations}
%\begin{align}
%C^E(k,\l)&=\frac{\varepsilon\,K^2_{\la} \,Q(k,\l) }{2 r K^2 + 2 \nu_4 K^6 }~,\\
%\Ncal &= 2(nk-m\l)\[\bit mn(k^2_+ - \l^2_+) - (m^2-n^2) k_+\l_+ \]=\nonumber\\
%&=(nk-m\l)^2 (K^2_s-K^2)~,\\
%\Dcal_\sigma &= K^2_\la K^2_{s,\la}~,\\
%\Dcal_0 &= r  \,(K^2 K^2_{s,\la} + K^2_{\la}K^2_{s}) + \nu_4  (K^6 K^2_{s,\la} + K^6_{s} K^2_{\la})~,\\
%\Dcal_\b &= k\,K^2_{s,\la} -(k+m)K^2_{\la}~.
%\end{align}
%\end{subequations}
%with
%\begin{subequations}
%\begin{align}
%N^2 = m^2+n^2~~&,~~N^2_\la = N^2+\la^2~,\\
%K^2 = k^2+\l^2~~&,~~K^2_\la = K^2+\la^2~,\\
%K^2_{s} = (k+m)^2+(\l+n)^2~~&,~~K^2_{s,\la} = K^2_{s}+\la^2~.
%\end{align}
%\end{subequations}
%%    B1 = K2la.^2.*Ks2la;
%%    B2 = r*K2la.*(K2.*Ks2la + K2la.*Ks2) + nu4*K2la.*(K2.^3.*Ks2la + Ks2.^3.*K2la);
%%    B3 = beta*K2la.*(k.*Ks2la -(k+m).*K2la);
%%        
%%    Denom = s*B1+B2+1i*B3 ;
%%    
%%    SP_f  =   A1    ./ Denom;
%


==> chapters/app-S3Tgr_lambda_v2.tex <==
% !TEX root = ../thesis.tex



\chapter{Derivation of the eigenvalue relation for the S3T stability of a homogeneous equilibrium with finite deformation radius}
\label{app:S3Tgr_lambda}

Here we present the S3T eigenvalue relation $\s$ that determines the stability of the homogeneous turbulent equilibrium with finite deformation radius, $1/\lambda$ (cf.~chapter~\textcolor{red}{??}). In this case the potential vorticity, which is materially conserved in the absence of forcing and dissipation, is $q=\z-\la^2\psi+f_0+\bv\cdot\xv$, and the forced-dissipative NL system is:
\begin{align}
\partial_t \pV + J\(\psi,\pV+\bv\cdot\xv\bit\) =\sqrt{\varepsilon}\xi +\Diss\,\pV
\end{align}
where $\pV\equiv\Delta \psi - \lambda^2 \psi$ is the relative potential vorticity and $\Diss$ is the dissipation. We can choose to either dissipate potential vorticity, i.e., $\Diss = -1- (-1)^h\nu_{2h} \Delta^{h}$ or dissipate relative vorticity, i.e., $\Diss = [-1- (-1)^h\nu_{2h} \Delta^{h}]\Del\Del_\la^{-1}$, where $\Del_\la\equiv\Del-\la^2$ and $\Del_\la^{-1}$ its inverse.


After decomposing the flow fields into mean fields $\Pv\equiv\tav{\pV}$, and deviations from the mean $\pV'=\pV-\Pv$, and also defining the eddy potential vorticity covariance $C(\xv_a,\xv_b,t)=\<\pV'(\xv_a,t)\pV'(\xv_b,t)\>$ and using the ergodic hypothesis that $\Tcal(\bullet) = \<\bullet\>$, we arrive to the QL and S3T systems\begin{subequations}
\begin{align}
\partial_t \Pv &+ J \(\Psi, \Pv+  {\bm\beta}\cdot\mathbf{x} \) = -\tav{ J \(\psi', \pV'\) }+\Diss\,\Pv \ ,\label{eq:eqlla_mean}\\
\partial_t \pV' &=\Acal(\Uv)\,\pV'+\sqrt{\e}\,\xi \ .\label{eq:eqlla_pert}
\end{align}\label{eq:eqlla}\end{subequations}
and\begin{subequations}
\begin{align}
\partial_t \Pv &+ J \(\Psi, \Pv +  {\bm\beta}\cdot\mathbf{x} \) = \Rcal_\la( C )+\Diss\Pv\ ,\label{eq:s3tla_mean}\\
\partial_t C_{ab} & = \[\bit\Acal_a(\Uv) + \Acal_b(\Uv)\]C_{ab} +\e\,Q_{ab}\ .\label{eq:s3tla_C}
\end{align}\label{eq:s3tla}\end{subequations}
with the only difference that $\Acal(\Uv)$ is\begin{subequations}
\be
\Acal(\Uv)=-\Uv\cdot\nablav + \[\bit(\Del_\la\Uv)\cdot\nablav + \hat{\mathbf{z}}\cdot(\bv\times\nablav)\]\Del^{-1}_\la +\Diss\ ,
\ee
and
\be
\Rcal_\la(C)\equiv-\nablav\cdot\[\zhat\times \frac1{2}\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) C\]_{\xv_a=\xv_b}\ .
\ee\label{eq:defs_R_Acal_la}\end{subequations}
Definitions~\eqref{eq:defs_R_Acal_la} reduce to~\eqref{eq:def_Acal} and~\eqref{eq:def_Rcal} for the infinite deformation radius case ($\la=0$).


\section{Case dissipating potential vorticity}

Consider the case where the potential vorticity is being dissipated, $\Diss = -1- (-1)^h\nu_{2h} \Delta^{h}$. Then for homogeneous forcing covariance, $Q$, the homogeneous solution with no mean flow $\Pv^e=0$ and equilibrium potential vorticity eddy covariance $C^e$ with spectrum:
\be
\hat{C}^e(\kv) = \frac{\varepsilon\,\hat{Q}(\kv)}{2(1+\nu_{2h} k^{2h})}\ ,
\ee
is a solution of~\eqref{eq:s3tla}. Following the methodology described in Appendix~\ref{app-S3Tgr} we derive the eigenvalue relation that determines the stability of this homogeneous equilibrium to be:
\begin{align}
\sigma + 1 + \nu_{2h} n^{2h} &= \int\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv)}{\s+2 + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv,\la}+\om_{\nv,\la} - \om_{\kv+\nv,\la}\)}\ ,  %\\
%&= \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(k^2_{\la,s}-k^2_{\la}\)\(k^2_{\la}-n^2_\la\)\,\hat{C}^e(\kv)}{k_{\la,s}^2k_{\la}^4 n_\la^2 \[\s+2r + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv} +\om_{\nv}- \om_{\kv+\nv}\)\bit\]}  
\end{align}
with $\kv_s\equiv \kv+\nv$ and $k_s\equiv|\kv_s|$ and
\be
\om_{\kv,\la} = \frac{\zhat\cdot(\bv\times\kv)}{k^2+\la^2}~.
\ee



{\color{red}

\begin{align}
\sigma + 1 + \nu_{2h} n^{2h} &= \int\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv)}{\s+2 + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv,\la}+\om_{\nv,\la} - \om_{\kv+\nv,\la}\)}\ ,  %\\
\end{align}

\be
f(\s) = \int \frac{\df^2 \kv}{(2\pi)^2}\;\frac{|\mathbf{k}\times{\mathbf{n}}|^2\, (k^2_s-k^2) (k^2-n^2) }{k^4_\la k^2_{\la,s} n_\la^2  \[ (\s+2) +\i\( \om_{\kv+\nv,\la}- \om_{\nv,\la} - \om_{\kv,\la} \)\bit \] }\frac{\hat{Q}(\kv)}{2}\ , \label{eq:f_factorla}
\ee
with $\kv_s=\kv+\nv$ and $k_s=|\kv_s|$ and the dispersion relation for the stability of the homogeneous equilibrium is 
\be
\s+1 =  \e\int \frac{\df^2 \kv}{(2\pi)^2}\;\frac{|\mathbf{k}\times{\mathbf{n}}|^2\, (k^2_s-k^2) (k^2-n^2) }{k^4_\la k^2_{\la,s} n_\la^2  \[ (\s+2) +\i\( \om_{\kv+\nv,\la}- \om_{\nv,\la} - \om_{\kv,\la} \)\bit \] }\frac{\hat{Q}(\kv)}{2} \ .\label{eq:s3tgr_z_nz_la}
\ee


}

\subsection{dissipate only kinetic energy, $-r\Delta\psi$}
We will write with red only the differences from $- rq$. 

For the NL system:
\begin{align}
\partial_t q + J(\psi,q) + \beta v  =\xi +\textrm{Diss}
\end{align}
with
\begin{align}
\textrm{Diss}&= - r \textcolor{red}{\Delta \psi} - (-1)^h\nu_{2h} \Delta^{h}\textcolor{red}{\Delta \psi} = -\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Delta \psi}\ \\
q &=\Delta \psi - \lambda^2 \psi~~,~~u =-\partial_y \psi ~~,~~v= \partial_x \psi~.
\end{align}
$h=1$ is diffusion, $h>1$ hyperdiffusion

Define $q=Q+q'$, etc. Then
\begin{align}
&\partial_t Q + J(\Psi,Q + \bv\cdot\xv) =- r \textcolor{red}{\Del\Psi} - (-1)^h\nu_{2h}  \Delta^{h}\textcolor{red}{\Del\Psi} - \Tcal[ J(\psi',q') ]~\\
&\partial_t q' = \Acal(\Uv) \,q' + f_{\textrm{nl}} + \xi
\end{align}
with
\begin{align}
\Acal(\Uv)&=-\Uv\cdot\nablav + \[\bit(\Del_\la\Uv)\cdot\nablav + \hat{\mathbf{z}}\cdot(\bv\times\nablav)\]\Del^{-1}_\la - \[r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Del\Del_\la^{-1}}~\\
f_{\textrm{nl}}&=\Tcal[ J(\psi',q') ]-J(\psi',q')
\end{align}

Eddy vorticity covariance is again $C(\xv_a,\xv_b,t)=\<q'(\xv_a,t)q'(\xv_b,t)\>$ and using the ergodic hypothesis $\Tcal(\bullet) = \<\bullet\>$ the Reynolds stress divergence can be expressed as:
\begin{align}
 -\Tcal[ J(\psi',q') ]&=-\nablav\cdot \<(\uv'\,q')\>\\
    &  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\times\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) C\]_{\xv_a=\xv_b}\nonumber\\
  &\equiv \Rcal(C)\ .
\end{align}


S3T system is
\begin{align}
\partial_t \, Q &+ J \(\Psi,Q+ {\bm\beta}\cdot\mathbf{x} \) = \Rcal( C )-\[r+(-1)^{h}\nu_{2h} \Del^h\]\,\textcolor{red}{\Del\Del_\la^{-1}}Q\ ,\\
\partial_t \, C & = \[\bit\Acal_a(\Uv) + \Acal_b(\Uv) \] C +\varepsilon\,Q\ ,
\end{align}

Consider a homogeneous, stationary equilibrium solution, $Q^e$, $C^e(\xv_a-\xv_b)$. Expanding $C^e$ as
\be
C^e(\xv_a-\xv_b) = \int\frac{\df^2\kv}{(2\pi)^2}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}
\ee
(and similarly for $Q(\xv_a-\xv_b)$), we find that
\be
\textcolor{red}{\hat{C}^e(\kv) }= \frac{\varepsilon\,\hat{Q}(\kv)}{2(r+\nu_{2h} k^{2h})}\textcolor{red}{\frac{k^2_\la}{k^2}}\ ,
\ee

Perturbations $\d Q$, $\d C$ about this equilibrium satisfy:
\begin{align}
\partial_t \,\d Q &+ J \(\d\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d C )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\,\textcolor{red}{\Del\Del_\la^{-1}}\d Q\ ,\label{eq1}\\
\partial_t \,\d C & = \(\bit\Acal^e_a + \Acal^e_b \)\d C +\(\bit\d\Acal_a + \d\Acal_b\)C^e\ ,\label{eq2}
\end{align}


The spatial component of the eigenfunction, $\d Q = \d\tilde{Q}\,e^{\s t}$, $\d C = \d\tilde{C}\,e^{\s t}$ about the homogeneous equilibrium are
\begin{align}
\d\tilde{Q}(\xv) &= e^{\i\nv\cdot\xv} ~\\
\d\tilde{C}(\xv_a,\xv_b) &= C^{\textrm{(h)}}(\xv_a-\xv_b)\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with
\be
C^{\textrm{(h)}}(\xv_a-\xv_b) = \int\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}
\ee
and satisfy
\begin{align}
\s \,\d \tilde{Q} &+ J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d\tilde C  )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Del\Del_\la^{-1}}\d \tilde{Q}\ ,\label{eq1}\\
\s \,\d \tilde{C} & = \(\bit\Acal^e_a + \Acal^e_b \)\d \tilde C +\(\bit\d\tilde\Acal_a + \d\tilde\Acal_b\)C^e\ ,\label{eq2}
\end{align}
with
\begin{align}
\d\Acal&=-\d\Uv\cdot\nablav + \[\bit(\Del_\la\,\d\Uv)\cdot\nablav \]\Del^{-1}_\la ~
\end{align}

Since $\d\tilde Q=e^{\i\nv\cdot\xv}$ we have
\be
\d\tilde\Psi = -\frac{\d\tilde Q}{n^2+\la^2}~,~\d\tilde U = \frac{\i n_y \d\tilde Q}{n^2+\la^2}~,~\d\tilde V = -\frac{\i n_x\,\d\tilde Q}{n^2+\la^2}~.
\ee

 Define Rossby wave frequency as:
\be
\om_{\kv} = \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k^2+\la^2} \equiv  \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k_\la^2}
\ee

Calculate each term of~\eqref{eq1} and \eqref{eq2}.

\begin{enumerate}
\item
\be\boxed{
J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \frac{\i(\b_x n_y-\b_y n_x)}{n^2+\la^2}\d\tilde Q = \i\om_{\nv}\d\tilde Q }
\ee
\item
\be\boxed{
\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Del\Del_\la^{-1}}\d \tilde{Q}= \[ r+\nu_{2h} n^{2h}\]\textcolor{red}{(n^2/n^2_\la)}\d\tilde Q  }
\ee
\item
\begin{align}
\[ 2r\textcolor{red}{(\Del_a\Del_{\la,a}^{-1}+\Del_b\Del_{\la,b}^{-1})}+(-1)^h\nu_{2h} (\Delta_a^{h}\textcolor{red}{\Del_a\Del_{\la,a}^{-1}}+\Delta_b^{h}\textcolor{red}{\Del_b\Del_{\la,b}^{-1}})\]\d\tilde C=?
\end{align}
We have that
\begin{align}
\nablav_a \,\d\tilde C &= \int\frac{\df^2\kv}{(2\pi)^2} (\i\kv_+)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
\nablav_b \, \d\tilde C &= \int\frac{\df^2\kv}{(2\pi)^2} (-\i\kv_-)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with $\kv_{\pm} = \kv\pm\nv/2$. Therefore $\[ 2r\textcolor{red}{(\Del_a\Del_{\la,a}^{-1}+\Del_b\Del_{\la,b}^{-1})}+(-1)^h\nu_{2h} (\Delta_a^{h}\textcolor{red}{\Del_a\Del_{\la,a}^{-1}}+\Delta_b^{h}\textcolor{red}{\Del_b\Del_{\la,b}^{-1}})\]\d\tilde C$ translated in wavenumber space as
\begin{align}
&\[ 2r\textcolor{red}{(\Del_a\Del_{\la,a}^{-1}+\Del_b\Del_{\la,b}^{-1})}+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C \leftrightarrow \nonumber\\
&\qquad\leftrightarrow \[ 2r\textcolor{red}{(k^2_+/ k^2_{\la,+} + k^2_-/ k^2_{\la,-})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_+/k^2_{\la,+} + k^{2h+2}_-/k^2_{\la,-}})\]\hat{C}^{\textrm{(h)}}(\kv)
\end{align}
\item
\begin{align}
& \[\bit\hat{\mathbf{z}}\cdot(\bv\times\nablav_a) \Del^{-1}_{\la,a}+\hat{\mathbf{z}}\cdot(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\d\tilde C= \nonumber\\
%&\qquad= \hat{\mathbf{z}}\cdot \[\bit(\bv\times\nablav_a) \Del^{-1}_{\la,a}+(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\Del_{\la,a}\Del_{\la,b}\d\tilde S ~\nonumber\\
% &\qquad=  \hat{\mathbf{z}}\cdot\[\bit(\bv\times\nablav_a) \Del_{\la,b}+(\bv\times\nablav_b) \Del_{\la,a}\] \d\tilde S \leftrightarrow~\\
 &\leftrightarrow \hat{\mathbf{z}}\cdot\[\i\bit(\bv\times \kv_{+} ) /(-k^2_{\la+})-\i\bit(\bv\times \kv_{-} ) /(-k^2_{\la-})\] \hat{C}^{\textrm{(h)}}(\kv)\\
% &\qquad=  -\i k^2_{\la+} k^2_{\la-}\, \hat{\mathbf{z}}\cdot\[\bit(\bv\times \kv_{+} )/k^2_{\la+} -\bit(\bv\times \kv_{-} )/ k^2_{\la-} \] \hat{S}^{\textrm{(h)}}(\kv)\\
 &\qquad=  -\i \, \( \om_{\kv_+} - \om_{\kv_-} \) \hat{C}^{\textrm{(h)}}(\kv)
\end{align}

Therefore
\be
\boxed{(\Acal^e_a+\Acal^e_b)\d\tilde C \leftrightarrow \[\bit- 2r \textcolor{red}{(k^2_+/ k^2_{\la,+} + k^2_-/ k^2_{\la,-})}- \nu_{2h} (\textcolor{red}{k^{2h+2}_+/k^2_{\la,+} + k^{2h+2}_-/k^2_{\la,-}}) -\i \, \( \om_{\kv_+} - \om_{\kv_-} \)\] \hat{C}^{\textrm{(h)}}(\kv)}
\ee
\end{enumerate}


Some useful identities:
\begin{align}
\uv\cdot\nablav F &= J(\psi,F) = \hat{\mathbf{z}}\cdot(\nablav\psi\times\nablav F)\\
(\Del_\la\uv)\cdot\nablav F &= J(q,F) = \hat{\mathbf{z}}\cdot(\nablav q\times\nablav F)
\end{align}
Using these we calculate the term $(\d\Acal_a+\d\Acal_b) C^e$. Everything is the same, except $C^e$.
%
%\begin{enumerate}
%\item
%\begin{align}
%(\d\Uv_a\cdot\nablav_a) C^e &= J_a(\d\tilde \Psi_a,C^e)\nonumber\\
%&= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)
%\end{align}
%we have that $\nablav_a\d\tilde \Psi_a = -\i\nv/(n^2_\la)\,e^{\i\nv\cdot\xv_a}$, where $n^2_\la = n^2+\la^2$ and therefore
%\begin{align}
%(\d\Uv_a\cdot\nablav_a) C^e &= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}(\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{n^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
%\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{n^2_\la}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\item similarly
%\begin{align}
%(\d\Uv_b\cdot\nablav_b) C^e &= \hat{\mathbf{z}}\cdot (\nablav_b\d\tilde \Psi_b\times\nablav_b C^E)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}(-\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{n^2_\la}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\item
%\begin{align}
%\[\bit(\Del_{\la,a}\d\Uv_a)\cdot\nablav_a\]\Del_{\la,a}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_a\d\tilde Q_a\times\nablav_a \Del_{\la,a}^{-1}C^e)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{k^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
%\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{k^2_{\la-}}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\item and similarly
%\begin{align}
%\[\bit(\Del_{\la,b}\d\Uv_b)\cdot\nablav_b\]\Del_{\la,b}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_b\d\tilde Q_b\times\nablav_b \Del_{\la,b}^{-1}C^e)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{k^2_{\la+}}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\end{enumerate}
Therefore
\begin{empheq}[box=\fbox]{align}
&(\d\Acal_a+\d\Acal_b) \textcolor{red}{C^e} = \nonumber\\
&\hspace{2em}=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\iint\frac{\df^2\kv}{(2\pi)^2}\[\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\frac1{k^2_{\la-}}-\frac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_-)}-\right.\nonumber\\
&\hspace{15em}\left.-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\frac1{k^2_{\la+}}-\frac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_+)}\]\,e^{\i\kv\cdot(\xv_a-\xv_b)} 
\end{empheq}


We are now in the position to solve the perturbation covariance equation and obtain $\hat{C}^{\textrm{(h)}}(\kv)$ as

\begin{empheq}[box=\fbox]{align}
&\hat{C}^{\textrm{(h)}}(\kv)=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\times\nonumber\\
 &\vspace{2em}\times\dfrac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\dfrac1{k^2_{\la-}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_-)}-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\dfrac1{k^2_{\la+}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_+)}}{\s+2r\textcolor{red}{(k^2_+/ k^2_{\la,+} + k^2_-/ k^2_{\la,-})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_+/k^2_{\la,+} + k^{2h+2}_-/k^2_{\la,-}}) -\i \, \( \om_{\kv_-} - \om_{\kv_+}\)}\nonumber\\
  &\vspace{1em}\equiv e^{\i\nv\cdot(\xv_a+\xv_b)/2} \[\bit F(\kv_-)-F(\kv_+)\]
\end{empheq}


How much is $\Rcal (\d C)$ ?

\begin{align}
\Rcal (\d C)    &   =-\nablav\cdot \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\times\(\frac{\i \kv}{k^2_{\la}}-\frac{\i (\kv+\nv)}{k^2_{\la,s}} \)\, \textcolor{red}{F(\kv)}  e^{\i \nv\cdot\xv} \nonumber\\
\end{align}

Now after some algebra we get that:
\begin{align}
\nablav\cdot\( \hat{\mathbf{z}}\times\kv\,e^{\i\nv\cdot\xv}\) &= -\i\hat{\mathbf{z}}\cdot(\nv\times\kv)\\
\nablav\cdot\( \hat{\mathbf{z}}\times\nv\,e^{\i\nv\cdot\xv}\) &= 0
\end{align}
therefore
\begin{align}
\Rcal (\d C)  &   = \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2_{\la,s}} -\frac1{k^2_{\la}}\)\, \textcolor{red}{F(\kv)}  e^{\i \nv\cdot\xv} \nonumber\\
&   =\d\tilde Q \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv)}}{\s+2r\textcolor{red}{(k^2_s/ k^2_{\la,s} + k^2/ k^2_{\la})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_s/k^2_{\la,s} + k^{2h+2}/k^2_{\la}}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  
\end{align}

Using the above we find that from the mean flow perturbation equation $\s$ must satisfy:
\begin{align}
&\sigma + (r + \nu_{2h} n^{2h})\textcolor{red}{(n^2/n^2_\la)} + \i\om_{\nv}=\nonumber\\
&\qquad= \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv)}}{\s+2r\textcolor{red}{(k^2_s/ k^2_{\la,s} + k^2/ k^2_{\la})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_s/k^2_{\la,s} + k^{2h+2}/k^2_{\la}}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  \\
&\qquad=  \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(k^2_{\la,s}-k^2_{\la}\)\(k^2_{\la}-n^2_\la\)\,\textcolor{red}{(k^2_\la/k^2)}\,\hat{C}^{e,OLD}(\kv)}{k_{\la,s}^2k_{\la}^4 n_\la^2 \[\s+2r\textcolor{red}{(k^2_s/ k^2_{\la,s} + k^2/ k^2_{\la})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_s/k^2_{\la,s} + k^{2h+2}/k^2_{\la}}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)\bit\]}  
\end{align}










%
%
%
%
%\textcolor{green}{H E R E }
%
%
%
%the generalized S3T dispersion relation is:
%\begin{align}
%\sigma\, N^2_\la/N^2+& r + \nu_4 N^4 - \i\b m/N^2 =\intinf\intinf\frac{\df k}{2\pi}\frac{\df \l}{2\pi} \frac{\Ncal~(K^2/N^2-1)}{K^2_\la\(\sigma \Dcal_\sigma +  \Dcal_0 + \i\b\,\Dcal_\b\)}\,C^E(k,\l)
%\end{align}
%
%
%where $\<\xi_a\xi_b\>=\d(t_a-t_b) Q(x_a-x_b,y_a-y_b)$ and 
%\begin{subequations}
%\begin{align}
%C^E(k,\l)&=\frac{\varepsilon\,K^2_{\la} \,Q(k,\l) }{2 r K^2 + 2 \nu_4 K^6 }~,\\
%\Ncal &= 2(nk-m\l)\[\bit mn(k^2_+ - \l^2_+) - (m^2-n^2) k_+\l_+ \]=\nonumber\\
%&=(nk-m\l)^2 (K^2_s-K^2)~,\\
%\Dcal_\sigma &= K^2_\la K^2_{s,\la}~,\\
%\Dcal_0 &= r  \,(K^2 K^2_{s,\la} + K^2_{\la}K^2_{s}) + \nu_4  (K^6 K^2_{s,\la} + K^6_{s} K^2_{\la})~,\\
%\Dcal_\b &= k\,K^2_{s,\la} -(k+m)K^2_{\la}~.
%\end{align}
%\end{subequations}
%with
%\begin{subequations}
%\begin{align}
%N^2 = m^2+n^2~~&,~~N^2_\la = N^2+\la^2~,\\
%K^2 = k^2+\l^2~~&,~~K^2_\la = K^2+\la^2~,\\
%K^2_{s} = (k+m)^2+(\l+n)^2~~&,~~K^2_{s,\la} = K^2_{s}+\la^2~.
%\end{align}
%\end{subequations}
%%    B1 = K2la.^2.*Ks2la;
%%    B2 = r*K2la.*(K2.*Ks2la + K2la.*Ks2) + nu4*K2la.*(K2.^3.*Ks2la + Ks2.^3.*K2la);
%%    B3 = beta*K2la.*(k.*Ks2la -(k+m).*K2la);
%%        
%%    Denom = s*B1+B2+1i*B3 ;
%%    
%%    SP_f  =   A1    ./ Denom;
%


==> chapters/app-S3Tlyap_10jan15.tex <==
% !TEX root = ../thesis.tex



\chapter{S3T stability of non-homogeneous equilibrium states}
\label{app:S3Tlyap}

In this appendix we describe the method by which we calculate the S3T stability of non-homogeneous stationary and non-stationary equilibria.


\clearpage

\section{Stability of finite amplitude traveling wave equilibria or mixed jet-traveling wave equilibria}


%\section{S3T generalized system}

S3T system allowing interaction of coherent structures described by streamfunction $\Psi(x,y)$ (from which all fields can be derived, $U=-\partial_y\Psi$, $V=\partial_x\Psi$, $Z=\Del\Psi$) with the turbulent eddy field, $C = \<\z'(x_a,y_a,t)\z'(x_b,y_b,t)\>$ is:\begin{subequations}
\begin{align}
&\partial_t  Z + U\partial_x Z + V\partial_y Z +\beta V =  - r Z -\nu_4 \Del^2 Z - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) C \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) C \right|_{\xv_a=\xv_b} \]\\
&\partial_t C  = \(\bit \Acal_a +\Acal_b\) C + Q~.
\end{align}\end{subequations}
with
\be
\Acal_a \equiv\left.\bit\Acal(\Psi)\right|_{\xv=\xv_a} = -U_a \partial_{x_a}-V_a \partial_{y_a} - \(\beta+Z_{y_a}\) \partial_{x_a} \Del_a^{-1} + Z_{x_a} \partial_{y_a}\Del_a^{-1} - r -\nu_4 \Del_a^2~.
\ee
This system can be written in matrix form:\begin{subequations}
\begin{align}
&\partial_t \Zv + \U \,\D_x  \Zv  +  \V \,\D_y \Zv  +\beta \, \Vv =  - r \, \Zv -\nu_4 \,\DDel^2 \Zv - \nonumber\\
&\qquad\qquad\qquad- \D_x \[ \vecd{\( - \D_y \DDel^{-1}\C\)}\] - \D_y \[\vecd{\( \D_x \DDel^{-1}\C\)}\]\\
&\partial_t\,\C  = \A\, \C+ \C\,\A^\transp + \Q~.
\end{align}\end{subequations}

This system admits equilibria with a coherent structure described by streamfunction $\Psi^e$ and an eddy vorticity covariance, $C^e$. Perturbations around one of these equilibria satisfy:
\begin{subequations}
\begin{align}
&\partial_t \,\d Z + \d U\, \partial_x Z^e + U^e\, \partial_x \d Z +  \d V \,\partial_y Z^e + V^e\, \partial_y \d Z  +\beta \,\d V =  - r \,\d Z -\nu_4 \,\Del^2 \d Z - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d C \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d C \right|_{\xv_a=\xv_b} \]\\
&\partial_t\,\d C  = \(\bit \Acal^e_a +\Acal^e_b\) \d C + \(\bit \d\Acal_a +\d\Acal_b\) C^e ~.
\end{align}\end{subequations}
with\begin{subequations}
\begin{align}
\Acal^e_a  &= \left.\bit\Acal(\Psi^e)\right|_{\xv=\xv_a}  ,\\
\d\Acal_a  &=\left.\bit\Acal(\Psi^e+\d \Psi)\right|_{\xv=\xv_a}- \left.\bit\Acal(\Psi^e)\right|_{\xv=\xv_a} \nonumber\\
&=  -\d U_a \partial_{x_a} -\d V_a \partial_{y_a} - \d Z_{y_a} \partial_{x_a} \Del_a^{-1} + \d Z_{x_a} \partial_{y_a}\Del_a^{-1} ~.
\end{align}\end{subequations}
or in matrix form:
\begin{subequations}
\begin{align}
&\partial_t \,\d \Zv + \d \U \,\D_x  \Zv^e + \U^e\,\D_x \d \Zv +  \d \V \,\D_y \Zv^e + \V^e\, \D_y \d \Zv  +\beta \,\d \Vv =  - r \,\d \Zv -\nu_4 \,\DDel^2 \d \Zv - \nonumber\\
&\qquad- \D_x \[ \vecd{\( - \D_y \DDel^{-1}\d\C\)}\] - \D_y \[\vecd{\( \D_x \DDel^{-1}\d\C\)}\]\\
&\partial_t\,\d\C  = \A^e \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp~.
\end{align}\end{subequations}

{\color{Green}
For jets, $\Zv^e=-\Uv^e_y$:
\begin{subequations}
\begin{align}
&\partial_t \,\d \Zv +  \d \V \,(-\Uv^e_{yy})  +\beta \,\d \Vv =  - r \,\d \Zv -\nu_4 \,\DDel^2 \d \Zv  - \D_y \[\vecd{\( \D_x \DDel^{-1}\d\C\)}\]\\
&\partial_t\,\d\C  = \A^e \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp~.
\end{align}\end{subequations}

}

The above is a real dynamical system. Searching for eigensolutions, $\d\Psi = \d\hat{\Psi} e^{\s t}$, $\d Z = \d\hat{Z} e^{\s t}$, $\d C = \d\hat{C} e^{ \s t}$:%s. With these substitution we have that $\d\Acal_a = \d\hat{\Acal}_a e^{\s t}$ and moreover:
\begin{subequations}
\begin{align}
&\s \,\d\hat{Z} + \d\hat{U}\, \partial_x Z^e + U^e\, \partial_x \d\hat{Z} +  \d\hat{V} \,\partial_y Z^e + V^e\, \partial_y \d\hat{Z}  +\beta \,\d \hat{V} =  - r \,\d \hat{Z} -\nu_4 \,\Del^2 \d \hat{Z} - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \]\\
&\s\,\d \hat{C}  = \(\bit \Acal^e_a +\Acal^e_b\) \d \hat{C} + \(\bit \d\hat{\Acal}_a +\d\hat{\Acal}_b\) C^e ~.
\end{align}\end{subequations}


\begin{subequations}
\begin{align}
&\s \,\d \Zv + \d \U \,\D_x  \Zv^e + \U^e\,\D_x \d \Zv +  \d \V \,\D_y \Zv^e + \V^e\, \D_y \d \Zv  +\beta \,\d \Vv =  - r \,\d \Zv -\nu_4 \,\DDel^2 \d \Zv - \nonumber\\
&\qquad- \D_x \[ \vecd{\( - \D_y \DDel^{-1}\d\C\)}\] - \D_y \[\vecd{\( \D_x \DDel^{-1}\d\C\)}\]\\
&\s\,\d\C  = \A^e \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp~.
\end{align}\label{eq:pert_S3Tgen}\end{subequations}

{\color{Green}
For jets:
\begin{subequations}
\begin{align}
&\s \,\d\hat{Z}  +  \d\hat{V} \,(-U_{yy}^e)  +\beta \,\d \hat{V} =  - r \,\d \hat{Z} -\nu_4 \,\Del^2 \d \hat{Z} - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \]\\
&\s\,\d \hat{C}  = \(\bit \Acal^e_a +\Acal^e_b\) \d \hat{C} + \(\bit \d\hat{\Acal}_a +\d\hat{\Acal}_b\) C^e ~.
\end{align}\end{subequations}


\begin{subequations}
\begin{align}
&\s \,\d \Zv +  \d \V \,(-\Uv^e_{yy}) + \beta \,\d \Vv =  - r \,\d \Zv -\nu_4 \,\DDel^2 \d \Zv  - \D_y \[\vecd{\( \D_x \DDel^{-1}\d\C\)}\]\\
&\s\,\d\C  = \A^e \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp~.
\end{align}\label{eq:pert_S3Tgen}\end{subequations}


with\begin{subequations}
\begin{align}
\Acal^e_a  &= \left.\bit\Acal(\Psi^e)\right|_{\xv=\xv_a}  = -U^e_a \partial_{x_a}- \(\beta+Z^e_{y_a}\) \partial_{x_a} \Del_a^{-1} - r -\nu_4 \Del_a^2~,\\
\d\Acal_a  &=\left.\bit\Acal(\Psi^e+\d \Psi)\right|_{\xv=\xv_a}- \left.\bit\Acal(\Psi^e)\right|_{\xv=\xv_a} =  -\d U_a \partial_{x_a} -\d V_a \partial_{y_a} - \d Z_{y_a} \partial_{x_a} \Del_a^{-1} + \d Z_{x_a} \partial_{y_a}\Del_a^{-1} ~.
\end{align}\end{subequations}


}




%\subsection{Petros thought}
%
%\be
%\d Z(x,y,t) = \d Z(x-v t,y)
%\ee
%
%Let us have a case with a homogeneous flow equilibrium in which the $\d Z_{mn} = e^{\i(mx+ny)}e^{(\s_r+\i\s_i)t}$ is an eigenfuction with eigenvalue $\s=\s_r+\i\s_i$.

\subsection{Continuous formalism}



S3T system with $Z(\xv,t)$, $C(\xv_a,\xv_b,t) = \Del_a \Del_b\,S(\xv_a,\xv_b,t)$:\begin{subequations}
\begin{align}
&\partial_t  Z + \Uv\cdot\nablav Z  +\beta V =  - r Z -\nu_4 \Del^2 Z - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) C \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) C \right|_{\xv_a=\xv_b} \]\\
&\partial_t C  = \(\bit \Acal_a +\Acal_b\) C + Q~.
\end{align}\end{subequations}
with
\be
\Acal_a \equiv\left.\bit\Acal(\Psi)\right|_{\xv=\xv_a} = -U_a \partial_{x_a}-V_a \partial_{y_a} - \(\beta+Z_{y_a}\) \partial_{x_a} \Del_a^{-1} + Z_{x_a} \partial_{y_a}\Del_a^{-1} - r -\nu_4 \Del_a^2~.
\ee
Perturbations around an equlibrium satisfy:
\begin{subequations}
\begin{align}
&\partial_t \,\d Z + \d U\, \partial_x Z^e + U^e\, \partial_x \d Z +  \d V \,\partial_y Z^e + V^e\, \partial_y \d Z  +\beta \,\d V =  - r \,\d Z -\nu_4 \,\Del^2 \d Z - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d C \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d C \right|_{\xv_a=\xv_b} \]\\
&\partial_t\,\d C  = \(\bit \Acal^e_a +\Acal^e_b\) \d C + \(\bit \d\Acal_a +\d\Acal_b\) C^e ~.
\end{align}\end{subequations}
with\begin{subequations}
\begin{align}
\Acal^e_a  &= \left.\bit\Acal(\Uv^e)\right|_{\xv=\xv_a}  = -U^e_a \partial_{x_a}-V^e_a \partial_{y_a} - \(\beta+Z^e_{y_a}\) \partial_{x_a} \Del_a^{-1} + Z^e_{x_a} \partial_{y_a}\Del_a^{-1} - r -\nu_4 \Del_a^2~,\\
\d\Acal_a  &=\left.\bit\Acal(\Psi^e+\d \Psi)\right|_{\xv=\xv_a}- \left.\bit\Acal(\Psi^e)\right|_{\xv=\xv_a} =  -\d U_a \partial_{x_a} -\d V_a \partial_{y_a} - \d Z_{y_a} \partial_{x_a} \Del_a^{-1} + \d Z_{x_a} \partial_{y_a}\Del_a^{-1} ~.
\end{align}\end{subequations}

The above is a real dynamical system. Searching for eigensolutions, $\d\Psi = \d\hat{\Psi} e^{\s t}$, $\d Z = \d\hat{Z} e^{\s t}$, $\d C = \d\hat{C} e^{ \s t}$:%s. With these substitution we have that $\d\Acal_a = \d\hat{\Acal}_a e^{\s t}$ and moreover:
\begin{subequations}
\begin{align}
&\s \,\d\hat{Z} + \d\hat{U}\, \partial_x Z^e + U^e\, \partial_x \d\hat{Z} +  \d\hat{V} \,\partial_y Z^e + V^e\, \partial_y \d\hat{Z}  +\beta \,\d \hat{V} =  - r \,\d \hat{Z} -\nu_4 \,\Del^2 \d \hat{Z} - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \]\\
&\s\,\d \hat{C}  = \(\bit \Acal^e_a +\Acal^e_b\) \d \hat{C} + \(\bit \d\hat{\Acal}_a +\d\hat{\Acal}_b\) C^e ~.\label{eq:pert_dC_s}
\end{align}\label{eq:pert_syst_cont}\end{subequations}


For a jet equilibrium, $U^e(y), V^e=0, C^e(x_a-x_b,y_a,y_b)$ the equilibrium covariance is homogeneous in $x$. Therefore we expect that the eigenfunction to be of the form:
\begin{subequations}\begin{align}
%\d S &= S_m(\xt,\yt,\yb)\,e^{\i m\xb} \\
%\nonumber\\
\d \Psi_m (x,y,t) &= e^{\i m x} e^{\s t} ~\textrm{`}\sum_n\textrm{'}~ a_n e^{\i n y}  ~,\label{eq:eig_dPsi}\\
\d C_m(x_a,y_a,x_b,y_b) &= e^{\i m(x_a+x_b)/2} ~\textrm{`}\sum_k\textrm{'} ~\d\hat{C}_{k,m} (y_a,y_b) e^{\i k(x_a-x_b)} ~.\label{eq:eig_dCm}
\end{align}\label{eq:eig_dPsim_dCm}\end{subequations}


{\color{Orange}
Where $~\textrm{`}\sum_n\textrm{'}$ can also denote integration if summated index takes values from a continuous domain.
Let us consider our equations confined in a periodic box $L_x$, $L_y$ then not all values of $k$ are allowed. Both $\d\Psi_m$ and $\d C_m$ must obey the periodic boundary conditions. Therefore they must obey:
\begin{subequations}\begin{align}
\d\Psi_m(x+L_x,y,t)&=\d\Psi_m(x,y+L_y,t)=\d\Psi_m(x,y,t)~,\label{eq:dPsi_period}\\
\d C_m(x_a+L_x,y_a,x_b,y_b,t)&=\d C_m(x_a,y_a,x_b+L_x,y_b,t) = \d C_m(x_a+L_x,y_a+L_y,x_b,y_b,t) \nonumber\\
&\qquad\qquad\qquad= \d C_m(x_a,y_a,x_b,y_b+L_y,t)= \d C_m(x_a,y_a,x_b,y_b,t)~.\label{eq:dC_period}
\end{align}\end{subequations}
From Eq.~\eqref{eq:dPsi_period} we have that
\begin{subequations}\begin{align}
e^{\i m L_x} &= 1 \Rightarrow m\textrm{ is an integer multiple of }2\pi/L_x ~,\\
 e^{\i n L_y} &= 1 \Rightarrow n\textrm{ is an integer multiple of }2\pi/L_y ~.
\end{align}\end{subequations}
and from Eq.~\eqref{eq:dC_period} we have that
\begin{subequations}\begin{align}
e^{\i m L_x/2}e^{\i k L_x} &= 1 \Rightarrow (k+m/2)\textrm{ is an integer multiple of }2\pi/L_x \nonumber\\
&\quad\;\;\; \Rightarrow \left\{
	\begin{array}{ll}
		  k = \kappa(2\pi/L_x)~,~\kappa\in\mathbb{Z}  & \textrm{, for $m$ even~,} \\
		 \\
		  k = \dfrac{2\kappa+1}{2}\,(2\pi/L_x)~,~\kappa\in\mathbb{Z}  & \textrm{, for $m$ odd~.} \\
	\end{array}\right.
\end{align}\end{subequations}

For $L_x=L_y=2\pi$ we have that Eqs.~\eqref{eq:eig_dPsim_dCm} take the form:
\begin{subequations}\begin{align}
%\d S &= S_m(\xt,\yt,\yb)\,e^{\i m\xb} \\
%\nonumber\\
\d \Psi_m (x,y,t) &= e^{\i m x} e^{\s t}\sum_{n=-\infty}^{+\infty} a_n e^{\i n y}  ~,m\in\mathbb{Z}~,\label{eq:eig_dPsi_k}\\
\d C_m(x_a,y_a,x_b,y_b) &= e^{\i m(x_a+x_b)/2} \sum_{k=-\infty}^{+\infty} \d\hat{C}_{k,m} (y_a,y_b) e^{\i (k-m/2)(x_a-x_b)} ~,m\in\mathbb{Z} ~,\label{eq:eig_dCm_k}
\end{align}\label{eq:eig_dPsim_dCm}\end{subequations}
Notice that $\d\hat{C}_{k,m} (y_a,y_b)$ corresponds to $e^{\i(k-m/2)(x_a-x_b)}$ which is different for each choice of $m$. We could have defined $\d\hat{C}_{k,m} (y_a,y_b)$ to be the Fourier coefficient corresponding to $e^{\i(k+m/2)(x_a-x_b)}$ but we have made the first choice.
}


If we denote $\d \Psi_{mn} = e^{\i(m x+ny)}$ then this induces:
\be
\[\d U_{mn},\d V_{mn},\d Z_{mn},(\d Z_x)_{mn},(\d Z_y)_{mn}\bit\] = \[\bit-\i n,\i m,-(m^2+n^2),-\i m(m^2+n^2),-\i n(m^2+n^2)\]\d \Psi_{mn} (x,y,t)~,
\ee
and would correspond to $\[\d U_{m},\d V_{m},\d Z_{m},(\d Z_x)_{mn},(\d Z_y)_{mn}\bit\] = e^{\s t} \sum_n a_n \[\d U_{m},\d V_{m},\d Z_{m},(\d Z_x)_{mn},(\d Z_y)_{mn}\bit\]$.

The S3T equilibrium covariance can be written as:
\begin{subequations}\begin{align}
C^e(x_a,y_a,x_b,y_b) &= \sum_{k=-N_k}^{N_k}\hat{C}^e_{k}(y_a,y_b) e^{\i k(x_a-x_b)}  \\
&= \frac1{2}\real{ \[\sum_{k=1}^{N_k} \hat{C}^e_{k}(y_a,y_b) e^{\i k(x_a-x_b)} \]}%\\
%&= \frac1{2} \sum_{k=1}^{N_k} \left\{ \hat{C}^{E,R}_{k}(y_a,y_b) \cos{ \[k(x_a-x_b) \]}-\hat{C}^{E,I}_{k}(y_a,y_b) \sin{ \[k(x_a-x_b) \]} \right\}
\end{align}\end{subequations}

\vspace*{1cm}

\textbf{Notes}\\
1.~~The last equality holds only if $\hat{C}_{k=0}^e=0$, which is true if the forcing covariance has $\hat{Q}_{k=0}=0$ regardless if $U^e$ is zero or not.

2.~~Both $\d C_m$ and $C^e$ have the symmetry that they remain the same under $\xv_a\leftrightarrow\xv_b$.

\vspace*{1cm}

It will be useful to calculate some partial derivatives of $\d C_m$ and $C^e$.\begin{subequations}\begin{align}
\partial_{x_a} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-\infty}^{+\infty} \i k\, \d\hat{C}_{k,m}(y_a,y_b) \,e^{\i (k-m/2)(x_a-x_b)} ~,\\
\partial_{x_b} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-\infty}^{+\infty} -\i\(k-m\) \d\hat{C}_{k,m}(y_a,y_b) \,e^{\i (k-m/2)(x_a-x_b)} ~,\\
\Del_{a} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-\infty}^{+\infty} \[ \partial^2_{y_a} - k^2 \bit\]\d\hat{C}_{k,m}(y_a,y_b) \,e^{\i (k-m/2)(x_a-x_b)} ~,\\
\Del_{\b} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-\infty}^{+\infty} \[ \partial^2_{y_b} - \(k-m\)^2 \]\d\hat{C}_{k,m}(y_a,y_b) \,e^{\i (k-m/2)(x_a-x_b)} ~.
\end{align}\end{subequations}

If the coherent streamfunction perturbation eigenfunction consists of only a single harmonic, $\d\Psi_{mn}$, after defining  $\d E_{n,a} =  e^{\i n y_a}$, some terms of Eq.~\eqref{eq:pert_dC_s} read:
\begin{subequations}\begin{align}
 -(U^e_a &\partial_{x_a} +U^e_b \partial_{x_b}) \,\d C_m = \nonumber\\
 &=e^{\i m(x_a+x_b)/2}\sum_{k=-\infty}^{+\infty}  \[  -\i k U^e_a\,\d\hat{C}_{k,m}(y_a,y_b) +  \i (k-m) U^e_b\,\d\hat{C}_{k,m}(y_a,y_b) \]\,e^{\i (k-m/2)(x_a-x_b)} ~,\\
 -(\d U_a &\partial_{x_a} + \d U_b \partial_{x_b} )  C^e = \nonumber\\
 &=-\sum_{k=-\infty}^{+\infty} \[\d U_a\, \i k \,\hat{C}^e_k(y_a,y_b) + \d U_b \(-\i k\) \hat{C}^e_k(y_a,y_b) \] \,e^{\i k(x_a-x_b)}\nonumber\\
%  &=\i n \sum_{k}  \[ e^{\i m x_a} e^{\i n y_a}\, \i k\,  \hat{C}^e_k(y_a,y_b) + e^{\i m x_b} e^{\i n y_b} \(-\i k\) \hat{C}^e_k(y_a,y_b) \] e^{\i k(x_a-x_b)}~\nonumber\\
%  &=\i n\, e^{\i m(x_a+x_b)/2} \sum_{k}  \[ e^{\i m (x_a-x_b)/2} e^{\i n y_a}\, \i k\,  \hat{C}^e_k(y_a,y_b) + e^{-\i m (x_a-x_b)/2} e^{\i n y_b} \(-\i k\) \hat{C}^e_k(y_a,y_b) \] e^{\i k(x_a-x_b)}\nonumber\\
  &=\i n \, e^{\i m(x_a+x_b)/2} \sum_{k=-\infty}^{+\infty} \left\{  \vphantom{\frac1{2}} \[  \(\i k\,\d E_a\)   \hat{C}^e_k(y_a,y_b) \] \,e^{\i (k+m/2) (x_a-x_b)} + \[   \hat{C}^e_k(y_a,y_b) \(-\i k\,\d E_b\) \] \,e^{\i (k-m/2) (x_a-x_b)}\right\}~.\label{eq:dUadUbCE}
 \end{align}\end{subequations}


The term $e^{\i m(x_a+x_b)/2}$ factors out of all terms of Eq.~\eqref{eq:pert_syst_cont}. After redefining $k\to k'= k+m$ in terms like the first one in Eq.~\eqref{eq:dUadUbCE} we can rewrite Eq.~\eqref{eq:pert_syst_cont} as a system of matrix equations for the perturbation covariances matrices, $\d\C_{k,m}$, which are defined as $\[\d\C_{k,m}\]_{a\b} =\d\hat{C}_{k,m}(y_a,y_b)$. These matrices satisfy:\begin{align}
\s\,\d \C_{k,m} &=  \A^{e,\textrm{L}}_{k}\,\d\C_{k,m} + \d\C_{k,m}\(\A^{e,\textrm{R}}_{k-m}\)^\transp + \sum_n a_n \[\vphantom{\frac1{2}}\d\A^{\rm L}_{k-m,m,n}\C^e_{k-m} + \C^e_{k}\(\d\A^{\rm R}_{k,m,n}\)^\transp\]
\label{eq:pert_dC_s_matr}\end{align}
with:\begin{subequations}\begin{align}
\A^{e,\textrm{L}}_{k} &= -\i k \U^e  -\i k \(\bit \beta -\U^e_{yy} \) \DDel^{-1}_{k}  - r - \nu_4  \DDel^2_{k}~,\\
\A^{e,\textrm{R}}_{k} &= +\i k\U^e  + \i k \(\bit \beta -\U^e_{yy} \) \DDel^{-1}_{k}  - r - \nu_4  \DDel^2_{k}~,\\
\d\A^{\textrm{L}}_{k,m,n} &= -\d\E_n\(+ nk\I+\i m \D_y\)\[\I+(m^2+n^2)\DDel^{-1}_k\]~,\\
\d\A^{\textrm{R}}_{k,m,n} &= -\d\E_n\(- nk\I+\i m \D_y\)\[\I+(m^2+n^2)\DDel^{-1}_k\]~,
\end{align}
\end{subequations}
Equation~\eqref{eq:pert_dC_s_matr} can be solved for $\d\C_{k,m}$ as a Sylvester equation and from $\d\C_{k,m}$ we get $\d C_m$ (Eq.~\eqref{eq:eig_dCm_k}).

\vspace*{2cm}
The following symmetries hold:
\begin{subequations}\begin{align}
\A^{e,\textrm{L}}_{-k} &= \A^{e,\textrm{R}}_{k}~,\\
\d\A^{\textrm{L}}_{-k,m,n} &= \d\A^{\textrm{R}}_{k,m,n} ~,\\
\d\A^{\textrm{L}}_{k,-m,n} &= -\d\A^{\textrm{R}}_{k,m,n} ~,\\
\end{align}
\end{subequations}
Also, because $\d\hat{C}$ and $C^e$ are symmetric in exchange $\xv_a\leftrightarrow\xv_b$ and furthermore $C^e$ is also real, we have that:
\bdm
\left.\begin{array}{ll}
	\C^e_{-k} &=\(\C^e_{k}\)^*~,\textrm{($C^e$ real)}\\
	\C^e_{-k} &=\(\C^e_{k}\)^\transp~,\textrm{($C^e$ symmetric)}
\end{array}\right\}\Rightarrow\nonumber\edm\begin{subequations}\begin{align}
\Rightarrow  \C^e_{k} &= \(\C^e_{k}\)^\dag~,\\
\d\C_{-k,m} &= \(\d\C_{k+m,m}\bit\)^\transp ~.\label{eq:symm_dCk}
\end{align}
If $\d\hat{C}$ is also real then Eq.~\eqref{eq:symm_dCk} becomes:
\be
\d\C_{-k,m} = \(\d\C_{k+m,m}\bit\)^\dag ~.\label{eq:symm_dCk_real}
\ee
\end{subequations}

In general, if $C^e$ has non-zero $\C_k$ for $k=0,\dots,N_k$ then for a fixed $m$ the $\d\C_{k,m}$ that would not be necessarily zero (since they will couple with at least one non-zero $\C^e_k$) will be the ones with $k=-(N_k+m),\dots,(N_k+m)$, which are a total of $2(N_k+m)+1$. However, one can only solve only for the first $N_k+2m$ perturbation covariances, $\d\C_{k,m}$, and deduce the rest $N_k+1$ using the symmetry of Eq.~\eqref{eq:symm_dCk}.

\vspace*{1cm}

\textbf{Note}: For $m=0$ perturbations, if $\C_{k=0}^e\ne0$ we can see that in principle we need to solve for $N_k+1$ perturbation covariances, $\d\C_{k,0}$, and not $N_k$ as it is claimed above. However, we can prove that $\d\C_{k=0,m=0}=0$, even if $\C_{k=0}^e\ne0$ and therefore only $N_k$ perturbation covariances are non-zero.

\vspace*{2cm}



The next step is to find the Reynolds stress divergence, $\d R_m$, that corresponds to $\d C_m$.
\begin{align}
\d R_m &= - \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \]
\end{align}

The term in the first brackets is $\d\<u'q'\>$, which reads:
\begin{align}
\d \<u'q'\> &=  \left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b}  \nonumber\\
&=-\frac1{2}  \left. \bit \sum_{k=-\infty}^{+\infty} \(\partial_{y_a} \Del_a^{-1}+\partial_{y_b} \Del_b^{-1}\) e^{\i m(x_a+x_b)/2} \,\d\hat{C}_{k,m} (y_a,y_b) \,e^{\i (k-m/2)(x_a-x_b)} \right|_{\xv_a=\xv_b} \nonumber\\
\end{align}
Discretizing the $y$-domain and representing $\d \<u'q'\>$ as a column vector we get using the matrix representation for $\d\hat{C}_{k,m}$:
\begin{subequations}\begin{align}
\d \<\mathbf{uq}\> &=-\frac1{2}  \left. \bit e^{\i m(x_a+x_b)/2} \sum_{k=-\infty}^{+\infty} \[\D_y \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\(\D_y\)^\transp\]_{a\b}  e^{\i (k-m/2)(x_a-x_b)} \right|_{\xv_a=\xv_b} \nonumber\\
&=-\frac1{2}   e^{\i m x} \vecd\[\sum_{k=-\infty}^{+\infty} \D_y \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\(\D_y\)^\transp\] ~,\label{eq:duqk}
\end{align}
and similarly for $\d\<v'q'\>$:
\begin{align}
\d \<\mathbf{vq}\> &=\frac1{2}  \left. \bit e^{\i m(x_a+x_b)/2} \sum_{k=-\infty}^{+\infty} \[ \i k \DDel^{-1}_{k}\, \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp \[-\i (k-m)\]\]_{a\b}  e^{\i (k-m/2)(x_a-x_b)} \right|_{\xv_a=\xv_b} \nonumber\\
&=\frac1{2}   e^{\i m x} \vecd\[ \sum_{k=-\infty}^{+\infty}  \i k \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\[-\i (k-m)\]\]~.\label{eq:dvqk}
\end{align}


Therefore $\d\Rv_m$ will be given by:
\begin{align}
\d \Rv_m &= -\partial_x\d \<\mathbf{uq}\> - \D_y\d \<\mathbf{vq}\>\nonumber\\
&=\frac{1}{2}e^{\i m x}  \left\{ \i m \, \vecd\[ \sum_k \D_y \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\(\D_y\)^\transp\] + \dotsb\right.\nonumber\\
&\qquad\qquad\qquad\dotsb+\left. \D_y \vecd\[ \sum_k  \i k \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\[-\i (k-m)\]\] \right\}
\end{align}
\end{subequations}

The Reynolds stress divergence that correspond to $\d\C_{k,m,n}$ are denoted with $\d\Rv_{mn}$. In general, the Reynolds stress divergence $\d\Rv_{mn}$ will be proportional to $e^{\i m x}$, but due to the non-homogeneous terms in $y$, ($U^e$, $U^e_{yy}$), it will not also be proportional to $e^{\i ny}$. The last will only be true in the case of the homogeneous equilibrium.

\vspace{1cm}
\textbf{Note}: In Eq.~\eqref{eq:duqk} for $k=0$ or $k=m$ the operators $\DDel^{-1}_k$ or $\DDel^{-1}_{k-m}$ are ill-defined. For the specific terms we have that $-\D_y  \DDel^{-1}_k = -\D_y^{-1}$. We calculate $\D_y^{-1}$ as the pseudoinverse of $\D_y$ using SVD decomposition and removing the zero singular values of $\D_y$.

%
%Navid
%Nai niko
%kane ti douleia sou, den thelo kati
%apla itan na do ena ypologismo
%
%diabasa tin paragrafo
%eisai sigouros gia to oti o oros den paizei rolo ?
%
%to βsin pou einai stin coherent eksisosi den paizei rolo sto growth rate
%afto mporeis na to deis an pareis Re and Imaginary part tou slanted dispersion (nomizo)
%kai episis ekana ypologismous (exei kairo) stous opoious ebgala ton oro kai pira ta idia growth rates (alla me lathos sigma_i)
%
%mou kanei entyposi, giati eixa kanei ki ego palia kai eixa kataliksei se anti8eto symperasma
%
%tote tha to ksanakano na bebaiotho
%
%o oros sto aristero melos, den einai tipota allo para to Rossby wave speed
%kai gia megalo b konta sto criticality, ta non-zonals exoune sxedon ayto gia sigma_i
%
%Tora, mias kai to deksi melos einai en genei migadiko, ena diaforetiko sigma_i 8a epireasei kai to growth rate
%
%8a to ksanado ki ego
%
%gia mikro b exo kanei ypologismo gia to poso epireazoun oi oroi me to sin\theta
%apla tous exo sto panepistimio
%
%gia megalo b den eixa kataferei na bro apotelesma
%
%a ok, gia mikro beta to ekana ki ego
%gia isotropiko bgainei afto pou exete sto JAS alla me b->bsin
%
%ahoxi, 8ymamai eixe dyo orous bcos\theta kai bsint\heta
%ah, ennoeis to ekanes prin petakseis kanenan oro
%
%nai de 8ymamai akribos
%prepei na koitaksoi tis simeioseis
%
%to poiotiko epixeirima ksexnao to bsin\theta kai to allo b einai meiomeno kata cos\theta douleyei (to exo grapsei p.x sto xarti pou 8a paei sto biblio (einai sto book_paper with Nikos)
%
%ypo tin ennoia oti eksigei p.x giati ta non-zonals einai pio asta8i molis allazei i kampyli ec=f(b) apo f8inousa se ayksousa
%
%kai giati p.x ta non-zonals einai pio asta8i gia NIF kai b<<1 (o oros me to b einai stabilizing) <--- afto den katalavaino ti ennoeis
%
%
%ta fluxes einai uv= A -b^2B (gia mi isotropiko)
%epomenos einai ligotera me b 
%
%afou ta non-zonals "blepoun" mikrotero b, ta fluxes gia ayta 8a einai megalytera -> pio asta8i
%
%B>0 ?
%nai an 8ymamai kala, ektos kai an kano la8os
%katse na skefto
%
%
%ego to bgazo:
%
%\d\<v'\z'\> = \frac{\mu}{8} \frac{\df^2\d U}{\df y^2} + \[\frac{3}{128} \bt^2 (\mu +2)+\frac{\mu }{8}\] \frac{\df^4\d U}{\df y^4}~.
%(an den exo kanei lathos)
%(afto einai to delta<vq>)
%
%
%poso arnitiko einai to mu ?
%
%to -1<mu<1
%
%ara o oros me to b einai 8etikos
%nai ego etsi bgazo
%ok Navid 8a to ksanakoitakso
%8ymomoun oti einai arnitikos, alla 8a to ksanado
%ki ego epeidi i pithanotita na kano lathos einai megali
%
%ok
%katse na do ti kanei o ypologismos kai feygo
%
%
%afto pou les esy A_B bgainei arnitiko
%alla yparxei ena - mprosta apo afto
%
%kalinyxta
%kalinixta
%
%
%
%
%
%B = 3/128 b^2(mu+2)+mu/8
%
%to NIF einai mu<0
%gia b=0 einai arnitiko
%gia b>apo mia krisimi timi ginetai thetiko
%
%
%
%alla den ksero giati


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% these were the first tries which were eventually wrong since dC was not periodic in all its elements

%\begin{subequations}\begin{align}
%\partial_{x_a} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-N_k}^{N_k} \i\(k+\frac{m}{2}\) \d\hat{C}_{k,m}(y_a,y_b) \,e^{\i k(x_a-x_b)} ~,\\
%\partial_{x_b} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-N_k}^{N_k}-\i\(k-\frac{m}{2}\) \d\hat{C}_{k,m}(y_a,y_b) \,e^{\i k(x_a-x_b)} ~,\\
%\Del_{a} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-N_k}^{N_k} \[ \partial^2_{y_a} - \(k+\frac{m}{2}\)^2 \]\d\hat{C}_{k,m}(y_a,y_b) \,e^{\i k(x_a-x_b)}~,\\
%\Del_{\b} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-N_k}^{N_k} \[ \partial^2_{y_b} - \(k-\frac{m}{2}\)^2 \]\d\hat{C}_{k,m}(y_a,y_b) \,e^{\i k(x_a-x_b)}~.
%\end{align}\end{subequations}\begin{subequations}\begin{align}
%\partial_{x_a} C^e = \sum_{k=-N_k}^{N_k} \i k \, \hat{C}^e_k(y_a,y_b) \,e^{\i k(x_a-x_b)} ~~&,~~
%\partial_{x_b} C^e = \sum_{k=-N_k}^{N_k} - \i k \, \hat{C}^e_k(y_a,y_b) \,e^{\i k(x_a-x_b)} ~,\\
%\Del_{a} C^e = \sum_{k=-N_k}^{N_k} \(\partial^2_{y_a}-k^2\) \hat{C}^e_k(y_a,y_b) \,e^{\i k(x_a-x_b)} ~~&,~~
%\Del_{\b} C^e = \sum_{k=-N_k}^{N_k} \(\partial^2_{y_b}-k^2\) \hat{C}^e_k(y_a,y_b) \,e^{\i k(x_a-x_b)} ~,
%\end{align}\end{subequations}
%
%If the coherent streamfunction perturbation eigenfunction consists of only a single harmonic, $\d\Psi_{mn}$, after defining $k_{\pm} = k\pm m/2$ and $\d E_{n,a} =  e^{\i n y_a}$, some terms of Eq.~\eqref{eq:pert_dC_s} read:
%\begin{subequations}\begin{align}
% -(U^e_a &\partial_{x_a} +U^e_b \partial_{x_b}) \,\d C_m = \nonumber\\
% &=e^{\i m(x_a+x_b)/2}\sum_{k=-N_k}^{N_k} \[  -\i k_+ U^e_a\,\d\hat{C}_{k,m}(y_a,y_b) +  \i k_- U^e_b\,\d\hat{C}_{k,m}(y_a,y_b) \]\,e^{\i k(x_a-x_b)} ~,\\
% -(\d U_a &\partial_{x_a} + \d U_b \partial_{x_b} )  C^e = \nonumber\\
% &=-\sum_{k=-N_k}^{N_k} \[\d U_a\, \i k \,\hat{C}^e_k(y_a,y_b) + \d U_b \(-\i k\) \hat{C}^e_k(y_a,y_b) \] \,e^{\i k(x_a-x_b)}\nonumber\\
%%  &=\i n \sum_{k}  \[ e^{\i m x_a} e^{\i n y_a}\, \i k\,  \hat{C}^e_k(y_a,y_b) + e^{\i m x_b} e^{\i n y_b} \(-\i k\) \hat{C}^e_k(y_a,y_b) \] e^{\i k(x_a-x_b)}~\nonumber\\
%%  &=\i n\, e^{\i m(x_a+x_b)/2} \sum_{k}  \[ e^{\i m (x_a-x_b)/2} e^{\i n y_a}\, \i k\,  \hat{C}^e_k(y_a,y_b) + e^{-\i m (x_a-x_b)/2} e^{\i n y_b} \(-\i k\) \hat{C}^e_k(y_a,y_b) \] e^{\i k(x_a-x_b)}\nonumber\\
%  &=\i n \, e^{\i m(x_a+x_b)/2} \sum_{k}\left\{  \vphantom{\frac1{2}} \[  \(\i k\,\d E_a\)   \hat{C}^e_k(y_a,y_b) \] \,e^{\i k_+ (x_a-x_b)} + \[   \hat{C}^e_k(y_a,y_b) \(-\i k\,\d E_b\) \] \,e^{\i k_- (x_a-x_b)}\right\}~.\label{eq:dUadUbCE}
% \end{align}\end{subequations}
%The term $e^{\i m(x_a+x_b)/2}$ factors out of all terms of Eq.~\eqref{eq:pert_syst_cont}, while in $(\d A_a+\d A_b)C^e$ the term $e^{\i k(x_a-x_b)}$ cannot be factored out.
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% these are totally wrong

{\color{Purple}
%For $k,k',m$ integers we have:
%\begin{align}
%\frac1{2\pi} \int_{0}^{2\pi} e^{-\i k' \xt } e^{\i (k+m/2)\xt}\,\df\xt &= \frac{e^{2\pi\i(k+m/2-k')}-1}{2\pi\i(k+m/2-k')} = \left\{
%	\begin{array}{ll}
%		 \d_{k,k'-m/2}  & \mbox{, if } m \textrm{ is even~,} \\
%		 \\
%		 \\
%		\dfrac1{\i \pi (k'-k-m/2)} & \mbox{, if } m \textrm{ is odd~.}
%	\end{array}
%\right.
%\end{align}
%%If $m$ is even, 
%%\be
%%\frac1{2\pi} \int_{0}^{2\pi} e^{-\i k' \xt } e^{\i (k+m/2)\xt}\,\df\xt = \d_{k,k'-m/2}
%%\ee
%%but in the case $m$ is odd then the numerator never vanishes and
%%\be
%%\frac1{2\pi} \int_{0}^{2\pi} e^{-\i k' \xt } e^{\i (k+m/2)\xt}\,\df\xt = \frac1{\i \pi (k'-k-m/2)}
%%\ee
%
%So, in the case $m$ is even, then by multiplying all terms all terms with $e^{-\i k' (x_a-x_b)} / (2\pi)$ and integrate over the whole domain we get Eq.~\eqref{eq:pert_dC_s_matr}. However, for $m$ odd we have that each $\d\hat{C}_{k,m}$ couples with all $\hat{C}^e_k$. For example, the term of Eq.~\eqref{eq:dUadUbCE} becomes:
%\begin{align}
%\s\,\d \hat{C}_{k,m} &=  \sum_n\, a_n\,\i n  \sum_{k'}\[  \vphantom{\frac1{2}} \frac{  \(\i k'\,\d E_a\)   \hat{C}^e_{k'}(y_a,y_b) }{\i \pi (k-k'-m/2)} + \frac{ \hat{C}^e_{k'}(y_a,y_b) \(-\i k'\,\d E_b\)  }{\i \pi (k-k'+m/2)} \]
%\end{align}
%Notice the summation over $k'$ for $\hat{C}^e_{k'}$. This equation can be written in matrix form:
%\begin{align}
%\s\,\d \C_{k,m} &= \sum_n\, a_n\, \i n   \sum_{k'}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \(\i k'\,\d \E_n\)   \C^e_{k'} }{k-k'-m/2} + \frac{ \C^e_{k'} \(-\i k'\,\d \E_n\)^\transp  }{k-k'+m/2} \]
%\end{align}
%
%
%We define $\d \C_{k,m,n}$ the solution of
%\begin{align}
%\(\A^{e,\textrm{L}}_{k,m}-\s\)\,\d\C_{k,m,n} + \d\C_{k,m,n}\(\A^{e,\textrm{R}}_{k,m}\)^\transp &+     \underbrace{\sum_{k'}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \d\A^{\textrm{L}}_{k',m,n}   \C^e_{k'} }{k-k'-m/2} + \frac{ \C^e_{k'} \(\d\A^{\textrm{R}}_{k',m,n}\)^\transp  }{k-k'+m/2} \]}_{\d\Q_{k,m,n}} =0~,\label{eq:dQkmn_def}
%\end{align}
%which consists of $\d\Psi_{mn}$ and we deduce therefore that $\d\C_{k,m}$ which solves the full
%\begin{align}
%\s\,\d \C_{k,m} &=\A^{e,\textrm{L}}_{k,m}\,\d\C_{k,m} + \d\C_{k,m}\(\A^{e,\textrm{R}}_{k,m}\)^\transp + \sum_n\, a_n\,    \sum_{k'}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \d\A^{\textrm{L}}_{k,m,n}   \C^e_{k'} }{k-k'-m/2} + \frac{ \C^e_{k'} \(\d\A^{\textrm{R}}_{k,m,n}\)^\transp  }{k-k'+m/2} \]
%\end{align}
%will be given as $\d\C_{k,m} = \sum_n  a_n\,\d\C_{k,m,n}$.
%
%
%In Eq.~\eqref{eq:dQkmn_def} the $\d\Q_{k,m,n}$ is defined with respect of the $\C_k^e$ matrices as:
%\be
%\d\Q_{k,m,n}=\sum_{k'=-N_k}^{N_k}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \d\A^{\textrm{L}}_{k,m,n}   \C^e_{k'} }{k-k'-m/2} + \frac{ \C^e_{k'} \(\d\A^{\textrm{R}}_{k,m,n}\)^\transp  }{k-k'+m/2} \]
%\ee
%Using the fact that $C^e$ is real and also symmetric in exchange $\xv_a\leftrightarrow\xv_b$ we have that $\C^e_{-k} = \(\C^e_k\)^\transp$. Also $ \d\A^{\textrm{L}}_{-k,m,n}= \d\A^{\textrm{R}}_{k,m,n}$ and $ \d\A^{\textrm{R}}_{-k,m,n}= \d\A^{\textrm{L}}_{k,m,n}$. Therefore $\d\Q_{k,m,n}$ becomes:
%\be
%\d\Q_{k,m,n}=\sum_{k'=1}^{N_k}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \d\A^{\textrm{L}}_{k,m,n}   \C^e_{k'} }{k-k'-m/2}+ \frac{  \d\A^{\textrm{R}}_{k',m,n}  \( \C^e_{k'} \)^\transp}{k+k'-m/2} + \frac{ \C^e_{k'} \(\d\A^{\textrm{R}}_{k,m,n}\)^\transp  }{k-k'+m/2} + \frac{  \( \C^e_{k'} \)^\transp\(\d\A^{\textrm{L}}_{k',m,n}\)^\transp  }{k'+k+m/2} \]
%\ee
%

%For example:
%\begin{align}
%\d C_m(x_a,y_a,x_b,y_b) &= e^{\i m(x_a+x_b)/2} \sum_{k=-N_k}^{N_k} \d\hat{C}_{k,m} (y_a,y_b) e^{\i k(x_a-x_b)} \nonumber\\
% &= e^{\i m(x_a+x_b)/2} \sum_{k=1}^{N_k} \[\d\hat{C}_{k,m} (y_a,y_b) e^{\i k(x_a-x_b)}+\d\hat{C}_{-k,m} (y_a,y_b) e^{-\i k(x_a-x_b)}\] ~.
%  \end{align}
%Since $\d C_m$ is symmetric to $\xv_a\leftrightarrow\xv_b$ we have that $\d\hat{C}_{-k,m} (y_a,y_b)=\d\hat{C}_{k,m} (y_b,y_a)$.
%\begin{align}
%\d C_m(x_a,y_a,x_b,y_b) &= e^{\i m(x_a+x_b)/2} \sum_{k=1}^{N_k} \[\d\hat{C}_{k,m} (y_a,y_b) e^{\i k(x_a-x_b)}+\d\hat{C}_{k,m} (y_b,y_a) e^{-\i k(x_a-x_b)}\] ~,\\
%C^e(x_a,y_a,x_b,y_b) &= \sum_{k=1}^{N_k} \[\hat{C}^e_{k}(y_a,y_b) e^{\i k(x_a-x_b)}+\hat{C}^e_{k}(y_b,y_a) e^{-\i k(x_a-x_b)}\] ~.
%  \end{align}
%  
%
%
%
%
%\begin{subequations}\begin{align}
% -(U^e_a &\partial_{x_a} +U^e_b \partial_{x_b}) \,\d C_m = \nonumber\\
% &=e^{\i m(x_a+x_b)/2} \sum_{k=-N_k}^{N_k} \[  -\i k_+ U^e_a\,\d\hat{C}_{k,m}(y_a,y_b) +  \i k_- U^e_b\,\d\hat{C}_{k,m}(y_a,y_b) \]e^{\i k(x_a-x_b)} ~,\\
% &=e^{\i m(x_a+x_b)/2}\sum_{k=1}^{N_k} \[\(-\i k_+\) U^e_a \d\hat{C}_{k,m} (y_a,y_b) e^{\i k(x_a-x_b)}+\(-\i k_-\) U^e_a\d\hat{C}_{k,m} (y_b,y_a) e^{-\i k(x_a-x_b)}+\dotsb\right.\nonumber\\
% &\qquad\qquad\qquad\qquad\qquad\dotsb+\left. \(\i k_-\) U^e_b \d\hat{C}_{k,m} (y_a,y_b) e^{\i k(x_a-x_b)}+\(\i k_+\) U^e_b\d\hat{C}_{k,m} (y_b,y_a) e^{-\i k(x_a-x_b)}\]  ~.
% \end{align}\end{subequations}
%
%
%\begin{subequations}\begin{align}
% -(\d U_a &\partial_{x_a} + \d U_b \partial_{x_b} )  C^e =\nonumber\\
% &=  -(\d U_a \partial_{x_a} + \d U_b \partial_{x_b} )\sum_{k=1}^{N_k} \[\hat{C}^e_{k}(y_a,y_b) e^{\i k(x_a-x_b)}+\hat{C}^e_{k}(y_b,y_a) e^{-\i k(x_a-x_b)}\]\nonumber\\
% &=\sum_{k} \[\(-\i k\)\,\d U_a\,\hat{C}^e_k(y_a,y_b) e^{\i k(x_a-x_b)}+\(+\i k\)\,\d U_a\,\hat{C}^e_k(y_b,y_a) e^{-\i k(x_a-x_b)}+\dotsb\right.\nonumber\\
% &\qquad\qquad\qquad\qquad\qquad\left.\dotsb+  \d U_b \(-\i k\) \hat{C}^e_k(y_a,y_b) e^{-\i k(x_a-x_b)}+  \d U_b \(+\i k\) \hat{C}^e_k(y_a,y_b) e^{\i k(x_a-x_b)}\] \nonumber\\
% &=e^{\i m(x_a+x_b)/2}\sum_{k} \[\(-\i k\)\,\(-\i n\)\d E_a\,\hat{C}^e_k(y_a,y_b) e^{\i k_+(x_a-x_b)}+\(+\i k\)\,\(-\i n\)\d E_a\,\hat{C}^e_k(y_b,y_a) e^{-\i k_-(x_a-x_b)}+\dotsb\right.\nonumber\\
% &\qquad\qquad\qquad\qquad\qquad\left.\dotsb+  \(-\i k\)\(-\i n\)\d E_b  \hat{C}^e_k(y_a,y_b) e^{-\i k_+(x_a-x_b)}+  \(+\i k\)\(-\i n\)\d E_b  \hat{C}^e_k(y_a,y_b) e^{\i k_-(x_a-x_b)}\] ~.
%  \end{align}\end{subequations}

}




%
%
%
%\subsection{Case with $m$ is even}
%
%
%After summing up for all $n$ to get the $\d A_{\a,\b}$ for the $\d\Psi_m$ (Eq.~\eqref{eq:eig_dPsi}) and also after denoting $\[\d\Ev_n\]_a = e^{\i n y_a}$, $\d\E_n = \diag\(\d\Ev_n\)$ the perturbation covariance perturbation (Eq.~\eqref{eq:pert_dC_s} becomes the matrix equation:
%%\begin{subequations}\begin{align}
%% -(U^e_a &\partial_{x_a} +U^e_a \partial_{x_a}) \d C_m =e^{\i m(x_a+x_b)/2}\sum_k \[ \(-\i k_+ \U^e\) \,\d\C_{k,m} +    \d\C_{k,m}\(\i  k_-\U^e\)^\transp \]_{\a\b}e^{\i k(x_a-x_b)} \\
%% -(\d U_a &\partial_{x_a} + \d U_b \partial_{x_b} )  C^e = \nonumber\\
%%& =\i n \, e^{\i m(x_a+x_b)/2}\sum_{k} \[  \(\i k\, \d\E_n\)   \C^e_k \]_{\a\b} e^{\i k_+ (x_a-x_b)} + \[ \C^e_k  \(-\i k\, \d\E_n\)^\transp \]_{\a\b} e^{\i k_-(x_a-x_b)}
%% \end{align}\end{subequations}
%\begin{align}
%\s\,\d\C_{k,m} &=  \A^{e,\textrm{L}}_{k,m}\,\d\C_{k,m} + \d\C_{k,m}\(\A^{e,\textrm{R}}_{k,m}\)^\transp + \sum_n a_n \[\vphantom{\frac1{2}}\d\A^{\rm L}_{k-m/2,m,n}\C^e_{k-m/2} + \C^e_{k+m/2}\(\d\A^{\rm R}_{k+m/2,m,n}\)^\transp\]
%\label{eq:pert_dC_s_matr}\end{align}
%with:
%\begin{subequations}\begin{align}
%\A^{e,\textrm{L}}_{k,m} &= -\i(k+m/2) \U^e  -\i(k +m/2) \(\bit \beta -\U^e_{yy} \) \DDel^{-1}_{k,+}  - r - \nu_4  \DDel^2_{k,+}~,\\
%\A^{e,\textrm{R}}_{k,m} &= +\i(k- m/2) \U^e  + \i(k- m/2) \(\bit \beta -\U^e_{yy} \) \DDel^{-1}_{k,-}  - r - \nu_4  \DDel^2_{k,-}~,\\
%\d\A^{\textrm{L}}_{k,m,n} &= -\d\E_n\(+ nk\I+\i m \D_y\)\[\I+(m^2+n^2)\DDel^{-1}_k\]~,\\
%\d\A^{\textrm{R}}_{k,m,n} &= -\d\E_n\(- nk\I+\i m \D_y\)\[\I+(m^2+n^2)\DDel^{-1}_k\]~,
%\end{align}
%and
%\begin{align}
%\DDel_{k,\pm }\equiv\DDel_{k\pm m/2} = \D^2 -\(k\pm m/2\)^2\I ~,
%\end{align}
%\end{subequations}
%Equation~\eqref{eq:pert_dC_s_matr} can be solved for $\d\C_{k,m}$ as a Sylvester equation and from $\d\C_{k,m}$ we get $\d C_m$ (Eq.~\eqref{eq:eig_dCm}).
%
%Note:
%If we denote with $\d\C_{k,m,n}$ the solution of:
%\be
%\s\,\d\C_{k,m,n} =  \A^{e,\textrm{L}}_{k,m}\,\d\C_{k,m,n} + \d\C_{k,m,n}\(\A^{e,\textrm{R}}_{k,m}\)^\transp +  \d\A^{\rm L}_{k-m/2,m,n}\C^e_{k-m/2} + \C^e_{k+m/2}\(\d\A^{\rm R}_{k+m/2,m,n}\)^\transp~.\label{eq:eig_dCkmn}
%\ee
%then $\d\C_{k,m} = \sum_n a_n \d\C_{k,m,n}$. 
%
%
%The next step is to find the Reynolds stress divergence, $\d R_m$, that corresponds to $\d C_m$.
%\begin{align}
%\d R_m &= - \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \]
%\end{align}
%
%The term in the first brackets is $\d\<u'q'\>$, which reads:
%\begin{align}
%\d \<u'q'\> &=  \left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b}  \nonumber\\
%&=-\frac1{2}  \left. \bit e^{\i m(x_a+x_b)/2} \sum_k \(\partial_{y_a} \Del_a^{-1}+\partial_{y_b} \Del_b^{-1}\) \d\hat{C}_{k,m} (y_a,y_b) \,e^{\i k(x_a-x_b)} \right|_{\xv_a=\xv_b} \nonumber\\
%\end{align}
%Discretizing the $y$-domain and representing $\d \<u'q'\>$ as a column vector we get using the matrix representation for $\d\hat{C}_{k,m}$:
%\begin{align}
%\d \<\mathbf{uq}\> &=-\frac1{2}  \left. \bit e^{\i m(x_a+x_b)/2} \sum_k \[\D_y \DDel^{-1}_{k,+} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp\(\D_y\)^\transp\]_{\a\b}  e^{\i k(x_a-x_b)} \right|_{\xv_a=\xv_b} \nonumber\\
%&=-\frac1{2}   e^{\i m x} \vecd\[\sum_k \D_y \DDel^{-1}_{k,+} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp\(\D_y\)^\transp\] \nonumber\\
%\end{align}
%and similarly for $\d\<v'q'\>$:
%\begin{align}
%\d \<\mathbf{vq}\> &=\frac1{2}  \left. \bit e^{\i m(x_a+x_b)/2} \sum_k \[ \i k_+ \DDel^{-1}_{k,+}\, \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp \(-\i k_-\)\]_{\a\b}  e^{\i k(x_a-x_b)} \right|_{\xv_a=\xv_b} \nonumber\\
%&=\frac1{2}   e^{\i m x} \vecd\[ \sum_k \i k_+ \DDel^{-1}_{k,+}\, \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp \(-\i k_-\)\] \nonumber\\
%\end{align}
%
%Therefore $\d\Rv_m$ will be given by:
%\begin{align}
%\d \Rv_m &= -\partial_x\d \<\mathbf{uq}\> - \D_y\d \<\mathbf{vq}\>\nonumber\\
%&=\frac{1}{2}e^{\i m x}  \left\{ \i m \, \vecd\[ \sum_k \D_y \DDel^{-1}_{k,+}\, \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp\(\D_y\)^\transp\] + \dotsb\right.\nonumber\\
%&\qquad\qquad\qquad\dotsb+\left. \D_y \vecd\[ \sum_k  \i k_+ \DDel^{-1}_{k,+} \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp \(-\i k_-\)\] \right\}
%\end{align}
%
%The Reynolds stress divergence that correspond to $\d\C_{k,m,n}$ are denoted with $\d\Rv_{mn}$. In general, due to the non-homogeneous terms in $y$, ($U^e$, $U^e_{yy}$), the Reynolds stress divergence $\d\Rv_{mn}$ will be proportional to $e^{\i m x}$ but not also  to $e^{\i ny}$. This will only be true in the case of the homogeneous equilibrium.
%
%\subsection{Case with $m$ is odd}
%Now we have
%
%\begin{align}
%\s\,\d\C_{k,m} &=  \A^{e,\textrm{L}}_{k,m}\,\d\C_{k,m} + \d\C_{k,m}\(\A^{e,\textrm{R}}_{k,m}\)^\transp + \sum_n a_n \sum_{k'} \frac1{\i\pi} \[\frac{\d\A^{\rm L}_{k',m,n}\,\C^e_{k'}}{k'-k+m/2} + \frac{\C^e_{k'}\(\d\A^{\rm R}_{k',m,n} \)^\transp}{k'-k-m/2}\]
%\label{eq:pert_dC_s_matr}\end{align}


\subsection{Corrolaries}

\subsubsection{For every equilibrium $(\Uv^e,C^e)$ the perturbation covariance that corresponds to $m=0$ has $\d\hat{C}_{k=0,m=0}=0$}

Proof: For $m=0$, $k=0$ we have that $\d\A^{\textrm{L}}_{0,0,n} = \d\A^{\textrm{R}}_{0,0,n}=0$, therefore the perturbation covariance $\d\hat{C}_{k=0,m=0}=0$ satisfies:
\be
\(\A^{e,\textrm{L}}_{0,0}-\s\I\)\,\d\C_{0,0} + \d\C_{0,0}\(\A^{e,\textrm{R}}_{0,0}\)^\transp=0 ~,\label{eq:dC00}
\ee
with
\begin{align}
\A^{e,\textrm{L}}_{0,0} &= \A^{e,\textrm{R}}_{0,0} =\(\A^{e,\textrm{R}}_{0,0}\)^\transp \equiv \A^e_{0,0}=   - r - \nu_4  \D_y^4~.
\end{align}
The Sylvester equation \eqref{eq:dC00} has a unique solution unless one of the eigenvalues of $\A^e_{0,0}-\s\I$ is equal to an eigenvalue of $-\A^e_{0,0}$. This happens only for $\s=-2r-\nu_4(m^4+n^4)$, for $m,n$ integers. Otherwise, the only solution is $\d\C_{0,0}=0$.


\vspace{2cm}

In order to solve the eigenproblem of a jet equilibrium we proceed as follows: We suppose a $\d\Psi_{m} = e^{\s t}e^{\i mx}\,\sum_n a_n \d \Psi_{mn}$ for some coefficients $a_n$ and choose a first guess for $\s$. For this given $\s$ we solve Eqs.~\eqref{eq:pert_dC_s_matr} and find all $\d\C_{k,m,n}$ and from that we find the corresponding $\d \hat{R}_{mn}$. We factor the $e^{\i m x}$ dependance out and expand $\d \Rv_{mn}$ in Fourier series in $y$:
\be
\d \hat{R}_{mn} = e^{\i m x}\,\sum_{n'} B^{(m)}_{n'n}\,e^{\i n' y}~.
\ee
Then we go to the perturbation equation for the coherent structure, which for a jet equilibrium takes the form:
\begin{align}
&\sum_n\,a_n\,\[ \s+r+\nu_4\Del^2 + \i m U^e -\frac{\i m}{m^2+n^2} \(\b-U^e_{yy}\) \]  [-(m^2+n^2)]\,\d\Psi_{mn} =   e^{\i m x}\sum_n a_n \(\sum_{n'} B^{(m)}_{n'n}\,e^{\i n' y}\)\nonumber\\
\end{align}
 The term, $e^{\i m x}$ factors out.


\begin{align}
&\sum_n\,-a_n\,(m^2+n^2)\[ \s+r+\nu_4(\partial_y^2-m^2)^2 + \i m U^e -\frac{\i m}{m^2+n^2} \(\b-U^e_{yy}\) \]  \,e^{\i n y} =   \sum_n a_n \(\sum_{n'} B^{(m)}_{n'n}\,e^{\i n' y}\)\nonumber\\
\end{align}


If this was a homogeneous equilibrium ($U^e=V^e=0$) then $B^{(m)}_{n'n} = b^{(m)}_n\,\d_{n'n}$ and the above equation simplifies to:\begin{subequations}
\begin{align}
\sum_{n,n'}\,a_n\, \[ \( \s+r+\nu_4(m^2+n^2)^2 -\frac{\i m\b}{m^2+n^2}  \)  (m^2+n^2)\,\d_{n'n}+ B^{(m)}_{n'n} \]\,e^{\i n' y} &=0~~\Leftrightarrow\label{eq:disp_s_nz_nn'}\\
\sum_n\,a_n\, \[ \( \s+r+\nu_4(m^2+n^2)^2 -\frac{\i m\b}{m^2+n^2}  \)  (m^2+n^2)+ b^{(m)}_{n} \]\,e^{\i n y}&=0~.\label{eq:disp_s_nz_n}
\end{align}
\end{subequations}
Since $e^{\i n y}$ are linearly independent Eq.~\eqref{eq:disp_s_nz_n} can be satisfied for a single $n=n_0$ and all other $a_n$ be set to zero, that is $a_{n_0}=1$ and $a_n=0$ for $n\ne n_0$. Another way to look at this is to notice that Eq.~\eqref{eq:disp_s_nz_nn'} again using the fact that $e^{\i n y}$ are linearly independent can be rewritten as:
\be
\sum_{n}\[-\frac{B^{(m)}_{n'n}}{m^2+n^2}  -\(r+\nu_4(m^2+n^2)^2 -\frac{\i m\b}{m^2+n^2}  \) \,\d_{n'n}\]\,a_n =\s\,\,a_n~~\Leftrightarrow\label{eq:disp_s_nz_eigen}\\
\ee
or in matrix form:
\be
\L^{(m)}\,\av = \s\,\av
\ee
where $\L^{m}$ is the matrix with elements:
\be
 L^{(m)}_{n'n} =-\frac{ B^{(m)}_{n'n} }{m^2+n^2} -\[r+\nu_4(m^2+n^2)^2 -\frac{\i m\b}{m^2+n^2}  \]  \d_{n'n}~.
\ee
and $\av$ is the vector with elements $[\av]_n=a_n$.
Since for the homogeneous equilibrium $B^{(m)}_{nn'} = b^{(m)}_n\,\d_{nn'}$, the matrix $\L^{(m)}$ is diagonal so its eigenvectors are the standard orthonormal basis, $\e_j$, with elements: $[\e_j]_{m} = \d_{jm}$.

\vspace{2cm}
For the jet equilibrium we can expand $U^e = \sum_p\hat{U}^e_p\,e^{\i p y}$. Neglecting $\nu_4$ we have:
\begin{align}
&\sum_n\,a_n\,\( \s+r  -\frac{\i m\b}{m^2+n^2}\)   (m^2+n^2)\,e^{\i n y} + \sum_{n,p} a_n\,\i m\hat{U}_p^e\( m^2+n^2-p^2 \)  \,e^{\i(n+p)y} + \sum_{n,n'} a_n \, B^{(m)}_{n'n}\,e^{\i n'y}=0
\end{align}
By changing summation variables $p\to q=p+n$ in the second sum and $n'\to q$ in the third sum, the above expression can be written:

\begin{align}
&\sum_{n,q}\,a_n\,\( \s+r  -\frac{\i m\b}{m^2+n^2}\)   (m^2+n^2)\,\d_{n,q} + \sum_{n,q} a_n\,\i m\hat{U}_{q-n}^e\[ m^2+n^2-(q-n)^2 \bit\]  + \sum_{n,q} a_n \, B^{(m)}_{q,n}=0\nonumber\\
&\sum_{n,q}\,a_n\,\left\{ \( \s+r  -\frac{\i m\b}{m^2+n^2}\)  \,\d_{n,q} + \i m\,\hat{U}_{q-n}^e\[ 1-\frac{(q-n)^2}{m^2+n^2} \]   +  \frac{B^{(m)}_{q,n}}{m^2+n^2} \right\} e^{\i q y}=0\nonumber\\
&\sum_n\,a_n\,\left\{ \( \s+r  -\frac{\i m\b}{m^2+n^2}\)  \,\d_{n,q} + \i m\,\hat{U}_{q-n}^e\[ 1-\frac{(q-n)^2}{m^2+n^2} \]   +  \frac{B^{(m)}_{q,n}}{m^2+n^2} \right\}=0\nonumber\\
&\sum_n\,a_n\,\left\{ -\( r  -\frac{\i m\b}{m^2+n^2}\)  \,\d_{n,q} - \i m\hat{U}_{q-n}^e\[ 1-\frac{(q-n)^2}{m^2+n^2} \]   - \frac{B^{(m)}_{q,n}}{m^2+n^2}\right\}=\s\,a_q~,
\end{align}
or else as
\be
\L^{(m,{U^e})}\,\av = \s\,\av
\ee
with $\L^{(m,{U^e})}$ the matrix with elements:
\be
\[\L^{(m,{U^e})}\]_{qn} = -\frac{B^{(m)}_{q,n}}{m^2+n^2} -\( r  -\frac{\i m\b}{m^2+n^2}\)  \,\d_{n,q} - \i m\hat{U}_{q-n}^e\[ 1-\frac{(q-n)^2}{m^2+n^2} \] ~.
\ee


\newpage
\subsection{Centroid-difference coordinates}

We write this system in centroid-difference coordinates, $\mathbf{\bar{x}}=(\mathbf{x}_a+\mathbf{x}_b)/2$, $\mathbf{\tilde{x}}=\mathbf{x}_a-\mathbf{x}_b$. This gives:\begin{subequations}
\begin{align}
x_a = \xb + \frac1{2}\xt ~~,~~x_b = \xb - \frac1{2}\yt ~,\\
y_a = \yb + \frac1{2}\yt ~~,~~y_b = \yb - \frac1{2}\yt ~,
\end{align}\end{subequations}
and the derivatives transform to:\begin{subequations}
\begin{align}
\partial_{x_a} = \frac1{2}\partial_{\xb} + \partial_{\xt} ~~&,~~ \partial_{x_b} = \frac1{2}\partial_{\xb} - \partial_{\xt} ~,\\
\partial_{y_a} = \frac1{2}\partial_{\yb} + \partial_{\yt} ~~&,~~ \partial_{y_b} = \frac1{2}\partial_{\yb} - \partial_{\yt}  ~,\\
\Del_a   = \Delt +\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\) +  \frac1{4}\Delb~~&,~~ \Del_b   = \Delt -\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\) +  \frac1{4}\Delb~,\\
\Del_a\Del_b   = \( \Delt+\frac1{4}\Delb\)^2 & - \(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)^2~,\\
\partial_{x_a} \Del_b + \partial_{x_b} \Del_a   = \partial_{\xb}&\( \Delt+\frac1{4}\Delb\) - 2\partial_{\xt}\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)~,\\
\partial_{y_a} \Del_b + \partial_{y_b} \Del_a   = \partial_{\yb}&\( \Delt+\frac1{4}\Delb\) - 2\partial_{\yt}\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)~.
\end{align}

%\begin{subequations}
%\begin{align}
%-U^e_a \partial_{x_a} -U^e_b \partial_{x_b} & = -\Ub^e \partial_{\xb}-\Ut^e \partial_{\xt} ~,\\
%-U^e_a \partial_{x_a} \Del_b -U^e_b \partial_{x_b} \Del_a & = -\(\Ub^e\partial_{\xb} + \Ut^e\partial_{\xt}\)\(\Del+\frac1{4}\Delb\) + 2\(\Ub^e\partial_{\xt} + \frac1{4} \Ut^e\partial_{\xb}\)\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\) ~,\\
%U_{y_a y_a}^e \partial_{x_a} \Del_b + U_{y_b y_b}^e \partial_{x_b} \Del_a & = \(\Ub''^e\partial_{\xb} + \Ut''^e\partial_{\xt}\)\(\Del+\frac1{4}\Delb\) - 2\(\Ub''^e\partial_{\xt} + \frac1{4} \Ut''^e\partial_{\xb}\)\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\) ~,\\
%-\d U_a \partial_{x\a} \Del_b -\d U_b \partial_{x_b} \Del_a &=
%\end{align}\end{subequations}


In general, we also have the following transformations of various quantities:
\begin{align}
\Phi_a \partial_{x_a} +\Phi_b \partial_{x_b} & = \Phib\, \partial_{\xb}+\Phit\, \partial_{\xt} ~~,~~ \Phi_a \partial_{y_a} +\Phi_b \partial_{y_b}  = \Phib\, \partial_{\yb}+\Phit\, \partial_{\yt} ~,\\
\Phi_a \partial_{x_a} \Del_b +\Phi_b \partial_{x_b} \Del_a &=\(\Phib\,\partial_{\xb} + \Phit\,\partial_{\xt}\)\(\Del+\frac1{4}\Delb\) - 2\(\Phib\,\partial_{\xt} + \frac1{4} \Phit\,\partial_{\xb}\)\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)~,\\
\Phi_a \partial_{y_a} \Del_b +\Phi_b \partial_{y_b} \Del_a &=\(\Phib\,\partial_{\yb} + \Phit\,\partial_{\yt}\)\(\Del+\frac1{4}\Delb\) - 2\(\Phib\,\partial_{\yt} + \frac1{4} \Phit\,\partial_{\yb}\)\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)~,
\end{align}\end{subequations}
where we have defined: $\Phib = (\Phi_a+\Phi_b)/2$ and $\Phit = \Phi_a-\Phi_b$.




\subsection{Homogeneous equilibrium}

For the homogeneous equilibrium Eqs.~\eqref{eq:pert_S3Tgen} take the form:\begin{subequations}
\begin{align}
&\( \bit \s + r + \nu_4 \DDel^2   +\beta \,\D_x \DDel^{-1} \)\d \Zv  =  \d\Rv \label{eq:dZ}\\
&\(\A^e-\sigma\) \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp = 0 ~. \label{eq:dC}
\end{align}\label{eqs:pert_hom}\end{subequations}
where we have defined the Reynolds stress divergence $\d\Rv= - \D_x \[\bit \vecd{\( - \D_y \DDel^{-1}\d\C\)}\] - \D_y \[\bit\vecd{\( \D_x \DDel^{-1}\d\C\)}\]$. The equilibrium operator is $\A^e = - \beta \,\D_x \DDel^{-1}-r -\nu_4 \DDel^2$ and
\be
\d\A = -\d\U\,\D_x-\d\V\,\D_y - \d\Z_y\,\D_x\DDel^{-1}+ \d\Z_x\,\D_y\DDel^{-1}~.
\ee
The eigenfunctions of this system are harmonics, $e^{\i(mx+ny)}$.

We assume $\d\Zv_{m,n} = e^{\i(mx+ny)}$ and a corresponding eigenvalue $\s_{m,n}$. We calculate $\d\C_{m,n}$ from Eq.~\eqref{eq:dC} and from that the corresponding Reynolds stress divergence, $\d\Rv_{m,n}$, that corresponds to the $(\d\Zv_{m,n},\s_{m,n})$. We expand the $\d\Rv_{m,n}$ as:
\be
\d\Rv_{m,n} = \sum_{m',n'}  \hat{\R}_{mnm'n'}\,e^{\i(m'x+n'y)}~.
\ee
It can be proven that $\d\Rv_{mn}$ will be proportional to $\d\Z_{mn}$, that is: $\hat{\Rv}_{mnm'n'}=r_{mn}\d_{mm'}\d_{nn'}$ (with $r_{mn}$ in general complex). This way Eq.~\eqref{eq:dZ} is written:
\be
 \( \bit \s + r + \nu_4 (m^2+n^2)^2   -\frac{\i m\beta }{m^2+n^2} - r_{mn}\) \,e^{\i(mx+ny)}  = 0\\
\ee
So our new guess for the eigenvalue, $\s'$ is:
\be
\s' = -r +\frac{\i m\beta }{m^2+n^2} + r_{mn}~.
\ee
We continue this iteration until convergence, that is until $|\s'-\s|\big/|\s'|<\tol$.

\vspace{2cm}

This method works very well in reproducing the results of the non-zonal dispersion relation for every choice of $(m,n)$ and it converges to the unstable eigenvalue even if our initial guess is very far away from that.

%Let us define a ``symbolic'' index $P$ for $m,n$ and $Q$ for $m',n'$ then the above is written: 
%\begin{align}
%\sum_{Q} \[ \( \bit \s + r + \nu_4 (m^2+n^2)^2   -\,\frac{\i m\beta }{m^2+n^2}\)\d_{P,Q} - \r_P \d_{P,Q}\] \,\e_Q  = 0~.\label{eq:eigRhat}
%\end{align}
%Definie diagonal matrix $\L$:
%\be
%\L_{PQ} = \[\r_{P} -\(r +\nu_4 (m^2+n^2)^2   -\,\frac{\i m\beta }{m^2+n^2}\)\]\d_{PQ}~,
%\ee
%we can interpret Eq.~\eqref{eq:eigRhat} as $\v$ being an eigenvector of $\L$ with eigenvalue $\s$.


\subsection{Non Homogeneous equilibrium }

For the homogeneous equilibrium Eqs.~\eqref{eq:pert_S3Tgen} take the form:
\begin{align}
&\( \bit \s + r + \nu_4 \DDel^2   +\beta \,\D_x \DDel^{-1} \)\d \Zv  =  \d\Rv \label{eq:dZ}\\
&\(\A^e-\sigma\) \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp = 0 ~. \label{eq:dC}
\end{align}\label{eqs:pert_hom}

\begin{subequations}
\begin{align}
\[ \bit \s + r + \nu_4 \DDel^2   + \U^e\,\D_x +\(\beta -\U_{yy}^e\)\D_x \DDel^{-1} \]\d \Zv  &=  \d\Rv \label{eq:dZ_UE}\\
\(\A^e-\sigma\) \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp &= 0 ~. \label{eq:dC_UE}
\end{align}\end{subequations}
where now $\A^e= -\U^e\D_x  - \(\beta -\U_{yy}^e\)\D_x \DDel^{-1}-r -\nu_4 \DDel^2$ and we have defined the Reynolds stress divergence $\d\Rv= - \D_x \[\bit \vecd{\( - \D_y \DDel^{-1}\d\C\)}\] - \D_y \[\bit\vecd{\( \D_x \DDel^{-1}\d\C\)}\]$ and
\be
\d\A = -\d\U\,\D_x-\d\V\,\D_y - \d\Z_y\,\D_x\DDel^{-1}+ \d\Z_x\,\D_y\DDel^{-1}~.
\ee
The eigenfunctions of this system are harmonics, $e^{\i(mx+ny)}$.

We assume $\d\Zv_{m} = e^{\i mx} f(y)$ and a corresponding eigenvalue $\s_{m}$. We calculate $\d\C_{m,n}$ from Eq.~\eqref{eq:dC} and from that the corresponding Reynolds stress divergence, $\d\Rv_{m,n}$, that corresponds to the $(\d\Zv_{m,n},\s_{m,n})$. We expand the $\d\Rv_{m,n}$ as:
\be
\d\Rv_{m} = e^{\i mx} \sum_{n'}  \hat{\R}_{mn'}\,e^{\i n'y}~.
\ee



\be
C^e(x_a-x_b,y_a,y_b) = \sum_k e^{\i k (x_a-x_b)} \, C^e_k(y_a,y_b)
\ee


It can be proven that $\d\Rv_{mn}$ will be proportional to $\d\Z_{mn}$, that is: $\hat{\Rv}_{mnm'n'}=r_{mn}\d_{mm'}\d_{nn'}$ (with $r_{mn}$ in general complex). This way Eq.~\eqref{eq:dZ} is written:
\be
 \( \bit \s + r + \nu_4 (m^2+n^2)^2   -\frac{\i m\beta }{m^2+n^2} - r_{mn}\) \,e^{\i(mx+ny)}  = 0\\
\ee
So our new guess for the eigenvalue, $\s'$ is:
\be
\s' = -r +\frac{\i m\beta }{m^2+n^2} + r_{mn}~.
\ee
We continue this iteration until convergence, that is until $|\s'-\s|\big/|\s'|<\tol$.

\vspace{2cm}

This method works very well in reproducing the results of the non-zonal dispersion relation for every choice of $(m,n)$ and it converges to the unstable eigenvalue even if our initial guess is very far away from that.

%Let us define a ``symbolic'' index $P$ for $m,n$ and $Q$ for $m',n'$ then the above is written: 
%\begin{align}
%\sum_{Q} \[ \( \bit \s + r + \nu_4 (m^2+n^2)^2   -\,\frac{\i m\beta }{m^2+n^2}\)\d_{P,Q} - \r_P \d_{P,Q}\] \,\e_Q  = 0~.\label{eq:eigRhat}
%\end{align}
%Definie diagonal matrix $\L$:
%\be
%\L_{PQ} = \[\r_{P} -\(r +\nu_4 (m^2+n^2)^2   -\,\frac{\i m\beta }{m^2+n^2}\)\]\d_{PQ}~,
%\ee
%we can interpret Eq.~\eqref{eq:eigRhat} as $\v$ being an eigenvector of $\L$ with eigenvalue $\s$.



\subsection{Jet equilibrium ($U^e\ne0,V^e=0$)}

Consider now a jet equilibrium $\(\Psi^e(y),C^e\)$. Since the streamfunction is only a function of $y$ the coherent mean flow will have only a streamwise component that is varied in $y$, $\(U^e(y),V^e=0\)$. Also the equilibrium perturbation vorticity covariance, $C^e$ will be homogeneous in $x$, that is it will depend only in the difference coordinate in $x$: $C^e(x_a-x_b,y_a,y_b)$. Therefore it can be readily shown that the perturbation equations take the form:\begin{subequations}
\begin{align}
\[ \bit \s + r + \nu_4 \DDel^2   + \U^e\,\D_x +\(\beta -\U_{yy}^e\)\D_x \DDel^{-1} \]\d \Zv  &=  \d\Rv \label{eq:dZ_UE}\\
\(\A^e-\sigma\) \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp &= 0 ~. \label{eq:dC_UE}
\end{align}\end{subequations}
where now $\A^e= -\U^e\D_x  - \(\beta -\U_{yy}^e\)\D_x \DDel^{-1}-r -\nu_4 \DDel^2$.

The perturbation vorticity eigenfunction will not be a single harmonic function, can it will in general be a sum of harmonics:
\be
\d Z = \sum_{\substack{m,n\\m,n\ne0}} \a_{mn}\,e^{\i\(mx+ny\)}\label{eq:dZ_gen}~,
\ee
(the $m,n\ne 0$ will be omitted from now on).
Let us denote $\d\Zv_{mn} = e^{\i\(mx+ny\)}$ and also let $\d\C_{mn}$ the solution of:
\be
\(\A^e-\sigma\) \d\C_{mn}+ \d\C_{mn}\,\(\A^e\)^\transp + \d\A_{mn}\,\C^e +\C^e\,\(\d\A_{mn}\)^\transp = 0 ~. 
\ee
If $\d\Zv$ is given by Eq.~\eqref{eq:dZ_gen} then we have that 
\be
\d\A = \sum_{m,n} \a_{mn}\,\d\A_{mn}~,
\ee
and therefore:
\begin{align}
\sum_{m,n} \a_{mn}\,\[ \(\A^e-\sigma\) \d\C_{mn}+ \d\C_{mn}\,\(\A^e\)^\transp + \d\A_{mn}\,\C^e +\C^e\,\(\d\A_{mn}\)^\transp \] &= 0~\Leftrightarrow\nonumber\\
 \(\A^e-\sigma\) \(\sum_{m,n} \a_{mn} \d\C_{mn}\)+ \(\sum_{m,n}\a_{mn} \d\C_{mn}\)\,\(\A^e\)^\transp  + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp&= 0~
\end{align}
Therefore the solution $\d\C$ of Eq.~\eqref{eq:dC_UE} is also expanded as:
\be
\d\C = \sum_{m,n} \a_{mn}\,\d\C_{mn}~.
\ee

What is the Reynold stress convergence $\d\Rv$ that is induced by $\d\C$? If we denote $\d\Rv_{mn}$ the Reynold stress convergence induced by $\d\C_{mn}$ then the total $\d\Rv$ will be:
\be
\d\Rv = \sum_{m,n} \a_{mn}\,\d\Rv_{mn}~.
\ee
The $\d\Rv_{mn}$ can be written as a Fourier expansion:
\be
\d\Rv_{mn} = \sum_{m',n'} \hat{R}_{m'n'mn}\,\d\Zv_{m'n'}~.
\ee

From \eqref{eq:dZ_UE} (neglecting $\nu_4$)
\begin{align}
\sum_{m,n} \[ \bit \s + r  + \U^e\,\D_x +\(\beta -\U_{yy}^e\)\D_x \DDel^{-1} \] \a_{mn}\,\d \Zv_{mn}  =  \sum_{m,n,m',n'} \a_{mn} \hat{R}_{m'n'mn}\,\d\Zv_{m'n'} ~\Leftrightarrow\nonumber\\
\sum_{m,n,m',n'} \left\{ \[ \bit \s + r +\U^e\,\D_x +\(\beta -\U_{yy}^e\)\D_x \DDel^{-1} \]\d_{mm'}\d_{nn'}  -    \hat{R}_{m'n'mn} \right\} \a_{mn}\,\d\Zv_{m'n'} ~\Leftrightarrow\nonumber\\
\end{align}

The equilibrium $U^e$ can be also written as $U^e=\sum_p \hat{U}^e_p e^{\i p y}$, $U^e_{yy}=\sum_p -p^2 \hat{U}^e_p e^{\i p y}$.
\be
\sum_{m,n,m',n'} \left\{ \[ \bit \s + r  - \frac{\i m\beta}{m^2+n^2} + \sum_p\i m\(1 - \frac{p^2}{m^2+n^2}  \)\hat{U}_p^e\,e^{\i p y} \]\,\d_{mm'}\d_{nn'}  -    \hat{R}_{m'n'mn} \right\} \a_{mn}\,\d\Zv_{m'n'} ~\nonumber\\
\ee


Let us neglect also the nonlinear advection terms in the equation for the coherent structure and also define a ``symbolic'' index $P$ for $m,n$ and $Q$ for $m',n'$ then the above is written: 
\be
\sum_{P,Q} \left\{ \[ \bit \s + r  - \frac{\i m\beta}{m^2+n^2}  \]\,\d_{QP}  -    \hat{R}_{QP} \right\} \a_{P}\,\d\Zv_{Q} ~\nonumber\\
\ee
Since $\d\Z_Q$ are linearly independent then each
\be
\sum_{P} \left\{ \[ \bit \s + r  - \frac{\i m\beta}{m^2+n^2}  \]\,\d_{QP}  -    \hat{R}_{QP} \right\} \a_{P}
\ee
must be zero, which is equivalent with $\a$ being an eigenvector of $\L=\R-r\I - \vecd(\i m \beta/(m^2+n^2))$ with eigenvalue $\s$. We find the eigenvalues of $\s$, choose the one with the maximum real part and repeat iteration.

==> chapters/app-S3Tlyap_copy.tex <==
% !TEX root = ../thesis.tex



\chapter{S3T stability of non-homogeneous equilibrium states}
\label{app:S3Tlyap}

In this appendix we describe the method by which we calculate the S3T stability of non-homogeneous stationary and non-stationary equilibria.


\clearpage

\section{Stability of finite amplitude traveling wave equilibria or mixed jet-traveling wave equilibria}


%\section{S3T generalized system}

S3T system allowing interaction of coherent structures described by streamfunction $\Psi(x,y)$ (from which all fields can be derived, $U=-\partial_y\Psi$, $V=\partial_x\Psi$, $Z=\Del\Psi$) with the turbulent eddy field, $C = \<\z'(x_a,y_a,t)\z'(x_b,y_b,t)\>$ is:\begin{subequations}
\begin{align}
&\partial_t  Z + U\partial_x Z + V\partial_y Z +\beta V =  - r Z -\nu_4 \Del^2 Z - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) C \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) C \right|_{\xv_a=\xv_b} \]\\
&\partial_t C  = \(\bit \Acal_a +\Acal_b\) C + Q~.
\end{align}\end{subequations}
with
\be
\Acal_a \equiv\left.\bit\Acal(\Psi)\right|_{\xv=\xv_a} = -U_a \partial_{x_a}-V_a \partial_{y_a} - \(\beta+Z_{y_a}\) \partial_{x_a} \Del_a^{-1} + Z_{x_a} \partial_{y_a}\Del_a^{-1} - r -\nu_4 \Del_a^2~.
\ee
This system can be written in matrix form:\begin{subequations}
\begin{align}
&\partial_t \Zv + \U \,\D_x  \Zv  +  \V \,\D_y \Zv  +\beta \, \Vv =  - r \, \Zv -\nu_4 \,\DDel^2 \Zv - \nonumber\\
&\qquad\qquad\qquad- \D_x \[ \vecd{\( - \D_y \DDel^{-1}\C\)}\] - \D_y \[\vecd{\( \D_x \DDel^{-1}\C\)}\]\\
&\partial_t\,\C  = \A\, \C+ \C\,\A^\transp + \Q~.
\end{align}\end{subequations}

This system admits equilibria with a coherent structure described by streamfunction $\Psi^e$ and an eddy vorticity covariance, $C^e$. Perturbations around one of these equilibria satisfy:
\begin{subequations}
\begin{align}
&\partial_t \,\d Z + \d U\, \partial_x Z^e + U^e\, \partial_x \d Z +  \d V \,\partial_y Z^e + V^e\, \partial_y \d Z  +\beta \,\d V =  - r \,\d Z -\nu_4 \,\Del^2 \d Z - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d C \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d C \right|_{\xv_a=\xv_b} \]\\
&\partial_t\,\d C  = \(\bit \Acal^e_a +\Acal^e_b\) \d C + \(\bit \d\Acal_a +\d\Acal_b\) C^e ~.
\end{align}\end{subequations}
with\begin{subequations}
\begin{align}
\Acal^e_a  &= \left.\bit\Acal(\Psi^e)\right|_{\xv=\xv_a}  ,\\
\d\Acal_a  &=\left.\bit\Acal(\Psi^e+\d \Psi)\right|_{\xv=\xv_a}- \left.\bit\Acal(\Psi^e)\right|_{\xv=\xv_a} \nonumber\\
&=  -\d U_a \partial_{x_a} -\d V_a \partial_{y_a} - \d Z_{y_a} \partial_{x_a} \Del_a^{-1} + \d Z_{x_a} \partial_{y_a}\Del_a^{-1} ~.
\end{align}\end{subequations}
or in matrix form:
\begin{subequations}
\begin{align}
&\partial_t \,\d \Zv + \d \U \,\D_x  \Zv^e + \U^e\,\D_x \d \Zv +  \d \V \,\D_y \Zv^e + \V^e\, \D_y \d \Zv  +\beta \,\d \Vv =  - r \,\d \Zv -\nu_4 \,\DDel^2 \d \Zv - \nonumber\\
&\qquad- \D_x \[ \vecd{\( - \D_y \DDel^{-1}\d\C\)}\] - \D_y \[\vecd{\( \D_x \DDel^{-1}\d\C\)}\]\\
&\partial_t\,\d\C  = \A^e \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp~.
\end{align}\end{subequations}

{\color{Green}
For jets, $\Zv^e=-\Uv^e_y$:
\begin{subequations}
\begin{align}
&\partial_t \,\d \Zv +  \d \V \,(-\Uv^e_{yy})  +\beta \,\d \Vv =  - r \,\d \Zv -\nu_4 \,\DDel^2 \d \Zv  - \D_y \[\vecd{\( \D_x \DDel^{-1}\d\C\)}\]\\
&\partial_t\,\d\C  = \A^e \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp~.
\end{align}\end{subequations}

}

The above is a real dynamical system. Searching for eigensolutions, $\d\Psi = \d\hat{\Psi} e^{\s t}$, $\d Z = \d\hat{Z} e^{\s t}$, $\d C = \d\hat{C} e^{ \s t}$:%s. With these substitution we have that $\d\Acal_a = \d\hat{\Acal}_a e^{\s t}$ and moreover:
\begin{subequations}
\begin{align}
&\s \,\d\hat{Z} + \d\hat{U}\, \partial_x Z^e + U^e\, \partial_x \d\hat{Z} +  \d\hat{V} \,\partial_y Z^e + V^e\, \partial_y \d\hat{Z}  +\beta \,\d \hat{V} =  - r \,\d \hat{Z} -\nu_4 \,\Del^2 \d \hat{Z} - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \]\\
&\s\,\d \hat{C}  = \(\bit \Acal^e_a +\Acal^e_b\) \d \hat{C} + \(\bit \d\hat{\Acal}_a +\d\hat{\Acal}_b\) C^e ~.
\end{align}\end{subequations}


\begin{subequations}
\begin{align}
&\s \,\d \Zv + \d \U \,\D_x  \Zv^e + \U^e\,\D_x \d \Zv +  \d \V \,\D_y \Zv^e + \V^e\, \D_y \d \Zv  +\beta \,\d \Vv =  - r \,\d \Zv -\nu_4 \,\DDel^2 \d \Zv - \nonumber\\
&\qquad- \D_x \[ \vecd{\( - \D_y \DDel^{-1}\d\C\)}\] - \D_y \[\vecd{\( \D_x \DDel^{-1}\d\C\)}\]\\
&\s\,\d\C  = \A^e \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp~.
\end{align}\label{eq:pert_S3Tgen}\end{subequations}

{\color{Green}
For jets:
\begin{subequations}
\begin{align}
&\s \,\d\hat{Z}  +  \d\hat{V} \,(-U_{yy}^e)  +\beta \,\d \hat{V} =  - r \,\d \hat{Z} -\nu_4 \,\Del^2 \d \hat{Z} - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \]\\
&\s\,\d \hat{C}  = \(\bit \Acal^e_a +\Acal^e_b\) \d \hat{C} + \(\bit \d\hat{\Acal}_a +\d\hat{\Acal}_b\) C^e ~.
\end{align}\end{subequations}


\begin{subequations}
\begin{align}
&\s \,\d \Zv +  \d \V \,(-\Uv^e_{yy}) + \beta \,\d \Vv =  - r \,\d \Zv -\nu_4 \,\DDel^2 \d \Zv  - \D_y \[\vecd{\( \D_x \DDel^{-1}\d\C\)}\]\\
&\s\,\d\C  = \A^e \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp~.
\end{align}\label{eq:pert_S3Tgen}\end{subequations}


with\begin{subequations}
\begin{align}
\Acal^e_a  &= \left.\bit\Acal(\Psi^e)\right|_{\xv=\xv_a}  = -U^e_a \partial_{x_a}- \(\beta+Z^e_{y_a}\) \partial_{x_a} \Del_a^{-1} - r -\nu_4 \Del_a^2~,\\
\d\Acal_a  &=\left.\bit\Acal(\Psi^e+\d \Psi)\right|_{\xv=\xv_a}- \left.\bit\Acal(\Psi^e)\right|_{\xv=\xv_a} =  -\d U_a \partial_{x_a} -\d V_a \partial_{y_a} - \d Z_{y_a} \partial_{x_a} \Del_a^{-1} + \d Z_{x_a} \partial_{y_a}\Del_a^{-1} ~.
\end{align}\end{subequations}


}




%\subsection{Petros thought}
%
%\be
%\d Z(x,y,t) = \d Z(x-v t,y)
%\ee
%
%Let us have a case with a homogeneous flow equilibrium in which the $\d Z_{mn} = e^{\i(mx+ny)}e^{(\s_r+\i\s_i)t}$ is an eigenfuction with eigenvalue $\s=\s_r+\i\s_i$.

\subsection{Continuous formalism}



S3T system with $Z(\xv,t)$, $C(\xv_a,\xv_b,t) = \Del_a \Del_b\,S(\xv_a,\xv_b,t)$:\begin{subequations}
\begin{align}
&\partial_t  Z + \Uv\cdot\nablav Z  +\beta V =  - r Z -\nu_4 \Del^2 Z - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) C \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) C \right|_{\xv_a=\xv_b} \]\\
&\partial_t C  = \(\bit \Acal_a +\Acal_b\) C + Q~.
\end{align}\end{subequations}
with
\be
\Acal_a \equiv\left.\bit\Acal(\Psi)\right|_{\xv=\xv_a} = -U_a \partial_{x_a}-V_a \partial_{y_a} - \(\beta+Z_{y_a}\) \partial_{x_a} \Del_a^{-1} + Z_{x_a} \partial_{y_a}\Del_a^{-1} - r -\nu_4 \Del_a^2~.
\ee
Perturbations around an equlibrium satisfy:
\begin{subequations}
\begin{align}
&\partial_t \,\d Z + \d U\, \partial_x Z^e + U^e\, \partial_x \d Z +  \d V \,\partial_y Z^e + V^e\, \partial_y \d Z  +\beta \,\d V =  - r \,\d Z -\nu_4 \,\Del^2 \d Z - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d C \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d C \right|_{\xv_a=\xv_b} \]\\
&\partial_t\,\d C  = \(\bit \Acal^e_a +\Acal^e_b\) \d C + \(\bit \d\Acal_a +\d\Acal_b\) C^e ~.
\end{align}\end{subequations}
with\begin{subequations}
\begin{align}
\Acal^e_a  &= \left.\bit\Acal(\Uv^e)\right|_{\xv=\xv_a}  = -U^e_a \partial_{x_a}-V^e_a \partial_{y_a} - \(\beta+Z^e_{y_a}\) \partial_{x_a} \Del_a^{-1} + Z^e_{x_a} \partial_{y_a}\Del_a^{-1} - r -\nu_4 \Del_a^2~,\\
\d\Acal_a  &=\left.\bit\Acal(\Psi^e+\d \Psi)\right|_{\xv=\xv_a}- \left.\bit\Acal(\Psi^e)\right|_{\xv=\xv_a} =  -\d U_a \partial_{x_a} -\d V_a \partial_{y_a} - \d Z_{y_a} \partial_{x_a} \Del_a^{-1} + \d Z_{x_a} \partial_{y_a}\Del_a^{-1} ~.
\end{align}\end{subequations}

The above is a real dynamical system. Searching for eigensolutions, $\d\Psi = \d\hat{\Psi} e^{\s t}$, $\d Z = \d\hat{Z} e^{\s t}$, $\d C = \d\hat{C} e^{ \s t}$:%s. With these substitution we have that $\d\Acal_a = \d\hat{\Acal}_a e^{\s t}$ and moreover:
\begin{subequations}
\begin{align}
&\s \,\d\hat{Z} + \d\hat{U}\, \partial_x Z^e + U^e\, \partial_x \d\hat{Z} +  \d\hat{V} \,\partial_y Z^e + V^e\, \partial_y \d\hat{Z}  +\beta \,\d \hat{V} =  - r \,\d \hat{Z} -\nu_4 \,\Del^2 \d \hat{Z} - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \]\\
&\s\,\d \hat{C}  = \(\bit \Acal^e_a +\Acal^e_b\) \d \hat{C} + \(\bit \d\hat{\Acal}_a +\d\hat{\Acal}_b\) C^e ~.\label{eq:pert_dC_s}
\end{align}\label{eq:pert_syst_cont}\end{subequations}


For a jet equilibrium, $U^e(y), V^e=0, C^e(x_a-x_b,y_a,y_b)$ the equilibrium covariance is homogeneous in $x$. Therefore we expect that the eigenfunction to be of the form:
\begin{subequations}\begin{align}
%\d S &= S_m(\xt,\yt,\yb)\,e^{\i m\xb} \\
%\nonumber\\
\d \Psi_m (x,y,t) &= e^{\i m x} e^{\s t} ~\textrm{`}\sum_n\textrm{'}~ a_n e^{\i n y}  ~,\label{eq:eig_dPsi}\\
\d C_m(x_a,y_a,x_b,y_b) &= e^{\i m(x_a+x_b)/2} ~\textrm{`}\sum_k\textrm{'} ~\d\hat{C}_{k,m} (y_a,y_b) e^{\i k(x_a-x_b)} ~.\label{eq:eig_dCm}
\end{align}\label{eq:eig_dPsim_dCm}\end{subequations}


{\color{Orange}
Where $~\textrm{`}\sum_n\textrm{'}$ can also denote integration if summated index takes values from a continuous domain.
Let us consider our equations confined in a periodic box $L_x$, $L_y$ then not all values of $k$ are allowed. Both $\d\Psi_m$ and $\d C_m$ must obey the periodic boundary conditions. Therefore they must obey:
\begin{subequations}\begin{align}
\d\Psi_m(x+L_x,y,t)&=\d\Psi_m(x,y+L_y,t)=\d\Psi_m(x,y,t)~,\label{eq:dPsi_period}\\
\d C_m(x_a+L_x,y_a,x_b,y_b,t)&=\d C_m(x_a,y_a,x_b+L_x,y_b,t) = \d C_m(x_a+L_x,y_a+L_y,x_b,y_b,t) \nonumber\\
&\qquad\qquad\qquad= \d C_m(x_a,y_a,x_b,y_b+L_y,t)= \d C_m(x_a,y_a,x_b,y_b,t)~.\label{eq:dC_period}
\end{align}\end{subequations}
From Eq.~\eqref{eq:dPsi_period} we have that
\begin{subequations}\begin{align}
e^{\i m L_x} &= 1 \Rightarrow m\textrm{ is an integer multiple of }2\pi/L_x ~,\\
 e^{\i n L_y} &= 1 \Rightarrow n\textrm{ is an integer multiple of }2\pi/L_y ~.
\end{align}\end{subequations}
and from Eq.~\eqref{eq:dC_period} we have that
\begin{subequations}\begin{align}
e^{\i m L_x/2}e^{\i k L_x} &= 1 \Rightarrow (k+m/2)\textrm{ is an integer multiple of }2\pi/L_x \nonumber\\
&\quad\;\;\; \Rightarrow \left\{
	\begin{array}{ll}
		  k = \kappa(2\pi/L_x)~,~\kappa\in\mathbb{Z}  & \textrm{, for $m$ even~,} \\
		 \\
		  k = \dfrac{2\kappa+1}{2}\,(2\pi/L_x)~,~\kappa\in\mathbb{Z}  & \textrm{, for $m$ odd~.} \\
	\end{array}\right.
\end{align}\end{subequations}

For $L_x=L_y=2\pi$ we have that Eqs.~\eqref{eq:eig_dPsim_dCm} take the form:
\begin{subequations}\begin{align}
%\d S &= S_m(\xt,\yt,\yb)\,e^{\i m\xb} \\
%\nonumber\\
\d \Psi_m (x,y,t) &= e^{\i m x} e^{\s t}\sum_{n=-\infty}^{+\infty} a_n e^{\i n y}  ~,m\in\mathbb{Z}~,\label{eq:eig_dPsi_k}\\
\d C_m(x_a,y_a,x_b,y_b) &= e^{\i m(x_a+x_b)/2} \sum_{k=-\infty}^{+\infty} \d\hat{C}_{k,m} (y_a,y_b) e^{\i (k-m/2)(x_a-x_b)} ~,m\in\mathbb{Z} ~,\label{eq:eig_dCm_k}
\end{align}\label{eq:eig_dPsim_dCm}\end{subequations}
Notice that $\d\hat{C}_{k,m} (y_a,y_b)$ corresponds to $e^{\i(k-m/2)(x_a-x_b)}$ which is different for each choice of $m$. We could have defined $\d\hat{C}_{k,m} (y_a,y_b)$ to be the Fourier coefficient corresponding to $e^{\i(k+m/2)(x_a-x_b)}$ but we have made the first choice.
}


If we denote $\d \Psi_{mn} = e^{\i(m x+ny)}$ then this induces:
\be
\[\d U_{mn},\d V_{mn},\d Z_{mn},(\d Z_x)_{mn},(\d Z_y)_{mn}\bit\] = \[\bit-\i n,\i m,-(m^2+n^2),-\i m(m^2+n^2),-\i n(m^2+n^2)\]\d \Psi_{mn} (x,y,t)~,
\ee
and would correspond to $\[\d U_{m},\d V_{m},\d Z_{m},(\d Z_x)_{mn},(\d Z_y)_{mn}\bit\] = e^{\s t} \sum_n a_n \[\d U_{m},\d V_{m},\d Z_{m},(\d Z_x)_{mn},(\d Z_y)_{mn}\bit\]$.

The S3T equilibrium covariance can be written as:
\begin{subequations}\begin{align}
C^e(x_a,y_a,x_b,y_b) &= \sum_{k=-N_k}^{N_k}\hat{C}^e_{k}(y_a,y_b) e^{\i k(x_a-x_b)}  \\
&= \frac1{2}\real{ \[\sum_{k=1}^{N_k} \hat{C}^e_{k}(y_a,y_b) e^{\i k(x_a-x_b)} \]}%\\
%&= \frac1{2} \sum_{k=1}^{N_k} \left\{ \hat{C}^{E,R}_{k}(y_a,y_b) \cos{ \[k(x_a-x_b) \]}-\hat{C}^{E,I}_{k}(y_a,y_b) \sin{ \[k(x_a-x_b) \]} \right\}
\end{align}\end{subequations}

\vspace*{1cm}

\textbf{Notes}\\
1.~~The last equality holds only if $\hat{C}_{k=0}^e=0$, which is true if the forcing covariance has $\hat{Q}_{k=0}=0$ regardless if $U^e$ is zero or not.

2.~~Both $\d C_m$ and $C^e$ have the symmetry that they remain the same under $\xv_a\leftrightarrow\xv_b$.

\vspace*{1cm}

It will be useful to calculate some partial derivatives of $\d C_m$ and $C^e$.\begin{subequations}\begin{align}
\partial_{x_a} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-\infty}^{+\infty} \i k\, \d\hat{C}_{k,m}(y_a,y_b) \,e^{\i (k-m/2)(x_a-x_b)} ~,\\
\partial_{x_b} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-\infty}^{+\infty} -\i\(k-m\) \d\hat{C}_{k,m}(y_a,y_b) \,e^{\i (k-m/2)(x_a-x_b)} ~,\\
\Del_{a} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-\infty}^{+\infty} \[ \partial^2_{y_a} - k^2 \bit\]\d\hat{C}_{k,m}(y_a,y_b) \,e^{\i (k-m/2)(x_a-x_b)} ~,\\
\Del_{\b} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-\infty}^{+\infty} \[ \partial^2_{y_b} - \(k-m\)^2 \]\d\hat{C}_{k,m}(y_a,y_b) \,e^{\i (k-m/2)(x_a-x_b)} ~.
\end{align}\end{subequations}

If the coherent streamfunction perturbation eigenfunction consists of only a single harmonic, $\d\Psi_{mn}$, after defining  $\d E_{n,a} =  e^{\i n y_a}$, some terms of Eq.~\eqref{eq:pert_dC_s} read:
\begin{subequations}\begin{align}
 -(U^e_a &\partial_{x_a} +U^e_b \partial_{x_b}) \,\d C_m = \nonumber\\
 &=e^{\i m(x_a+x_b)/2}\sum_{k=-\infty}^{+\infty}  \[  -\i k U^e_a\,\d\hat{C}_{k,m}(y_a,y_b) +  \i (k-m) U^e_b\,\d\hat{C}_{k,m}(y_a,y_b) \]\,e^{\i (k-m/2)(x_a-x_b)} ~,\\
 -(\d U_a &\partial_{x_a} + \d U_b \partial_{x_b} )  C^e = \nonumber\\
 &=-\sum_{k=-\infty}^{+\infty} \[\d U_a\, \i k \,\hat{C}^e_k(y_a,y_b) + \d U_b \(-\i k\) \hat{C}^e_k(y_a,y_b) \] \,e^{\i k(x_a-x_b)}\nonumber\\
%  &=\i n \sum_{k}  \[ e^{\i m x_a} e^{\i n y_a}\, \i k\,  \hat{C}^e_k(y_a,y_b) + e^{\i m x_b} e^{\i n y_b} \(-\i k\) \hat{C}^e_k(y_a,y_b) \] e^{\i k(x_a-x_b)}~\nonumber\\
%  &=\i n\, e^{\i m(x_a+x_b)/2} \sum_{k}  \[ e^{\i m (x_a-x_b)/2} e^{\i n y_a}\, \i k\,  \hat{C}^e_k(y_a,y_b) + e^{-\i m (x_a-x_b)/2} e^{\i n y_b} \(-\i k\) \hat{C}^e_k(y_a,y_b) \] e^{\i k(x_a-x_b)}\nonumber\\
  &=\i n \, e^{\i m(x_a+x_b)/2} \sum_{k=-\infty}^{+\infty} \left\{  \vphantom{\frac1{2}} \[  \(\i k\,\d E_a\)   \hat{C}^e_k(y_a,y_b) \] \,e^{\i (k+m/2) (x_a-x_b)} + \[   \hat{C}^e_k(y_a,y_b) \(-\i k\,\d E_b\) \] \,e^{\i (k-m/2) (x_a-x_b)}\right\}~.\label{eq:dUadUbCE}
 \end{align}\end{subequations}


The term $e^{\i m(x_a+x_b)/2}$ factors out of all terms of Eq.~\eqref{eq:pert_syst_cont}. After redefining $k\to k'= k+m$ in terms like the first one in Eq.~\eqref{eq:dUadUbCE} we can rewrite Eq.~\eqref{eq:pert_syst_cont} as a system of matrix equations for the perturbation covariances matrices, $\d\C_{k,m}$, which are defined as $\[\d\C_{k,m}\]_{a\b} =\d\hat{C}_{k,m}(y_a,y_b)$. These matrices satisfy:\begin{align}
\s\,\d \C_{k,m} &=  \A^{e,\textrm{L}}_{k}\,\d\C_{k,m} + \d\C_{k,m}\(\A^{e,\textrm{R}}_{k-m}\)^\transp + \sum_n a_n \[\vphantom{\frac1{2}}\d\A^{\rm L}_{k-m,m,n}\C^e_{k-m} + \C^e_{k}\(\d\A^{\rm R}_{k,m,n}\)^\transp\]
\label{eq:pert_dC_s_matr}\end{align}
with:\begin{subequations}\begin{align}
\A^{e,\textrm{L}}_{k} &= -\i k \U^e  -\i k \(\bit \beta -\U^e_{yy} \) \DDel^{-1}_{k}  - r - \nu_4  \DDel^2_{k}~,\\
\A^{e,\textrm{R}}_{k} &= +\i k\U^e  + \i k \(\bit \beta -\U^e_{yy} \) \DDel^{-1}_{k}  - r - \nu_4  \DDel^2_{k}~,\\
\d\A^{\textrm{L}}_{k,m,n} &= -\d\E_n\(+ nk\I+\i m \D_y\)\[\I+(m^2+n^2)\DDel^{-1}_k\]~,\\
\d\A^{\textrm{R}}_{k,m,n} &= -\d\E_n\(- nk\I+\i m \D_y\)\[\I+(m^2+n^2)\DDel^{-1}_k\]~,
\end{align}
\end{subequations}
Equation~\eqref{eq:pert_dC_s_matr} can be solved for $\d\C_{k,m}$ as a Sylvester equation and from $\d\C_{k,m}$ we get $\d C_m$ (Eq.~\eqref{eq:eig_dCm_k}).

\vspace*{2cm}
The following symmetries hold:
\begin{subequations}\begin{align}
\A^{e,\textrm{L}}_{-k} &= \A^{e,\textrm{R}}_{k}~,\\
\d\A^{\textrm{L}}_{-k,m,n} &= \d\A^{\textrm{R}}_{k,m,n} ~,\\
\d\A^{\textrm{L}}_{k,-m,n} &= -\d\A^{\textrm{R}}_{k,m,n} ~,\\
\end{align}
\end{subequations}
Also, because $\d\hat{C}$ and $C^e$ are symmetric in exchange $\xv_a\leftrightarrow\xv_b$ and furthermore $C^e$ is also real, we have that:
\bdm
\left.\begin{array}{ll}
	\C^e_{-k} &=\(\C^e_{k}\)^*~,\textrm{($C^e$ real)}\\
	\C^e_{-k} &=\(\C^e_{k}\)^\transp~,\textrm{($C^e$ symmetric)}
\end{array}\right\}\Rightarrow\nonumber\edm\begin{subequations}\begin{align}
\Rightarrow  \C^e_{k} &= \(\C^e_{k}\)^\dag~,\\
\d\C_{-k,m} &= \(\d\C_{k+m,m}\bit\)^\transp ~.\label{eq:symm_dCk}
\end{align}
If $\d\hat{C}$ is also real then Eq.~\eqref{eq:symm_dCk} becomes:
\be
\d\C_{-k,m} = \(\d\C_{k+m,m}\bit\)^\dag ~.\label{eq:symm_dCk_real}
\ee
\end{subequations}

In general, if $C^e$ has non-zero $\C_k$ for $k=0,\dots,N_k$ then for a fixed $m$ the $\d\C_{k,m}$ that would not be necessarily zero (since they will couple with at least one non-zero $\C^e_k$) will be the ones with $k=-(N_k+m),\dots,(N_k+m)$, which are a total of $2(N_k+m)+1$. However, one can only solve only for the first $N_k+2m$ perturbation covariances, $\d\C_{k,m}$, and deduce the rest $N_k+1$ using the symmetry of Eq.~\eqref{eq:symm_dCk}.

\vspace*{1cm}

\textbf{Note}: For $m=0$ perturbations, if $\C_{k=0}^e\ne0$ we can see that in principle we need to solve for $N_k+1$ perturbation covariances, $\d\C_{k,0}$, and not $N_k$ as it is claimed above. However, we can prove that $\d\C_{k=0,m=0}=0$, even if $\C_{k=0}^e\ne0$ and therefore only $N_k$ perturbation covariances are non-zero.

\vspace*{2cm}



The next step is to find the Reynolds stress divergence, $\d R_m$, that corresponds to $\d C_m$.
\begin{align}
\d R_m &= - \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \]
\end{align}

The term in the first brackets is $\d\<u'q'\>$, which reads:
\begin{align}
\d \<u'q'\> &=  \left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b}  \nonumber\\
&=-\frac1{2}  \left. \bit \sum_{k=-\infty}^{+\infty} \(\partial_{y_a} \Del_a^{-1}+\partial_{y_b} \Del_b^{-1}\) e^{\i m(x_a+x_b)/2} \,\d\hat{C}_{k,m} (y_a,y_b) \,e^{\i (k-m/2)(x_a-x_b)} \right|_{\xv_a=\xv_b} \nonumber\\
\end{align}
Discretizing the $y$-domain and representing $\d \<u'q'\>$ as a column vector we get using the matrix representation for $\d\hat{C}_{k,m}$:
\begin{subequations}\begin{align}
\d \<\mathbf{uq}\> &=-\frac1{2}  \left. \bit e^{\i m(x_a+x_b)/2} \sum_{k=-\infty}^{+\infty} \[\D_y \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\(\D_y\)^\transp\]_{a\b}  e^{\i (k-m/2)(x_a-x_b)} \right|_{\xv_a=\xv_b} \nonumber\\
&=-\frac1{2}   e^{\i m x} \vecd\[\sum_{k=-\infty}^{+\infty} \D_y \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\(\D_y\)^\transp\] ~,\label{eq:duqk}
\end{align}
and similarly for $\d\<v'q'\>$:
\begin{align}
\d \<\mathbf{vq}\> &=\frac1{2}  \left. \bit e^{\i m(x_a+x_b)/2} \sum_{k=-\infty}^{+\infty} \[ \i k \DDel^{-1}_{k}\, \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp \[-\i (k-m)\]\]_{a\b}  e^{\i (k-m/2)(x_a-x_b)} \right|_{\xv_a=\xv_b} \nonumber\\
&=\frac1{2}   e^{\i m x} \vecd\[ \sum_{k=-\infty}^{+\infty}  \i k \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\[-\i (k-m)\]\]~.\label{eq:dvqk}
\end{align}


Therefore $\d\Rv_m$ will be given by:
\begin{align}
\d \Rv_m &= -\partial_x\d \<\mathbf{uq}\> - \D_y\d \<\mathbf{vq}\>\nonumber\\
&=\frac{1}{2}e^{\i m x}  \left\{ \i m \, \vecd\[ \sum_k \D_y \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\(\D_y\)^\transp\] + \dotsb\right.\nonumber\\
&\qquad\qquad\qquad\dotsb+\left. \D_y \vecd\[ \sum_k  \i k \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\[-\i (k-m)\]\] \right\}
\end{align}
\end{subequations}

The Reynolds stress divergence that correspond to $\d\C_{k,m,n}$ are denoted with $\d\Rv_{mn}$. In general, the Reynolds stress divergence $\d\Rv_{mn}$ will be proportional to $e^{\i m x}$, but due to the non-homogeneous terms in $y$, ($U^e$, $U^e_{yy}$), it will not also be proportional to $e^{\i ny}$. The last will only be true in the case of the homogeneous equilibrium.

\vspace{1cm}
\textbf{Note}: In Eq.~\eqref{eq:duqk} for $k=0$ or $k=m$ the operators $\DDel^{-1}_k$ or $\DDel^{-1}_{k-m}$ are ill-defined. For the specific terms we have that $-\D_y  \DDel^{-1}_k = -\D_y^{-1}$. We calculate $\D_y^{-1}$ as the pseudoinverse of $\D_y$ using SVD decomposition and removing the zero singular values of $\D_y$.

%
%Navid
%Nai niko
%kane ti douleia sou, den thelo kati
%apla itan na do ena ypologismo
%
%diabasa tin paragrafo
%eisai sigouros gia to oti o oros den paizei rolo ?
%
%to βsin pou einai stin coherent eksisosi den paizei rolo sto growth rate
%afto mporeis na to deis an pareis Re and Imaginary part tou slanted dispersion (nomizo)
%kai episis ekana ypologismous (exei kairo) stous opoious ebgala ton oro kai pira ta idia growth rates (alla me lathos sigma_i)
%
%mou kanei entyposi, giati eixa kanei ki ego palia kai eixa kataliksei se anti8eto symperasma
%
%tote tha to ksanakano na bebaiotho
%
%o oros sto aristero melos, den einai tipota allo para to Rossby wave speed
%kai gia megalo b konta sto criticality, ta non-zonals exoune sxedon ayto gia sigma_i
%
%Tora, mias kai to deksi melos einai en genei migadiko, ena diaforetiko sigma_i 8a epireasei kai to growth rate
%
%8a to ksanado ki ego
%
%gia mikro b exo kanei ypologismo gia to poso epireazoun oi oroi me to sin\theta
%apla tous exo sto panepistimio
%
%gia megalo b den eixa kataferei na bro apotelesma
%
%a ok, gia mikro beta to ekana ki ego
%gia isotropiko bgainei afto pou exete sto JAS alla me b->bsin
%
%ahoxi, 8ymamai eixe dyo orous bcos\theta kai bsint\heta
%ah, ennoeis to ekanes prin petakseis kanenan oro
%
%nai de 8ymamai akribos
%prepei na koitaksoi tis simeioseis
%
%to poiotiko epixeirima ksexnao to bsin\theta kai to allo b einai meiomeno kata cos\theta douleyei (to exo grapsei p.x sto xarti pou 8a paei sto biblio (einai sto book_paper with Nikos)
%
%ypo tin ennoia oti eksigei p.x giati ta non-zonals einai pio asta8i molis allazei i kampyli ec=f(b) apo f8inousa se ayksousa
%
%kai giati p.x ta non-zonals einai pio asta8i gia NIF kai b<<1 (o oros me to b einai stabilizing) <--- afto den katalavaino ti ennoeis
%
%
%ta fluxes einai uv= A -b^2B (gia mi isotropiko)
%epomenos einai ligotera me b 
%
%afou ta non-zonals "blepoun" mikrotero b, ta fluxes gia ayta 8a einai megalytera -> pio asta8i
%
%B>0 ?
%nai an 8ymamai kala, ektos kai an kano la8os
%katse na skefto
%
%
%ego to bgazo:
%
%\d\<v'\z'\> = \frac{\mu}{8} \frac{\df^2\d U}{\df y^2} + \[\frac{3}{128} \bt^2 (\mu +2)+\frac{\mu }{8}\] \frac{\df^4\d U}{\df y^4}~.
%(an den exo kanei lathos)
%(afto einai to delta<vq>)
%
%
%poso arnitiko einai to mu ?
%
%to -1<mu<1
%
%ara o oros me to b einai 8etikos
%nai ego etsi bgazo
%ok Navid 8a to ksanakoitakso
%8ymomoun oti einai arnitikos, alla 8a to ksanado
%ki ego epeidi i pithanotita na kano lathos einai megali
%
%ok
%katse na do ti kanei o ypologismos kai feygo
%
%
%afto pou les esy A_B bgainei arnitiko
%alla yparxei ena - mprosta apo afto
%
%kalinyxta
%kalinixta
%
%
%
%
%
%B = 3/128 b^2(mu+2)+mu/8
%
%to NIF einai mu<0
%gia b=0 einai arnitiko
%gia b>apo mia krisimi timi ginetai thetiko
%
%
%
%alla den ksero giati


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% these were the first tries which were eventually wrong since dC was not periodic in all its elements

%\begin{subequations}\begin{align}
%\partial_{x_a} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-N_k}^{N_k} \i\(k+\frac{m}{2}\) \d\hat{C}_{k,m}(y_a,y_b) \,e^{\i k(x_a-x_b)} ~,\\
%\partial_{x_b} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-N_k}^{N_k}-\i\(k-\frac{m}{2}\) \d\hat{C}_{k,m}(y_a,y_b) \,e^{\i k(x_a-x_b)} ~,\\
%\Del_{a} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-N_k}^{N_k} \[ \partial^2_{y_a} - \(k+\frac{m}{2}\)^2 \]\d\hat{C}_{k,m}(y_a,y_b) \,e^{\i k(x_a-x_b)}~,\\
%\Del_{\b} \d C_m &= e^{\i m(x_a+x_b)/2}\sum_{k=-N_k}^{N_k} \[ \partial^2_{y_b} - \(k-\frac{m}{2}\)^2 \]\d\hat{C}_{k,m}(y_a,y_b) \,e^{\i k(x_a-x_b)}~.
%\end{align}\end{subequations}\begin{subequations}\begin{align}
%\partial_{x_a} C^e = \sum_{k=-N_k}^{N_k} \i k \, \hat{C}^e_k(y_a,y_b) \,e^{\i k(x_a-x_b)} ~~&,~~
%\partial_{x_b} C^e = \sum_{k=-N_k}^{N_k} - \i k \, \hat{C}^e_k(y_a,y_b) \,e^{\i k(x_a-x_b)} ~,\\
%\Del_{a} C^e = \sum_{k=-N_k}^{N_k} \(\partial^2_{y_a}-k^2\) \hat{C}^e_k(y_a,y_b) \,e^{\i k(x_a-x_b)} ~~&,~~
%\Del_{\b} C^e = \sum_{k=-N_k}^{N_k} \(\partial^2_{y_b}-k^2\) \hat{C}^e_k(y_a,y_b) \,e^{\i k(x_a-x_b)} ~,
%\end{align}\end{subequations}
%
%If the coherent streamfunction perturbation eigenfunction consists of only a single harmonic, $\d\Psi_{mn}$, after defining $k_{\pm} = k\pm m/2$ and $\d E_{n,a} =  e^{\i n y_a}$, some terms of Eq.~\eqref{eq:pert_dC_s} read:
%\begin{subequations}\begin{align}
% -(U^e_a &\partial_{x_a} +U^e_b \partial_{x_b}) \,\d C_m = \nonumber\\
% &=e^{\i m(x_a+x_b)/2}\sum_{k=-N_k}^{N_k} \[  -\i k_+ U^e_a\,\d\hat{C}_{k,m}(y_a,y_b) +  \i k_- U^e_b\,\d\hat{C}_{k,m}(y_a,y_b) \]\,e^{\i k(x_a-x_b)} ~,\\
% -(\d U_a &\partial_{x_a} + \d U_b \partial_{x_b} )  C^e = \nonumber\\
% &=-\sum_{k=-N_k}^{N_k} \[\d U_a\, \i k \,\hat{C}^e_k(y_a,y_b) + \d U_b \(-\i k\) \hat{C}^e_k(y_a,y_b) \] \,e^{\i k(x_a-x_b)}\nonumber\\
%%  &=\i n \sum_{k}  \[ e^{\i m x_a} e^{\i n y_a}\, \i k\,  \hat{C}^e_k(y_a,y_b) + e^{\i m x_b} e^{\i n y_b} \(-\i k\) \hat{C}^e_k(y_a,y_b) \] e^{\i k(x_a-x_b)}~\nonumber\\
%%  &=\i n\, e^{\i m(x_a+x_b)/2} \sum_{k}  \[ e^{\i m (x_a-x_b)/2} e^{\i n y_a}\, \i k\,  \hat{C}^e_k(y_a,y_b) + e^{-\i m (x_a-x_b)/2} e^{\i n y_b} \(-\i k\) \hat{C}^e_k(y_a,y_b) \] e^{\i k(x_a-x_b)}\nonumber\\
%  &=\i n \, e^{\i m(x_a+x_b)/2} \sum_{k}\left\{  \vphantom{\frac1{2}} \[  \(\i k\,\d E_a\)   \hat{C}^e_k(y_a,y_b) \] \,e^{\i k_+ (x_a-x_b)} + \[   \hat{C}^e_k(y_a,y_b) \(-\i k\,\d E_b\) \] \,e^{\i k_- (x_a-x_b)}\right\}~.\label{eq:dUadUbCE}
% \end{align}\end{subequations}
%The term $e^{\i m(x_a+x_b)/2}$ factors out of all terms of Eq.~\eqref{eq:pert_syst_cont}, while in $(\d A_a+\d A_b)C^e$ the term $e^{\i k(x_a-x_b)}$ cannot be factored out.
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% these are totally wrong

{\color{Purple}
%For $k,k',m$ integers we have:
%\begin{align}
%\frac1{2\pi} \int_{0}^{2\pi} e^{-\i k' \xt } e^{\i (k+m/2)\xt}\,\df\xt &= \frac{e^{2\pi\i(k+m/2-k')}-1}{2\pi\i(k+m/2-k')} = \left\{
%	\begin{array}{ll}
%		 \d_{k,k'-m/2}  & \mbox{, if } m \textrm{ is even~,} \\
%		 \\
%		 \\
%		\dfrac1{\i \pi (k'-k-m/2)} & \mbox{, if } m \textrm{ is odd~.}
%	\end{array}
%\right.
%\end{align}
%%If $m$ is even, 
%%\be
%%\frac1{2\pi} \int_{0}^{2\pi} e^{-\i k' \xt } e^{\i (k+m/2)\xt}\,\df\xt = \d_{k,k'-m/2}
%%\ee
%%but in the case $m$ is odd then the numerator never vanishes and
%%\be
%%\frac1{2\pi} \int_{0}^{2\pi} e^{-\i k' \xt } e^{\i (k+m/2)\xt}\,\df\xt = \frac1{\i \pi (k'-k-m/2)}
%%\ee
%
%So, in the case $m$ is even, then by multiplying all terms all terms with $e^{-\i k' (x_a-x_b)} / (2\pi)$ and integrate over the whole domain we get Eq.~\eqref{eq:pert_dC_s_matr}. However, for $m$ odd we have that each $\d\hat{C}_{k,m}$ couples with all $\hat{C}^e_k$. For example, the term of Eq.~\eqref{eq:dUadUbCE} becomes:
%\begin{align}
%\s\,\d \hat{C}_{k,m} &=  \sum_n\, a_n\,\i n  \sum_{k'}\[  \vphantom{\frac1{2}} \frac{  \(\i k'\,\d E_a\)   \hat{C}^e_{k'}(y_a,y_b) }{\i \pi (k-k'-m/2)} + \frac{ \hat{C}^e_{k'}(y_a,y_b) \(-\i k'\,\d E_b\)  }{\i \pi (k-k'+m/2)} \]
%\end{align}
%Notice the summation over $k'$ for $\hat{C}^e_{k'}$. This equation can be written in matrix form:
%\begin{align}
%\s\,\d \C_{k,m} &= \sum_n\, a_n\, \i n   \sum_{k'}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \(\i k'\,\d \E_n\)   \C^e_{k'} }{k-k'-m/2} + \frac{ \C^e_{k'} \(-\i k'\,\d \E_n\)^\transp  }{k-k'+m/2} \]
%\end{align}
%
%
%We define $\d \C_{k,m,n}$ the solution of
%\begin{align}
%\(\A^{e,\textrm{L}}_{k,m}-\s\)\,\d\C_{k,m,n} + \d\C_{k,m,n}\(\A^{e,\textrm{R}}_{k,m}\)^\transp &+     \underbrace{\sum_{k'}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \d\A^{\textrm{L}}_{k',m,n}   \C^e_{k'} }{k-k'-m/2} + \frac{ \C^e_{k'} \(\d\A^{\textrm{R}}_{k',m,n}\)^\transp  }{k-k'+m/2} \]}_{\d\Q_{k,m,n}} =0~,\label{eq:dQkmn_def}
%\end{align}
%which consists of $\d\Psi_{mn}$ and we deduce therefore that $\d\C_{k,m}$ which solves the full
%\begin{align}
%\s\,\d \C_{k,m} &=\A^{e,\textrm{L}}_{k,m}\,\d\C_{k,m} + \d\C_{k,m}\(\A^{e,\textrm{R}}_{k,m}\)^\transp + \sum_n\, a_n\,    \sum_{k'}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \d\A^{\textrm{L}}_{k,m,n}   \C^e_{k'} }{k-k'-m/2} + \frac{ \C^e_{k'} \(\d\A^{\textrm{R}}_{k,m,n}\)^\transp  }{k-k'+m/2} \]
%\end{align}
%will be given as $\d\C_{k,m} = \sum_n  a_n\,\d\C_{k,m,n}$.
%
%
%In Eq.~\eqref{eq:dQkmn_def} the $\d\Q_{k,m,n}$ is defined with respect of the $\C_k^e$ matrices as:
%\be
%\d\Q_{k,m,n}=\sum_{k'=-N_k}^{N_k}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \d\A^{\textrm{L}}_{k,m,n}   \C^e_{k'} }{k-k'-m/2} + \frac{ \C^e_{k'} \(\d\A^{\textrm{R}}_{k,m,n}\)^\transp  }{k-k'+m/2} \]
%\ee
%Using the fact that $C^e$ is real and also symmetric in exchange $\xv_a\leftrightarrow\xv_b$ we have that $\C^e_{-k} = \(\C^e_k\)^\transp$. Also $ \d\A^{\textrm{L}}_{-k,m,n}= \d\A^{\textrm{R}}_{k,m,n}$ and $ \d\A^{\textrm{R}}_{-k,m,n}= \d\A^{\textrm{L}}_{k,m,n}$. Therefore $\d\Q_{k,m,n}$ becomes:
%\be
%\d\Q_{k,m,n}=\sum_{k'=1}^{N_k}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \d\A^{\textrm{L}}_{k,m,n}   \C^e_{k'} }{k-k'-m/2}+ \frac{  \d\A^{\textrm{R}}_{k',m,n}  \( \C^e_{k'} \)^\transp}{k+k'-m/2} + \frac{ \C^e_{k'} \(\d\A^{\textrm{R}}_{k,m,n}\)^\transp  }{k-k'+m/2} + \frac{  \( \C^e_{k'} \)^\transp\(\d\A^{\textrm{L}}_{k',m,n}\)^\transp  }{k'+k+m/2} \]
%\ee
%

%For example:
%\begin{align}
%\d C_m(x_a,y_a,x_b,y_b) &= e^{\i m(x_a+x_b)/2} \sum_{k=-N_k}^{N_k} \d\hat{C}_{k,m} (y_a,y_b) e^{\i k(x_a-x_b)} \nonumber\\
% &= e^{\i m(x_a+x_b)/2} \sum_{k=1}^{N_k} \[\d\hat{C}_{k,m} (y_a,y_b) e^{\i k(x_a-x_b)}+\d\hat{C}_{-k,m} (y_a,y_b) e^{-\i k(x_a-x_b)}\] ~.
%  \end{align}
%Since $\d C_m$ is symmetric to $\xv_a\leftrightarrow\xv_b$ we have that $\d\hat{C}_{-k,m} (y_a,y_b)=\d\hat{C}_{k,m} (y_b,y_a)$.
%\begin{align}
%\d C_m(x_a,y_a,x_b,y_b) &= e^{\i m(x_a+x_b)/2} \sum_{k=1}^{N_k} \[\d\hat{C}_{k,m} (y_a,y_b) e^{\i k(x_a-x_b)}+\d\hat{C}_{k,m} (y_b,y_a) e^{-\i k(x_a-x_b)}\] ~,\\
%C^e(x_a,y_a,x_b,y_b) &= \sum_{k=1}^{N_k} \[\hat{C}^e_{k}(y_a,y_b) e^{\i k(x_a-x_b)}+\hat{C}^e_{k}(y_b,y_a) e^{-\i k(x_a-x_b)}\] ~.
%  \end{align}
%  
%
%
%
%
%\begin{subequations}\begin{align}
% -(U^e_a &\partial_{x_a} +U^e_b \partial_{x_b}) \,\d C_m = \nonumber\\
% &=e^{\i m(x_a+x_b)/2} \sum_{k=-N_k}^{N_k} \[  -\i k_+ U^e_a\,\d\hat{C}_{k,m}(y_a,y_b) +  \i k_- U^e_b\,\d\hat{C}_{k,m}(y_a,y_b) \]e^{\i k(x_a-x_b)} ~,\\
% &=e^{\i m(x_a+x_b)/2}\sum_{k=1}^{N_k} \[\(-\i k_+\) U^e_a \d\hat{C}_{k,m} (y_a,y_b) e^{\i k(x_a-x_b)}+\(-\i k_-\) U^e_a\d\hat{C}_{k,m} (y_b,y_a) e^{-\i k(x_a-x_b)}+\dotsb\right.\nonumber\\
% &\qquad\qquad\qquad\qquad\qquad\dotsb+\left. \(\i k_-\) U^e_b \d\hat{C}_{k,m} (y_a,y_b) e^{\i k(x_a-x_b)}+\(\i k_+\) U^e_b\d\hat{C}_{k,m} (y_b,y_a) e^{-\i k(x_a-x_b)}\]  ~.
% \end{align}\end{subequations}
%
%
%\begin{subequations}\begin{align}
% -(\d U_a &\partial_{x_a} + \d U_b \partial_{x_b} )  C^e =\nonumber\\
% &=  -(\d U_a \partial_{x_a} + \d U_b \partial_{x_b} )\sum_{k=1}^{N_k} \[\hat{C}^e_{k}(y_a,y_b) e^{\i k(x_a-x_b)}+\hat{C}^e_{k}(y_b,y_a) e^{-\i k(x_a-x_b)}\]\nonumber\\
% &=\sum_{k} \[\(-\i k\)\,\d U_a\,\hat{C}^e_k(y_a,y_b) e^{\i k(x_a-x_b)}+\(+\i k\)\,\d U_a\,\hat{C}^e_k(y_b,y_a) e^{-\i k(x_a-x_b)}+\dotsb\right.\nonumber\\
% &\qquad\qquad\qquad\qquad\qquad\left.\dotsb+  \d U_b \(-\i k\) \hat{C}^e_k(y_a,y_b) e^{-\i k(x_a-x_b)}+  \d U_b \(+\i k\) \hat{C}^e_k(y_a,y_b) e^{\i k(x_a-x_b)}\] \nonumber\\
% &=e^{\i m(x_a+x_b)/2}\sum_{k} \[\(-\i k\)\,\(-\i n\)\d E_a\,\hat{C}^e_k(y_a,y_b) e^{\i k_+(x_a-x_b)}+\(+\i k\)\,\(-\i n\)\d E_a\,\hat{C}^e_k(y_b,y_a) e^{-\i k_-(x_a-x_b)}+\dotsb\right.\nonumber\\
% &\qquad\qquad\qquad\qquad\qquad\left.\dotsb+  \(-\i k\)\(-\i n\)\d E_b  \hat{C}^e_k(y_a,y_b) e^{-\i k_+(x_a-x_b)}+  \(+\i k\)\(-\i n\)\d E_b  \hat{C}^e_k(y_a,y_b) e^{\i k_-(x_a-x_b)}\] ~.
%  \end{align}\end{subequations}

}




%
%
%
%\subsection{Case with $m$ is even}
%
%
%After summing up for all $n$ to get the $\d A_{\a,\b}$ for the $\d\Psi_m$ (Eq.~\eqref{eq:eig_dPsi}) and also after denoting $\[\d\Ev_n\]_a = e^{\i n y_a}$, $\d\E_n = \diag\(\d\Ev_n\)$ the perturbation covariance perturbation (Eq.~\eqref{eq:pert_dC_s} becomes the matrix equation:
%%\begin{subequations}\begin{align}
%% -(U^e_a &\partial_{x_a} +U^e_a \partial_{x_a}) \d C_m =e^{\i m(x_a+x_b)/2}\sum_k \[ \(-\i k_+ \U^e\) \,\d\C_{k,m} +    \d\C_{k,m}\(\i  k_-\U^e\)^\transp \]_{\a\b}e^{\i k(x_a-x_b)} \\
%% -(\d U_a &\partial_{x_a} + \d U_b \partial_{x_b} )  C^e = \nonumber\\
%%& =\i n \, e^{\i m(x_a+x_b)/2}\sum_{k} \[  \(\i k\, \d\E_n\)   \C^e_k \]_{\a\b} e^{\i k_+ (x_a-x_b)} + \[ \C^e_k  \(-\i k\, \d\E_n\)^\transp \]_{\a\b} e^{\i k_-(x_a-x_b)}
%% \end{align}\end{subequations}
%\begin{align}
%\s\,\d\C_{k,m} &=  \A^{e,\textrm{L}}_{k,m}\,\d\C_{k,m} + \d\C_{k,m}\(\A^{e,\textrm{R}}_{k,m}\)^\transp + \sum_n a_n \[\vphantom{\frac1{2}}\d\A^{\rm L}_{k-m/2,m,n}\C^e_{k-m/2} + \C^e_{k+m/2}\(\d\A^{\rm R}_{k+m/2,m,n}\)^\transp\]
%\label{eq:pert_dC_s_matr}\end{align}
%with:
%\begin{subequations}\begin{align}
%\A^{e,\textrm{L}}_{k,m} &= -\i(k+m/2) \U^e  -\i(k +m/2) \(\bit \beta -\U^e_{yy} \) \DDel^{-1}_{k,+}  - r - \nu_4  \DDel^2_{k,+}~,\\
%\A^{e,\textrm{R}}_{k,m} &= +\i(k- m/2) \U^e  + \i(k- m/2) \(\bit \beta -\U^e_{yy} \) \DDel^{-1}_{k,-}  - r - \nu_4  \DDel^2_{k,-}~,\\
%\d\A^{\textrm{L}}_{k,m,n} &= -\d\E_n\(+ nk\I+\i m \D_y\)\[\I+(m^2+n^2)\DDel^{-1}_k\]~,\\
%\d\A^{\textrm{R}}_{k,m,n} &= -\d\E_n\(- nk\I+\i m \D_y\)\[\I+(m^2+n^2)\DDel^{-1}_k\]~,
%\end{align}
%and
%\begin{align}
%\DDel_{k,\pm }\equiv\DDel_{k\pm m/2} = \D^2 -\(k\pm m/2\)^2\I ~,
%\end{align}
%\end{subequations}
%Equation~\eqref{eq:pert_dC_s_matr} can be solved for $\d\C_{k,m}$ as a Sylvester equation and from $\d\C_{k,m}$ we get $\d C_m$ (Eq.~\eqref{eq:eig_dCm}).
%
%Note:
%If we denote with $\d\C_{k,m,n}$ the solution of:
%\be
%\s\,\d\C_{k,m,n} =  \A^{e,\textrm{L}}_{k,m}\,\d\C_{k,m,n} + \d\C_{k,m,n}\(\A^{e,\textrm{R}}_{k,m}\)^\transp +  \d\A^{\rm L}_{k-m/2,m,n}\C^e_{k-m/2} + \C^e_{k+m/2}\(\d\A^{\rm R}_{k+m/2,m,n}\)^\transp~.\label{eq:eig_dCkmn}
%\ee
%then $\d\C_{k,m} = \sum_n a_n \d\C_{k,m,n}$. 
%
%
%The next step is to find the Reynolds stress divergence, $\d R_m$, that corresponds to $\d C_m$.
%\begin{align}
%\d R_m &= - \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_a} \Del_a^{-1}+\partial_{x_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b} \]
%\end{align}
%
%The term in the first brackets is $\d\<u'q'\>$, which reads:
%\begin{align}
%\d \<u'q'\> &=  \left. \bit \frac1{2}\(-\partial_{y_a} \Del_a^{-1}-\partial_{y_b} \Del_b^{-1}\) \d \hat{C} \right|_{\xv_a=\xv_b}  \nonumber\\
%&=-\frac1{2}  \left. \bit e^{\i m(x_a+x_b)/2} \sum_k \(\partial_{y_a} \Del_a^{-1}+\partial_{y_b} \Del_b^{-1}\) \d\hat{C}_{k,m} (y_a,y_b) \,e^{\i k(x_a-x_b)} \right|_{\xv_a=\xv_b} \nonumber\\
%\end{align}
%Discretizing the $y$-domain and representing $\d \<u'q'\>$ as a column vector we get using the matrix representation for $\d\hat{C}_{k,m}$:
%\begin{align}
%\d \<\mathbf{uq}\> &=-\frac1{2}  \left. \bit e^{\i m(x_a+x_b)/2} \sum_k \[\D_y \DDel^{-1}_{k,+} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp\(\D_y\)^\transp\]_{\a\b}  e^{\i k(x_a-x_b)} \right|_{\xv_a=\xv_b} \nonumber\\
%&=-\frac1{2}   e^{\i m x} \vecd\[\sum_k \D_y \DDel^{-1}_{k,+} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp\(\D_y\)^\transp\] \nonumber\\
%\end{align}
%and similarly for $\d\<v'q'\>$:
%\begin{align}
%\d \<\mathbf{vq}\> &=\frac1{2}  \left. \bit e^{\i m(x_a+x_b)/2} \sum_k \[ \i k_+ \DDel^{-1}_{k,+}\, \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp \(-\i k_-\)\]_{\a\b}  e^{\i k(x_a-x_b)} \right|_{\xv_a=\xv_b} \nonumber\\
%&=\frac1{2}   e^{\i m x} \vecd\[ \sum_k \i k_+ \DDel^{-1}_{k,+}\, \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp \(-\i k_-\)\] \nonumber\\
%\end{align}
%
%Therefore $\d\Rv_m$ will be given by:
%\begin{align}
%\d \Rv_m &= -\partial_x\d \<\mathbf{uq}\> - \D_y\d \<\mathbf{vq}\>\nonumber\\
%&=\frac{1}{2}e^{\i m x}  \left\{ \i m \, \vecd\[ \sum_k \D_y \DDel^{-1}_{k,+}\, \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp\(\D_y\)^\transp\] + \dotsb\right.\nonumber\\
%&\qquad\qquad\qquad\dotsb+\left. \D_y \vecd\[ \sum_k  \i k_+ \DDel^{-1}_{k,+} \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp \(-\i k_-\)\] \right\}
%\end{align}
%
%The Reynolds stress divergence that correspond to $\d\C_{k,m,n}$ are denoted with $\d\Rv_{mn}$. In general, due to the non-homogeneous terms in $y$, ($U^e$, $U^e_{yy}$), the Reynolds stress divergence $\d\Rv_{mn}$ will be proportional to $e^{\i m x}$ but not also  to $e^{\i ny}$. This will only be true in the case of the homogeneous equilibrium.
%
%\subsection{Case with $m$ is odd}
%Now we have
%
%\begin{align}
%\s\,\d\C_{k,m} &=  \A^{e,\textrm{L}}_{k,m}\,\d\C_{k,m} + \d\C_{k,m}\(\A^{e,\textrm{R}}_{k,m}\)^\transp + \sum_n a_n \sum_{k'} \frac1{\i\pi} \[\frac{\d\A^{\rm L}_{k',m,n}\,\C^e_{k'}}{k'-k+m/2} + \frac{\C^e_{k'}\(\d\A^{\rm R}_{k',m,n} \)^\transp}{k'-k-m/2}\]
%\label{eq:pert_dC_s_matr}\end{align}


\subsection{Corrolaries}

\subsubsection{For every equilibrium $(\Uv^e,C^e)$ the perturbation covariance that corresponds to $m=0$ has $\d\hat{C}_{k=0,m=0}=0$}

Proof: For $m=0$, $k=0$ we have that $\d\A^{\textrm{L}}_{0,0,n} = \d\A^{\textrm{R}}_{0,0,n}=0$, therefore the perturbation covariance $\d\hat{C}_{k=0,m=0}=0$ satisfies:
\be
\(\A^{e,\textrm{L}}_{0,0}-\s\I\)\,\d\C_{0,0} + \d\C_{0,0}\(\A^{e,\textrm{R}}_{0,0}\)^\transp=0 ~,\label{eq:dC00}
\ee
with
\begin{align}
\A^{e,\textrm{L}}_{0,0} &= \A^{e,\textrm{R}}_{0,0} =\(\A^{e,\textrm{R}}_{0,0}\)^\transp \equiv \A^e_{0,0}=   - r - \nu_4  \D_y^4~.
\end{align}
The Sylvester equation \eqref{eq:dC00} has a unique solution unless one of the eigenvalues of $\A^e_{0,0}-\s\I$ is equal to an eigenvalue of $-\A^e_{0,0}$. This happens only for $\s=-2r-\nu_4(m^4+n^4)$, for $m,n$ integers. Otherwise, the only solution is $\d\C_{0,0}=0$.


\vspace{2cm}

In order to solve the eigenproblem of a jet equilibrium we proceed as follows: We suppose a $\d\Psi_{m} = e^{\s t}e^{\i mx}\,\sum_n a_n \d \Psi_{mn}$ for some coefficients $a_n$ and choose a first guess for $\s$. For this given $\s$ we solve Eqs.~\eqref{eq:pert_dC_s_matr} and find all $\d\C_{k,m,n}$ and from that we find the corresponding $\d \hat{R}_{mn}$. We factor the $e^{\i m x}$ dependance out and expand $\d \Rv_{mn}$ in Fourier series in $y$:
\be
\d \hat{R}_{mn} = e^{\i m x}\,\sum_{n'} B^{(m)}_{n'n}\,e^{\i n' y}~.
\ee
Then we go to the perturbation equation for the coherent structure, which for a jet equilibrium takes the form:
\begin{align}
&\sum_n\,a_n\,\[ \s+r+\nu_4\Del^2 + \i m U^e -\frac{\i m}{m^2+n^2} \(\b-U^e_{yy}\) \]  [-(m^2+n^2)]\,\d\Psi_{mn} =   e^{\i m x}\sum_n a_n \(\sum_{n'} B^{(m)}_{n'n}\,e^{\i n' y}\)\nonumber\\
\end{align}
 The term, $e^{\i m x}$ factors out.


\begin{align}
&\sum_n\,-a_n\,(m^2+n^2)\[ \s+r+\nu_4(\partial_y^2-m^2)^2 + \i m U^e -\frac{\i m}{m^2+n^2} \(\b-U^e_{yy}\) \]  \,e^{\i n y} =   \sum_n a_n \(\sum_{n'} B^{(m)}_{n'n}\,e^{\i n' y}\)\nonumber\\
\end{align}


If this was a homogeneous equilibrium ($U^e=V^e=0$) then $B^{(m)}_{n'n} = b^{(m)}_n\,\d_{n'n}$ and the above equation simplifies to:\begin{subequations}
\begin{align}
\sum_{n,n'}\,a_n\, \[ \( \s+r+\nu_4(m^2+n^2)^2 -\frac{\i m\b}{m^2+n^2}  \)  (m^2+n^2)\,\d_{n'n}+ B^{(m)}_{n'n} \]\,e^{\i n' y} &=0~~\Leftrightarrow\label{eq:disp_s_nz_nn'}\\
\sum_n\,a_n\, \[ \( \s+r+\nu_4(m^2+n^2)^2 -\frac{\i m\b}{m^2+n^2}  \)  (m^2+n^2)+ b^{(m)}_{n} \]\,e^{\i n y}&=0~.\label{eq:disp_s_nz_n}
\end{align}
\end{subequations}
Since $e^{\i n y}$ are linearly independent Eq.~\eqref{eq:disp_s_nz_n} can be satisfied for a single $n=n_0$ and all other $a_n$ be set to zero, that is $a_{n_0}=1$ and $a_n=0$ for $n\ne n_0$. Another way to look at this is to notice that Eq.~\eqref{eq:disp_s_nz_nn'} again using the fact that $e^{\i n y}$ are linearly independent can be rewritten as:
\be
\sum_{n}\[-\frac{B^{(m)}_{n'n}}{m^2+n^2}  -\(r+\nu_4(m^2+n^2)^2 -\frac{\i m\b}{m^2+n^2}  \) \,\d_{n'n}\]\,a_n =\s\,\,a_n~~\Leftrightarrow\label{eq:disp_s_nz_eigen}\\
\ee
or in matrix form:
\be
\L^{(m)}\,\av = \s\,\av
\ee
where $\L^{m}$ is the matrix with elements:
\be
 L^{(m)}_{n'n} =-\frac{ B^{(m)}_{n'n} }{m^2+n^2} -\[r+\nu_4(m^2+n^2)^2 -\frac{\i m\b}{m^2+n^2}  \]  \d_{n'n}~.
\ee
and $\av$ is the vector with elements $[\av]_n=a_n$.
Since for the homogeneous equilibrium $B^{(m)}_{nn'} = b^{(m)}_n\,\d_{nn'}$, the matrix $\L^{(m)}$ is diagonal so its eigenvectors are the standard orthonormal basis, $\e_j$, with elements: $[\e_j]_{m} = \d_{jm}$.

\vspace{2cm}
For the jet equilibrium we can expand $U^e = \sum_p\hat{U}^e_p\,e^{\i p y}$. Neglecting $\nu_4$ we have:
\begin{align}
&\sum_n\,a_n\,\( \s+r  -\frac{\i m\b}{m^2+n^2}\)   (m^2+n^2)\,e^{\i n y} + \sum_{n,p} a_n\,\i m\hat{U}_p^e\( m^2+n^2-p^2 \)  \,e^{\i(n+p)y} + \sum_{n,n'} a_n \, B^{(m)}_{n'n}\,e^{\i n'y}=0
\end{align}
By changing summation variables $p\to q=p+n$ in the second sum and $n'\to q$ in the third sum, the above expression can be written:

\begin{align}
&\sum_{n,q}\,a_n\,\( \s+r  -\frac{\i m\b}{m^2+n^2}\)   (m^2+n^2)\,\d_{n,q} + \sum_{n,q} a_n\,\i m\hat{U}_{q-n}^e\[ m^2+n^2-(q-n)^2 \bit\]  + \sum_{n,q} a_n \, B^{(m)}_{q,n}=0\nonumber\\
&\sum_{n,q}\,a_n\,\left\{ \( \s+r  -\frac{\i m\b}{m^2+n^2}\)  \,\d_{n,q} + \i m\,\hat{U}_{q-n}^e\[ 1-\frac{(q-n)^2}{m^2+n^2} \]   +  \frac{B^{(m)}_{q,n}}{m^2+n^2} \right\} e^{\i q y}=0\nonumber\\
&\sum_n\,a_n\,\left\{ \( \s+r  -\frac{\i m\b}{m^2+n^2}\)  \,\d_{n,q} + \i m\,\hat{U}_{q-n}^e\[ 1-\frac{(q-n)^2}{m^2+n^2} \]   +  \frac{B^{(m)}_{q,n}}{m^2+n^2} \right\}=0\nonumber\\
&\sum_n\,a_n\,\left\{ -\( r  -\frac{\i m\b}{m^2+n^2}\)  \,\d_{n,q} - \i m\hat{U}_{q-n}^e\[ 1-\frac{(q-n)^2}{m^2+n^2} \]   - \frac{B^{(m)}_{q,n}}{m^2+n^2}\right\}=\s\,a_q~,
\end{align}
or else as
\be
\L^{(m,{U^e})}\,\av = \s\,\av
\ee
with $\L^{(m,{U^e})}$ the matrix with elements:
\be
\[\L^{(m,{U^e})}\]_{qn} = -\frac{B^{(m)}_{q,n}}{m^2+n^2} -\( r  -\frac{\i m\b}{m^2+n^2}\)  \,\d_{n,q} - \i m\hat{U}_{q-n}^e\[ 1-\frac{(q-n)^2}{m^2+n^2} \] ~.
\ee


\newpage
\subsection{Centroid-difference coordinates}

We write this system in centroid-difference coordinates, $\mathbf{\bar{x}}=(\mathbf{x}_a+\mathbf{x}_b)/2$, $\mathbf{\tilde{x}}=\mathbf{x}_a-\mathbf{x}_b$. This gives:\begin{subequations}
\begin{align}
x_a = \xb + \frac1{2}\xt ~~,~~x_b = \xb - \frac1{2}\yt ~,\\
y_a = \yb + \frac1{2}\yt ~~,~~y_b = \yb - \frac1{2}\yt ~,
\end{align}\end{subequations}
and the derivatives transform to:\begin{subequations}
\begin{align}
\partial_{x_a} = \frac1{2}\partial_{\xb} + \partial_{\xt} ~~&,~~ \partial_{x_b} = \frac1{2}\partial_{\xb} - \partial_{\xt} ~,\\
\partial_{y_a} = \frac1{2}\partial_{\yb} + \partial_{\yt} ~~&,~~ \partial_{y_b} = \frac1{2}\partial_{\yb} - \partial_{\yt}  ~,\\
\Del_a   = \Delt +\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\) +  \frac1{4}\Delb~~&,~~ \Del_b   = \Delt -\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\) +  \frac1{4}\Delb~,\\
\Del_a\Del_b   = \( \Delt+\frac1{4}\Delb\)^2 & - \(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)^2~,\\
\partial_{x_a} \Del_b + \partial_{x_b} \Del_a   = \partial_{\xb}&\( \Delt+\frac1{4}\Delb\) - 2\partial_{\xt}\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)~,\\
\partial_{y_a} \Del_b + \partial_{y_b} \Del_a   = \partial_{\yb}&\( \Delt+\frac1{4}\Delb\) - 2\partial_{\yt}\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)~.
\end{align}

%\begin{subequations}
%\begin{align}
%-U^e_a \partial_{x_a} -U^e_b \partial_{x_b} & = -\Ub^e \partial_{\xb}-\Ut^e \partial_{\xt} ~,\\
%-U^e_a \partial_{x_a} \Del_b -U^e_b \partial_{x_b} \Del_a & = -\(\Ub^e\partial_{\xb} + \Ut^e\partial_{\xt}\)\(\Del+\frac1{4}\Delb\) + 2\(\Ub^e\partial_{\xt} + \frac1{4} \Ut^e\partial_{\xb}\)\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\) ~,\\
%U_{y_a y_a}^e \partial_{x_a} \Del_b + U_{y_b y_b}^e \partial_{x_b} \Del_a & = \(\Ub''^e\partial_{\xb} + \Ut''^e\partial_{\xt}\)\(\Del+\frac1{4}\Delb\) - 2\(\Ub''^e\partial_{\xt} + \frac1{4} \Ut''^e\partial_{\xb}\)\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\) ~,\\
%-\d U_a \partial_{x\a} \Del_b -\d U_b \partial_{x_b} \Del_a &=
%\end{align}\end{subequations}


In general, we also have the following transformations of various quantities:
\begin{align}
\Phi_a \partial_{x_a} +\Phi_b \partial_{x_b} & = \Phib\, \partial_{\xb}+\Phit\, \partial_{\xt} ~~,~~ \Phi_a \partial_{y_a} +\Phi_b \partial_{y_b}  = \Phib\, \partial_{\yb}+\Phit\, \partial_{\yt} ~,\\
\Phi_a \partial_{x_a} \Del_b +\Phi_b \partial_{x_b} \Del_a &=\(\Phib\,\partial_{\xb} + \Phit\,\partial_{\xt}\)\(\Del+\frac1{4}\Delb\) - 2\(\Phib\,\partial_{\xt} + \frac1{4} \Phit\,\partial_{\xb}\)\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)~,\\
\Phi_a \partial_{y_a} \Del_b +\Phi_b \partial_{y_b} \Del_a &=\(\Phib\,\partial_{\yb} + \Phit\,\partial_{\yt}\)\(\Del+\frac1{4}\Delb\) - 2\(\Phib\,\partial_{\yt} + \frac1{4} \Phit\,\partial_{\yb}\)\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)~,
\end{align}\end{subequations}
where we have defined: $\Phib = (\Phi_a+\Phi_b)/2$ and $\Phit = \Phi_a-\Phi_b$.




\subsection{Homogeneous equilibrium}

For the homogeneous equilibrium Eqs.~\eqref{eq:pert_S3Tgen} take the form:\begin{subequations}
\begin{align}
&\( \bit \s + r + \nu_4 \DDel^2   +\beta \,\D_x \DDel^{-1} \)\d \Zv  =  \d\Rv \label{eq:dZ}\\
&\(\A^e-\sigma\) \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp = 0 ~. \label{eq:dC}
\end{align}\label{eqs:pert_hom}\end{subequations}
where we have defined the Reynolds stress divergence $\d\Rv= - \D_x \[\bit \vecd{\( - \D_y \DDel^{-1}\d\C\)}\] - \D_y \[\bit\vecd{\( \D_x \DDel^{-1}\d\C\)}\]$. The equilibrium operator is $\A^e = - \beta \,\D_x \DDel^{-1}-r -\nu_4 \DDel^2$ and
\be
\d\A = -\d\U\,\D_x-\d\V\,\D_y - \d\Z_y\,\D_x\DDel^{-1}+ \d\Z_x\,\D_y\DDel^{-1}~.
\ee
The eigenfunctions of this system are harmonics, $e^{\i(mx+ny)}$.

We assume $\d\Zv_{m,n} = e^{\i(mx+ny)}$ and a corresponding eigenvalue $\s_{m,n}$. We calculate $\d\C_{m,n}$ from Eq.~\eqref{eq:dC} and from that the corresponding Reynolds stress divergence, $\d\Rv_{m,n}$, that corresponds to the $(\d\Zv_{m,n},\s_{m,n})$. We expand the $\d\Rv_{m,n}$ as:
\be
\d\Rv_{m,n} = \sum_{m',n'}  \hat{\R}_{mnm'n'}\,e^{\i(m'x+n'y)}~.
\ee
It can be proven that $\d\Rv_{mn}$ will be proportional to $\d\Z_{mn}$, that is: $\hat{\Rv}_{mnm'n'}=r_{mn}\d_{mm'}\d_{nn'}$ (with $r_{mn}$ in general complex). This way Eq.~\eqref{eq:dZ} is written:
\be
 \( \bit \s + r + \nu_4 (m^2+n^2)^2   -\frac{\i m\beta }{m^2+n^2} - r_{mn}\) \,e^{\i(mx+ny)}  = 0\\
\ee
So our new guess for the eigenvalue, $\s'$ is:
\be
\s' = -r +\frac{\i m\beta }{m^2+n^2} + r_{mn}~.
\ee
We continue this iteration until convergence, that is until $|\s'-\s|\big/|\s'|<\tol$.

\vspace{2cm}

This method works very well in reproducing the results of the non-zonal dispersion relation for every choice of $(m,n)$ and it converges to the unstable eigenvalue even if our initial guess is very far away from that.

%Let us define a ``symbolic'' index $P$ for $m,n$ and $Q$ for $m',n'$ then the above is written: 
%\begin{align}
%\sum_{Q} \[ \( \bit \s + r + \nu_4 (m^2+n^2)^2   -\,\frac{\i m\beta }{m^2+n^2}\)\d_{P,Q} - \r_P \d_{P,Q}\] \,\e_Q  = 0~.\label{eq:eigRhat}
%\end{align}
%Definie diagonal matrix $\L$:
%\be
%\L_{PQ} = \[\r_{P} -\(r +\nu_4 (m^2+n^2)^2   -\,\frac{\i m\beta }{m^2+n^2}\)\]\d_{PQ}~,
%\ee
%we can interpret Eq.~\eqref{eq:eigRhat} as $\v$ being an eigenvector of $\L$ with eigenvalue $\s$.


\subsection{Non Homogeneous equilibrium }

For the homogeneous equilibrium Eqs.~\eqref{eq:pert_S3Tgen} take the form:
\begin{align}
&\( \bit \s + r + \nu_4 \DDel^2   +\beta \,\D_x \DDel^{-1} \)\d \Zv  =  \d\Rv \label{eq:dZ}\\
&\(\A^e-\sigma\) \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp = 0 ~. \label{eq:dC}
\end{align}\label{eqs:pert_hom}

\begin{subequations}
\begin{align}
\[ \bit \s + r + \nu_4 \DDel^2   + \U^e\,\D_x +\(\beta -\U_{yy}^e\)\D_x \DDel^{-1} \]\d \Zv  &=  \d\Rv \label{eq:dZ_UE}\\
\(\A^e-\sigma\) \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp &= 0 ~. \label{eq:dC_UE}
\end{align}\end{subequations}
where now $\A^e= -\U^e\D_x  - \(\beta -\U_{yy}^e\)\D_x \DDel^{-1}-r -\nu_4 \DDel^2$ and we have defined the Reynolds stress divergence $\d\Rv= - \D_x \[\bit \vecd{\( - \D_y \DDel^{-1}\d\C\)}\] - \D_y \[\bit\vecd{\( \D_x \DDel^{-1}\d\C\)}\]$ and
\be
\d\A = -\d\U\,\D_x-\d\V\,\D_y - \d\Z_y\,\D_x\DDel^{-1}+ \d\Z_x\,\D_y\DDel^{-1}~.
\ee
The eigenfunctions of this system are harmonics, $e^{\i(mx+ny)}$.

We assume $\d\Zv_{m} = e^{\i mx} f(y)$ and a corresponding eigenvalue $\s_{m}$. We calculate $\d\C_{m,n}$ from Eq.~\eqref{eq:dC} and from that the corresponding Reynolds stress divergence, $\d\Rv_{m,n}$, that corresponds to the $(\d\Zv_{m,n},\s_{m,n})$. We expand the $\d\Rv_{m,n}$ as:
\be
\d\Rv_{m} = e^{\i mx} \sum_{n'}  \hat{\R}_{mn'}\,e^{\i n'y}~.
\ee



\be
C^e(x_a-x_b,y_a,y_b) = \sum_k e^{\i k (x_a-x_b)} \, C^e_k(y_a,y_b)
\ee


It can be proven that $\d\Rv_{mn}$ will be proportional to $\d\Z_{mn}$, that is: $\hat{\Rv}_{mnm'n'}=r_{mn}\d_{mm'}\d_{nn'}$ (with $r_{mn}$ in general complex). This way Eq.~\eqref{eq:dZ} is written:
\be
 \( \bit \s + r + \nu_4 (m^2+n^2)^2   -\frac{\i m\beta }{m^2+n^2} - r_{mn}\) \,e^{\i(mx+ny)}  = 0\\
\ee
So our new guess for the eigenvalue, $\s'$ is:
\be
\s' = -r +\frac{\i m\beta }{m^2+n^2} + r_{mn}~.
\ee
We continue this iteration until convergence, that is until $|\s'-\s|\big/|\s'|<\tol$.

\vspace{2cm}

This method works very well in reproducing the results of the non-zonal dispersion relation for every choice of $(m,n)$ and it converges to the unstable eigenvalue even if our initial guess is very far away from that.

%Let us define a ``symbolic'' index $P$ for $m,n$ and $Q$ for $m',n'$ then the above is written: 
%\begin{align}
%\sum_{Q} \[ \( \bit \s + r + \nu_4 (m^2+n^2)^2   -\,\frac{\i m\beta }{m^2+n^2}\)\d_{P,Q} - \r_P \d_{P,Q}\] \,\e_Q  = 0~.\label{eq:eigRhat}
%\end{align}
%Definie diagonal matrix $\L$:
%\be
%\L_{PQ} = \[\r_{P} -\(r +\nu_4 (m^2+n^2)^2   -\,\frac{\i m\beta }{m^2+n^2}\)\]\d_{PQ}~,
%\ee
%we can interpret Eq.~\eqref{eq:eigRhat} as $\v$ being an eigenvector of $\L$ with eigenvalue $\s$.



\subsection{Jet equilibrium ($U^e\ne0,V^e=0$)}

Consider now a jet equilibrium $\(\Psi^e(y),C^e\)$. Since the streamfunction is only a function of $y$ the coherent mean flow will have only a streamwise component that is varied in $y$, $\(U^e(y),V^e=0\)$. Also the equilibrium perturbation vorticity covariance, $C^e$ will be homogeneous in $x$, that is it will depend only in the difference coordinate in $x$: $C^e(x_a-x_b,y_a,y_b)$. Therefore it can be readily shown that the perturbation equations take the form:\begin{subequations}
\begin{align}
\[ \bit \s + r + \nu_4 \DDel^2   + \U^e\,\D_x +\(\beta -\U_{yy}^e\)\D_x \DDel^{-1} \]\d \Zv  &=  \d\Rv \label{eq:dZ_UE}\\
\(\A^e-\sigma\) \d\C+ \d\C\,\(\A^e\)^\transp + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp &= 0 ~. \label{eq:dC_UE}
\end{align}\end{subequations}
where now $\A^e= -\U^e\D_x  - \(\beta -\U_{yy}^e\)\D_x \DDel^{-1}-r -\nu_4 \DDel^2$.

The perturbation vorticity eigenfunction will not be a single harmonic function, can it will in general be a sum of harmonics:
\be
\d Z = \sum_{\substack{m,n\\m,n\ne0}} \a_{mn}\,e^{\i\(mx+ny\)}\label{eq:dZ_gen}~,
\ee
(the $m,n\ne 0$ will be omitted from now on).
Let us denote $\d\Zv_{mn} = e^{\i\(mx+ny\)}$ and also let $\d\C_{mn}$ the solution of:
\be
\(\A^e-\sigma\) \d\C_{mn}+ \d\C_{mn}\,\(\A^e\)^\transp + \d\A_{mn}\,\C^e +\C^e\,\(\d\A_{mn}\)^\transp = 0 ~. 
\ee
If $\d\Zv$ is given by Eq.~\eqref{eq:dZ_gen} then we have that 
\be
\d\A = \sum_{m,n} \a_{mn}\,\d\A_{mn}~,
\ee
and therefore:
\begin{align}
\sum_{m,n} \a_{mn}\,\[ \(\A^e-\sigma\) \d\C_{mn}+ \d\C_{mn}\,\(\A^e\)^\transp + \d\A_{mn}\,\C^e +\C^e\,\(\d\A_{mn}\)^\transp \] &= 0~\Leftrightarrow\nonumber\\
 \(\A^e-\sigma\) \(\sum_{m,n} \a_{mn} \d\C_{mn}\)+ \(\sum_{m,n}\a_{mn} \d\C_{mn}\)\,\(\A^e\)^\transp  + \d\A\,\C^e +\C^e\,\(\d\A\)^\transp&= 0~
\end{align}
Therefore the solution $\d\C$ of Eq.~\eqref{eq:dC_UE} is also expanded as:
\be
\d\C = \sum_{m,n} \a_{mn}\,\d\C_{mn}~.
\ee

What is the Reynold stress convergence $\d\Rv$ that is induced by $\d\C$? If we denote $\d\Rv_{mn}$ the Reynold stress convergence induced by $\d\C_{mn}$ then the total $\d\Rv$ will be:
\be
\d\Rv = \sum_{m,n} \a_{mn}\,\d\Rv_{mn}~.
\ee
The $\d\Rv_{mn}$ can be written as a Fourier expansion:
\be
\d\Rv_{mn} = \sum_{m',n'} \hat{R}_{m'n'mn}\,\d\Zv_{m'n'}~.
\ee

From \eqref{eq:dZ_UE} (neglecting $\nu_4$)
\begin{align}
\sum_{m,n} \[ \bit \s + r  + \U^e\,\D_x +\(\beta -\U_{yy}^e\)\D_x \DDel^{-1} \] \a_{mn}\,\d \Zv_{mn}  =  \sum_{m,n,m',n'} \a_{mn} \hat{R}_{m'n'mn}\,\d\Zv_{m'n'} ~\Leftrightarrow\nonumber\\
\sum_{m,n,m',n'} \left\{ \[ \bit \s + r +\U^e\,\D_x +\(\beta -\U_{yy}^e\)\D_x \DDel^{-1} \]\d_{mm'}\d_{nn'}  -    \hat{R}_{m'n'mn} \right\} \a_{mn}\,\d\Zv_{m'n'} ~\Leftrightarrow\nonumber\\
\end{align}

The equilibrium $U^e$ can be also written as $U^e=\sum_p \hat{U}^e_p e^{\i p y}$, $U^e_{yy}=\sum_p -p^2 \hat{U}^e_p e^{\i p y}$.
\be
\sum_{m,n,m',n'} \left\{ \[ \bit \s + r  - \frac{\i m\beta}{m^2+n^2} + \sum_p\i m\(1 - \frac{p^2}{m^2+n^2}  \)\hat{U}_p^e\,e^{\i p y} \]\,\d_{mm'}\d_{nn'}  -    \hat{R}_{m'n'mn} \right\} \a_{mn}\,\d\Zv_{m'n'} ~\nonumber\\
\ee


Let us neglect also the nonlinear advection terms in the equation for the coherent structure and also define a ``symbolic'' index $P$ for $m,n$ and $Q$ for $m',n'$ then the above is written: 
\be
\sum_{P,Q} \left\{ \[ \bit \s + r  - \frac{\i m\beta}{m^2+n^2}  \]\,\d_{QP}  -    \hat{R}_{QP} \right\} \a_{P}\,\d\Zv_{Q} ~\nonumber\\
\ee
Since $\d\Z_Q$ are linearly independent then each
\be
\sum_{P} \left\{ \[ \bit \s + r  - \frac{\i m\beta}{m^2+n^2}  \]\,\d_{QP}  -    \hat{R}_{QP} \right\} \a_{P}
\ee
must be zero, which is equivalent with $\a$ being an eigenvector of $\L=\R-r\I - \vecd(\i m \beta/(m^2+n^2))$ with eigenvalue $\s$. We find the eigenvalues of $\s$, choose the one with the maximum real part and repeat iteration.

==> chapters/app-dispersion_lambda.tex <==
% !TEX root = ../thesis.tex


\chapter{Calculation of the S3T growth rates for the homogeneous turbulent equilibrium}
\label{app:S3Tgr_lambda}






\section{Generalized S3T dispersion with deformation}


\subsection{dissipate kinetic and potential energy, $-r\,q$}
For the NL system:
\begin{align}
\partial_t q + J(\psi,q+\bv\cdot\xv) =\sqrt{\varepsilon}\xi +\textrm{Diss}
\end{align}
with
\begin{align}
\textrm{Diss}&=- r q - (-1)^h\nu_{2h} \Delta^{h}q = -\[ r+(-1)^h\nu_{2h} \Delta^{h}\]q\ \\
q &=\Delta \psi - \lambda^2 \psi~~,~~u =-\partial_y \psi ~~,~~v= \partial_x \psi~.
\end{align}
$h=1$ is diffusion, $h>1$ hyperdiffusion

Define $q=Q+q'$, etc. Then
\begin{align}
&\partial_t Q + J(\Psi,Q + \bv\cdot\xv) =- \[ r+(-1)^h\nu_{2h} \Delta^{h}\] Q - \Tcal[ J(\psi',q') ]~\\
&\partial_t q' = \Acal(\Uv) \,q' + f_{\textrm{nl}} + \xi
\end{align}
with
\begin{align}
\Acal(\Uv)&=-\Uv\cdot\nablav + \[\bit(\Del_\la\Uv)\cdot\nablav + \hat{\mathbf{z}}\cdot(\bv\times\nablav)\]\Del^{-1}_\la - \[r+(-1)^h\nu_{2h} \Delta^{h}\]~\\
f_{\textrm{nl}}&=\Tcal[ J(\psi',q') ]-J(\psi',q')
\end{align}

After defining the eddy vorticity covariance as $C(\xv_a,\xv_b,t)=\<q'(\xv_a,t)q'(\xv_b,t)\>$ and using the ergodic hypothesis that $\Tcal(\bullet) = \<\bullet\>$, the Reynolds stress divergence can be expressed as: $\Rcal(C)=-\nablav\cdot\[\zhat\times \frac1{2}\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) C\]_{\xv_a=\xv_b}$ (cf.~\eqref{eq:def_Rcal}).


S3T system is
\begin{align}
\partial_t \, Q &+ J \(\Psi,Q+ {\bm\beta}\cdot\mathbf{x} \) = \Rcal( C )-(r+\nu_4 \Del^2)\,Q\ ,\\
\partial_t \, C & = \[\bit\Acal_a(\Uv) + \Acal_b(\Uv) \] C +\varepsilon\,Q\ ,
\end{align}

Consider a homogeneous, stationary equilibrium solution, $Q^e$, $C^e(\xv_a-\xv_b)$. Expanding $C^e$ as
\be
C^e(\xv_a-\xv_b) = \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}
\ee
(and similarly for $Q(\xv_a-\xv_b)$), we find that
\be
\hat{C}^e(\kv) = \frac{\varepsilon\,\hat{Q}(\kv)}{2(r+\nu_{2h} k^{2h})}\ ,
\ee

Perturbations $\d Q$, $\d C$ about this equilibrium satisfy:
\begin{align}
\partial_t \,\d Q &+ J \(\d\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d C )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\,\d Q\ ,\label{eq1}\\
\partial_t \,\d C & = \(\bit\Acal^e_a + \Acal^e_b \)\d C +\(\bit\d\Acal_a + \d\Acal_b\)C^e\ ,\label{eq2}
\end{align}


The spatial component of the eigenfunction, $\d Q = \d\tilde{Q}\,e^{\s t}$, $\d C = \d\tilde{C}\,e^{\s t}$ about the homogeneous equilibrium are
\begin{align}
\d\tilde{Q}(\xv) &= e^{\i\nv\cdot\xv} ~\\
\d\tilde{C}(\xv_a,\xv_b) &= C^{\textrm{(h)}}(\xv_a-\xv_b)\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with
\be
C^{\textrm{(h)}}(\xv_a-\xv_b) = \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}
\ee
and satisfy
\begin{align}
\s \,\d \tilde{Q} &+ J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d\tilde C  )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\,\d \tilde{Q}\ ,\label{eq1}\\
\s \,\d \tilde{C} & = \(\bit\Acal^e_a + \Acal^e_b \)\d \tilde C +\(\bit\d\tilde\Acal_a + \d\tilde\Acal_b\)C^e\ ,\label{eq2}
\end{align}
with
\begin{align}
\d\Acal&=-\d\Uv\cdot\nablav + \[\bit(\Del_\la\,\d\Uv)\cdot\nablav \]\Del^{-1}_\la ~
\end{align}

Since $\d\tilde Q=e^{\i\nv\cdot\xv}$ we have
\be
\d\tilde\Psi = -\frac{\d\tilde Q}{n^2+\la^2}~,~\d\tilde U = \frac{\i n_y \d\tilde Q}{n^2+\la^2}~,~\d\tilde V = -\frac{\i n_x\,\d\tilde Q}{n^2+\la^2}~.
\ee

{\color{red} Define Rossby wave frequency as:
\be
\om_{\kv} = \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k^2+\la^2} \equiv  \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k_\la^2}
\ee
}

Calculate each term of~\eqref{eq1} and \eqref{eq2}.

\begin{enumerate}
\item
\be\boxed{
J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \frac{\i(\b_x n_y-\b_y n_x)}{n^2+\la^2}\d\tilde Q = \i\om_{\nv}\d\tilde Q }
\ee
\item
\be\boxed{
\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\,\d \tilde{Q}= \[ r+\nu_{2h} n^{2h}\]\d\tilde Q  }
\ee
\item
\begin{align}
\[ 2r+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C=?
\end{align}
We have that
\begin{align}
\nablav_a \,\d\tilde C &= \nablav_a \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
&= \iint\frac{\df^2\kv}{(2\pi)^2} (\i\kv_+)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
\nablav_b \, \d\tilde C &= \nablav_b \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
&= \iint\frac{\df^2\kv}{(2\pi)^2} (-\i\kv_-)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with $\kv_{\pm} = \kv\pm\nv/2$. Therefore $\[ 2r+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C$ translated in wavenumber space as
\begin{align}
\[ 2r+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C &=  \iint\frac{\df^2\kv}{(2\pi)^2} \[ 2r + \nu_{2h} (k^{2h}_+ + k^{2h}_-)\]\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\end{align}
or 
\begin{align}
\[ 2r+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C &\leftrightarrow  \[ 2r + \nu_{2h} (k^{2h}_+ + k^{2h}_-)\]\hat{C}^{\textrm{(h)}}(\kv)
\end{align}
\item
\begin{align}
& \[\bit\hat{\mathbf{z}}\cdot(\bv\times\nablav_a) \Del^{-1}_{\la,a}+\hat{\mathbf{z}}\cdot(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\d\tilde C= \nonumber\\
%&\qquad= \hat{\mathbf{z}}\cdot \[\bit(\bv\times\nablav_a) \Del^{-1}_{\la,a}+(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\Del_{\la,a}\Del_{\la,b}\d\tilde S ~\nonumber\\
% &\qquad=  \hat{\mathbf{z}}\cdot\[\bit(\bv\times\nablav_a) \Del_{\la,b}+(\bv\times\nablav_b) \Del_{\la,a}\] \d\tilde S \leftrightarrow~\\
 &\leftrightarrow \hat{\mathbf{z}}\cdot\[\i\bit(\bv\times \kv_{+} ) /(-k^2_{\la+})-\i\bit(\bv\times \kv_{-} ) /(-k^2_{\la-})\] \hat{C}^{\textrm{(h)}}(\kv)\\
% &\qquad=  -\i k^2_{\la+} k^2_{\la-}\, \hat{\mathbf{z}}\cdot\[\bit(\bv\times \kv_{+} )/k^2_{\la+} -\bit(\bv\times \kv_{-} )/ k^2_{\la-} \] \hat{S}^{\textrm{(h)}}(\kv)\\
 &\qquad=  -\i \, \( \om_{\kv_+} - \om_{\kv_-} \) \hat{C}^{\textrm{(h)}}(\kv)
\end{align}

Therefore
\be
\boxed{(\Acal^e_a+\Acal^e_b)\d\tilde C \leftrightarrow \[\bit- 2r - \nu_{2h} (k^{2h}_+ + k^{2h}_-) -\i \, \( \om_{\kv_+} - \om_{\kv_-} \)\] \hat{C}^{\textrm{(h)}}(\kv)}
\ee
\end{enumerate}


Some useful identities:
\begin{align}
\uv\cdot\nablav F &= J(\psi,F) = \hat{\mathbf{z}}\cdot(\nablav\psi\times\nablav F)\\
(\Del_\la\uv)\cdot\nablav F &= J(q,F) = \hat{\mathbf{z}}\cdot(\nablav q\times\nablav F)
\end{align}
Using these we calculate the term $(\d\Acal_a+\d\Acal_b) C^e$.

\begin{enumerate}
\item
\begin{align}
(\d\Uv_a\cdot\nablav_a) C^e &= J_a(\d\tilde \Psi_a,C^e)\nonumber\\
&= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)
\end{align}
we have that $\nablav_a\d\tilde \Psi_a = -\i\nv/(n^2_\la)\,e^{\i\nv\cdot\xv_a}$, where $n^2_\la = n^2+\la^2$ and therefore
\begin{align}
(\d\Uv_a\cdot\nablav_a) C^e &= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)\nonumber\\
&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}(\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{n^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{n^2_\la}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
\end{align}
\item similarly
\begin{align}
(\d\Uv_b\cdot\nablav_b) C^e &= \hat{\mathbf{z}}\cdot (\nablav_b\d\tilde \Psi_b\times\nablav_b C^E)\nonumber\\
&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}(-\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{n^2_\la}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
\end{align}
\item
\begin{align}
\[\bit(\Del_{\la,a}\d\Uv_a)\cdot\nablav_a\]\Del_{\la,a}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_a\d\tilde Q_a\times\nablav_a \Del_{\la,a}^{-1}C^e)\nonumber\\
&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{k^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{k^2_{\la-}}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
\end{align}
\item and similarly
\begin{align}
\[\bit(\Del_{\la,b}\d\Uv_b)\cdot\nablav_b\]\Del_{\la,b}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_b\d\tilde Q_b\times\nablav_b \Del_{\la,b}^{-1}C^e)\nonumber\\
&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{k^2_{\la+}}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
\end{align}
\end{enumerate}


Therefore
\begin{empheq}[box=\fbox]{align}
&(\d\Acal_a+\d\Acal_b) C^e = \nonumber\\
&\hspace{2em}=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\iint\frac{\df^2\kv}{(2\pi)^2}\[\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\frac1{k^2_{\la-}}-\frac1{n^2_\la}\)\,\hat{C}^e(\kv_-)-\right.\nonumber\\
&\hspace{15em}\left.-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\frac1{k^2_{\la+}}-\frac1{n^2_\la}\)\,\hat{C}^e(\kv_+)\]\,e^{\i\kv\cdot(\xv_a-\xv_b)} 
\end{empheq}


We are now in the position to solve the perturbation covariance equation and obtain $\hat{C}^{\textrm{(h)}}(\kv)$ as

\begin{empheq}[box=\fbox]{align}
&\hat{C}^{\textrm{(h)}}(\kv)=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\times\nonumber\\
 &\vspace{2em}\times\dfrac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\dfrac1{k^2_{\la-}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv_-)-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\dfrac1{k^2_{\la+}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv_+)}{\s+2r + \nu_{2h} (k^{2h}_+ + k^{2h}_-) -\i \, \( \om_{\kv_-} - \om_{\kv_+}\)}\nonumber\\
  &\vspace{1em}\equiv e^{\i\nv\cdot(\xv_a+\xv_b)/2} \[\bit F(\kv_-)-F(\kv_+)\]
\end{empheq}


How much is $\Rcal (\dC)$ ?

\begin{align}
&\Rcal (\dC)     =\nonumber\\
&\hspace{.3em}  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\!\times\!\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) \dC\]_{\xv_a=\xv_b}\nonumber\\
%&  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\times\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) \iint\frac{\df^2\kv}{(2\pi)^2} \hat{C}^{\textrm{(h)}}(\kv) e^{\i\kv\cdot(\xv_a-\xv_b)} \]_{\xv_a=\xv_b}\nonumber\\
&\hspace{.3em}  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\!\times\!\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) \iint\!\frac{\df^2\kv}{(2\pi)^2} \[\bit F(\kv_-)-F(\kv_+)\] e^{\i\nv\cdot(\xv_a+\xv_b)/2}e^{\i\kv\cdot(\xv_a-\xv_b)} \]_{\xv_a=\xv_b}\nonumber\\
%&  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\times \iint\frac{\df^2\kv}{(2\pi)^2} \(\frac{\i \kv_+}{-k^2_{\la+}}-\frac{\i \kv_-}{-k^2_{\la-}} \)\[\bit F(\kv_-)-F(\kv_+)\] e^{\i (\kv_+\cdot \xv_a-\kv_-\xv_b)} \]_{\xv_a=\xv_b}\nonumber\\
&\hspace{.3em}  =-\nablav\cdot \iint\!\frac{\df^2\kv}{(2\pi)^2} \frac{\hat{\mathbf{z}}}{2}\!\times\!\(\frac{\i \kv_-}{k^2_{\la-}}-\frac{\i \kv_+}{k^2_{\la+}} \)\[\bit F(\kv_-)-F(\kv_+)\] e^{\i \nv\cdot\xv}
\end{align}
Moreover, since under $\kv\to-\kv$ we have that $\kv_+ \to- \kv_-$, $k^2_{\la+} \to k^2_{\la-}$ and $F(\kv_+)\to -F(\kv_-)$ we get that 
\begin{align}
\Rcal (\dC)    &   =-\nablav\cdot \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\times\(\frac{\i \kv_-}{k^2_{\la-}}-\frac{\i \kv_+}{k^2_{\la+}} \)\, F(\kv_-)  e^{\i \nv\cdot\xv}~.
\end{align}
It is easy to derive that for any vector $\pv$,
\be
\nablav\cdot\( \hat{\mathbf{z}}\times\pv\,e^{\i\nv\cdot\xv}\) = -\i\,\hat{\mathbf{z}}\cdot(\nv\times\pv)\,e^{\i\nv\cdot\xv}\ ,
\ee
and therefore
\begin{align}
\Rcal (\dC)  &   = \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2_{\la,+}} -\frac1{k^2_{\la,-}}\)\, F(\kv_-)  e^{\i \nv\cdot\xv} \nonumber\\
& = \d\tilde Q\iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2_{\la,s}} -\frac1{k^2_{\la}}\)\, F(\kv)   \nonumber\\
&   =\d\tilde Q \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv)}{\s+2r + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  
\end{align}

Using the above we find that from the mean flow perturbation equation $\s$ must satisfy:
\begin{align}
\sigma + r + \nu_{2h} n^{2h} + \i\om_{\nv}&= \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\hat{C}^e(\kv)}{\s+2r + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  \\
&= \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(k^2_{\la,s}-k^2_{\la}\)\(k^2_{\la}-n^2_\la\)\,\hat{C}^e(\kv)}{k_{\la,s}^2k_{\la}^4 n_\la^2 \[\s+2r + \nu_{2h} (k^{2h}_s + k^{2h}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)\bit\]}  
\end{align}





\subsection{dissipate only kinetic energy, $-r\Delta\psi$}
We will write with red only the differences from $- rq$. 

For the NL system:
\begin{align}
\partial_t q + J(\psi,q) + \beta v  =\xi +\textrm{Diss}
\end{align}
with
\begin{align}
\textrm{Diss}&= - r \textcolor{red}{\Delta \psi} - (-1)^h\nu_{2h} \Delta^{h}\textcolor{red}{\Delta \psi} = -\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Delta \psi}\ \\
q &=\Delta \psi - \lambda^2 \psi~~,~~u =-\partial_y \psi ~~,~~v= \partial_x \psi~.
\end{align}
$h=1$ is diffusion, $h>1$ hyperdiffusion

Define $q=Q+q'$, etc. Then
\begin{align}
&\partial_t Q + J(\Psi,Q + \bv\cdot\xv) =- r \textcolor{red}{\Del\Psi} - (-1)^h\nu_{2h}  \Delta^{h}\textcolor{red}{\Del\Psi} - \Tcal[ J(\psi',q') ]~\\
&\partial_t q' = \Acal(\Uv) \,q' + f_{\textrm{nl}} + \xi
\end{align}
with
\begin{align}
\Acal(\Uv)&=-\Uv\cdot\nablav + \[\bit(\Del_\la\Uv)\cdot\nablav + \hat{\mathbf{z}}\cdot(\bv\times\nablav)\]\Del^{-1}_\la - \[r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Del\Del_\la^{-1}}~\\
f_{\textrm{nl}}&=\Tcal[ J(\psi',q') ]-J(\psi',q')
\end{align}

Eddy vorticity covariance is again $C(\xv_a,\xv_b,t)=\<q'(\xv_a,t)q'(\xv_b,t)\>$ and using the ergodic hypothesis $\Tcal(\bullet) = \<\bullet\>$ the Reynolds stress divergence can be expressed as:
\begin{align}
 -\Tcal[ J(\psi',q') ]&=-\nablav\cdot \<(\uv'\,q')\>\\
    &  =-\nablav\cdot\[\frac{\hat{\mathbf{z}}}{2}\times\(\nablav_a \Del_{\la,a}^{-1}+\nablav_b \Del_{\la,b}^{-1}\) C\]_{\xv_a=\xv_b}\nonumber\\
  &\equiv \Rcal(C)\ .
\end{align}


S3T system is
\begin{align}
\partial_t \, Q &+ J \(\Psi,Q+ {\bm\beta}\cdot\mathbf{x} \) = \Rcal( C )-\[r+(-1)^{h}\nu_{2h} \Del^h\]\,\textcolor{red}{\Del\Del_\la^{-1}}Q\ ,\\
\partial_t \, C & = \[\bit\Acal_a(\Uv) + \Acal_b(\Uv) \] C +\varepsilon\,Q\ ,
\end{align}

Consider a homogeneous, stationary equilibrium solution, $Q^e$, $C^e(\xv_a-\xv_b)$. Expanding $C^e$ as
\be
C^e(\xv_a-\xv_b) = \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}
\ee
(and similarly for $Q(\xv_a-\xv_b)$), we find that
\be
\textcolor{red}{\hat{C}^e(\kv) }= \frac{\varepsilon\,\hat{Q}(\kv)}{2(r+\nu_{2h} k^{2h})}\textcolor{red}{\frac{k^2_\la}{k^2}}\ ,
\ee

Perturbations $\d Q$, $\d C$ about this equilibrium satisfy:
\begin{align}
\partial_t \,\d Q &+ J \(\d\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d C )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\,\textcolor{red}{\Del\Del_\la^{-1}}\d Q\ ,\label{eq1}\\
\partial_t \,\d C & = \(\bit\Acal^e_a + \Acal^e_b \)\d C +\(\bit\d\Acal_a + \d\Acal_b\)C^e\ ,\label{eq2}
\end{align}


The spatial component of the eigenfunction, $\d Q = \d\tilde{Q}\,e^{\s t}$, $\d C = \d\tilde{C}\,e^{\s t}$ about the homogeneous equilibrium are
\begin{align}
\d\tilde{Q}(\xv) &= e^{\i\nv\cdot\xv} ~\\
\d\tilde{C}(\xv_a,\xv_b) &= C^{\textrm{(h)}}(\xv_a-\xv_b)\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with
\be
C^{\textrm{(h)}}(\xv_a-\xv_b) = \iint\frac{\df^2\kv}{(2\pi)^2}\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}
\ee
and satisfy
\begin{align}
\s \,\d \tilde{Q} &+ J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \Rcal( \d\tilde C  )-\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Del\Del_\la^{-1}}\d \tilde{Q}\ ,\label{eq1}\\
\s \,\d \tilde{C} & = \(\bit\Acal^e_a + \Acal^e_b \)\d \tilde C +\(\bit\d\tilde\Acal_a + \d\tilde\Acal_b\)C^e\ ,\label{eq2}
\end{align}
with
\begin{align}
\d\Acal&=-\d\Uv\cdot\nablav + \[\bit(\Del_\la\,\d\Uv)\cdot\nablav \]\Del^{-1}_\la ~
\end{align}

Since $\d\tilde Q=e^{\i\nv\cdot\xv}$ we have
\be
\d\tilde\Psi = -\frac{\d\tilde Q}{n^2+\la^2}~,~\d\tilde U = \frac{\i n_y \d\tilde Q}{n^2+\la^2}~,~\d\tilde V = -\frac{\i n_x\,\d\tilde Q}{n^2+\la^2}~.
\ee

 Define Rossby wave frequency as:
\be
\om_{\kv} = \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k^2+\la^2} \equiv  \frac{\hat{\mathbf{z}}\cdot(\bv\times\kv)}{k_\la^2}
\ee

Calculate each term of~\eqref{eq1} and \eqref{eq2}.

\begin{enumerate}
\item
\be\boxed{
J \(\d\tilde\Psi, {\bm\beta}\cdot\mathbf{x} \) = \frac{\i(\b_x n_y-\b_y n_x)}{n^2+\la^2}\d\tilde Q = \i\om_{\nv}\d\tilde Q }
\ee
\item
\be\boxed{
\[ r+(-1)^h\nu_{2h} \Delta^{h}\]\textcolor{red}{\Del\Del_\la^{-1}}\d \tilde{Q}= \[ r+\nu_{2h} n^{2h}\]\textcolor{red}{(n^2/n^2_\la)}\d\tilde Q  }
\ee
\item
\begin{align}
\[ 2r\textcolor{red}{(\Del_a\Del_{\la,a}^{-1}+\Del_b\Del_{\la,b}^{-1})}+(-1)^h\nu_{2h} (\Delta_a^{h}\textcolor{red}{\Del_a\Del_{\la,a}^{-1}}+\Delta_b^{h}\textcolor{red}{\Del_b\Del_{\la,b}^{-1}})\]\d\tilde C=?
\end{align}
We have that
\begin{align}
\nablav_a \,\d\tilde C &= \iint\frac{\df^2\kv}{(2\pi)^2} (\i\kv_+)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}\\
\nablav_b \, \d\tilde C &= \iint\frac{\df^2\kv}{(2\pi)^2} (-\i\kv_-)\hat{C}^{\textrm{(h)}}(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)}\,e^{\i\nv\cdot(\xv_a+\xv_b)/2}
\end{align}
with $\kv_{\pm} = \kv\pm\nv/2$. Therefore $\[ 2r\textcolor{red}{(\Del_a\Del_{\la,a}^{-1}+\Del_b\Del_{\la,b}^{-1})}+(-1)^h\nu_{2h} (\Delta_a^{h}\textcolor{red}{\Del_a\Del_{\la,a}^{-1}}+\Delta_b^{h}\textcolor{red}{\Del_b\Del_{\la,b}^{-1}})\]\d\tilde C$ translated in wavenumber space as
\begin{align}
&\[ 2r\textcolor{red}{(\Del_a\Del_{\la,a}^{-1}+\Del_b\Del_{\la,b}^{-1})}+(-1)^h\nu_{2h} (\Delta_a^{h}+\Delta_b^{h})\]\d\tilde C \leftrightarrow \nonumber\\
&\qquad\leftrightarrow \[ 2r\textcolor{red}{(k^2_+/ k^2_{\la,+} + k^2_-/ k^2_{\la,-})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_+/k^2_{\la,+} + k^{2h+2}_-/k^2_{\la,-}})\]\hat{C}^{\textrm{(h)}}(\kv)
\end{align}
\item
\begin{align}
& \[\bit\hat{\mathbf{z}}\cdot(\bv\times\nablav_a) \Del^{-1}_{\la,a}+\hat{\mathbf{z}}\cdot(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\d\tilde C= \nonumber\\
%&\qquad= \hat{\mathbf{z}}\cdot \[\bit(\bv\times\nablav_a) \Del^{-1}_{\la,a}+(\bv\times\nablav_b) \Del^{-1}_{\la,b}\]\Del_{\la,a}\Del_{\la,b}\d\tilde S ~\nonumber\\
% &\qquad=  \hat{\mathbf{z}}\cdot\[\bit(\bv\times\nablav_a) \Del_{\la,b}+(\bv\times\nablav_b) \Del_{\la,a}\] \d\tilde S \leftrightarrow~\\
 &\leftrightarrow \hat{\mathbf{z}}\cdot\[\i\bit(\bv\times \kv_{+} ) /(-k^2_{\la+})-\i\bit(\bv\times \kv_{-} ) /(-k^2_{\la-})\] \hat{C}^{\textrm{(h)}}(\kv)\\
% &\qquad=  -\i k^2_{\la+} k^2_{\la-}\, \hat{\mathbf{z}}\cdot\[\bit(\bv\times \kv_{+} )/k^2_{\la+} -\bit(\bv\times \kv_{-} )/ k^2_{\la-} \] \hat{S}^{\textrm{(h)}}(\kv)\\
 &\qquad=  -\i \, \( \om_{\kv_+} - \om_{\kv_-} \) \hat{C}^{\textrm{(h)}}(\kv)
\end{align}

Therefore
\be
\boxed{(\Acal^e_a+\Acal^e_b)\d\tilde C \leftrightarrow \[\bit- 2r \textcolor{red}{(k^2_+/ k^2_{\la,+} + k^2_-/ k^2_{\la,-})}- \nu_{2h} (\textcolor{red}{k^{2h+2}_+/k^2_{\la,+} + k^{2h+2}_-/k^2_{\la,-}}) -\i \, \( \om_{\kv_+} - \om_{\kv_-} \)\] \hat{C}^{\textrm{(h)}}(\kv)}
\ee
\end{enumerate}


Some useful identities:
\begin{align}
\uv\cdot\nablav F &= J(\psi,F) = \hat{\mathbf{z}}\cdot(\nablav\psi\times\nablav F)\\
(\Del_\la\uv)\cdot\nablav F &= J(q,F) = \hat{\mathbf{z}}\cdot(\nablav q\times\nablav F)
\end{align}
Using these we calculate the term $(\d\Acal_a+\d\Acal_b) C^e$. Everything is the same, except $C^e$.
%
%\begin{enumerate}
%\item
%\begin{align}
%(\d\Uv_a\cdot\nablav_a) C^e &= J_a(\d\tilde \Psi_a,C^e)\nonumber\\
%&= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)
%\end{align}
%we have that $\nablav_a\d\tilde \Psi_a = -\i\nv/(n^2_\la)\,e^{\i\nv\cdot\xv_a}$, where $n^2_\la = n^2+\la^2$ and therefore
%\begin{align}
%(\d\Uv_a\cdot\nablav_a) C^e &= \hat{\mathbf{z}}\cdot (\nablav_a\d\tilde \Psi_a\times\nablav_a C^E)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}(\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{n^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
%\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{n^2_\la}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\item similarly
%\begin{align}
%(\d\Uv_b\cdot\nablav_b) C^e &= \hat{\mathbf{z}}\cdot (\nablav_b\d\tilde \Psi_b\times\nablav_b C^E)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(-\frac{\i\nv}{n^2_\la}\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}(-\i\kv)\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{n^2_\la}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\item
%\begin{align}
%\[\bit(\Del_{\la,a}\d\Uv_a)\cdot\nablav_a\]\Del_{\la,a}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_a\d\tilde Q_a\times\nablav_a \Del_{\la,a}^{-1}C^e)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_a}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%&=  \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv)}{k^2_\la}\,\hat{C}^e(\kv)\,e^{\i(\kv+\nv)\cdot\xv_a-\i\kv\cdot\xv_b} \nonumber\\
%\textrm{(after $\kv\to\kv'=\kv+\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-)}{k^2_{\la-}}\,\hat{C}^e(\kv_-)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\item and similarly
%\begin{align}
%\[\bit(\Del_{\la,b}\d\Uv_b)\cdot\nablav_b\]\Del_{\la,b}^{-1}C^e &=\hat{\mathbf{z}}\cdot (\nablav_b\d\tilde Q_b\times\nablav_b \Del_{\la,b}^{-1}C^e)\nonumber\\
%&= \hat{\mathbf{z}}\cdot \(\i\nv\,e^{\i\nv\cdot\xv_b}\times\iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\i\kv}{-k^2_\la}\hat{C}^e(\kv)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \)\nonumber\\
%\textrm{(after $\kv\to\kv'=\kv-\nv/2$)}&=  e^{\i\nv\cdot(\xv_a+\xv_b)/2} \iint\frac{\df^2\kv}{(2\pi)^2}\frac{-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)}{k^2_{\la+}}\,\hat{C}^e(\kv_+)\,e^{\i\kv\cdot(\xv_a-\xv_b)} \nonumber\\
%\end{align}
%\end{enumerate}
Therefore
\begin{empheq}[box=\fbox]{align}
&(\d\Acal_a+\d\Acal_b) \textcolor{red}{C^e} = \nonumber\\
&\hspace{2em}=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\iint\frac{\df^2\kv}{(2\pi)^2}\[\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\frac1{k^2_{\la-}}-\frac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_-)}-\right.\nonumber\\
&\hspace{15em}\left.-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\frac1{k^2_{\la+}}-\frac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_+)}\]\,e^{\i\kv\cdot(\xv_a-\xv_b)} 
\end{empheq}


We are now in the position to solve the perturbation covariance equation and obtain $\hat{C}^{\textrm{(h)}}(\kv)$ as

\begin{empheq}[box=\fbox]{align}
&\hat{C}^{\textrm{(h)}}(\kv)=e^{\i\nv\cdot(\xv_a+\xv_b)/2}\times\nonumber\\
 &\vspace{2em}\times\dfrac{\hat{\mathbf{z}}\cdot(\nv\times\kv_-) \(\dfrac1{k^2_{\la-}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_-)}-\hat{\mathbf{z}}\cdot(\nv\times\kv_+)\(\dfrac1{k^2_{\la+}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv_+)}}{\s+2r\textcolor{red}{(k^2_+/ k^2_{\la,+} + k^2_-/ k^2_{\la,-})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_+/k^2_{\la,+} + k^{2h+2}_-/k^2_{\la,-}}) -\i \, \( \om_{\kv_-} - \om_{\kv_+}\)}\nonumber\\
  &\vspace{1em}\equiv e^{\i\nv\cdot(\xv_a+\xv_b)/2} \[\bit F(\kv_-)-F(\kv_+)\]
\end{empheq}


How much is $\Rcal (\d C)$ ?

\begin{align}
\Rcal (\d C)    &   =-\nablav\cdot \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\times\(\frac{\i \kv}{k^2_{\la}}-\frac{\i (\kv+\nv)}{k^2_{\la,s}} \)\, \textcolor{red}{F(\kv)}  e^{\i \nv\cdot\xv} \nonumber\\
\end{align}

Now after some algebra we get that:
\begin{align}
\nablav\cdot\( \hat{\mathbf{z}}\times\kv\,e^{\i\nv\cdot\xv}\) &= -\i\hat{\mathbf{z}}\cdot(\nv\times\kv)\\
\nablav\cdot\( \hat{\mathbf{z}}\times\nv\,e^{\i\nv\cdot\xv}\) &= 0
\end{align}
therefore
\begin{align}
\Rcal (\d C)  &   = \iint\frac{\df^2\kv}{(2\pi)^2} \hat{\mathbf{z}}\cdot(\nv\times\kv)\(\frac1{k^2_{\la,s}} -\frac1{k^2_{\la}}\)\, \textcolor{red}{F(\kv)}  e^{\i \nv\cdot\xv} \nonumber\\
&   =\d\tilde Q \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv)}}{\s+2r\textcolor{red}{(k^2_s/ k^2_{\la,s} + k^2/ k^2_{\la})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_s/k^2_{\la,s} + k^{2h+2}/k^2_{\la}}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  
\end{align}

Using the above we find that from the mean flow perturbation equation $\s$ must satisfy:
\begin{align}
&\sigma + (r + \nu_{2h} n^{2h})\textcolor{red}{(n^2/n^2_\la)} + \i\om_{\nv}=\nonumber\\
&\qquad= \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(\dfrac1{k^2_{\la,s}}-\dfrac1{k^2_{\la}} \)\(\dfrac1{k^2_{\la}}-\dfrac1{n^2_\la}\)\,\textcolor{red}{\hat{C}^e(\kv)}}{\s+2r\textcolor{red}{(k^2_s/ k^2_{\la,s} + k^2/ k^2_{\la})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_s/k^2_{\la,s} + k^{2h+2}/k^2_{\la}}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)}  \\
&\qquad=  \iint\frac{\df^2\kv}{(2\pi)^2} \dfrac{|\nv\times\kv|^2 \(k^2_{\la,s}-k^2_{\la}\)\(k^2_{\la}-n^2_\la\)\,\textcolor{red}{(k^2_\la/k^2)}\,\hat{C}^{e,OLD}(\kv)}{k_{\la,s}^2k_{\la}^4 n_\la^2 \[\s+2r\textcolor{red}{(k^2_s/ k^2_{\la,s} + k^2/ k^2_{\la})} + \nu_{2h} (\textcolor{red}{k^{2h+2}_s/k^2_{\la,s} + k^{2h+2}/k^2_{\la}}) -\i \, \( \om_{\kv} - \om_{\kv+\nv}\)\bit\]}  
\end{align}














\textcolor{green}{H E R E }



the generalized S3T dispersion relation is:
\begin{align}
\sigma\, N^2_\la/N^2+& r + \nu_4 N^4 - \i\b m/N^2 =\intinf\intinf\frac{\df k}{2\pi}\frac{\df \l}{2\pi} \frac{\Ncal~(K^2/N^2-1)}{K^2_\la\(\sigma \Dcal_\sigma +  \Dcal_0 + \i\b\,\Dcal_\b\)}\,C^E(k,\l)
\end{align}


where $\<\xi_a\xi_b\>=\d(t_a-t_b) Q(x_a-x_b,y_a-y_b)$ and 
\begin{subequations}
\begin{align}
C^E(k,\l)&=\frac{\varepsilon\,K^2_{\la} \,Q(k,\l) }{2 r K^2 + 2 \nu_4 K^6 }~,\\
\Ncal &= 2(nk-m\l)\[\bit mn(k^2_+ - \l^2_+) - (m^2-n^2) k_+\l_+ \]=\nonumber\\
&=(nk-m\l)^2 (K^2_s-K^2)~,\\
\Dcal_\sigma &= K^2_\la K^2_{s,\la}~,\\
\Dcal_0 &= r  \,(K^2 K^2_{s,\la} + K^2_{\la}K^2_{s}) + \nu_4  (K^6 K^2_{s,\la} + K^6_{s} K^2_{\la})~,\\
\Dcal_\b &= k\,K^2_{s,\la} -(k+m)K^2_{\la}~.
\end{align}
\end{subequations}
with
\begin{subequations}
\begin{align}
N^2 = m^2+n^2~~&,~~N^2_\la = N^2+\la^2~,\\
K^2 = k^2+\l^2~~&,~~K^2_\la = K^2+\la^2~,\\
K^2_{s} = (k+m)^2+(\l+n)^2~~&,~~K^2_{s,\la} = K^2_{s}+\la^2~.
\end{align}
\end{subequations}
%    B1 = K2la.^2.*Ks2la;
%    B2 = r*K2la.*(K2.*Ks2la + K2la.*Ks2) + nu4*K2la.*(K2.^3.*Ks2la + Ks2.^3.*K2la);
%    B3 = beta*K2la.*(k.*Ks2la -(k+m).*K2la);
%        
%    Denom = s*B1+B2+1i*B3 ;
%    
%    SP_f  =   A1    ./ Denom;



==> chapters/app-rednoise.tex <==
\chapter{Calculation of S3T growth rates for the homogeneous equilibrium for red-noise stochastic forcing}
\label{app:rednoise}

Let us introduce red-noise stochastic forcing with decorrelation time $\tau=1/\a$. This system is described by:
\begin{align}
\partial_t \z'_a &= \Acal_a\,\z'_a + \eta_a~,\\
\partial_t \eta_a &=-\a\,\eta_a + \xi_a~.
\end{align}
where $\z'=\z'(\xv,t)$, $\eta_a=\eta(\xv,t)$,
\be
\mathcal{A}_a = -U_\a\,\partial_{x_a} - \(\beta-U''_\a\)\partial_{x_a}\Del_\a^{-1}-r~,
\ee
and $\xi_\a=\xi(x_\a,y_\a,t)$ is white noise forcing with:
\be
\<\xi(\xv_a,t)\xi(\xv_b,t')\> = \d(t-t')\,Q(\xv_a-\xv_b)~.
\ee

Let us define the state $\zeta_\a = \[q_\a,\eta_\a\]^\transp$ and $f_\a = \[0,\xi_\a\]^\transp$ so that the above system can be written as:
\be
\partial_t \zeta_\a = \tilde{\cal A}_\a\,\zeta_\a + f_\a~,\label{eq:zeta_a}
\ee
where $\tilde{\cal A}_\a$ is the expanded operator:
\be
\tilde{\cal A}_\a = \left(
\begin{array}{cc}
  {\cal A}_\a &  1   \\
   0 & -a   
\end{array}
\right)
\ee
We can as before define the two point same time perturbation field covariance,
\be
\tilde{\cal C}_{\a\b} = \< \zeta_\a\,\zeta_\b^\transp \>= \left(
\begin{array}{cc}
  \<q_\a q_\b\> &  \<q_\a\eta_\b\>   \\
   \<\eta_\a q_\b\> & \<\eta_\a\eta_\b\>   
\end{array}
\right)
\equiv \left(
\begin{array}{cc}
  \cal{C}_{\a\b} &  \Sigma^{(1)}_{\a\b}   \\
   \Sigma^{(2)}_{\a\b} & \cal{H}_{\a\b}   
\end{array}
\right)
\ee
It can be verified that~\footnote{The easiest way to do that is to work with~\eqref{eq:zeta_a}. Suppose that $\zeta_\a$ and $f_\a$ are  $2N\times 1$ column vectors and $f_\a = F \xi_\a$ where $F$ is a $2N\times N$ matrix with the upper square part zero and the lower square part the identity and $\xi_\a$ is an $N\times 1$ column vector. We can calculate $\<\zeta_\a \,f_\b\>$ using that $\zeta_\a = \int^t \[e^{\mathcal{A}(t-s)}\]_{\a m} F_{mn} \xi_n(s)\,\df s$ as:\bdm \<\zeta_\a \,f_\b\> = \int^t \[e^{\mathcal{A}(t-s)}\]_{\a m} F_{mn}  F_{bk} \<\xi_n(s)\xi_k(t)\>\,\df s = \int^t \[e^{\mathcal{A}(t-s)}\]_{\a m} F_{mn}  F_{\b k} \frac1{2}\Xi_{nk}\d(t-s)\,\df s\edm\bdm = \frac1{2} \d_{\a m} F_{mn}  F_{\b k}\Xi_{nk} = \frac1{2} F_{\a n} \Xi_{nk} \[F^\transp\]_{k\b}   \edm This is a $2N\times 2N$ matrix with only the lower right $N\times N$ part nonzero and equal to $\Xi/2$. Therefore we have Eqs.~\eqref{eq:64}.}\begin{subequations}
\begin{align}
\<\xi_\a \eta_\b + \eta_\a\xi_\b\> & = \Xi_{\a\b}~,\\
\<\xi_\a q_\b \> = \<\xi_\b q_\a \> &= 0~.\label{eq:doubt}
\end{align}\label{eq:64}\end{subequations}
so the equations for the evolution of each of the components of $\tilde{\cal C}_{\a\b}$ are:\begin{subequations}
\begin{align}
\partial_t {\cal C}_{\a\b} &=\({\cal A}_\a +{\cal A}_\b\) {\cal C}_{\a\b} +  \Sigma^{(1)}_{\a\b}+\Sigma^{(2)}_{\a\b}~,\\
\partial_t  \Sigma^{(1)}_{\a\b} &=\({\cal A}_\a-a\)  \Sigma^{(1)}_{\a\b}  +  {\cal H}_{\a\b} ~,\\
\partial_t  \Sigma^{(2)}_{\a\b} &=\({\cal A}_\b-a\)  \Sigma^{(2)}_{\a\b}  + {\cal H}_{\a\b} ~,\\
\partial_t {\cal H}_{\a\b} &=-2a {\cal H}_{\a\b}  + \Xi_{\a\b}~.
\end{align}\end{subequations}

The state with no mean flow $U=0$ will be an equilibrium if we can find such (homogeneous) components of $\tilde{\mathcal{C}}$ so that the left-hand sides of the above equations go to zero. Thus we have:\begin{subequations}\begin{align}
0 &=\({\cal A}^E_\a +{\cal A}^E_\b\) {\cal C}^E_{\a\b} +  \Sigma^{(1),E}_{\a\b}+\Sigma^{(2),E}_{\a\b}~,\label{eq:Cab}\\
0 &=\({\cal A}^E_\a-a\)  \Sigma^{(1),E}_{\a\b}  + {\cal H}^E_{\a\b} ~,\label{eq:Sigma1}\\
0 &=\({\cal A}^E_\b-a\)  \Sigma^{(2),E}_{\a\b}  + {\cal H}^E_{\a\b} ~,\label{eq:Sigma2}\\
0 &=-2a {\cal H}^E_{\a\b}  + \Xi_{\a\b}~.
\end{align}\end{subequations}
The last one immediately gives
\be
{\cal H}^E_{\a\b} =\frac{ \Xi_{\a\b}}{2a}~.
\ee
We define ${\Psi}$ and ${\cal S}^{(1,2)}$ as:\begin{subequations}
\begin{align}
{\cal C}_{\a\b}  &= \<q_\a q_\b\> = \Del_\a\Del_\b\<\psi_\a\psi_\b\>= \Del_\a\Del_\b \Psi_{\a\b}~,\label{eq:Psi}\\
\Sigma^{(1)}_{\a\b}  &= \<q_\a\eta_\b\> = \Del_\a\<\psi_\a\eta_\b\>  = \Del_\a\,{\cal S}^{(1)}_{\a\b}~,\\
\Sigma^{(2)}_{\a\b}  &= \<\eta_\a q_\b\> = \Del_\b\<\eta_\a\psi_\b\>  = \Del_\b\,{\cal S}^{(2)}_{\a\b}~.
\end{align}\end{subequations}
The equilibrium is homogeneous, that is when we change to centroid-difference coordinates all components of $\tilde{\mathcal{C}}$ depend only on the difference coordinates:\begin{subequations}\begin{align}
{\cal C}^E_{\a\b} &\rightarrow {\cal C}^E(\tilde{x},\tilde{y})  \\
{\Psi}^E_{\a\b} &\rightarrow {\Psi}^E(\tilde{x},\tilde{y})  \\
\Sigma^{(j),E}_{\a\b} &\rightarrow \Sigma^{(j),E}(\tilde{x},\tilde{y})   = \tilde{\Del}\, {\cal S}^{(j),E}(\tilde{x},\tilde{y})~,\quad j=1,2~,\\
{\cal H}^E_{\a\b} &\rightarrow {\cal H}^E(\tilde{x},\tilde{y}) ~.
\end{align}\end{subequations}

Using that the equilibrium operator for $U=0$ is:
\be
{\cal A}^E_\a = -r - \beta\partial_{x_\a} \Del^{-1}_\a
\ee
the Eqs.~\eqref{eq:Cab}-\eqref{eq:Sigma2} in centroid-difference coordinates become:
\begin{subequations}\begin{align}
0 &=-2r\tilde{\Del}^2\Psi^E(\tilde{x},\tilde{y})+ \Sigma^{(1),E}(\tilde{x},\tilde{y})+\Sigma^{(2),E}(\tilde{x},\tilde{y})~,\label{eq:Psi}\\
0 &=-(r+a)\,\tilde{\Del}\,{\cal S}^{(1),E}(\tilde{x},\tilde{y})  - \beta\partial_{\tilde{x}} \, {\cal S}^{(1),E}(\tilde{x},\tilde{y})   + {\cal H}^E(\tilde{x},\tilde{y}) ~,\label{eq:S1}\\
0 &=-(r+a)\,\tilde{\Del}\,{\cal S}^{(2),E}(\tilde{x},\tilde{y}) + \beta\partial_{\tilde{x}} \, {\cal S}^{(2),E}(\tilde{x},\tilde{y})   + {\cal H}^E(\tilde{x},\tilde{y}) ~,\label{eq:S2}
\end{align}\end{subequations}
Therefore they have solutions:
\begin{subequations}\begin{align}
{\cal \hat{S}}^{(1),E}(k,\l) &=\frac{-{\cal\hat{H}}^E(k,\l)}{(r+a) K^2 -\i \beta k} = \frac{-{\hat{\Xi}}(k,\l)}{2a(r+a) K^2-2a\i \beta k} ~,\label{eq:Skl1}\\
{\cal \hat{S}}^{(2),E}(k,\l) &=\frac{-{\cal\hat{H}}^E(k,\l)}{(r+a) K^2 +\i \beta k} = \frac{-{\hat{\Xi}}(k,\l)}{2a(r+a) K^2+2a\i \beta k} ~,\label{eq:Skl2}
\end{align}\end{subequations}
\begin{subequations}\begin{align}
{\hat{\Sigma}}^{(1),E}(k,\l) &= \frac{ K^2{\hat{\Xi}}(k,\l)}{2a\[(r+a) K^2 -\i \beta k\]} ~,\label{eq:Sigmakl1}\\
{\hat{\Sigma}}^{(2),E}(k,\l) &= \frac{ K^2{\hat{\Xi}}(k,\l)}{2a\[(r+a) K^2 +\i \beta k\]} ~.\label{eq:Sigmakl2}\\
{\hat{{\Psi}}}^{E}(k,\l) &=\frac{(r+a)}{2ar \left[ (r+a)^2 K^4+k^2 \beta ^2\right]}{\hat{\Xi}}(k,\l)~.\label{eq:Psikl}
\end{align}\label{eqs:equilibria_red}\end{subequations}
or from Eq.~\eqref{eq:Psi}
\be
{\hat{{\cal C}}}^{E}(k,\l) =\frac{(r+a)K^4}{2ar \left[ (r+a)^2 K^4+k^2 \beta ^2\right]}{\hat{\Xi}}(k,\l)~.\\
\ee
%\be
%\partial_t C_{\a\b} = ({\cal A}_\a + {\cal A}_\b) C_{\a\b} + \Xi_{\a\b}~,\label{eq:ssst_cont_la_Cab}
%\ee
%where
%\be
%{\cal A}_\a = -U_\a \partial_{x_\a} - Q'_\a \partial_{x_\a} (\Del_\a)^{-1}_\la - r +\nu_2 \Del_\a - \nu_4 \Del^2_\a~.
%\ee
In order to check the stability of this equilibrium we perturb it and write the evolution equation for the perturbations.\begin{subequations}
\begin{align}
\partial_t \, {\d\cal C}_{\a\b} &=\({\cal A}^E_\a +{\cal A}^E_\b\)\, {\d\cal C}_{\a\b} + \({\d\cal A}_\a +{\d\cal A}_\b\)\, {\cal C}^E_{\a\b} +  \d\Sigma^{(1)}_{\a\b}+\d\Sigma^{(2)}_{\a\b}~,\\
\partial_t  \,\d\Sigma^{(1)}_{\a\b} &=\({\cal A}^E_\a-a\)  \d\Sigma^{(1)}_{\a\b} +\d{\cal A}_\a\,\Sigma^{(1),E}_{\a\b} ~,\\
\partial_t  \,\d\Sigma^{(2)}_{\a\b} &=\({\cal A}^E_\b-a\)  \d\Sigma^{(2)}_{\a\b} +\d{\cal A}_\b\,\Sigma^{(2),E}_{\a\b} ~,\\
\partial_t\, {\d\cal H}_{\a\b} &=-2a\, {\d\cal H}_{\a\b} ~.
\end{align}\end{subequations}

In the above
\be
\d\mathcal{A}_a = -(\d U)_\a\,\partial_{x_a} +(\d U'')_\a \,\partial_{x_a}\Del_\a^{-1}~,
\ee

\begin{subequations}
\begin{align}
\partial_t \, {\d\mathcal{C}}_{\a\b} &=\(-2r-\beta\partial_{x_\a}\Del_\b-\beta\partial_{x_\b}\Del_\a\)\,\d\Psi_{\a\b} +  \({\d\cal A}_\a +{\d\cal A}_\b\)\, {\cal C}^E_{\a\b} +  \d\Sigma^{(1)}_{\a\b}+\d\Sigma^{(2)}_{\a\b}~,\\
\partial_t  \,\d\Sigma^{(1)}_{\a\b} &=\[\bit-(r+a)\Del_\a-\beta\partial_{x_\a} \]\,\d\mathcal{S}^{(1)}_{\a\b} +\d{\cal A}_\a\,\Sigma^{(1),E}_{\a\b} ~,\\
\partial_t  \,\d\Sigma^{(2)}_{\a\b} &=\[\bit-(r+a)\Del_\b-\beta\partial_{x_\b} \]\,\d\mathcal{S}^{(2)}_{\a\b} +\d{\cal A}_\b\,\Sigma^{(2),E}_{\a\b} ~,\\
\partial_t\, {\d\cal H}_{\a\b} &=-2a\, {\d\cal H}_{\a\b} ~.
\end{align}\end{subequations}

In centroid-difference coordinates:\begin{subequations}
\begin{align}
\Del_\a &= \tilde{\Del} + \frac1{4}\partial^2_{\bar{y}\bar{y}} + \partial^2_{\bar{y}\tilde{y}}~,\\
\Del_\b &= \tilde{\Del} + \frac1{4}\partial^2_{\bar{y}\bar{y}} - \partial^2_{\bar{y}\tilde{y}}~,
\end{align}
\end{subequations}
We would like to calculate $ \({\d\cal A}_\a +{\d\cal A}_\b\)\, {\cal C}^E_{\a\b}$ in the new coordinates.
\begin{align}
 \({\d\cal A}_\a +{\d\cal A}_\b\)\, {\cal C}^E_{\a\b} & =  \({\d\cal A}_\a +{\d\cal A}_\b\)\,\Del_\a\Del_\b {\Psi}^E_{\a\b}\nonumber\\
 & =  \[\bit-(\d U)_\a\,\partial_{x_a} -(\d U)_\b\,\partial_{x_b} \]\Del_\a\Del_\b {\Psi}^E_{\a\b} +\nonumber\\
 &\qquad+ \[\bit (\d U'')_\a \,\partial_{x_a}\Del_\b +(\d U'')_\b \,\partial_{x_b}\Del_\a\]\, {\Psi}^E_{\a\b}\rightarrow\\
 &\rightarrow \[\bit-\d U(\bar{y}+\tilde{y}/2)+\d U(\bar{y}-\tilde{y}/2) \] \partial_{\tilde{x}} \tilde{\Del}^2 {\Psi}^E +\nonumber\\
 &\qquad+ \[\bit \d U''(\bar{y}+\tilde{y}/2) -\d U''(\bar{y}-\tilde{y}/2) \]\, \partial_{\tilde{x}} \tilde{\Del} {\Psi}^E \nonumber
\end{align}
and for a $\d U = e^{\i ny}$
\begin{align}
\({\d\cal A}_\a +{\d\cal A}_\b\)\, {\cal C}^E_{\a\b} &\rightarrow -e^{\i n \bar{y}} \(e^{\i n \tilde{y}/2}-e^{-\i n \tilde{y}/2} \) \partial_{\tilde{x}} \tilde{\Del}^2 {\Psi}^E + n^2\,e^{\i n \bar{y}} \(e^{\i n \tilde{y}/2}-e^{-\i n \tilde{y}/2} \) \, \partial_{\tilde{x}} \tilde{\Del} {\Psi}^E \end{align}

Similarly we can calculate $\d\mathcal{A}_\a \Del_\a \,\d \mathcal{S}^{(1)}_{\a\b}$ and  $\d\mathcal{A}_\b \Del_\b \,\d \mathcal{S}^{(2)}_{\a\b}$
therefore the above equations trasform to:\begin{subequations}
\begin{align}
\partial_t \, {\d\mathcal{C}} &=-2r{\d\mathcal{C}} +2\beta\partial^3_{\tilde{x}\tilde{y}\bar{y}}\,\d\Psi +  \[\bit-\d U(\bar{y}+\tilde{y}/2)+\d U(\bar{y}-\tilde{y}/2) \] \partial_{\tilde{x}} \tilde{\Del}^2 {\Psi}^E +\nonumber\\
 &\qquad\qquad\qquad+ \[\bit \d U''(\bar{y}+\tilde{y}/2) -\d U''(\bar{y}-\tilde{y}/2) \]\, \partial_{\tilde{x}} \tilde{\Del} {\Psi}^E  +  \d\Sigma^{(1)}+\d\Sigma^{(2)}~,\label{eq:calC}\\
\partial_t  \,\Del_\a\,\d\mathcal{S}^{(1)} &=\[\bit-(r+a)\Del_\a-\beta\partial_{\tilde{x}} \]\,\d\mathcal{S}^{(1)} +\[-\d U(\bar{y}+\tilde{y}/2)\tilde{\Del} + \d U''(\bar{y}+\tilde{y}/2)\]\partial_{\tilde{x}}\,\mathcal{S}^{(1),E} ~,\label{eq:calS1}\\
\partial_t  \,\Del_\b\,\d\mathcal{S}^{(2)} &=\[\bit-(r+a)\Del_\b+\beta\partial_{\tilde{x}} \]\,\d\mathcal{S}^{(2)} +\[-\d U(\bar{y}-\tilde{y}/2)\tilde{\Del} + \d U''(\bar{y}-\tilde{y}/2)\]\(-\partial_{\tilde{x}}\)\,\mathcal{S}^{(2),E} ~,\label{eq:calS2}\\
\partial_t\, {\d\cal H}_{\a\b} &=-2a\, {\d\cal H}_{\a\b} ~.\label{eq:calH}
\end{align}

Plus we have the mean flow perturbation equation:
\be
\partial_t\,\d U = -\left.\bit\partial^3_{\tilde{x}\tilde{y}\bar{y}}\,\d\Psi\right|_{\tilde{x}=\tilde{y}=0} - \rU\d U~.\label{eq:calU}
\ee\label{eqs:eigensystem_rednoise}
\end{subequations}
Eigenvalues of the system of Eqs.~\eqref{eqs:eigensystem_rednoise} will determine the stability of the homogeneous equilibrium.

Let us assume perturbations in the form:
\begin{align}
\d U_n(y,t) &= e^{\i n y+\sigma t}~,\\
\d \Psi_n(\tilde{x},\tilde{y},\bar{y},t) &= e^{\i n \bar{y}+\sigma t}\,\Psi_n(\tilde{x},\tilde{y})~,\\
\d \mathcal{S}^{(1,2)}_n(\tilde{x},\tilde{y},\bar{y},t) &= e^{\i n \bar{y}+\sigma t}\,\mathcal{S}_n(\tilde{x},\tilde{y})~.
\end{align}
and also consider the expansion of the homogeneous part of the eigensolutions,
\begin{align}
\Phi_n(\tilde{x},\tilde{y}) = \iint \frac{\df k\,\df\l}{(2\pi)^2}\,\hat{\Phi}_n(k,\l)\,e^{\i(k\tilde{x}+\l\tilde{y})}
\end{align}

From Eqs.~\eqref{eq:calS1} and \eqref{eq:calS2} we solve $\d\mathcal{S}_n^{(1,2)}$
\begin{align}
%\hat{\mathcal{S}}^{(1)}_n &=\frac{rK^2-\i k\beta}{(\sigma+r+a)  K^2_{+} - \i k \beta}\,\hat{\mathcal{S}}^{(1),E} ~,\\
\hat{\mathcal{S}}^{(1)}_n &=\frac{-\i k (K_{-}^2-n^2)}{(\sigma+r+a)  K_{+}^2 - \i k \beta}\,\hat{\mathcal{S}}^{(1),E}_{-} ~,\\
%\hat{\mathcal{S}}^{(2)}_n &=\frac{rK^2+\i k\beta}{(\sigma+r+a)  K^2_{-} + \i k \beta}\,\hat{\mathcal{S}}^{(2),E} ~,\\
\hat{\mathcal{S}}^{(2)}_n &=\frac{\i k (K_{+}^2-n^2)}{(\sigma+r+a)  K_{-}^2 + \i k \beta}\,\hat{\mathcal{S}}^{(2),E}_{+} ~.
\end{align}
or
\begin{align}
%\hat{\Sigma}^{(1)}_n &=- \frac{rK^2K^2_{+}-\i k\beta K^2_{+}}{(\sigma+r+a)  K^2_{+} - \i k \beta}\,\hat{\mathcal{S}}^{(1),E} ~,\\
\hat{\Sigma}^{(1)}_n &=\frac{\i k (K_{-}^2-n^2)}{(\sigma+r+a)  K_{+}^2 - \i k \beta}\,K^2_{+}\,\hat{\mathcal{S}}^{(1),E}_{-} ~,\\
%\hat{\Sigma}^{(2)}_n &=-\frac{rK^2K^2_{-} +\i k\beta K^2_{-} }{(\sigma+r+a)  K^2_{-} + \i k \beta}\,\hat{\mathcal{S}}^{(2),E} ~.
\hat{\Sigma}^{(2)}_n &=\frac{-\i k (K_{+}^2-n^2)}{(\sigma+r+a)  K_{-}^2 + \i k \beta}\,K^2_{-}\,\hat{\mathcal{S}}^{(2),E}_{+} ~.
\end{align}

\be
(\sigma+2r) \, {\d\mathcal{C}}=-2\beta\partial^3_{\tilde{x}\tilde{y}\bar{y}}\,\d\Psi +  \[\bit-\d U(\bar{y}+\tilde{y}/2)+\d U(\bar{y}-\tilde{y}/2) \] \partial_{\tilde{x}} \tilde{\Del}^2 {\Psi}^E +\nonumber\\
\ee
Now Eq.~\eqref{eq:calC} gives us $\d\mathcal{C}_n$ which we enter in Eq.~\eqref{eq:calU}.
%\begin{align}
%&\[\bit(\sigma+2r) K^2_{+}K^2_{-} +2\i\beta n k \l \]\hat{\Psi}_n= \nonumber\\
%&\qquad= \sin{(n\tilde{y}/2)}\[2 k K^2(K^2-n^2)\] {\Psi}^E - \nonumber\\
%&\qquad\qquad- \frac{rK^2K^2_{+}-\i k\beta K^2_{+}}{(\sigma+r+a)  K^2_{+} - \i k \beta}\,\hat{\mathcal{S}}^{(1),E} -\frac{rK^2K^2_{-} +\i k\beta K^2_{-} }{(\sigma+r+a)  K^2_{-} + \i k \beta}\,\hat{\mathcal{S}}^{(2),E} ~,\label{eq:sol_psi_n}
%\end{align}
%
\begin{align}
&\[\bit(\sigma+2r) K^2_{+}K^2_{-} +2\i\beta n k \l \]\hat{\Psi}_n= \nonumber\\
&\qquad= \i k \(K^4_{+}-K^2_{+} n^2\)\hat{\Psi}^E_+ - \i k\(K^4_{-}-K^2_{-} n^2\)\hat{\Psi}^E_- \,+ \nonumber\\
&\qquad\qquad+\frac{\i k (K_{-}^2-n^2)}{(\sigma+r+a)  K_{+}^2 - \i k \beta}\,K^2_{+}\,\hat{\mathcal{S}}^{(1),E}_{-} - \frac{\i k (K_{+}^2-n^2)}{(\sigma+r+a)  K_{-}^2 + \i k \beta}\,K^2_{-}\,\hat{\mathcal{S}}^{(2),E}_{+} ~,\label{eq:sol_psi_n}
\end{align}
where $\hat{\Psi}^E_{\pm}(k,\l)  = \hat{\Psi}^E(k,\l\pm n/2)$
%
%
%\begin{align}
%\hat{\Psi}_n(k,\l) &= \i k \frac{\(K^4_{+}-K^2_{+} n^2\)\hat{\Psi}^E_+ - \(K^4_{-}-K^2_{-} n^2\)\hat{\Psi}^E_-}{(\sigma+2r)K^2_{+}K^2_{-} + 2\i n\b k\l}~.
%\end{align}




And thus the dispersion equation is:\be
\sigma+\rU = n \(\Lambda_{-} - \Lambda_{+}  + R_2 -R_1 \)
\ee
with\begin{subequations}\begin{align}
\Lambda_{\pm} &=  \iint \frac{\df k\,\df\l}{(2\pi)^2}\, \frac{ k^2\l \(K^4_{\pm}-K^2_{\pm} \,n^2\)}{(\sigma+2r) K^2_{+}K^2_{-} +2\i\beta n k \l} \hat{\Psi}^E_\pm\\
R_{1} &=  \iint \frac{\df k\,\df\l}{(2\pi)^2}\, \frac{ k^2\l (K_{-}^2-n^2)K^2_{+}}{\[(\sigma+r+a)  K_{+}^2 - \i k \beta\]\[(\sigma+2r) K^2_{+}K^2_{-} +2\i\beta n k \l\]}\,\hat{\mathcal{S}}_{-}^{(1),E}\\
R_{2} &=  \iint \frac{\df k\,\df\l}{(2\pi)^2}\, \frac{k^2\l (K_{+}^2-n^2)K^2_{-}}{\[(\sigma+r+a)  K_{-}^2 + \i k \beta\]\[(\sigma+2r) K^2_{+}K^2_{-} +2\i\beta n k \l\]}\,\hat{\mathcal{S}}_{+}^{(2),E}
\end{align}\end{subequations}
where $\hat{\Psi}_n(k,\l)$ is given by Eq.~\eqref{eq:sol_psi_n}. Can this be simplified any more?
We notice that with a change of variables $(k,\l)\to(-k,-\l)$ then $\Lambda_{+}\to-\Lambda_{-}$ and $R_2\to -R_1$. Therefore:
\be
\sigma+\rU = 2n \( \Lambda_{-} - R_1\)
\ee
and furthermore, in the $\Lambda_{-}$ if we change $\lambda\to\lambda-n/2$ then:\begin{subequations}\begin{align}
\Lambda_{-} &=  \iint \frac{\df k\,\df\l}{(2\pi)^2}\, \frac{ k^2(\l+n/2) K^2 \(K^2-n^2\)}{(\sigma+2r) K^2_{++}K^2 +2\i\beta n k (\l+n/2)} \hat{\Psi}^E\\
R_{1} &=  \iint \frac{\df k\,\df\l}{(2\pi)^2}\, \frac{ k^2(\l+n/2) (K^2-n^2)K^2_{++}}{\[(\sigma+r+a)  K_{++}^2 - \i k \beta\]\[(\sigma+2r) K^2_{++}K^2 +2\i\beta n k (\l+n/2)\]}\,\hat{\mathcal{S}}^{(1),E}\end{align}\end{subequations}

Therefore, the eigenvalue $\sigma$ satisfies:


\begin{align}
\sigma+\rU &= \iint \frac{\df k\,\df\l}{(2\pi)^2}\,\[\frac{ 2nk^2(\l+n/2) K^2 \(K^2-n^2\)}{(\sigma+2r) K^2_{++}K^2 +2\i\beta n k (\l+n/2)} \hat{\Psi}^E - \right.\\
&\qquad\qquad-\left.\frac{ 2nk^2(\l+n/2) (K^2-n^2)K^2_{++}}{\[(\sigma+r+a)  K_{++}^2 - \i k \beta\]\[(\sigma+2r) K^2_{++}K^2 +2\i\beta n k (\l+n/2)\]}\,\hat{\mathcal{S}}^{(1),E}\]
\end{align}


\vspace*{2cm}
In the limit of zero correlation time $\tau$, or $a\to+\infty$ we must gain the white-noise dispersion relation. Consider the equilibria~\eqref{eqs:equilibria_red} and let $\hat{\Xi}(k,\l)\to\varepsilon\,\hat{\Xi}(k,\l)$. Then if we take the limit $a\to+\infty$ while $\varepsilon/a^2=\epsilon$ then we end up whith
\begin{align}
{\hat{\Sigma}}^{(1,2),E}(k,\l) &= \frac{\epsilon}{2}\hat{\Xi}(k,\l)~,\\
\hat{\mathcal{C}}^{E}(k,\l) &= K^4{\hat{{\Psi}}}^{E}(k,\l)=\frac{\epsilon}{2r} \hat{\Xi}(k,\l)~.
\end{align}
The $\Psi$ equilibrium goes to the ``white noise'' version. But $\Sigma$ do not go to zero. However, if we take this limit then the integrals $R_{1,2}$ go to zero recovering therefore in this way our previous dispersion relation.

\vspace*{3cm}
What would change if the operator $\mathcal{A}$ and also the mean flow were also dissipated with diffusion and hyperdiffusion?
\be
\mathcal{A}_a = -U_\a\,\partial_{x_a} - \(\beta-U''_\a\)\partial_{x_a}\Del_\a^{-1}-r +\nu_2\Del_\a-\nu_4\Del_\a^2~.
\ee

If we define\begin{subequations}\begin{align}
r'&\equiv r+\nu_2 K^2+\nu_4 K^4~,\\
r'_{\pm}&\equiv r+\nu_2 K^2_{\pm}+\nu_4 K^4_{\pm}~,
\end{align}\end{subequations}
then equilibria are the same as before with $r\to r'$:\begin{subequations}\begin{align}
\hat{\Sigma}_\nu^{(1),E}(k,\l) &= \frac{K^2\,\hat{\Xi}(k,\l)}{2a\left\{(r'+a)K^2 -\i \beta k\right\}}~~,~~\hat{\mathcal{S}}_\nu^{(1),E}(k,\l) &= \frac{-\hat{\Xi}(k,\l)}{2a\left\{(r'+a)K^2 -\i \beta k\right\}} ~,\label{eq:Skl1_nu}\\
\hat{\Sigma}_\nu^{(2),E}(k,\l) &= \frac{K^2\,\hat{\Xi}(k,\l)}{2a\left\{(r'+a)K^2 +\i \beta k\right\}}~~,~~\hat{\mathcal{S}}_\nu^{(2),E}(k,\l) &= \frac{-\hat{\Xi}(k,\l)}{2a\left\{(r'+a)K^2 +\i \beta k\right\}},\label{eq:Skl2_nu}\\
{\hat{{\Psi}}}_\nu^{E}(k,\l) &=\frac{(a+r')}{2a r'\, \left[ (a+r')^2 K^4+k^2 \beta ^2\right]}\,\hat{\Xi}(k,\l)~,\label{eq:Psikl_nu}
\end{align}\end{subequations}
%\begin{subequations}\begin{align}
%\hat{\Sigma}^{(1),E}(k,\l) &= \frac{K^2{\hat{\Xi}}(k,\l)}{2a\left\{\[(r+a)+\nu_2 K^2+\nu_4 K^4\]K^2 -\i \beta k\right\}} ~,\label{eq:Skl1_nu}\\
%\hat{\Sigma}^{(2),E}(k,\l) &= \frac{K^2{\hat{\Xi}}(k,\l)}{2a\left\{\[(r+a)+\nu_2 K^2+\nu_4 K^4\]K^2 +\i \beta k\right\}} ~,\label{eq:Skl2_nu}\\
%{\hat{{\Psi}}}^{E}(k,\l) &=\frac{(a+r+\nu_2 K^2+\nu_4 K^4)}{2a\(r+\nu_2 K^2+\nu_4 K^4\) \left[ (a+r+\nu_2 K^2+\nu_4 K^4)^2 K^4+k^2 \beta ^2\right]}{\hat{\Xi}}(k,\l)~.\label{eq:Psikl_nu}
%\end{align}\end{subequations}
while the perturbation eigenfunctions change to:
\begin{subequations}\begin{align}
%\hat{\mathcal{S}}^{(1)}_n &=\frac{rK^2-\i k\beta}{(\sigma+r+a)  K^2_{+} - \i k \beta}\,\hat{\mathcal{S}}^{(1),E} ~,\\
\hat{\mathcal{S}}^{(1)}_{\nu,n} &=\frac{-\i k (K_{-}^2-n^2)}{(\sigma+r'_{+}+a)  K_{+}^2 - \i k \beta}\,\hat{\mathcal{S}}^{(1),E}_{-} ~~,~~\hat{\Sigma}^{(1)}_{\nu,n} =\frac{\i k (K_{-}^2-n^2)}{(\sigma+r'_{+}+a)  K_{+}^2 - \i k \beta}\,K_{+}^2\,\hat{\mathcal{S}}^{(1),E}_{-} ~,\\
%\hat{\mathcal{S}}^{(2)}_n &=\frac{rK^2+\i k\beta}{(\sigma+r+a)  K^2_{-} + \i k \beta}\,\hat{\mathcal{S}}^{(2),E} ~,\\
\hat{\mathcal{S}}^{(2)}_{\nu,n} &=\frac{\i k (K_{+}^2-n^2)}{(\sigma+r'_{-}+a)  K_{-}^2 + \i k \beta}\,\hat{\mathcal{S}}^{(2),E}_{+} ~~,~~\hat{\Sigma}^{(2)}_{\nu,n} =\frac{-\i k (K_{+}^2-n^2)}{(\sigma+r'_{-}+a)  K_{-}^2 + \i k \beta}\,K_{-}^2\,\hat{\mathcal{S}}^{(2),E}_{+} ~,
\end{align}
and
\begin{align}
&\[\bit(\sigma+r'_{+}+r'_{-}) K^2_{+}K^2_{-} +2\i\beta n k \l \]\hat{\Psi}_{\nu,n}= \nonumber\\
&\qquad= \i k \(K^4_{+}-K^2_{+} n^2\)\hat{\Psi}^E_{\nu,+} - \i k\(K^4_{-}-K^2_{-} n^2\)\hat{\Psi}^E_{\nu,-} + \nonumber\\
&\qquad\qquad+\frac{\i k (K_{-}^2-n^2)}{(\sigma+r'_{+}+a)  K_{+}^2 - \i k \beta}\,K_{+}^2\,\hat{\mathcal{S}}^{(1),E}_{\nu,-}-\frac{\i k (K_{+}^2-n^2)}{(\sigma+r'_{-}+a)  K_{-}^2 + \i k \beta}\,K^2_{-}\,\hat{\mathcal{S}}^{(2),E}_{\nu,+}  ~.\label{eq:sol_psi_n}
\end{align}
\end{subequations}

\vspace*{1cm}

Thus the dispersion relation is:
\begin{align}
\sigma&+\rU+\nu_2 n^2+\nu_4 n^4 = \\
&\qquad=\iint \frac{\df k\,\df\l}{(2\pi)^2}\,\[\frac{ 2nk^2(\l+n/2) K^2 \(K^2-n^2\)}{(\sigma+r'_{++}+r') K^2_{++}K^2 +2\i\beta n k (\l+n/2)} \hat{\Psi}_\nu^E \,- \right.\\
&\qquad\qquad-\left.\frac{2n k^2(\l+n/2) (K^2-n^2)K^2_{++}}{\[(\sigma+r'_{++}+a)  K_{++}^2 - \i k \beta\]\[(\sigma+r'_{++}+r') K^2_{++}K^2 +2\i\beta n k (\l+n/2)\]}\,\hat{\mathcal{S}}_\nu^{(1),E}\]
\end{align}






\textcolor{red}{ . . .  to be continued }



==> chapters/chap-S3TnonhomNL.tex <==
%\begin{savequote}[75mm] 
%This is some random quote to start off the chapter.
%\qauthor{Firstname lastname} 
%\end{savequote}

\chapter{Finite amplitude states predicted by S3T and its reflection in nonlinear simulations}

\section{ ? ? }


==> chapters/chap-finite_nonhom.tex <==
%\begin{savequote}[75mm] 
%This is some random quote to start off the chapter.
%\qauthor{Firstname lastname} 
%\end{savequote}

\chapter{S3T stability of inhomogeneous equilibria}

In this chapter we will deploy methods with which we can address the S3T stability of inhomogeneous equilibrium solutions, that is solutions that are dominated either by zonal jets or non-zonal propagating coherent structures..



\section{S3T generalized system}

S3T system allowing interaction of coherent structures described by streamfunction $\Psi(x,y)$ (from which all fields can be derived, $U=-\partial_y\Psi$, $V=\partial_x\Psi$, $Z=\Del\Psi$) with the turbulent eddy field, $C = \<\z'(x_\a,y_\a,t)\z'(x_\b,y_\b,t)\>$ is:\begin{subequations}
\begin{align}
&\partial_t  Z + U\partial_x Z + V\partial_y Z +\beta V =  - r Z -\nu_4 \Del^2 Z - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_\a} \Del_\a^{-1}-\partial_{y_\b} \Del_\b^{-1}\) C \right|_{\x_\a=\x_\b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_\a} \Del_\a^{-1}+\partial_{x_\b} \Del_\b^{-1}\) C \right|_{\x_\a=\x_\b} \]\\
&\partial_t C  = \(\bit \Acal_\a +\Acal_\b\) C + Q~.
\end{align}\end{subequations}
with
\be
\Acal_\a \equiv\left.\bit\Acal(\Psi)\right|_{\x=\x_a} = -U_a \partial_{x_\a}-V_a \partial_{y_\a} - \(\beta+Z_{y_\a}\) \partial_{x_\a} \Del_\a^{-1} + Z_{x_\a} \partial_{y_\a}\Del_\a^{-1} - r -\nu_4 \Del_\a^2~.
\ee
This system can be written in matrix form:\begin{subequations}
\begin{align}
&\partial_t \Zv + \U \,\D_x  \Zv  +  \V \,\D_y \Zv  +\beta \, \Vv =  - r \, \Zv -\nu_4 \,\DDel^2 \Zv - \nonumber\\
&\qquad\qquad\qquad- \D_x \[ \vecd{\( - \D_y \DDel^{-1}\C\)}\] - \D_y \[\vecd{\( \D_x \DDel^{-1}\C\)}\]\\
&\partial_t\,\C  = \A\, \C+ \C\,\A^\transp + \Q~.
\end{align}\end{subequations}

This system admits equilibria with a coherent structure described by streamfunction $\Psi^E$ and an eddy vorticity covariance, $C^E$. Perturbations around one of these equilibria satisfy:
\begin{subequations}
\begin{align}
&\partial_t \,\d Z + \d U\, \partial_x Z^E + U^E\, \partial_x \d Z +  \d V \,\partial_y Z^E + V^E\, \partial_y \d Z  +\beta \,\d V =  - r \,\d Z -\nu_4 \,\Del^2 \d Z - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_\a} \Del_\a^{-1}-\partial_{y_\b} \Del_\b^{-1}\) \d C \right|_{\x_\a=\x_\b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_\a} \Del_\a^{-1}+\partial_{x_\b} \Del_\b^{-1}\) \d C \right|_{\x_\a=\x_\b} \]\\
&\partial_t\,\d C  = \(\bit \Acal^E_\a +\Acal^E_\b\) \d C + \(\bit \d\Acal_\a +\d\Acal_\b\) C^E ~.
\end{align}\end{subequations}
with\begin{subequations}
\begin{align}
\Acal^E_\a  &= \left.\bit\Acal(\Psi^E)\right|_{\x=\x_a}  ,\\
\d\Acal_\a  &=\left.\bit\Acal(\Psi^E+\d \Psi)\right|_{\x=\x_a}- \left.\bit\Acal(\Psi^E)\right|_{\x=\x_a} \nonumber\\
&=  -\d U_a \partial_{x_\a} -\d V_a \partial_{y_\a} - \d Z_{y_\a} \partial_{x_\a} \Del_\a^{-1} + \d Z_{x_\a} \partial_{y_\a}\Del_\a^{-1} ~.
\end{align}\end{subequations}
or in matrix form:
\begin{subequations}
\begin{align}
&\partial_t \,\d \Zv + \d \U \,\D_x  \Zv^E + \U^E\,\D_x \d \Zv +  \d \V \,\D_y \Zv^E + \V^E\, \D_y \d \Zv  +\beta \,\d \Vv =  - r \,\d \Zv -\nu_4 \,\DDel^2 \d \Zv - \nonumber\\
&\qquad- \D_x \[ \vecd{\( - \D_y \DDel^{-1}\d\C\)}\] - \D_y \[\vecd{\( \D_x \DDel^{-1}\d\C\)}\]\\
&\partial_t\,\d\C  = \A^E \d\C+ \d\C\,\(\A^E\)^\transp + \d\A\,\C^E +\C^E\,\(\d\A\)^\transp~.
\end{align}\end{subequations}

{\color{Green}
For jets, $\Zv^E=-\Uv^E_y$:
\begin{subequations}
\begin{align}
&\partial_t \,\d \Zv +  \d \V \,(-\Uv^E_{yy})  +\beta \,\d \Vv =  - r \,\d \Zv -\nu_4 \,\DDel^2 \d \Zv  - \D_y \[\vecd{\( \D_x \DDel^{-1}\d\C\)}\]\\
&\partial_t\,\d\C  = \A^E \d\C+ \d\C\,\(\A^E\)^\transp + \d\A\,\C^E +\C^E\,\(\d\A\)^\transp~.
\end{align}\end{subequations}

}

The above is a real dynamical system. Searching for eigensolutions, $\d\Psi = \d\hat{\Psi} e^{\s t}$, $\d Z = \d\hat{Z} e^{\s t}$, $\d C = \d\hat{C} e^{ \s t}$:%s. With these substitution we have that $\d\Acal_\a = \d\hat{\Acal}_\a e^{\s t}$ and moreover:
\begin{subequations}
\begin{align}
&\s \,\d\hat{Z} + \d\hat{U}\, \partial_x Z^E + U^E\, \partial_x \d\hat{Z} +  \d\hat{V} \,\partial_y Z^E + V^E\, \partial_y \d\hat{Z}  +\beta \,\d \hat{V} =  - r \,\d \hat{Z} -\nu_4 \,\Del^2 \d \hat{Z} - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_\a} \Del_\a^{-1}-\partial_{y_\b} \Del_\b^{-1}\) \d \hat{C} \right|_{\x_\a=\x_\b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_\a} \Del_\a^{-1}+\partial_{x_\b} \Del_\b^{-1}\) \d \hat{C} \right|_{\x_\a=\x_\b} \]\\
&\s\,\d \hat{C}  = \(\bit \Acal^E_\a +\Acal^E_\b\) \d \hat{C} + \(\bit \d\hat{\Acal}_\a +\d\hat{\Acal}_\b\) C^E ~.
\end{align}\end{subequations}


\begin{subequations}
\begin{align}
&\s \,\d \Zv + \d \U \,\D_x  \Zv^E + \U^E\,\D_x \d \Zv +  \d \V \,\D_y \Zv^E + \V^E\, \D_y \d \Zv  +\beta \,\d \Vv =  - r \,\d \Zv -\nu_4 \,\DDel^2 \d \Zv - \nonumber\\
&\qquad- \D_x \[ \vecd{\( - \D_y \DDel^{-1}\d\C\)}\] - \D_y \[\vecd{\( \D_x \DDel^{-1}\d\C\)}\]\\
&\s\,\d\C  = \A^E \d\C+ \d\C\,\(\A^E\)^\transp + \d\A\,\C^E +\C^E\,\(\d\A\)^\transp~.
\end{align}\label{eq:pert_S3Tgen}\end{subequations}

{\color{Green}
For jets:
\begin{subequations}
\begin{align}
&\s \,\d\hat{Z}  +  \d\hat{V} \,(-U_{yy}^E)  +\beta \,\d \hat{V} =  - r \,\d \hat{Z} -\nu_4 \,\Del^2 \d \hat{Z} - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_\a} \Del_\a^{-1}+\partial_{x_\b} \Del_\b^{-1}\) \d \hat{C} \right|_{\x_\a=\x_\b} \]\\
&\s\,\d \hat{C}  = \(\bit \Acal^E_\a +\Acal^E_\b\) \d \hat{C} + \(\bit \d\hat{\Acal}_\a +\d\hat{\Acal}_\b\) C^E ~.
\end{align}\end{subequations}


\begin{subequations}
\begin{align}
&\s \,\d \Zv +  \d \V \,(-\Uv^E_{yy}) + \beta \,\d \Vv =  - r \,\d \Zv -\nu_4 \,\DDel^2 \d \Zv  - \D_y \[\vecd{\( \D_x \DDel^{-1}\d\C\)}\]\\
&\s\,\d\C  = \A^E \d\C+ \d\C\,\(\A^E\)^\transp + \d\A\,\C^E +\C^E\,\(\d\A\)^\transp~.
\end{align}\label{eq:pert_S3Tgen}\end{subequations}


with\begin{subequations}
\begin{align}
\Acal^E_\a  &= \left.\bit\Acal(\Psi^E)\right|_{\x=\x_a}  = -U^E_a \partial_{x_\a}- \(\beta+Z^E_{y_\a}\) \partial_{x_\a} \Del_\a^{-1} - r -\nu_4 \Del_\a^2~,\\
\d\Acal_\a  &=\left.\bit\Acal(\Psi^E+\d \Psi)\right|_{\x=\x_a}- \left.\bit\Acal(\Psi^E)\right|_{\x=\x_a} =  -\d U_a \partial_{x_\a} -\d V_a \partial_{y_\a} - \d Z_{y_\a} \partial_{x_\a} \Del_\a^{-1} + \d Z_{x_\a} \partial_{y_\a}\Del_\a^{-1} ~.
\end{align}\end{subequations}


}




%\subsection{Petros thought}
%
%\be
%\d Z(x,y,t) = \d Z(x-v t,y)
%\ee
%
%Let us have a case with a homogeneous flow equilibrium in which the $\d Z_{mn} = e^{\i(mx+ny)}e^{(\s_r+\i\s_i)t}$ is an eigenfuction with eigenvalue $\s=\s_r+\i\s_i$.

\subsection{Continuous formalism}



S3T system with $Z(x,y,t)$, $C(x_\a,y_\a,x_\b,y_\b) = \Del_\a \Del_\b\,S(x_\a,y_\a,x_\b,y_\b)$:\begin{subequations}
\begin{align}
&\partial_t  Z + U\partial_x Z + V\partial_y Z +\beta V =  - r Z -\nu_4 \Del^2 Z - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_\a} \Del_\a^{-1}-\partial_{y_\b} \Del_\b^{-1}\) C \right|_{\x_\a=\x_\b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_\a} \Del_\a^{-1}+\partial_{x_\b} \Del_\b^{-1}\) C \right|_{\x_\a=\x_\b} \]\\
&\partial_t C  = \(\bit \Acal_\a +\Acal_\b\) C + Q~.
\end{align}\end{subequations}
with
\be
\Acal_\a \equiv\left.\bit\Acal(\Psi)\right|_{\xv=\xv_a} = -U_a \partial_{x_\a}-V_a \partial_{y_\a} - \(\beta+Z_{y_\a}\) \partial_{x_\a} \Del_\a^{-1} + Z_{x_\a} \partial_{y_\a}\Del_\a^{-1} - r -\nu_4 \Del_\a^2~.
\ee
Perturbations around an equlibrium satisfy:
\begin{subequations}
\begin{align}
&\partial_t \,\d Z + \d U\, \partial_x Z^E + U^E\, \partial_x \d Z +  \d V \,\partial_y Z^E + V^E\, \partial_y \d Z  +\beta \,\d V =  - r \,\d Z -\nu_4 \,\Del^2 \d Z - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_\a} \Del_\a^{-1}-\partial_{y_\b} \Del_\b^{-1}\) \d C \right|_{\x_\a=\x_\b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_\a} \Del_\a^{-1}+\partial_{x_\b} \Del_\b^{-1}\) \d C \right|_{\x_\a=\x_\b} \]\\
&\partial_t\,\d C  = \(\bit \Acal^E_\a +\Acal^E_\b\) \d C + \(\bit \d\Acal_\a +\d\Acal_\b\) C^E ~.
\end{align}\end{subequations}
with\begin{subequations}
\begin{align}
\Acal^E_\a  &= \left.\bit\Acal(\Psi^E)\right|_{\x=\x_a}  = -U^E_a \partial_{x_\a}-V^E_a \partial_{y_\a} - \(\beta+Z^E_{y_\a}\) \partial_{x_\a} \Del_\a^{-1} + Z^E_{x_\a} \partial_{y_\a}\Del_\a^{-1} - r -\nu_4 \Del_\a^2~,\\
\d\Acal_\a  &=\left.\bit\Acal(\Psi^E+\d \Psi)\right|_{\x=\x_a}- \left.\bit\Acal(\Psi^E)\right|_{\x=\x_a} =  -\d U_a \partial_{x_\a} -\d V_a \partial_{y_\a} - \d Z_{y_\a} \partial_{x_\a} \Del_\a^{-1} + \d Z_{x_\a} \partial_{y_\a}\Del_\a^{-1} ~.
\end{align}\end{subequations}

The above is a real dynamical system. Searching for eigensolutions, $\d\Psi = \d\hat{\Psi} e^{\s t}$, $\d Z = \d\hat{Z} e^{\s t}$, $\d C = \d\hat{C} e^{ \s t}$:%s. With these substitution we have that $\d\Acal_\a = \d\hat{\Acal}_\a e^{\s t}$ and moreover:
\begin{subequations}
\begin{align}
&\s \,\d\hat{Z} + \d\hat{U}\, \partial_x Z^E + U^E\, \partial_x \d\hat{Z} +  \d\hat{V} \,\partial_y Z^E + V^E\, \partial_y \d\hat{Z}  +\beta \,\d \hat{V} =  - r \,\d \hat{Z} -\nu_4 \,\Del^2 \d \hat{Z} - \nonumber\\
&\qquad- \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_\a} \Del_\a^{-1}-\partial_{y_\b} \Del_\b^{-1}\) \d \hat{C} \right|_{\x_\a=\x_\b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_\a} \Del_\a^{-1}+\partial_{x_\b} \Del_\b^{-1}\) \d \hat{C} \right|_{\x_\a=\x_\b} \]\\
&\s\,\d \hat{C}  = \(\bit \Acal^E_\a +\Acal^E_\b\) \d \hat{C} + \(\bit \d\hat{\Acal}_\a +\d\hat{\Acal}_\b\) C^E ~.\label{eq:pert_dC_s}
\end{align}\label{eq:pert_syst_cont}\end{subequations}


For a jet equilibrium, $U^E(y), V^E=0, C^E(x_\a-x_\b,y_\a,y_\b)$ the equilibrium covariance is homogeneous in $x$. Therefore we expect that the eigenfunction to be of the form:
\begin{subequations}\begin{align}
%\d S &= S_m(\xt,\yt,\yb)\,e^{\i m\xb} \\
%\nonumber\\
\d \Psi_m (x,y,t) &= e^{\i m x} e^{\s t} ~\textrm{`}\sum_n\textrm{'}~ a_n e^{\i n y}  ~,\label{eq:eig_dPsi}\\
\d C_m(x_\a,y_\a,x_\b,y_\b) &= e^{\i m(x_\a+x_\b)/2} ~\textrm{`}\sum_k\textrm{'} ~\d\hat{C}_{k,m} (y_\a,y_\b) e^{\i k(x_\a-x_\b)} ~.\label{eq:eig_dCm}
\end{align}\label{eq:eig_dPsim_dCm}\end{subequations}


{\color{Orange}
Where $~\textrm{`}\sum_n\textrm{'}$ can also denote integration if summated index takes values from a continuous domain.
Let us consider our equations confined in a periodic box $L_x$, $L_y$ then not all values of $k$ are allowed. Both $\d\Psi_m$ and $\d C_m$ must obey the periodic boundary conditions. Therefore they must obey:
\begin{subequations}\begin{align}
\d\Psi_m(x+L_x,y,t)&=\d\Psi_m(x,y+L_y,t)=\d\Psi_m(x,y,t)~,\label{eq:dPsi_period}\\
\d C_m(x_\a+L_x,y_\a,x_\b,y_\b,t)&=\d C_m(x_\a,y_\a,x_\b+L_x,y_\b,t) = \d C_m(x_\a+L_x,y_\a+L_y,x_\b,y_\b,t) \nonumber\\
&\qquad\qquad\qquad= \d C_m(x_\a,y_\a,x_\b,y_\b+L_y,t)= \d C_m(x_\a,y_\a,x_\b,y_\b,t)~.\label{eq:dC_period}
\end{align}\end{subequations}
From Eq.~\eqref{eq:dPsi_period} we have that
\begin{subequations}\begin{align}
e^{\i m L_x} &= 1 \Rightarrow m\textrm{ is an integer multiple of }2\pi/L_x ~,\\
 e^{\i n L_y} &= 1 \Rightarrow n\textrm{ is an integer multiple of }2\pi/L_y ~.
\end{align}\end{subequations}
and from Eq.~\eqref{eq:dC_period} we have that
\begin{subequations}\begin{align}
e^{\i m L_x/2}e^{\i k L_x} &= 1 \Rightarrow (k+m/2)\textrm{ is an integer multiple of }2\pi/L_x \nonumber\\
&\quad\;\;\; \Rightarrow \left\{
	\begin{array}{ll}
		  k = \kappa(2\pi/L_x)~,~\kappa\in\mathbb{Z}  & \textrm{, for $m$ even~,} \\
		 \\
		  k = \dfrac{2\kappa+1}{2}\,(2\pi/L_x)~,~\kappa\in\mathbb{Z}  & \textrm{, for $m$ odd~.} \\
	\end{array}\right.
\end{align}\end{subequations}

For $L_x=L_y=2\pi$ we have that Eqs.~\eqref{eq:eig_dPsim_dCm} take the form:
\begin{subequations}\begin{align}
%\d S &= S_m(\xt,\yt,\yb)\,e^{\i m\xb} \\
%\nonumber\\
\d \Psi_m (x,y,t) &= e^{\i m x} e^{\s t}\sum_{n=-\infty}^{+\infty} a_n e^{\i n y}  ~,m\in\mathbb{Z}~,\label{eq:eig_dPsi_k}\\
\d C_m(x_\a,y_\a,x_\b,y_\b) &= e^{\i m(x_\a+x_\b)/2} \sum_{k=-\infty}^{+\infty} \d\hat{C}_{k,m} (y_\a,y_\b) e^{\i (k-m/2)(x_\a-x_\b)} ~,m\in\mathbb{Z} ~,\label{eq:eig_dCm_k}
\end{align}\label{eq:eig_dPsim_dCm}\end{subequations}
Notice that $\d\hat{C}_{k,m} (y_\a,y_\b)$ corresponds to $e^{\i(k-m/2)(x_\a-x_\b)}$ which is different for each choice of $m$. We could have defined $\d\hat{C}_{k,m} (y_\a,y_\b)$ to be the Fourier coefficient corresponding to $e^{\i(k+m/2)(x_\a-x_\b)}$ but we have made the first choice.
}


If we denote $\d \Psi_{mn} = e^{\i(m x+ny)}$ then this induces:
\be
\[\d U_{mn},\d V_{mn},\d Z_{mn},(\d Z_x)_{mn},(\d Z_y)_{mn}\bit\] = \[\bit-\i n,\i m,-(m^2+n^2),-\i m(m^2+n^2),-\i n(m^2+n^2)\]\d \Psi_{mn} (x,y,t)~,
\ee
and would correspond to $\[\d U_{m},\d V_{m},\d Z_{m},(\d Z_x)_{mn},(\d Z_y)_{mn}\bit\] = e^{\s t} \sum_n a_n \[\d U_{m},\d V_{m},\d Z_{m},(\d Z_x)_{mn},(\d Z_y)_{mn}\bit\]$.

The S3T equilibrium covariance can be written as:
\begin{subequations}\begin{align}
C^E(x_\a,y_\a,x_\b,y_\b) &= \sum_{k=-N_k}^{N_k}\hat{C}^E_{k}(y_\a,y_\b) e^{\i k(x_\a-x_\b)}  \\
&= \frac1{2}\real{ \[\sum_{k=1}^{N_k} \hat{C}^E_{k}(y_\a,y_\b) e^{\i k(x_\a-x_\b)} \]}%\\
%&= \frac1{2} \sum_{k=1}^{N_k} \left\{ \hat{C}^{E,R}_{k}(y_\a,y_\b) \cos{ \[k(x_\a-x_\b) \]}-\hat{C}^{E,I}_{k}(y_\a,y_\b) \sin{ \[k(x_\a-x_\b) \]} \right\}
\end{align}\end{subequations}

\vspace*{1cm}

\textbf{Notes}\\
1.~~The last equality holds only if $\hat{C}_{k=0}^E=0$, which is true if the forcing covariance has $\hat{Q}_{k=0}=0$ regardless if $U^E$ is zero or not.

2.~~Both $\d C_m$ and $C^E$ have the symmetry that they remain the same under $\x_\a\leftrightarrow\x_\b$.

\vspace*{1cm}

It will be useful to calculate some partial derivatives of $\d C_m$ and $C^E$.\begin{subequations}\begin{align}
\partial_{x_\a} \d C_m &= e^{\i m(x_\a+x_\b)/2}\sum_{k=-\infty}^{+\infty} \i k\, \d\hat{C}_{k,m}(y_\a,y_\b) \,e^{\i (k-m/2)(x_\a-x_\b)} ~,\\
\partial_{x_\b} \d C_m &= e^{\i m(x_\a+x_\b)/2}\sum_{k=-\infty}^{+\infty} -\i\(k-m\) \d\hat{C}_{k,m}(y_\a,y_\b) \,e^{\i (k-m/2)(x_\a-x_\b)} ~,\\
\Del_{\a} \d C_m &= e^{\i m(x_\a+x_\b)/2}\sum_{k=-\infty}^{+\infty} \[ \partial^2_{y_\a} - k^2 \bit\]\d\hat{C}_{k,m}(y_\a,y_\b) \,e^{\i (k-m/2)(x_\a-x_\b)} ~,\\
\Del_{\b} \d C_m &= e^{\i m(x_\a+x_\b)/2}\sum_{k=-\infty}^{+\infty} \[ \partial^2_{y_\b} - \(k-m\)^2 \]\d\hat{C}_{k,m}(y_\a,y_\b) \,e^{\i (k-m/2)(x_\a-x_\b)} ~.
\end{align}\end{subequations}

If the coherent streamfunction perturbation eigenfunction consists of only a single harmonic, $\d\Psi_{mn}$, after defining  $\d E_{n,a} =  e^{\i n y_\a}$, some terms of Eq.~\eqref{eq:pert_dC_s} read:
\begin{subequations}\begin{align}
 -(U^E_\a &\partial_{x_\a} +U^E_\b \partial_{x_\b}) \,\d C_m = \nonumber\\
 &=e^{\i m(x_\a+x_\b)/2}\sum_{k=-\infty}^{+\infty}  \[  -\i k U^E_\a\,\d\hat{C}_{k,m}(y_\a,y_\b) +  \i (k-m) U^E_\b\,\d\hat{C}_{k,m}(y_\a,y_\b) \]\,e^{\i (k-m/2)(x_\a-x_\b)} ~,\\
 -(\d U_\a &\partial_{x_\a} + \d U_\b \partial_{x_\b} )  C^E = \nonumber\\
 &=-\sum_{k=-\infty}^{+\infty} \[\d U_\a\, \i k \,\hat{C}^E_k(y_\a,y_\b) + \d U_\b \(-\i k\) \hat{C}^E_k(y_\a,y_\b) \] \,e^{\i k(x_\a-x_\b)}\nonumber\\
%  &=\i n \sum_{k}  \[ e^{\i m x_\a} e^{\i n y_\a}\, \i k\,  \hat{C}^E_k(y_\a,y_\b) + e^{\i m x_\b} e^{\i n y_\b} \(-\i k\) \hat{C}^E_k(y_\a,y_\b) \] e^{\i k(x_\a-x_\b)}~\nonumber\\
%  &=\i n\, e^{\i m(x_\a+x_\b)/2} \sum_{k}  \[ e^{\i m (x_\a-x_\b)/2} e^{\i n y_\a}\, \i k\,  \hat{C}^E_k(y_\a,y_\b) + e^{-\i m (x_\a-x_\b)/2} e^{\i n y_\b} \(-\i k\) \hat{C}^E_k(y_\a,y_\b) \] e^{\i k(x_\a-x_\b)}\nonumber\\
  &=\i n \, e^{\i m(x_\a+x_\b)/2} \sum_{k=-\infty}^{+\infty} \left\{  \vphantom{\frac1{2}} \[  \(\i k\,\d E_\a\)   \hat{C}^E_k(y_\a,y_\b) \] \,e^{\i (k+m/2) (x_\a-x_\b)} + \[   \hat{C}^E_k(y_\a,y_\b) \(-\i k\,\d E_\b\) \] \,e^{\i (k-m/2) (x_\a-x_\b)}\right\}~.\label{eq:dUadUbCE}
 \end{align}\end{subequations}


The term $e^{\i m(x_\a+x_\b)/2}$ factors out of all terms of Eq.~\eqref{eq:pert_syst_cont}. After redefining $k\to k'= k+m$ in terms like the first one in Eq.~\eqref{eq:dUadUbCE} we can rewrite Eq.~\eqref{eq:pert_syst_cont} as a system of matrix equations for the perturbation covariances matrices, $\d\C_{k,m}$, which are defined as $\[\d\C_{k,m}\]_{\a\b} =\d\hat{C}_{k,m}(y_\a,y_\b)$. These matrices satisfy:\begin{align}
\s\,\d \C_{k,m} &=  \A^{E,\textrm{L}}_{k}\,\d\C_{k,m} + \d\C_{k,m}\(\A^{E,\textrm{R}}_{k-m}\)^\transp + \sum_n a_n \[\vphantom{\frac1{2}}\d\A^{\rm L}_{k-m,m,n}\C^E_{k-m} + \C^E_{k}\(\d\A^{\rm R}_{k,m,n}\)^\transp\]
\label{eq:pert_dC_s_matr}\end{align}
with:\begin{subequations}\begin{align}
\A^{E,\textrm{L}}_{k} &= -\i k \U^E  -\i k \(\bit \beta -\U^E_{yy} \) \DDel^{-1}_{k}  - r - \nu_4  \DDel^2_{k}~,\\
\A^{E,\textrm{R}}_{k} &= +\i k\U^E  + \i k \(\bit \beta -\U^E_{yy} \) \DDel^{-1}_{k}  - r - \nu_4  \DDel^2_{k}~,\\
\d\A^{\textrm{L}}_{k,m,n} &= -\d\E_n\(+ nk\I+\i m \D_y\)\[\I+(m^2+n^2)\DDel^{-1}_k\]~,\\
\d\A^{\textrm{R}}_{k,m,n} &= -\d\E_n\(- nk\I+\i m \D_y\)\[\I+(m^2+n^2)\DDel^{-1}_k\]~,
\end{align}
\end{subequations}
Equation~\eqref{eq:pert_dC_s_matr} can be solved for $\d\C_{k,m}$ as a Sylvester equation and from $\d\C_{k,m}$ we get $\d C_m$ (Eq.~\eqref{eq:eig_dCm_k}).

\vspace*{2cm}
The following symmetries hold:
\begin{subequations}\begin{align}
\A^{E,\textrm{L}}_{-k} &= \A^{E,\textrm{R}}_{k}~,\\
\d\A^{\textrm{L}}_{-k,m,n} &= \d\A^{\textrm{R}}_{k,m,n} ~,\\
\d\A^{\textrm{L}}_{k,-m,n} &= -\d\A^{\textrm{R}}_{k,m,n} ~,\\
\end{align}
\end{subequations}
Also, because $\d\hat{C}$ and $C^E$ are symmetric in exchange $\x_\a\leftrightarrow\x_\b$ and furthermore $C^E$ is also real, we have that:
\bdm
\left.\begin{array}{ll}
	\C^{E}_{-k} &=\(\C^{E}_{k}\)^*~,\textrm{($C^E$ real)}\\
	\C^{E}_{-k} &=\(\C^{E}_{k}\)^\transp~,\textrm{($C^E$ symmetric)}
\end{array}\right\}\Rightarrow\nonumber\edm\begin{subequations}\begin{align}
\Rightarrow  \C^{E}_{k} &= \(\C^{E}_{k}\)^\dag~,\\
\d\C_{-k,m} &= \(\d\C_{k+m,m}\bit\)^\transp ~.\label{eq:symm_dCk}
\end{align}
If $\d\hat{C}$ is also real then Eq.~\eqref{eq:symm_dCk} becomes:
\be
\d\C_{-k,m} = \(\d\C_{k+m,m}\bit\)^\dag ~.\label{eq:symm_dCk_real}
\ee
\end{subequations}

In general, if $C^E$ has non-zero $\C_k$ for $k=0,\dots,N_k$ then for a fixed $m$ the $\d\C_{k,m}$ that would not be necessarily zero (since they will couple with at least one non-zero $\C^E_k$) will be the ones with $k=-(N_k+m),\dots,(N_k+m)$, which are a total of $2(N_k+m)+1$. However, one can only solve only for the first $N_k+2m$ perturbation covariances, $\d\C_{k,m}$, and deduce the rest $N_k+1$ using the symmetry of Eq.~\eqref{eq:symm_dCk}.

\vspace*{1cm}

\textbf{Note}: For $m=0$ perturbations, if $\C_{k=0}^E\ne0$ we can see that in principle we need to solve for $N_k+1$ perturbation covariances, $\d\C_{k,0}$, and not $N_k$ as it is claimed above. However, we can prove that $\d\C_{k=0,m=0}=0$, regardless if $\C_{k=0}^E\ne0$ and therefore one $N_k$ perturbation covariances are non-zero.

\vspace*{2cm}



The next step is to find the Reynolds stress divergence, $\d R_m$, that corresponds to $\d C_m$.
\begin{align}
\d R_m &= - \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_\a} \Del_\a^{-1}-\partial_{y_\b} \Del_\b^{-1}\) \d \hat{C} \right|_{\x_\a=\x_\b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_\a} \Del_\a^{-1}+\partial_{x_\b} \Del_\b^{-1}\) \d \hat{C} \right|_{\x_\a=\x_\b} \]
\end{align}

The term in the first brackets is $\d\<u'q'\>$, which reads:
\begin{align}
\d \<u'q'\> &=  \left. \bit \frac1{2}\(-\partial_{y_\a} \Del_\a^{-1}-\partial_{y_\b} \Del_\b^{-1}\) \d \hat{C} \right|_{\x_\a=\x_\b}  \nonumber\\
&=-\frac1{2}  \left. \bit \sum_{k=-\infty}^{+\infty} \(\partial_{y_\a} \Del_\a^{-1}+\partial_{y_\b} \Del_\b^{-1}\) e^{\i m(x_\a+x_\b)/2} \,\d\hat{C}_{k,m} (y_\a,y_\b) \,e^{\i (k-m/2)(x_\a-x_\b)} \right|_{\x_\a=\x_\b} \nonumber\\
\end{align}
Discretizing the $y$-domain and representing $\d \<u'q'\>$ as a column vector we get using the matrix representation for $\d\hat{C}_{k,m}$:
\begin{subequations}\begin{align}
\d \<\mathbf{uq}\> &=-\frac1{2}  \left. \bit e^{\i m(x_\a+x_\b)/2} \sum_{k=-\infty}^{+\infty} \[\D_y \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\(\D_y\)^\transp\]_{\a\b}  e^{\i (k-m/2)(x_\a-x_\b)} \right|_{\x_\a=\x_\b} \nonumber\\
&=-\frac1{2}   e^{\i m x} \vecd\[\sum_{k=-\infty}^{+\infty} \D_y \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\(\D_y\)^\transp\] ~,\label{eq:duqk}
\end{align}
and similarly for $\d\<v'q'\>$:
\begin{align}
\d \<\mathbf{vq}\> &=\frac1{2}  \left. \bit e^{\i m(x_\a+x_\b)/2} \sum_{k=-\infty}^{+\infty} \[ \i k \DDel^{-1}_{k}\, \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp \[-\i (k-m)\]\]_{\a\b}  e^{\i (k-m/2)(x_\a-x_\b)} \right|_{\x_\a=\x_\b} \nonumber\\
&=\frac1{2}   e^{\i m x} \vecd\[ \sum_{k=-\infty}^{+\infty}  \i k \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\[-\i (k-m)\]\]~.\label{eq:dvqk}
\end{align}


Therefore $\d\Rv_m$ will be given by:
\begin{align}
\d \Rv_m &= -\partial_x\d \<\mathbf{uq}\> - \D_y\d \<\mathbf{vq}\>\nonumber\\
&=\frac{1}{2}e^{\i m x}  \left\{ \i m \, \vecd\[ \sum_k \D_y \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\(\D_y\)^\transp\] + \dotsb\right.\nonumber\\
&\qquad\qquad\qquad\dotsb+\left. \D_y \vecd\[ \sum_k  \i k \DDel^{-1}_{k} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k-m}\)^\transp\[-\i (k-m)\]\] \right\}
\end{align}
\end{subequations}

The Reynolds stress divergence that correspond to $\d\C_{k,m,n}$ are denoted with $\d\Rv_{mn}$. In general, the Reynolds stress divergence $\d\Rv_{mn}$ will be proportional to $e^{\i m x}$, but due to the non-homogeneous terms in $y$, ($U^E$, $U^E_{yy}$), it will not also be proportional to $e^{\i ny}$. The last will only be true in the case of the homogeneous equilibrium.

\vspace{1cm}
\textbf{Note}: In Eq.~\eqref{eq:duqk} for $k=0$ or $k=m$ the operators $\DDel^{-1}_k$ or $\DDel^{-1}_{k-m}$ are ill-defined. For the specific terms we have that $-\D_y  \DDel^{-1}_k = -\D_y^{-1}$. We calculate $\D_y^{-1}$ as the pseudoinverse of $\D_y$ using SVD decomposition and removing the zero singular values of $\D_y$.

%
%Navid
%Nai niko
%kane ti douleia sou, den thelo kati
%apla itan na do ena ypologismo
%
%diabasa tin paragrafo
%eisai sigouros gia to oti o oros den paizei rolo ?
%
%to βsin pou einai stin coherent eksisosi den paizei rolo sto growth rate
%afto mporeis na to deis an pareis Re and Imaginary part tou slanted dispersion (nomizo)
%kai episis ekana ypologismous (exei kairo) stous opoious ebgala ton oro kai pira ta idia growth rates (alla me lathos sigma_i)
%
%mou kanei entyposi, giati eixa kanei ki ego palia kai eixa kataliksei se anti8eto symperasma
%
%tote tha to ksanakano na bebaiotho
%
%o oros sto aristero melos, den einai tipota allo para to Rossby wave speed
%kai gia megalo b konta sto criticality, ta non-zonals exoune sxedon ayto gia sigma_i
%
%Tora, mias kai to deksi melos einai en genei migadiko, ena diaforetiko sigma_i 8a epireasei kai to growth rate
%
%8a to ksanado ki ego
%
%gia mikro b exo kanei ypologismo gia to poso epireazoun oi oroi me to sin\theta
%apla tous exo sto panepistimio
%
%gia megalo b den eixa kataferei na bro apotelesma
%
%a ok, gia mikro beta to ekana ki ego
%gia isotropiko bgainei afto pou exete sto JAS alla me b->bsin
%
%ahoxi, 8ymamai eixe dyo orous bcos\theta kai bsint\heta
%ah, ennoeis to ekanes prin petakseis kanenan oro
%
%nai de 8ymamai akribos
%prepei na koitaksoi tis simeioseis
%
%to poiotiko epixeirima ksexnao to bsin\theta kai to allo b einai meiomeno kata cos\theta douleyei (to exo grapsei p.x sto xarti pou 8a paei sto biblio (einai sto book_paper with Nikos)
%
%ypo tin ennoia oti eksigei p.x giati ta non-zonals einai pio asta8i molis allazei i kampyli ec=f(b) apo f8inousa se ayksousa
%
%kai giati p.x ta non-zonals einai pio asta8i gia NIF kai b<<1 (o oros me to b einai stabilizing) <--- afto den katalavaino ti ennoeis
%
%
%ta fluxes einai uv= A -b^2B (gia mi isotropiko)
%epomenos einai ligotera me b 
%
%afou ta non-zonals "blepoun" mikrotero b, ta fluxes gia ayta 8a einai megalytera -> pio asta8i
%
%B>0 ?
%nai an 8ymamai kala, ektos kai an kano la8os
%katse na skefto
%
%
%ego to bgazo:
%
%\d\<v'\z'\> = \frac{\mu}{8} \frac{\df^2\d U}{\df y^2} + \[\frac{3}{128} \bt^2 (\mu +2)+\frac{\mu }{8}\] \frac{\df^4\d U}{\df y^4}~.
%(an den exo kanei lathos)
%(afto einai to delta<vq>)
%
%
%poso arnitiko einai to mu ?
%
%to -1<mu<1
%
%ara o oros me to b einai 8etikos
%nai ego etsi bgazo
%ok Navid 8a to ksanakoitakso
%8ymomoun oti einai arnitikos, alla 8a to ksanado
%ki ego epeidi i pithanotita na kano lathos einai megali
%
%ok
%katse na do ti kanei o ypologismos kai feygo
%
%
%afto pou les esy A_B bgainei arnitiko
%alla yparxei ena - mprosta apo afto
%
%kalinyxta
%kalinixta
%
%
%
%
%
%B = 3/128 b^2(mu+2)+mu/8
%
%to NIF einai mu<0
%gia b=0 einai arnitiko
%gia b>apo mia krisimi timi ginetai thetiko
%
%
%
%alla den ksero giati


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% these were the first tries which were eventually wrong since dC was not periodic in all its elements

%\begin{subequations}\begin{align}
%\partial_{x_\a} \d C_m &= e^{\i m(x_\a+x_\b)/2}\sum_{k=-N_k}^{N_k} \i\(k+\frac{m}{2}\) \d\hat{C}_{k,m}(y_\a,y_\b) \,e^{\i k(x_\a-x_\b)} ~,\\
%\partial_{x_\b} \d C_m &= e^{\i m(x_\a+x_\b)/2}\sum_{k=-N_k}^{N_k}-\i\(k-\frac{m}{2}\) \d\hat{C}_{k,m}(y_\a,y_\b) \,e^{\i k(x_\a-x_\b)} ~,\\
%\Del_{\a} \d C_m &= e^{\i m(x_\a+x_\b)/2}\sum_{k=-N_k}^{N_k} \[ \partial^2_{y_\a} - \(k+\frac{m}{2}\)^2 \]\d\hat{C}_{k,m}(y_\a,y_\b) \,e^{\i k(x_\a-x_\b)}~,\\
%\Del_{\b} \d C_m &= e^{\i m(x_\a+x_\b)/2}\sum_{k=-N_k}^{N_k} \[ \partial^2_{y_\b} - \(k-\frac{m}{2}\)^2 \]\d\hat{C}_{k,m}(y_\a,y_\b) \,e^{\i k(x_\a-x_\b)}~.
%\end{align}\end{subequations}\begin{subequations}\begin{align}
%\partial_{x_\a} C^E = \sum_{k=-N_k}^{N_k} \i k \, \hat{C}^E_k(y_\a,y_\b) \,e^{\i k(x_\a-x_\b)} ~~&,~~
%\partial_{x_\b} C^E = \sum_{k=-N_k}^{N_k} - \i k \, \hat{C}^E_k(y_\a,y_\b) \,e^{\i k(x_\a-x_\b)} ~,\\
%\Del_{\a} C^E = \sum_{k=-N_k}^{N_k} \(\partial^2_{y_\a}-k^2\) \hat{C}^E_k(y_\a,y_\b) \,e^{\i k(x_\a-x_\b)} ~~&,~~
%\Del_{\b} C^E = \sum_{k=-N_k}^{N_k} \(\partial^2_{y_\b}-k^2\) \hat{C}^E_k(y_\a,y_\b) \,e^{\i k(x_\a-x_\b)} ~,
%\end{align}\end{subequations}
%
%If the coherent streamfunction perturbation eigenfunction consists of only a single harmonic, $\d\Psi_{mn}$, after defining $k_{\pm} = k\pm m/2$ and $\d E_{n,a} =  e^{\i n y_\a}$, some terms of Eq.~\eqref{eq:pert_dC_s} read:
%\begin{subequations}\begin{align}
% -(U^E_\a &\partial_{x_\a} +U^E_\b \partial_{x_\b}) \,\d C_m = \nonumber\\
% &=e^{\i m(x_\a+x_\b)/2}\sum_{k=-N_k}^{N_k} \[  -\i k_+ U^E_\a\,\d\hat{C}_{k,m}(y_\a,y_\b) +  \i k_- U^E_\b\,\d\hat{C}_{k,m}(y_\a,y_\b) \]\,e^{\i k(x_\a-x_\b)} ~,\\
% -(\d U_\a &\partial_{x_\a} + \d U_\b \partial_{x_\b} )  C^E = \nonumber\\
% &=-\sum_{k=-N_k}^{N_k} \[\d U_\a\, \i k \,\hat{C}^E_k(y_\a,y_\b) + \d U_\b \(-\i k\) \hat{C}^E_k(y_\a,y_\b) \] \,e^{\i k(x_\a-x_\b)}\nonumber\\
%%  &=\i n \sum_{k}  \[ e^{\i m x_\a} e^{\i n y_\a}\, \i k\,  \hat{C}^E_k(y_\a,y_\b) + e^{\i m x_\b} e^{\i n y_\b} \(-\i k\) \hat{C}^E_k(y_\a,y_\b) \] e^{\i k(x_\a-x_\b)}~\nonumber\\
%%  &=\i n\, e^{\i m(x_\a+x_\b)/2} \sum_{k}  \[ e^{\i m (x_\a-x_\b)/2} e^{\i n y_\a}\, \i k\,  \hat{C}^E_k(y_\a,y_\b) + e^{-\i m (x_\a-x_\b)/2} e^{\i n y_\b} \(-\i k\) \hat{C}^E_k(y_\a,y_\b) \] e^{\i k(x_\a-x_\b)}\nonumber\\
%  &=\i n \, e^{\i m(x_\a+x_\b)/2} \sum_{k}\left\{  \vphantom{\frac1{2}} \[  \(\i k\,\d E_\a\)   \hat{C}^E_k(y_\a,y_\b) \] \,e^{\i k_+ (x_\a-x_\b)} + \[   \hat{C}^E_k(y_\a,y_\b) \(-\i k\,\d E_\b\) \] \,e^{\i k_- (x_\a-x_\b)}\right\}~.\label{eq:dUadUbCE}
% \end{align}\end{subequations}
%The term $e^{\i m(x_\a+x_\b)/2}$ factors out of all terms of Eq.~\eqref{eq:pert_syst_cont}, while in $(\d A_\a+\d A_\b)C^E$ the term $e^{\i k(x_a-x_b)}$ cannot be factored out.
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% these are totally wrong

{\color{Purple}
%For $k,k',m$ integers we have:
%\begin{align}
%\frac1{2\pi} \int_{0}^{2\pi} e^{-\i k' \xt } e^{\i (k+m/2)\xt}\,\df\xt &= \frac{e^{2\pi\i(k+m/2-k')}-1}{2\pi\i(k+m/2-k')} = \left\{
%	\begin{array}{ll}
%		 \d_{k,k'-m/2}  & \mbox{, if } m \textrm{ is even~,} \\
%		 \\
%		 \\
%		\dfrac1{\i \pi (k'-k-m/2)} & \mbox{, if } m \textrm{ is odd~.}
%	\end{array}
%\right.
%\end{align}
%%If $m$ is even, 
%%\be
%%\frac1{2\pi} \int_{0}^{2\pi} e^{-\i k' \xt } e^{\i (k+m/2)\xt}\,\df\xt = \d_{k,k'-m/2}
%%\ee
%%but in the case $m$ is odd then the numerator never vanishes and
%%\be
%%\frac1{2\pi} \int_{0}^{2\pi} e^{-\i k' \xt } e^{\i (k+m/2)\xt}\,\df\xt = \frac1{\i \pi (k'-k-m/2)}
%%\ee
%
%So, in the case $m$ is even, then by multiplying all terms all terms with $e^{-\i k' (x_\a-x_\b)} / (2\pi)$ and integrate over the whole domain we get Eq.~\eqref{eq:pert_dC_s_matr}. However, for $m$ odd we have that each $\d\hat{C}_{k,m}$ couples with all $\hat{C}^E_k$. For example, the term of Eq.~\eqref{eq:dUadUbCE} becomes:
%\begin{align}
%\s\,\d \hat{C}_{k,m} &=  \sum_n\, a_n\,\i n  \sum_{k'}\[  \vphantom{\frac1{2}} \frac{  \(\i k'\,\d E_\a\)   \hat{C}^E_{k'}(y_\a,y_\b) }{\i \pi (k-k'-m/2)} + \frac{ \hat{C}^E_{k'}(y_\a,y_\b) \(-\i k'\,\d E_\b\)  }{\i \pi (k-k'+m/2)} \]
%\end{align}
%Notice the summation over $k'$ for $\hat{C}^E_{k'}$. This equation can be written in matrix form:
%\begin{align}
%\s\,\d \C_{k,m} &= \sum_n\, a_n\, \i n   \sum_{k'}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \(\i k'\,\d \E_n\)   \C^E_{k'} }{k-k'-m/2} + \frac{ \C^E_{k'} \(-\i k'\,\d \E_n\)^\transp  }{k-k'+m/2} \]
%\end{align}
%
%
%We define $\d \C_{k,m,n}$ the solution of
%\begin{align}
%\(\A^{E,\textrm{L}}_{k,m}-\s\)\,\d\C_{k,m,n} + \d\C_{k,m,n}\(\A^{E,\textrm{R}}_{k,m}\)^\transp &+     \underbrace{\sum_{k'}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \d\A^{\textrm{L}}_{k',m,n}   \C^E_{k'} }{k-k'-m/2} + \frac{ \C^E_{k'} \(\d\A^{\textrm{R}}_{k',m,n}\)^\transp  }{k-k'+m/2} \]}_{\d\Q_{k,m,n}} =0~,\label{eq:dQkmn_def}
%\end{align}
%which consists of $\d\Psi_{mn}$ and we deduce therefore that $\d\C_{k,m}$ which solves the full
%\begin{align}
%\s\,\d \C_{k,m} &=\A^{E,\textrm{L}}_{k,m}\,\d\C_{k,m} + \d\C_{k,m}\(\A^{E,\textrm{R}}_{k,m}\)^\transp + \sum_n\, a_n\,    \sum_{k'}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \d\A^{\textrm{L}}_{k,m,n}   \C^E_{k'} }{k-k'-m/2} + \frac{ \C^E_{k'} \(\d\A^{\textrm{R}}_{k,m,n}\)^\transp  }{k-k'+m/2} \]
%\end{align}
%will be given as $\d\C_{k,m} = \sum_n  a_n\,\d\C_{k,m,n}$.
%
%
%In Eq.~\eqref{eq:dQkmn_def} the $\d\Q_{k,m,n}$ is defined with respect of the $\C_k^E$ matrices as:
%\be
%\d\Q_{k,m,n}=\sum_{k'=-N_k}^{N_k}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \d\A^{\textrm{L}}_{k,m,n}   \C^E_{k'} }{k-k'-m/2} + \frac{ \C^E_{k'} \(\d\A^{\textrm{R}}_{k,m,n}\)^\transp  }{k-k'+m/2} \]
%\ee
%Using the fact that $C^E$ is real and also symmetric in exchange $\x_\a\leftrightarrow\x_\b$ we have that $\C^{E}_{-k} = \(\C^E_k\)^\transp$. Also $ \d\A^{\textrm{L}}_{-k,m,n}= \d\A^{\textrm{R}}_{k,m,n}$ and $ \d\A^{\textrm{R}}_{-k,m,n}= \d\A^{\textrm{L}}_{k,m,n}$. Therefore $\d\Q_{k,m,n}$ becomes:
%\be
%\d\Q_{k,m,n}=\sum_{k'=1}^{N_k}\frac1{\i\pi}\[  \vphantom{\frac1{2}} \frac{  \d\A^{\textrm{L}}_{k,m,n}   \C^E_{k'} }{k-k'-m/2}+ \frac{  \d\A^{\textrm{R}}_{k',m,n}  \( \C^E_{k'} \)^\transp}{k+k'-m/2} + \frac{ \C^E_{k'} \(\d\A^{\textrm{R}}_{k,m,n}\)^\transp  }{k-k'+m/2} + \frac{  \( \C^E_{k'} \)^\transp\(\d\A^{\textrm{L}}_{k',m,n}\)^\transp  }{k'+k+m/2} \]
%\ee
%

%For example:
%\begin{align}
%\d C_m(x_\a,y_\a,x_\b,y_\b) &= e^{\i m(x_\a+x_\b)/2} \sum_{k=-N_k}^{N_k} \d\hat{C}_{k,m} (y_\a,y_\b) e^{\i k(x_\a-x_\b)} \nonumber\\
% &= e^{\i m(x_\a+x_\b)/2} \sum_{k=1}^{N_k} \[\d\hat{C}_{k,m} (y_\a,y_\b) e^{\i k(x_\a-x_\b)}+\d\hat{C}_{-k,m} (y_\a,y_\b) e^{-\i k(x_\a-x_\b)}\] ~.
%  \end{align}
%Since $\d C_m$ is symmetric to $\x_\a\leftrightarrow\x_\b$ we have that $\d\hat{C}_{-k,m} (y_\a,y_\b)=\d\hat{C}_{k,m} (y_\b,y_\a)$.
%\begin{align}
%\d C_m(x_\a,y_\a,x_\b,y_\b) &= e^{\i m(x_\a+x_\b)/2} \sum_{k=1}^{N_k} \[\d\hat{C}_{k,m} (y_\a,y_\b) e^{\i k(x_\a-x_\b)}+\d\hat{C}_{k,m} (y_\b,y_\a) e^{-\i k(x_\a-x_\b)}\] ~,\\
%C^E(x_\a,y_\a,x_\b,y_\b) &= \sum_{k=1}^{N_k} \[\hat{C}^E_{k}(y_\a,y_\b) e^{\i k(x_\a-x_\b)}+\hat{C}^E_{k}(y_\b,y_\a) e^{-\i k(x_\a-x_\b)}\] ~.
%  \end{align}
%  
%
%
%
%
%\begin{subequations}\begin{align}
% -(U^E_\a &\partial_{x_\a} +U^E_\b \partial_{x_\b}) \,\d C_m = \nonumber\\
% &=e^{\i m(x_\a+x_\b)/2} \sum_{k=-N_k}^{N_k} \[  -\i k_+ U^E_\a\,\d\hat{C}_{k,m}(y_\a,y_\b) +  \i k_- U^E_\b\,\d\hat{C}_{k,m}(y_\a,y_\b) \]e^{\i k(x_\a-x_\b)} ~,\\
% &=e^{\i m(x_\a+x_\b)/2}\sum_{k=1}^{N_k} \[\(-\i k_+\) U^E_\a \d\hat{C}_{k,m} (y_\a,y_\b) e^{\i k(x_\a-x_\b)}+\(-\i k_-\) U^E_\a\d\hat{C}_{k,m} (y_\b,y_\a) e^{-\i k(x_\a-x_\b)}+\dotsb\right.\nonumber\\
% &\qquad\qquad\qquad\qquad\qquad\dotsb+\left. \(\i k_-\) U^E_\b \d\hat{C}_{k,m} (y_\a,y_\b) e^{\i k(x_\a-x_\b)}+\(\i k_+\) U^E_\b\d\hat{C}_{k,m} (y_\b,y_\a) e^{-\i k(x_\a-x_\b)}\]  ~.
% \end{align}\end{subequations}
%
%
%\begin{subequations}\begin{align}
% -(\d U_\a &\partial_{x_\a} + \d U_\b \partial_{x_\b} )  C^E =\nonumber\\
% &=  -(\d U_\a \partial_{x_\a} + \d U_\b \partial_{x_\b} )\sum_{k=1}^{N_k} \[\hat{C}^E_{k}(y_\a,y_\b) e^{\i k(x_\a-x_\b)}+\hat{C}^E_{k}(y_\b,y_\a) e^{-\i k(x_\a-x_\b)}\]\nonumber\\
% &=\sum_{k} \[\(-\i k\)\,\d U_\a\,\hat{C}^E_k(y_\a,y_\b) e^{\i k(x_\a-x_\b)}+\(+\i k\)\,\d U_\a\,\hat{C}^E_k(y_\b,y_\a) e^{-\i k(x_\a-x_\b)}+\dotsb\right.\nonumber\\
% &\qquad\qquad\qquad\qquad\qquad\left.\dotsb+  \d U_\b \(-\i k\) \hat{C}^E_k(y_\a,y_\b) e^{-\i k(x_\a-x_\b)}+  \d U_\b \(+\i k\) \hat{C}^E_k(y_\a,y_\b) e^{\i k(x_\a-x_\b)}\] \nonumber\\
% &=e^{\i m(x_\a+x_\b)/2}\sum_{k} \[\(-\i k\)\,\(-\i n\)\d E_\a\,\hat{C}^E_k(y_\a,y_\b) e^{\i k_+(x_\a-x_\b)}+\(+\i k\)\,\(-\i n\)\d E_\a\,\hat{C}^E_k(y_\b,y_\a) e^{-\i k_-(x_\a-x_\b)}+\dotsb\right.\nonumber\\
% &\qquad\qquad\qquad\qquad\qquad\left.\dotsb+  \(-\i k\)\(-\i n\)\d E_\b  \hat{C}^E_k(y_\a,y_\b) e^{-\i k_+(x_\a-x_\b)}+  \(+\i k\)\(-\i n\)\d E_\b  \hat{C}^E_k(y_\a,y_\b) e^{\i k_-(x_\a-x_\b)}\] ~.
%  \end{align}\end{subequations}

}




%
%
%
%\subsection{Case with $m$ is even}
%
%
%After summing up for all $n$ to get the $\d A_{\a,\b}$ for the $\d\Psi_m$ (Eq.~\eqref{eq:eig_dPsi}) and also after denoting $\[\d\Ev_n\]_\a = e^{\i n y_\a}$, $\d\E_n = \diag\(\d\Ev_n\)$ the perturbation covariance perturbation (Eq.~\eqref{eq:pert_dC_s} becomes the matrix equation:
%%\begin{subequations}\begin{align}
%% -(U^E_a &\partial_{x_\a} +U^E_a \partial_{x_\a}) \d C_m =e^{\i m(x_\a+x_\b)/2}\sum_k \[ \(-\i k_+ \U^E\) \,\d\C_{k,m} +    \d\C_{k,m}\(\i  k_-\U^E\)^\transp \]_{\a\b}e^{\i k(x_\a-x_\b)} \\
%% -(\d U_\a &\partial_{x_\a} + \d U_\b \partial_{x_\b} )  C^E = \nonumber\\
%%& =\i n \, e^{\i m(x_\a+x_\b)/2}\sum_{k} \[  \(\i k\, \d\E_n\)   \C^E_k \]_{\a\b} e^{\i k_+ (x_\a-x_\b)} + \[ \C^E_k  \(-\i k\, \d\E_n\)^\transp \]_{\a\b} e^{\i k_-(x_\a-x_\b)}
%% \end{align}\end{subequations}
%\begin{align}
%\s\,\d\C_{k,m} &=  \A^{E,\textrm{L}}_{k,m}\,\d\C_{k,m} + \d\C_{k,m}\(\A^{E,\textrm{R}}_{k,m}\)^\transp + \sum_n a_n \[\vphantom{\frac1{2}}\d\A^{\rm L}_{k-m/2,m,n}\C^E_{k-m/2} + \C^E_{k+m/2}\(\d\A^{\rm R}_{k+m/2,m,n}\)^\transp\]
%\label{eq:pert_dC_s_matr}\end{align}
%with:
%\begin{subequations}\begin{align}
%\A^{E,\textrm{L}}_{k,m} &= -\i(k+m/2) \U^E  -\i(k +m/2) \(\bit \beta -\U^E_{yy} \) \DDel^{-1}_{k,+}  - r - \nu_4  \DDel^2_{k,+}~,\\
%\A^{E,\textrm{R}}_{k,m} &= +\i(k- m/2) \U^E  + \i(k- m/2) \(\bit \beta -\U^E_{yy} \) \DDel^{-1}_{k,-}  - r - \nu_4  \DDel^2_{k,-}~,\\
%\d\A^{\textrm{L}}_{k,m,n} &= -\d\E_n\(+ nk\I+\i m \D_y\)\[\I+(m^2+n^2)\DDel^{-1}_k\]~,\\
%\d\A^{\textrm{R}}_{k,m,n} &= -\d\E_n\(- nk\I+\i m \D_y\)\[\I+(m^2+n^2)\DDel^{-1}_k\]~,
%\end{align}
%and
%\begin{align}
%\DDel_{k,\pm }\equiv\DDel_{k\pm m/2} = \D^2 -\(k\pm m/2\)^2\I ~,
%\end{align}
%\end{subequations}
%Equation~\eqref{eq:pert_dC_s_matr} can be solved for $\d\C_{k,m}$ as a Sylvester equation and from $\d\C_{k,m}$ we get $\d C_m$ (Eq.~\eqref{eq:eig_dCm}).
%
%Note:
%If we denote with $\d\C_{k,m,n}$ the solution of:
%\be
%\s\,\d\C_{k,m,n} =  \A^{E,\textrm{L}}_{k,m}\,\d\C_{k,m,n} + \d\C_{k,m,n}\(\A^{E,\textrm{R}}_{k,m}\)^\transp +  \d\A^{\rm L}_{k-m/2,m,n}\C^E_{k-m/2} + \C^E_{k+m/2}\(\d\A^{\rm R}_{k+m/2,m,n}\)^\transp~.\label{eq:eig_dCkmn}
%\ee
%then $\d\C_{k,m} = \sum_n a_n \d\C_{k,m,n}$. 
%
%
%The next step is to find the Reynolds stress divergence, $\d R_m$, that corresponds to $\d C_m$.
%\begin{align}
%\d R_m &= - \partial_x \[\left. \bit \frac1{2}\(-\partial_{y_\a} \Del_\a^{-1}-\partial_{y_\b} \Del_\b^{-1}\) \d \hat{C} \right|_{\x_\a=\x_\b} \] - \partial_y \[\left. \bit \frac1{2}\(\partial_{x_\a} \Del_\a^{-1}+\partial_{x_\b} \Del_\b^{-1}\) \d \hat{C} \right|_{\x_\a=\x_\b} \]
%\end{align}
%
%The term in the first brackets is $\d\<u'q'\>$, which reads:
%\begin{align}
%\d \<u'q'\> &=  \left. \bit \frac1{2}\(-\partial_{y_\a} \Del_\a^{-1}-\partial_{y_\b} \Del_\b^{-1}\) \d \hat{C} \right|_{\x_\a=\x_\b}  \nonumber\\
%&=-\frac1{2}  \left. \bit e^{\i m(x_\a+x_\b)/2} \sum_k \(\partial_{y_\a} \Del_\a^{-1}+\partial_{y_\b} \Del_\b^{-1}\) \d\hat{C}_{k,m} (y_\a,y_\b) \,e^{\i k(x_\a-x_\b)} \right|_{\x_\a=\x_\b} \nonumber\\
%\end{align}
%Discretizing the $y$-domain and representing $\d \<u'q'\>$ as a column vector we get using the matrix representation for $\d\hat{C}_{k,m}$:
%\begin{align}
%\d \<\mathbf{uq}\> &=-\frac1{2}  \left. \bit e^{\i m(x_\a+x_\b)/2} \sum_k \[\D_y \DDel^{-1}_{k,+} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp\(\D_y\)^\transp\]_{\a\b}  e^{\i k(x_\a-x_\b)} \right|_{\x_\a=\x_\b} \nonumber\\
%&=-\frac1{2}   e^{\i m x} \vecd\[\sum_k \D_y \DDel^{-1}_{k,+} \,\d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp\(\D_y\)^\transp\] \nonumber\\
%\end{align}
%and similarly for $\d\<v'q'\>$:
%\begin{align}
%\d \<\mathbf{vq}\> &=\frac1{2}  \left. \bit e^{\i m(x_\a+x_\b)/2} \sum_k \[ \i k_+ \DDel^{-1}_{k,+}\, \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp \(-\i k_-\)\]_{\a\b}  e^{\i k(x_\a-x_\b)} \right|_{\x_\a=\x_\b} \nonumber\\
%&=\frac1{2}   e^{\i m x} \vecd\[ \sum_k \i k_+ \DDel^{-1}_{k,+}\, \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp \(-\i k_-\)\] \nonumber\\
%\end{align}
%
%Therefore $\d\Rv_m$ will be given by:
%\begin{align}
%\d \Rv_m &= -\partial_x\d \<\mathbf{uq}\> - \D_y\d \<\mathbf{vq}\>\nonumber\\
%&=\frac{1}{2}e^{\i m x}  \left\{ \i m \, \vecd\[ \sum_k \D_y \DDel^{-1}_{k,+}\, \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp\(\D_y\)^\transp\] + \dotsb\right.\nonumber\\
%&\qquad\qquad\qquad\dotsb+\left. \D_y \vecd\[ \sum_k  \i k_+ \DDel^{-1}_{k,+} \d\C_{k,m} + \d\C_{k,m} \(\DDel^{-1}_{k,-}\)^\transp \(-\i k_-\)\] \right\}
%\end{align}
%
%The Reynolds stress divergence that correspond to $\d\C_{k,m,n}$ are denoted with $\d\Rv_{mn}$. In general, due to the non-homogeneous terms in $y$, ($U^E$, $U^E_{yy}$), the Reynolds stress divergence $\d\Rv_{mn}$ will be proportional to $e^{\i m x}$ but not also  to $e^{\i ny}$. This will only be true in the case of the homogeneous equilibrium.
%
%\subsection{Case with $m$ is odd}
%Now we have
%
%\begin{align}
%\s\,\d\C_{k,m} &=  \A^{E,\textrm{L}}_{k,m}\,\d\C_{k,m} + \d\C_{k,m}\(\A^{E,\textrm{R}}_{k,m}\)^\transp + \sum_n a_n \sum_{k'} \frac1{\i\pi} \[\frac{\d\A^{\rm L}_{k',m,n}\,\C^E_{k'}}{k'-k+m/2} + \frac{\C^E_{k'}\(\d\A^{\rm R}_{k',m,n} \)^\transp}{k'-k-m/2}\]
%\label{eq:pert_dC_s_matr}\end{align}


\subsection{Corrolaries}

\subsubsection{For every equilibrium $(U^E,V^E,C^E)$ the perturbation covariance that corresponds to $m=0$ has $\d\hat{C}_{k=0,m=0}=0$}

Proof: For $m=0$, $k=0$ we have that $\d\A^{\textrm{L}}_{0,0,n} = \d\A^{\textrm{R}}_{0,0,n}=0$, therefore the perturbation covariance $\d\hat{C}_{k=0,m=0}=0$ satisfies:
\be
\(\A^{E,\textrm{L}}_{0,0}-\s\I\)\,\d\C_{0,0} + \d\C_{0,0}\(\A^{E,\textrm{R}}_{0,0}\)^\transp=0 ~,\label{eq:dC00}
\ee
with
\begin{align}
\A^{E,\textrm{L}}_{0,0} &= \A^{E,\textrm{R}}_{0,0} =\(\A^{E,\textrm{R}}_{0,0}\)^\transp \equiv \A^{E}_{0,0}=   - r - \nu_4  \D_y^4~.
\end{align}
The Sylvester equation \eqref{eq:dC00} has a unique solution unless one of the eigenvalues of $\A^{E}_{0,0}-\s\I$ is equal to an eigenvalue of $-\A^{E}_{0,0}$. This happens only for $\s=-2r-\nu_4(m^4+n^4)$, for $m,n$ integers. Otherwise, the only solution is $\d\C_{0,0}=0$.


\vspace{2cm}

In order to solve the eigenproblem of a jet equilibrium we proceed as follows: We suppose a $\d\Psi_{m} = e^{\s t}e^{\i mx}\,\sum_n a_n \d \Psi_{mn}$ for some coefficients $a_n$ and choose a first guess for $\s$. For this given $\s$ we solve Eqs.~\eqref{eq:pert_dC_s_matr} and find all $\d\C_{k,m,n}$ and from that we find the corresponding $\d \hat{R}_{mn}$. We factor the $e^{\i m x}$ dependance out and expand $\d \Rv_{mn}$ in Fourier series in $y$:
\be
\d \hat{R}_{mn} = e^{\i m x}\,\sum_{n'} B^{(m)}_{n'n}\,e^{\i n' y}~.
\ee
Then we go to the perturbation equation for the coherent structure, which for a jet equilibrium takes the form:
\begin{align}
&\sum_n\,a_n\,\[ \s+r+\nu_4\Del^2 + \i m U^E -\frac{\i m}{m^2+n^2} \(\b-U^E_{yy}\) \]  [-(m^2+n^2)]\,\d\Psi_{mn} =   e^{\i m x}\sum_n a_n \(\sum_{n'} B^{(m)}_{n'n}\,e^{\i n' y}\)\nonumber\\
\end{align}
 The term, $e^{\i m x}$ factors out.


\begin{align}
&\sum_n\,-a_n\,(m^2+n^2)\[ \s+r+\nu_4(\partial_y^2-m^2)^2 + \i m U^E -\frac{\i m}{m^2+n^2} \(\b-U^E_{yy}\) \]  \,e^{\i n y} =   \sum_n a_n \(\sum_{n'} B^{(m)}_{n'n}\,e^{\i n' y}\)\nonumber\\
\end{align}


If this was a homogeneous equilibrium ($U^E=V^E=0$) then $B^{(m)}_{n'n} = b^{(m)}_n\,\d_{n'n}$ and the above equation simplifies to:\begin{subequations}
\begin{align}
\sum_{n,n'}\,a_n\, \[ \( \s+r+\nu_4(m^2+n^2)^2 -\frac{\i m\b}{m^2+n^2}  \)  (m^2+n^2)\,\d_{n'n}+ B^{(m)}_{n'n} \]\,e^{\i n' y} &=0~~\Leftrightarrow\label{eq:disp_s_nz_nn'}\\
\sum_n\,a_n\, \[ \( \s+r+\nu_4(m^2+n^2)^2 -\frac{\i m\b}{m^2+n^2}  \)  (m^2+n^2)+ b^{(m)}_{n} \]\,e^{\i n y}&=0~.\label{eq:disp_s_nz_n}
\end{align}
\end{subequations}
Since $e^{\i n y}$ are linearly independent Eq.~\eqref{eq:disp_s_nz_n} can be satisfied for a single $n=n_0$ and all other $a_n$ be set to zero, that is $a_{n_0}=1$ and $a_n=0$ for $n\ne n_0$. Another way to look at this is to notice that Eq.~\eqref{eq:disp_s_nz_nn'} again using the fact that $e^{\i n y}$ are linearly independent can be rewritten as:
\be
\sum_{n}\[-\frac{B^{(m)}_{n'n}}{m^2+n^2}  -\(r+\nu_4(m^2+n^2)^2 -\frac{\i m\b}{m^2+n^2}  \) \,\d_{n'n}\]\,a_n =\s\,\,a_n~~\Leftrightarrow\label{eq:disp_s_nz_eigen}\\
\ee
or in matrix form:
\be
\L^{(m)}\,\av = \s\,\av
\ee
where $\L^{m}$ is the matrix with elements:
\be
 L^{(m)}_{n'n} =-\frac{ B^{(m)}_{n'n} }{m^2+n^2} -\[r+\nu_4(m^2+n^2)^2 -\frac{\i m\b}{m^2+n^2}  \]  \d_{n'n}~.
\ee
and $\av$ is the vector with elements $[\av]_n=a_n$.
Since for the homogeneous equilibrium $B^{(m)}_{nn'} = b^{(m)}_n\,\d_{nn'}$, the matrix $\L^{(m)}$ is diagonal so its eigenvectors are the standard orthonormal basis, $\e_j$, with elements: $[\e_j]_{m} = \d_{jm}$.

\vspace{2cm}
For the jet equilibrium we can expand $U^E = \sum_p\hat{U}^E_p\,e^{\i p y}$. Neglecting $\nu_4$ we have:
\begin{align}
&\sum_n\,a_n\,\( \s+r  -\frac{\i m\b}{m^2+n^2}\)   (m^2+n^2)\,e^{\i n y} + \sum_{n,p} a_n\,\i m\hat{U}_p^E\( m^2+n^2-p^2 \)  \,e^{\i(n+p)y} + \sum_{n,n'} a_n \, B^{(m)}_{n'n}\,e^{\i n'y}=0
\end{align}
By changing summation variables $p\to q=p+n$ in the second sum and $n'\to q$ in the third sum, the above expression can be written:

\begin{align}
&\sum_{n,q}\,a_n\,\( \s+r  -\frac{\i m\b}{m^2+n^2}\)   (m^2+n^2)\,\d_{n,q} + \sum_{n,q} a_n\,\i m\hat{U}_{q-n}^E\[ m^2+n^2-(q-n)^2 \bit\]  + \sum_{n,q} a_n \, B^{(m)}_{q,n}=0\nonumber\\
&\sum_{n,q}\,a_n\,\left\{ \( \s+r  -\frac{\i m\b}{m^2+n^2}\)  \,\d_{n,q} + \i m\,\hat{U}_{q-n}^E\[ 1-\frac{(q-n)^2}{m^2+n^2} \]   +  \frac{B^{(m)}_{q,n}}{m^2+n^2} \right\} e^{\i q y}=0\nonumber\\
&\sum_n\,a_n\,\left\{ \( \s+r  -\frac{\i m\b}{m^2+n^2}\)  \,\d_{n,q} + \i m\,\hat{U}_{q-n}^E\[ 1-\frac{(q-n)^2}{m^2+n^2} \]   +  \frac{B^{(m)}_{q,n}}{m^2+n^2} \right\}=0\nonumber\\
&\sum_n\,a_n\,\left\{ -\( r  -\frac{\i m\b}{m^2+n^2}\)  \,\d_{n,q} - \i m\hat{U}_{q-n}^E\[ 1-\frac{(q-n)^2}{m^2+n^2} \]   - \frac{B^{(m)}_{q,n}}{m^2+n^2}\right\}=\s\,a_q~,
\end{align}
or else as
\be
\L^{(m,{U^E})}\,\av = \s\,\av
\ee
with $\L^{(m,{U^E})}$ the matrix with elements:
\be
\[\L^{(m,{U^E})}\]_{qn} = -\frac{B^{(m)}_{q,n}}{m^2+n^2} -\( r  -\frac{\i m\b}{m^2+n^2}\)  \,\d_{n,q} - \i m\hat{U}_{q-n}^E\[ 1-\frac{(q-n)^2}{m^2+n^2} \] ~.
\ee


\newpage
\subsection{Centroid-difference coordinates}

We write this system in centroid-difference coordinates, $\mathbf{\bar{x}}=(\mathbf{x}_\a+\mathbf{x}_\b)/2$, $\mathbf{\tilde{x}}=\mathbf{x}_\a-\mathbf{x}_\b$. This gives:\begin{subequations}
\begin{align}
x_\a = \xb + \frac1{2}\xt ~~,~~x_\b = \xb - \frac1{2}\yt ~,\\
y_\a = \yb + \frac1{2}\yt ~~,~~y_\b = \yb - \frac1{2}\yt ~,
\end{align}\end{subequations}
and the derivatives transform to:\begin{subequations}
\begin{align}
\partial_{x_\a} = \frac1{2}\partial_{\xb} + \partial_{\xt} ~~&,~~ \partial_{x_\b} = \frac1{2}\partial_{\xb} - \partial_{\xt} ~,\\
\partial_{y_\a} = \frac1{2}\partial_{\yb} + \partial_{\yt} ~~&,~~ \partial_{y_\b} = \frac1{2}\partial_{\yb} - \partial_{\yt}  ~,\\
\Del_\a   = \Delt +\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\) +  \frac1{4}\Delb~~&,~~ \Del_\b   = \Delt -\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\) +  \frac1{4}\Delb~,\\
\Del_\a\Del_\b   = \( \Delt+\frac1{4}\Delb\)^2 & - \(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)^2~,\\
\partial_{x_\a} \Del_\b + \partial_{x_\b} \Del_\a   = \partial_{\xb}&\( \Delt+\frac1{4}\Delb\) - 2\partial_{\xt}\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)~,\\
\partial_{y_\a} \Del_\b + \partial_{y_\b} \Del_\a   = \partial_{\yb}&\( \Delt+\frac1{4}\Delb\) - 2\partial_{\yt}\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)~.
\end{align}

%\begin{subequations}
%\begin{align}
%-U^E_\a \partial_{x_\a} -U^E_\b \partial_{x_\b} & = -\Ub^E \partial_{\xb}-\Ut^E \partial_{\xt} ~,\\
%-U^E_\a \partial_{x_\a} \Del_\b -U^E_\b \partial_{x_\b} \Del_\a & = -\(\Ub^E\partial_{\xb} + \Ut^E\partial_{\xt}\)\(\Del+\frac1{4}\Delb\) + 2\(\Ub^E\partial_{\xt} + \frac1{4} \Ut^E\partial_{\xb}\)\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\) ~,\\
%U_{y_\a y_\a}^E \partial_{x_\a} \Del_\b + U_{y_\b y_\b}^E \partial_{x_\b} \Del_\a & = \(\Ub''^E\partial_{\xb} + \Ut''^E\partial_{\xt}\)\(\Del+\frac1{4}\Delb\) - 2\(\Ub''^E\partial_{\xt} + \frac1{4} \Ut''^E\partial_{\xb}\)\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\) ~,\\
%-\d U_\a \partial_{x\a} \Del_\b -\d U_\b \partial_{x_\b} \Del_\a &=
%\end{align}\end{subequations}


In general, we also have the following transformations of various quantities:
\begin{align}
\Phi_\a \partial_{x_\a} +\Phi_\b \partial_{x_\b} & = \Phib\, \partial_{\xb}+\Phit\, \partial_{\xt} ~~,~~ \Phi_\a \partial_{y_\a} +\Phi_\b \partial_{y_\b}  = \Phib\, \partial_{\yb}+\Phit\, \partial_{\yt} ~,\\
\Phi_\a \partial_{x_\a} \Del_\b +\Phi_\b \partial_{x_\b} \Del_\a &=\(\Phib\,\partial_{\xb} + \Phit\,\partial_{\xt}\)\(\Del+\frac1{4}\Delb\) - 2\(\Phib\,\partial_{\xt} + \frac1{4} \Phit\,\partial_{\xb}\)\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)~,\\
\Phi_\a \partial_{y_\a} \Del_\b +\Phi_\b \partial_{y_\b} \Del_\a &=\(\Phib\,\partial_{\yb} + \Phit\,\partial_{\yt}\)\(\Del+\frac1{4}\Delb\) - 2\(\Phib\,\partial_{\yt} + \frac1{4} \Phit\,\partial_{\yb}\)\(\bit\partial_{\xb\xt}+\partial_{\yb\yt}\)~,
\end{align}\end{subequations}
where we have defined: $\Phib = (\Phi_\a+\Phi_\b)/2$ and $\Phit = \Phi_\a-\Phi_\b$.




\subsection{Homogeneous equilibrium}

For the homogeneous equilibrium Eqs.~\eqref{eq:pert_S3Tgen} take the form:\begin{subequations}
\begin{align}
&\( \bit \s + r + \nu_4 \DDel^2   +\beta \,\D_x \DDel^{-1} \)\d \Zv  =  \d\Rv \label{eq:dZ}\\
&\(\A^E-\sigma\) \d\C+ \d\C\,\(\A^E\)^\transp + \d\A\,\C^E +\C^E\,\(\d\A\)^\transp = 0 ~. \label{eq:dC}
\end{align}\label{eqs:pert_hom}\end{subequations}
where we have defined the Reynolds stress divergence $\d\Rv= - \D_x \[\bit \vecd{\( - \D_y \DDel^{-1}\d\C\)}\] - \D_y \[\bit\vecd{\( \D_x \DDel^{-1}\d\C\)}\]$. The equilibrium operator is $\A^E = - \beta \,\D_x \DDel^{-1}-r -\nu_4 \DDel^2$ and
\be
\d\A = -\d\U\,\D_x-\d\V\,\D_y - \d\Z_y\,\D_x\DDel^{-1}+ \d\Z_x\,\D_y\DDel^{-1}~.
\ee
The eigenfunctions of this system are harmonics, $e^{\i(mx+ny)}$.

We assume $\d\Zv_{m,n} = e^{\i(mx+ny)}$ and a corresponding eigenvalue $\s_{m,n}$. We calculate $\d\C_{m,n}$ from Eq.~\eqref{eq:dC} and from that the corresponding Reynolds stress divergence, $\d\Rv_{m,n}$, that corresponds to the $(\d\Zv_{m,n},\s_{m,n})$. We expand the $\d\Rv_{m,n}$ as:
\be
\d\Rv_{m,n} = \sum_{m',n'}  \hat{\R}_{mnm'n'}\,e^{\i(m'x+n'y)}~.
\ee
It can be proven that $\d\Rv_{mn}$ will be proportional to $\d\Z_{mn}$, that is: $\hat{\Rv}_{mnm'n'}=r_{mn}\d_{mm'}\d_{nn'}$ (with $r_{mn}$ in general complex). This way Eq.~\eqref{eq:dZ} is written:
\be
 \( \bit \s + r + \nu_4 (m^2+n^2)^2   -\frac{\i m\beta }{m^2+n^2} - r_{mn}\) \,e^{\i(mx+ny)}  = 0\\
\ee
So our new guess for the eigenvalue, $\s'$ is:
\be
\s' = -r +\frac{\i m\beta }{m^2+n^2} + r_{mn}~.
\ee
We continue this iteration until convergence, that is until $|\s'-\s|\big/|\s'|<\tol$.

\vspace{2cm}

This method works very well in reproducing the results of the non-zonal dispersion relation for every choice of $(m,n)$ and it converges to the unstable eigenvalue even if our initial guess is very far away from that.

%Let us define a ``symbolic'' index $P$ for $m,n$ and $Q$ for $m',n'$ then the above is written: 
%\begin{align}
%\sum_{Q} \[ \( \bit \s + r + \nu_4 (m^2+n^2)^2   -\,\frac{\i m\beta }{m^2+n^2}\)\d_{P,Q} - \r_P \d_{P,Q}\] \,\e_Q  = 0~.\label{eq:eigRhat}
%\end{align}
%Definie diagonal matrix $\L$:
%\be
%\L_{PQ} = \[\r_{P} -\(r +\nu_4 (m^2+n^2)^2   -\,\frac{\i m\beta }{m^2+n^2}\)\]\d_{PQ}~,
%\ee
%we can interpret Eq.~\eqref{eq:eigRhat} as $\v$ being an eigenvector of $\L$ with eigenvalue $\s$.


\subsection{Non Homogeneous equilibrium }

For the homogeneous equilibrium Eqs.~\eqref{eq:pert_S3Tgen} take the form:
\begin{align}
&\( \bit \s + r + \nu_4 \DDel^2   +\beta \,\D_x \DDel^{-1} \)\d \Zv  =  \d\Rv \label{eq:dZ}\\
&\(\A^E-\sigma\) \d\C+ \d\C\,\(\A^E\)^\transp + \d\A\,\C^E +\C^E\,\(\d\A\)^\transp = 0 ~. \label{eq:dC}
\end{align}\label{eqs:pert_hom}

\begin{subequations}
\begin{align}
\[ \bit \s + r + \nu_4 \DDel^2   + \U^E\,\D_x +\(\beta -\U_{yy}^E\)\D_x \DDel^{-1} \]\d \Zv  &=  \d\Rv \label{eq:dZ_UE}\\
\(\A^E-\sigma\) \d\C+ \d\C\,\(\A^E\)^\transp + \d\A\,\C^E +\C^E\,\(\d\A\)^\transp &= 0 ~. \label{eq:dC_UE}
\end{align}\end{subequations}
where now $\A^E= -\U^E\D_x  - \(\beta -\U_{yy}^E\)\D_x \DDel^{-1}-r -\nu_4 \DDel^2$ and we have defined the Reynolds stress divergence $\d\Rv= - \D_x \[\bit \vecd{\( - \D_y \DDel^{-1}\d\C\)}\] - \D_y \[\bit\vecd{\( \D_x \DDel^{-1}\d\C\)}\]$ and
\be
\d\A = -\d\U\,\D_x-\d\V\,\D_y - \d\Z_y\,\D_x\DDel^{-1}+ \d\Z_x\,\D_y\DDel^{-1}~.
\ee
The eigenfunctions of this system are harmonics, $e^{\i(mx+ny)}$.

We assume $\d\Zv_{m} = e^{\i mx} f(y)$ and a corresponding eigenvalue $\s_{m}$. We calculate $\d\C_{m,n}$ from Eq.~\eqref{eq:dC} and from that the corresponding Reynolds stress divergence, $\d\Rv_{m,n}$, that corresponds to the $(\d\Zv_{m,n},\s_{m,n})$. We expand the $\d\Rv_{m,n}$ as:
\be
\d\Rv_{m} = e^{\i mx} \sum_{n'}  \hat{\R}_{mn'}\,e^{\i n'y}~.
\ee



\be
C^E(x_\a,x_\b,y_\a,y_\b) = \sum_k e^{\i k (x_\a-x_\b)} \, C^E_k(y_a,y_b)
\ee


It can be proven that $\d\Rv_{mn}$ will be proportional to $\d\Z_{mn}$, that is: $\hat{\Rv}_{mnm'n'}=r_{mn}\d_{mm'}\d_{nn'}$ (with $r_{mn}$ in general complex). This way Eq.~\eqref{eq:dZ} is written:
\be
 \( \bit \s + r + \nu_4 (m^2+n^2)^2   -\frac{\i m\beta }{m^2+n^2} - r_{mn}\) \,e^{\i(mx+ny)}  = 0\\
\ee
So our new guess for the eigenvalue, $\s'$ is:
\be
\s' = -r +\frac{\i m\beta }{m^2+n^2} + r_{mn}~.
\ee
We continue this iteration until convergence, that is until $|\s'-\s|\big/|\s'|<\tol$.

\vspace{2cm}

This method works very well in reproducing the results of the non-zonal dispersion relation for every choice of $(m,n)$ and it converges to the unstable eigenvalue even if our initial guess is very far away from that.

%Let us define a ``symbolic'' index $P$ for $m,n$ and $Q$ for $m',n'$ then the above is written: 
%\begin{align}
%\sum_{Q} \[ \( \bit \s + r + \nu_4 (m^2+n^2)^2   -\,\frac{\i m\beta }{m^2+n^2}\)\d_{P,Q} - \r_P \d_{P,Q}\] \,\e_Q  = 0~.\label{eq:eigRhat}
%\end{align}
%Definie diagonal matrix $\L$:
%\be
%\L_{PQ} = \[\r_{P} -\(r +\nu_4 (m^2+n^2)^2   -\,\frac{\i m\beta }{m^2+n^2}\)\]\d_{PQ}~,
%\ee
%we can interpret Eq.~\eqref{eq:eigRhat} as $\v$ being an eigenvector of $\L$ with eigenvalue $\s$.



\subsection{Jet equilibrium ($U^E\ne0,V^E=0$)}

Consider now a jet equilibrium $\(\Psi^E(y),C^E\)$. Since the streamfunction is only a function of $y$ the coherent mean flow will have only a streamwise component that is varied in $y$, $\(U^E(y),V^E=0\)$. Also the equilibrium perturbation vorticity covariance, $C^E$ will be homogeneous in $x$, that is it will depend only in the difference coordinate in $x$: $C^E(x_\a-x_\b,y_\a,y_\b)$. Therefore it can be readily shown that the perturbation equations take the form:\begin{subequations}
\begin{align}
\[ \bit \s + r + \nu_4 \DDel^2   + \U^E\,\D_x +\(\beta -\U_{yy}^E\)\D_x \DDel^{-1} \]\d \Zv  &=  \d\Rv \label{eq:dZ_UE}\\
\(\A^E-\sigma\) \d\C+ \d\C\,\(\A^E\)^\transp + \d\A\,\C^E +\C^E\,\(\d\A\)^\transp &= 0 ~. \label{eq:dC_UE}
\end{align}\end{subequations}
where now $\A^E= -\U^E\D_x  - \(\beta -\U_{yy}^E\)\D_x \DDel^{-1}-r -\nu_4 \DDel^2$.

The perturbation vorticity eigenfunction will not be a single harmonic function, can it will in general be a sum of harmonics:
\be
\d Z = \sum_{\substack{m,n\\m,n\ne0}} \a_{mn}\,e^{\i\(mx+ny\)}\label{eq:dZ_gen}~,
\ee
(the $m,n\ne 0$ will be omitted from now on).
Let us denote $\d\Zv_{mn} = e^{\i\(mx+ny\)}$ and also let $\d\C_{mn}$ the solution of:
\be
\(\A^E-\sigma\) \d\C_{mn}+ \d\C_{mn}\,\(\A^E\)^\transp + \d\A_{mn}\,\C^E +\C^E\,\(\d\A_{mn}\)^\transp = 0 ~. 
\ee
If $\d\Zv$ is given by Eq.~\eqref{eq:dZ_gen} then we have that 
\be
\d\A = \sum_{m,n} \a_{mn}\,\d\A_{mn}~,
\ee
and therefore:
\begin{align}
\sum_{m,n} \a_{mn}\,\[ \(\A^E-\sigma\) \d\C_{mn}+ \d\C_{mn}\,\(\A^E\)^\transp + \d\A_{mn}\,\C^E +\C^E\,\(\d\A_{mn}\)^\transp \] &= 0~\Leftrightarrow\nonumber\\
 \(\A^E-\sigma\) \(\sum_{m,n} \a_{mn} \d\C_{mn}\)+ \(\sum_{m,n}\a_{mn} \d\C_{mn}\)\,\(\A^E\)^\transp  + \d\A\,\C^E +\C^E\,\(\d\A\)^\transp&= 0~
\end{align}
Therefore the solution $\d\C$ of Eq.~\eqref{eq:dC_UE} is also expanded as:
\be
\d\C = \sum_{m,n} \a_{mn}\,\d\C_{mn}~.
\ee

What is the Reynold stress convergence $\d\Rv$ that is induced by $\d\C$? If we denote $\d\Rv_{mn}$ the Reynold stress convergence induced by $\d\C_{mn}$ then the total $\d\Rv$ will be:
\be
\d\Rv = \sum_{m,n} \a_{mn}\,\d\Rv_{mn}~.
\ee
The $\d\Rv_{mn}$ can be written as a Fourier expansion:
\be
\d\Rv_{mn} = \sum_{m',n'} \hat{R}_{m'n'mn}\,\d\Zv_{m'n'}~.
\ee

From \eqref{eq:dZ_UE} (neglecting $\nu_4$)
\begin{align}
\sum_{m,n} \[ \bit \s + r  + \U^E\,\D_x +\(\beta -\U_{yy}^E\)\D_x \DDel^{-1} \] \a_{mn}\,\d \Zv_{mn}  =  \sum_{m,n,m',n'} \a_{mn} \hat{R}_{m'n'mn}\,\d\Zv_{m'n'} ~\Leftrightarrow\nonumber\\
\sum_{m,n,m',n'} \left\{ \[ \bit \s + r +\U^E\,\D_x +\(\beta -\U_{yy}^E\)\D_x \DDel^{-1} \]\d_{mm'}\d_{nn'}  -    \hat{R}_{m'n'mn} \right\} \a_{mn}\,\d\Zv_{m'n'} ~\Leftrightarrow\nonumber\\
\end{align}

The equilibrium $U^E$ can be also written as $U^E=\sum_p \hat{U}^E_p e^{\i p y}$, $U^E_{yy}=\sum_p -p^2 \hat{U}^E_p e^{\i p y}$.
\be
\sum_{m,n,m',n'} \left\{ \[ \bit \s + r  - \frac{\i m\beta}{m^2+n^2} + \sum_p\i m\(1 - \frac{p^2}{m^2+n^2}  \)\hat{U}_p^E\,e^{\i p y} \]\,\d_{mm'}\d_{nn'}  -    \hat{R}_{m'n'mn} \right\} \a_{mn}\,\d\Zv_{m'n'} ~\nonumber\\
\ee


Let us neglect also the nonlinear advection terms in the equation for the coherent structure and also define a ``symbolic'' index $P$ for $m,n$ and $Q$ for $m',n'$ then the above is written: 
\be
\sum_{P,Q} \left\{ \[ \bit \s + r  - \frac{\i m\beta}{m^2+n^2}  \]\,\d_{QP}  -    \hat{R}_{QP} \right\} \a_{P}\,\d\Zv_{Q} ~\nonumber\\
\ee
Since $\d\Z_Q$ are linearly independent then each
\be
\sum_{P} \left\{ \[ \bit \s + r  - \frac{\i m\beta}{m^2+n^2}  \]\,\d_{QP}  -    \hat{R}_{QP} \right\} \a_{P}
\ee
must be zero, which is equivalent with $\a$ being an eigenvector of $\L=\R-r\I - \vecd(\i m \beta/(m^2+n^2))$ with eigenvalue $\s$. We find the eigenvalues of $\s$, choose the one with the maximum real part and repeat iteration.

==> frontmatter/abstract.tex <==
% !TEX root = ../thesis.tex

% the abstract


This thesis presents a newly developed theory for the formation and maintenance of eddy-driven jets in planetary turbulence. The novelty is that jet formation and maintenance is studied as a dynamics of the statistics of the flow rather than dynamics of individual realizations. This is pursued using Stochastic Structural Stability Theory (S3T) which studies the closed dynamics of the first two cumulants of the full statistical state dynamics of the flow by neglecting or parameterizing the third and higher-order cumulants. S3T is an analytical, predictive and quantitative theory for turbulence that proceeds directly from the equations of motion and provides a way of finding turbulent statistical equilibria and determining their stability. Instability of the statistics of the flow signifies transition of the turbulent regime to a new regime.

With this statistical closure large-scale structure formation is studied in barotropic turbulence on a $\b$-plane. By studying the dynamics of the statistical state novel phenomena are predicted such as: the instability of homogeneous turbulence to jet formation, the establishment of turbulent equilibria, the prediction of multiple turbulent equilibria, jet merging bifurcations, and the existence of latent jets. Although these phenomena cannot be predicted by analysis of the dynamics of single realizations of the flow, it is demonstrated that the predictions of the statistical theory are reflected in individual realizations of the flow.

It is further demonstrated that at analytically predicted critical parameter values the homogeneous turbulent state undergoes a bifurcation and becomes inhomogeneous with the emergence of large-scale zonal and/or non-zonal flows. The mechanisms by which the turbulent Reynolds stresses organize to reinforce infinitesimal mean flow inhomogeneities, thus leading to this statistical state instability, are extensively studied for various regimes of parameter values (planetary vorticity gradient, dissipation rate and turbulent energy injection rate) and it is shown that for small and modest values of planetary vorticity gradient, $\b$, the upgradient fluxes responsible for the formation and maintenance of large-scale structure are induced by the Orr mechanism, while for large $\b$ by resonant wave triads. It is demonstrated that the S3T instabilities equilibrate to finite amplitude jets, in agreement with the jets that develop in individual simulations. The relation between the formation of large-scale structure through modulational instability and the S3T instability of the homogeneous turbulent state is also investigated and it is shown that the modulational instability results are subsumed by the S3T results.

The study of the S3T stability of inhomogeneous turbulent jet equilibria is also presented and the relation with the phenomenon of jet merging is investigated. Methods for finding inhomogeneous statistical turbulent equilibria and also for studying their stability are developed.



==> frontmatter/abstractgreek.tex <==


% the abstract

Παρουσιάζεται μία θεωρία που αναπτύχθηκε πρόσφατα για το σχηματισμό και την συντήρηση αεροχείμαρρων στις ατμόσφαιρες πλανητών. Η καινοτομία της θεωρίας αυτής είναι ότι αντιμετωπίζει το σχηματισμό και τη συντήρηση των αεροχείμαρρων όχι μέσω της μελέτης της δυναμικής ανεξαρτήτων τροχιών του ρευστού στο θεσεογραφικό χώρο αλλά μέσω της μελέτης της δυναμικής που υπακούει η ίδια η στατιστική των τροχιών αυτών. Αυτό επιτυγχάνεται μέσω της Θεωρίας Στοχαστικής Δομικής Ευστάθειας (Stochastic Structural Stability Theory -- S3T) η οποία μελετά το κλειστό δυναμικό σύστημα που περιγράφει τη δυναμική των δύο πρώτων στατιστικών ροπών της πλήρους στατιστικής δυναμικής της ροής, αγνοώντας ή παραμετροποιώντας ροπές τρίτης και ανώτερης τάξεως. Η S3T αποτελεί μια αναλυτική, προγνωστική και ποσοτική θεωρία της τυρβώδους κατάστασης η οποία προκύπτει απευθείας από τις εξισώσεις κινήσεις. Μας παρέχει ένα τρόπο εύρεσης στατιστικών τυρβώδων καταστάσεων ισορροπίας και επίσης τρόπο μελέτης της ευστάθειας αυτών. Αστάθεια της στατιστικής δυναμικής της ροής υπονοεί μετάβαση της τύρβης σε μια κατάσταση.

Μέσω αυτού του στατιστικού κλεισίματος (closure) γίνεται μελέτη του σχηματισμού δομών μεγάλης κλίμακας σε βαροτροπική τύρβη σε $\b$-επίπεδο. Μελετώντας τη δυναμικής της στατιστικής κατάστασης μία σειρά από νέα φαινόμενα μπορούν να προβλεφθούν, όπως: η ύπαρξη στατιστικών τυρβώδων καταστάσεων ισορροπίας, η αστάθεια τις ομοιογενούς τυρβώδους κατάστασης ως προς το σχηματισμό ζωνικών ροών, συγχωνεύσεις αεροχείμαρρων ως διακλαδώσεις της στατιστικής δυναμικής και η ύπαρξη λανθανουσών ζωνικών ροών (latent jets). Ενώ όλα αυτά τα φαινόμενα δεν μπορούν να προβλεφθούν με τη μελέτης της δυναμικής ανεξαρτήτων τροχιών του ρευστού στο θεσεογραφικό χώρο, επιδεικνύεται ότι οι προβλέψεις της στατιστικής δυναμικής αντικατοπτρίζονται σε τέτοιες τροχιές της ροής.

Ως προς το σχηματισμό των δομών μεγάλης κλίμακας δείχνεται ότι σε κάποιες κρίσιμες τιμές των παραμέτρων, οι οποίες προβλέπονται αναλυτικά, γίνεται μία διακλάδωση και η στατιστικά ομοιογενής τυρβώδης κατάσταση γίνεται ανομοιογενής με την εμφάνιση είτε ζωνικών είτε μη-ζωνικών ροών μεγάλης κλίμακας. Οι μηχανισμοί με τους οποίους οι τάσεις Reynolds από τις τυρβώδεις κινήσεις του υγρού οργανώνονται ούτως ώστε να ενισχύσουν μία απειροστή μέση ροή, οδηγώντας έτσι σε στατιστική αστάθεια, μελετώνται διεξοδικά για διάφορες περιοχές των παραμέτρων (της κλίσης της πλανητικής στροβιλότητας, του ρυθμού ανάλωσης λόγω απόσβεσης και του ρυθμού εισροής ενέργειας στη ροή). Δείχνεται ότι για μικρές και μεσαίες τιμές της κλίσης της πλανητικής στροβιλότητας, $\b$, η ροή ορμής σε κατεύθυνση αντίθετα από αυτήν της βαθμίδας (upgradient momentum flux), η οποία είναι υπεύθυνη για το σχηματισμό των δομών μεγάλης κλίμακας, επάγεται μέσω του μηχανισμού Orr, ενώ για μεγάλες τιμές της $\b$ μέσω συντονισμού από τριάδες κυμάτων. Δείχνεται επίσης ότι οι S3T αστάθειες εξισορροπούνται σε πεπερασμένο πλάτος, σε συμφωνία με τις ζωνικές ροές που σχηματίζονται σε αριθμητικές προσομοιώσεις των εξισώσεων κίνησης. Διερευνάται επίσης η σχέση μεταξύ του σχηματισμού δομών μεγάλης κλίμακας μέσω της διαμορφωτικής αστάθειας (modulational instability) και της S3T αστάθειας της ομοιογενούς τυρβώδους κατάστασης και δείχνεται ότι η διαμορφωτική αστάθεια δεν είναι παρά μία ειδική περίπτωση της S3T αστάθειας.

Τέλος, γίνεται μελέτη της  S3T ευστάθειας ανομοιογενών στατιστικών τυρβώδων καταστάσεων στις οποίες υπάρχουν ζωνικές ροές μεγάλης κλίμακας και διερευνάται η σχέση των S3T ασταθειών που προκύπτουν με το φαινόμενο συγχώνευσης αεροχείμαρρων. Αναπτύσσονται μέθοδοι εύρεσης ανομοιογενών στατιστικών τυρβώδων καταστάσεων καθώς επίσης και μελέτης της ευστάθειας αυτών.


==> frontmatter/abstractturkish.tex <==
% the abstract

This is the turkish version of the abstract


==> frontmatter/authorlist.tex <==
\noindent The following authors contributed to Chapter 1: Albert Einstein, George Gamow and Pief Panofsky.

\noindent The following authors contributed to Chapter 2: I. I. Rabi, Niels Bohr and Norman Ramsey.

\noindent The following authors contributed to Chapter 3: Ramon y Cajal, Andrew Huxley. 


==> frontmatter/coverpage.tex <==
% some details about the thesis
\title{Formation of large-scale structures by turbulence in rotating planets}
\author{Navid C. Constantinou}
\advisor{Petros J. Ioannou}

\titlegreek{Σχηματισμός δομών μεγάλης κλίμακας από την τύρβη\\ σε περιστρεφόμενους πλανήτες}
\authorgreek{Ναβίτ Κ. Κωνσταντίνου}
\advisorgreek{Πέτρος Ι. Ιωάννου}

% about the degree
\degree{Doctor of Philosophy}
\field{Physics}
\degreeyear{2015}
\degreemonth{July}

% about the university
\department{Department of Physics}
\university{National and Kapodistrian University of Athens}
\universitycity{Athens}
\universitystate{Greece}






==> frontmatter/efkaristo.tex <==
% !TEX root = thesis.tex



% the acknowledgments section

% the acknowledgments section

%\newthought{I would like to thank} everyone. Also the Pope of Rome and his fabulous cat.


%
%Often I am being asked the question ``what do you study in your Ph.D.?''. Usually I answer this question in two different ways, depending whether I am being asked by a person who is also in science or not.
%The latter category usually accompanies their question with an expression of fear, being sure that they will not understand anything of what I am about to say. To them, I answer "I study weather" and as a result their first fear disappears. Of course one of the next question is: ``So how will the weather going to be the next days?'' which I am incapable of answering. To fellow scientists I explain in more detail that I study geophysical fluid dynamics  . . . Their next question is ``How did you choose this subject? Did you liked it all along?''.
%
%Indeed, eventually I ended up liking the subject very much 
%However, I only chose the subject because it was the area of interest of my teacher, Petros Ioannou. In fact, when I decided to pursue doctoral studies I did not choose the field to study but I chose the teacher to study with.
%
%In fact I did not liked it all along
%





%One of the most common questions somebody asks a person pursuing doctoral studies is why he chose to study the specific subject. Personally, I have not chosen the particular subject to study but rather I chose the teacher with who I wanted to study with.



Γνώρισα τον Πέτρο Ιωάννου το 2004 όταν στο δεύτερο έτος των προπτυχιακών μου σπουδών παρακολούθησα το μάθημα της Θεωρητικής Μηχανικής που συνδιδάσκει μαζί με τον Θεοχάρη Αποστολάτο. Οι ζωντανές, γεμάτες έμπνευση και συχνά διασκεδαστικές διαλέξεις τους άλλαξαν από τότε τον τρόπο με τον οποίο αντιλαμβάνομαι τη Φυσική. Ήταν, θυμάμαι, πρώτη φορά στο μάθημα της Μηχανικής  που αντιλήφθηκα τι ακριβώς εστί θεωρητική φυσική. Κατά τη διάρκεια των τελευταίων 10 ετών και οι δύο του έχουν επηρεάσει σε μεγάλο βαθμό τον τρόπο με τον οποίο σκέφτομαι .

Φτάνοντας στο τέλος των διδακτορικών μου σπουδών θα ήθελα πρωτίστως να ευχαριστήσω 




I met Petros Ioannou in 2004 when I was in my second year of undergraduate studies. I had taken then a course that he and Theocharis Apostolatos taught on Newtonian Mechanics.  Their inspiring, lively and often entertaining lectures changed my way of viewing physics. It was during this Mechanics course that I got my first taste of what physics is all about. During the last 10 years both of them have influenced my scientific way of thinking immensely.

Now that my doctoral studies have completed I would like to thank first and foremost my thesis advisor Petros Ioannou. He has been a tutor and a mentor for me during these years. His clear physical and mathematical intuition, along with his immense passion and enthusiasm for attacking physical problems have both been sources of inspiration for me. I really hope that some day I will be able to convey but a fraction of his passion and clarity to any future student that I might have.

Next I want to say thank you to Nikos Bakas. He has been my older academic ``brother" and my officemate. I thank him for the multitude of discussions we had regarding the scientific problems and also for the many times that he has help me out when I could not overcome a specific calculation. 

Also a special thanks should go to Brian Farrell and to Theocharis Apostolatos both for being readily available for anything I wanted to discuss regarding my research.

I also want to thank Fokion Hatziioannou. The afternoon discussion sessions that were organized during the period when I was an undergraduate and in the early years of my graduate studies helped me become acquainted with subjects that were not approached in the lectures and also revisit subjects that I had been taught in the lectures but through a completely different perspective.  Also, for the organization of the famous ``Physic Department excursions'' and the long hikes in the mountains all over Greece. The majority my friends from the Physics Department I had either met them in one of these field trips, or, if I had already met them before, it was in this excursions that we came really close to each other for the first time.


I would like to thank Javier Jim\'enez for inviting me to the First Multiflow Summer Workshop during June 2013 in Madrid.  Also I would like to thank the IPAM (Institute for Pure and Applied Mathematics), UCLA for the invitation to the Mathematics of Turbulence Long program (September to December 2014) as a core participant and their hospitality. Much of this manuscript was written during my time at IPAM.

It is my pleasure to acknowledge the Alexander S. Onassis Public Benefit Foundation for the financial support they have provided me during the period 2009-2014. Also, my friend A. Koudounas for partially supporting me during the last six months of my doctoral studies.

Special thanks goes to my parents Ntinos \& Ntina and the rest of my family for their continuous support, love and understanding the last eleven years of both my undergraduate and post-graduate studies.

Last but not least I would like to take this opportunity to collaboratively thank all of my friends who have been close supporters of me throughout these years. Indicatively I should mention: 
Giannis M. for helping me pack and move all my stuff away from my apartment before departing for the IPAM workshop in L.A. and also for his hospitality in Lefkosia in January 2015; 
Savvas~K. for his hospitality in Archanes during COMECAP 2014 conference;
Haris \& Kyriaki for their hospitality in Lefkada during both summers of 2011 and 2014 where we enjoyed Lefkada's crystal clear waters and parts of this manuscript were written;
Petros for joining me to innumerable bicycle rides up the mountains around Athens;
Theodore~D. for his company during the IPAM workshop and for reading and commenting on parts of this manuscript;
Savvas~S. for his hospitality in Lefkosia both in September 2011 and December 2012;
Andreas~K. and Mairi for their hospitality in Lefkosia in January 2013;
Andreas~A. who except from being a friend also was an extremely helpful neighbor in Exarchia;
Andreas~S. for the great moments we had in the university in Athens, for introducing me to Pandelis gastronomical experience, and for his support even after he left Athens towards the colder, higher, Scandinavian latitudes.  Finally, and perhaps most importantly, my Antigoni for caring.



%
%\vspace{2em}
%
%\begin{flushright}
%\emph{Navid\\
%Athens, Feb. 2015}
%\end{flushright}
%





